Planetary Candidates Observed by Kepler. VII. The First Fully Uniform Catalog Based on The Entire 48 Month Dataset (Q1-Q17 DR24)

We present the seventh Kepler planet candidate catalog, which is the first to be based on the entire, uniformly processed, 48 month Kepler dataset. This is the first fully automated catalog, employing robotic vetting procedures to uniformly evaluate every periodic signal detected by the Q1-Q17 Data Release 24 (DR24) Kepler pipeline. While we prioritize uniform vetting over the absolute correctness of individual objects, we find that our robotic vetting is overall comparable to, and in most cases is superior to, the human vetting procedures employed by past catalogs. This catalog is the first to utilize artificial transit injection to evaluate the performance of our vetting procedures and quantify potential biases, which are essential for accurate computation of planetary occurrence rates. With respect to the cumulative Kepler Object of Interest (KOI) catalog, we designate 1,478 new KOIs, of which 402 are dispositioned as planet candidates (PCs). Also, 237 KOIs dispositioned as false positives (FPs) in previous Kepler catalogs have their disposition changed to PC and 118 PCs have their disposition changed to FP. This brings the total number of known KOIs to 8,826 and PCs to 4,696. We compare the Q1-Q17 DR24 KOI catalog to previous KOI catalogs, as well as ancillary Kepler catalogs, finding good agreement between them. We highlight new PCs that are both potentially rocky and potentially in the habitable zone of their host stars, many of which orbit solar-type stars. This work represents significant progress in accurately determining the fraction of Earth-size planets in the habitable zone of Sun-like stars. The full catalog is publicly available at the NASA Exoplanet Archive.

==> ebexclude-full.tex <==
001433410\\
001572353\\
001573836\\
001868650\\
002012362\\
002141697\\
002159783\\
002162283\\
002302092\\
002305277\\
002435971\\
002437038\\
002444187\\
002448320\\
002449084\\
002450566\\
002453212\\
002570289\\
002571439\\
002577756\\
002694741\\
002695740\\
002715007\\
002715417\\
002717141\\
002720096\\
002831632\\
002835289\\
002851474\\
002854432\\
002854752\\
002858322\\
002972514\\
002983113\\
002988984\\
002996347\\
003104113\\
003119295\\
003127873\\
003218683\\
003221207\\
003228863\\
003232823\\
003240976\\
003245776\\
003339563\\
003342425\\
003353233\\
003354616\\
003431321\\
003437778\\
003437800\\
003439180\\
003443519\\
003448245\\
003454864\\
003545476\\
003547111\\
003547874\\
003549994\\
003557421\\
003558822\\
003560212\\
003633901\\
003641446\\
003729724\\
003730067\\
003732732\\
003734660\\
003735597\\
003743834\\
003745184\\
003749404\\
003756730\\
003765708\\
003832382\\
003833859\\
003837677\\
003839964\\
003848042\\
003851320\\
003853259\\
003862171\\
003935319\\
003936357\\
003953981\\
003956545\\
003956881\\
003958488\\
003965556\\
003969362\\
003972629\\
004036687\\
004066203\\
004071600\\
004073678\\
004074532\\
004074708\\
004138301\\
004150136\\
004168013\\
004169521\\
004241946\\
004244929\\
004248941\\
004249218\\
004273411\\
004281068\\
004349483\\
004350454\\
004357272\\
004359851\\
004372379\\
004372705\\
004385109\\
004450976\\
004451148\\
004458989\\
004464999\\
004466691\\
004474193\\
004476900\\
004545729\\
004547067\\
004547308\\
004550750\\
004554004\\
004563150\\
004569923\\
004570326\\
004647652\\
004649324\\
004651526\\
004659476\\
004660997\\
004661397\\
004669592\\
004672934\\
004677321\\
004738426\\
004743626\\
004758092\\
004762887\\
004843222\\
004847343\\
004847369\\
004850874\\
004853067\\
004857282\\
004859432\\
004904304\\
004909422\\
004921906\\
004936334\\
004936680\\
004937217\\
004941060\\
004945588\\
004945857\\
004947528\\
004949194\\
004949770\\
004950505\\
004954113\\
004991959\\
004999260\\
004999357\\
005005570\\
005008287\\
005015926\\
005017127\\
005022573\\
005022908\\
005025261\\
005033682\\
005041843\\
005041975\\
005077994\\
005104097\\
005123176\\
005127005\\
005128972\\
005129777\\
005166136\\
005174346\\
005175668\\
005195137\\
005196301\\
005197256\\
005198934\\
005199489\\
005201619\\
005211385\\
005215999\\
005218385\\
005219580\\
005259926\\
005264818\\
005282464\\
005283266\\
005283839\\
005284262\\
005286221\\
005290305\\
005296276\\
005296877\\
005307780\\
005310387\\
005353374\\
005353653\\
005357682\\
005357882\\
005358200\\
005369419\\
005371109\\
005374883\\
005374999\\
005376552\\
005377349\\
005389616\\
005390351\\
005425950\\
005439790\\
005440746\\
005450322\\
005458880\\
005459373\\
005461570\\
005468295\\
005475624\\
005477524\\
005478466\\
005511076\\
005535061\\
005543482\\
005557368\\
005563814\\
005567438\\
005606644\\
005611561\\
005611763\\
005615528\\
005615815\\
005617953\\
005620981\\
005623923\\
005685072\\
005699617\\
005703230\\
005707897\\
005733154\\
005733384\\
005737474\\
005770431\\
005770860\\
005771961\\
005773205\\
005783368\\
005783676\\
005785551\\
005786545\\
005790912\\
005791886\\
005792093\\
005802834\\
005809827\\
005809868\\
005818706\\
005820209\\
005821050\\
005823121\\
005872506\\
005872696\\
005877364\\
005878081\\
005878836\\
005881838\\
005891963\\
005944240\\
005951553\\
005955731\\
005956588\\
005957123\\
005960283\\
005960989\\
005961327\\
005966237\\
005975712\\
005977736\\
005978521\\
005984000\\
005985314\\
005988465\\
006024572\\
006026204\\
006034812\\
006042191\\
006044543\\
006045264\\
006046061\\
006050116\\
006057829\\
006061139\\
006067735\\
006072195\\
006072578\\
006105491\\
006106771\\
006118779\\
006128248\\
006137885\\
006141791\\
006143826\\
006144827\\
006153219\\
006197319\\
006209824\\
006213131\\
006223646\\
006262882\\
006264091\\
006265720\\
006267702\\
006281103\\
006286402\\
006287172\\
006290740\\
006292925\\
006302051\\
006302592\\
006344429\\
006350020\\
006353203\\
006359771\\
006368316\\
006370361\\
006370558\\
006370665\\
006390205\\
006424124\\
006431545\\
006436038\\
006443538\\
006446219\\
006447430\\
006462057\\
006467389\\
006471048\\
006504095\\
006507541\\
006549491\\
006593575\\
006615041\\
006633929\\
006669809\\
006670812\\
006671698\\
006677225\\
006689368\\
006692340\\
006693555\\
006695510\\
006699679\\
006766325\\
006775034\\
006791604\\
006794131\\
006803335\\
006805779\\
006836140\\
006843507\\
006844489\\
006853229\\
006863229\\
006865626\\
006871716\\
006880727\\
006881709\\
006929869\\
006964796\\
006966265\\
007013934\\
007023917\\
007035139\\
007037319\\
007038831\\
007039026\\
007060333\\
007091476\\
007117153\\
007118621\\
007118656\\
007119757\\
007119876\\
007130044\\
007173910\\
007176440\\
007198474\\
007199183\\
007199353\\
007204041\\
007217866\\
007259722\\
007259917\\
007269797\\
007269843\\
007272739\\
007273033\\
007280704\\
007282128\\
007304911\\
007335517\\
007339123\\
007339345\\
007348206\\
007350038\\
007362751\\
007366145\\
007367833\\
007368451\\
007373255\\
007373555\\
007375612\\
007378178\\
007382250\\
007383021\\
007387296\\
007431703\\
007432479\\
007433513\\
007440742\\
007457163\\
007458285\\
007501230\\
007506164\\
007506446\\
007511416\\
007512381\\
007516345\\
007518816\\
007529123\\
007533807\\
007542091\\
007546429\\
007546791\\
007584739\\
007584826\\
007590728\\
007591456\\
007597095\\
007601767\\
007610486\\
007620664\\
007627059\\
007630690\\
007657914\\
007672068\\
007676610\\
007680593\\
007685689\\
007686918\\
007690843\\
007691553\\
007696778\\
007697065\\
007698650\\
007700181\\
007709086\\
007740302\\
007740566\\
007744173\\
007748113\\
007749504\\
007765894\\
007766185\\
007773380\\
007777443\\
007816201\\
007818448\\
007821450\\
007830460\\
007835348\\
007839027\\
007871200\\
007877062\\
007878402\\
007884426\\
007884842\\
007887124\\
007889628\\
007890379\\
007897952\\
007907688\\
007936219\\
007938870\\
007941050\\
007950962\\
007953796\\
007959612\\
007968880\\
007973970\\
007975824\\
007976783\\
007977261\\
008004839\\
008027591\\
008029708\\
008039225\\
008043961\\
008045121\\
008053107\\
008074045\\
008087799\\
008095275\\
008097539\\
008097553\\
008097902\\
008099615\\
008108785\\
008111387\\
008122124\\
008123430\\
008143757\\
008144355\\
008145477\\
008151107\\
008166095\\
008177958\\
008183850\\
008189196\\
008190491\\
008190613\\
008192840\\
008197368\\
008211618\\
008222945\\
008230815\\
008231231\\
008241252\\
008242493\\
008245326\\
008248812\\
008257903\\
008263940\\
008264490\\
008264510\\
008264534\\
008265951\\
008280135\\
008285349\\
008298344\\
008309175\\
008311255\\
008314879\\
008322564\\
008328376\\
008330092\\
008360184\\
008382182\\
008386048\\
008386198\\
008386865\\
008386982\\
008394040\\
008397460\\
008428136\\
008430210\\
008431389\\
008431390\\
008431611\\
008432859\\
008452840\\
008456774\\
008456998\\
008481574\\
008496820\\
008508485\\
008523194\\
008539720\\
008539850\\
008545456\\
008548416\\
008554005\\
008555573\\
008559716\\
008563964\\
008579707\\
008587792\\
008608310\\
008624778\\
008625469\\
008626039\\
008647309\\
008652599\\
008654097\\
008677949\\
008682849\\
008685306\\
008690104\\
008694926\\
008696274\\
008696442\\
008703528\\
008715667\\
008739802\\
008758716\\
008800998\\
008804824\\
008816790\\
008823666\\
008838070\\
008842170\\
008846978\\
008868650\\
008872737\\
008878719\\
008892722\\
008893936\\
008894630\\
008904448\\
008906039\\
008912308\\
008912468\\
008912911\\
008913061\\
008934111\\
008956957\\
008957887\\
008958670\\
008977390\\
008982501\\
008982514\\
009002076\\
009004380\\
009005043\\
009016693\\
009020289\\
009021397\\
009026766\\
009028024\\
009030509\\
009030817\\
009032671\\
009051716\\
009071104\\
009071373\\
009075704\\
009077796\\
009083523\\
009085955\\
009087918\\
009091810\\
009092303\\
009094335\\
009097798\\
009108579\\
009110213\\
009137992\\
009142964\\
009145707\\
009145846\\
009151972\\
009161428\\
009164561\\
009164694\\
009179806\\
009181877\\
009220600\\
009228778\\
009237533\\
009237755\\
009238207\\
009239684\\
009245929\\
009268105\\
009272276\\
009274472\\
009283826\\
009288175\\
009290838\\
009307423\\
009345163\\
009345838\\
009347868\\
009350889\\
009353234\\
009356753\\
009357030\\
009365025\\
009388303\\
009389122\\
009392331\\
009392682\\
009402652\\
009408183\\
009412114\\
009414905\\
009419603\\
009426970\\
009450883\\
009451598\\
009453192\\
009466316\\
009470054\\
009470175\\
009472174\\
009475663\\
009478836\\
009480516\\
009480977\\
009481674\\
009489411\\
009508052\\
009508954\\
009512958\\
009514070\\
009519590\\
009527167\\
009532219\\
009532591\\
009533508\\
009533706\\
009536053\\
009541127\\
009544350\\
009552668\\
009592145\\
009596037\\
009602542\\
009612468\\
009637239\\
009637265\\
009639265\\
009639491\\
009644680\\
009649493\\
009651298\\
009654476\\
009655187\\
009657096\\
009662581\\
009664382\\
009665086\\
009700154\\
009701423\\
009702641\\
009703626\\
009711769\\
009713664\\
009716456\\
009717924\\
009722737\\
009724080\\
009725155\\
009760531\\
009767437\\
009772642\\
009776718\\
009777987\\
009784371\\
009786798\\
009788113\\
009790355\\
009821923\\
009827122\\
009832227\\
009833618\\
009833806\\
009835416\\
009838047\\
009840412\\
009843451\\
009848190\\
009851944\\
009882280\\
009892651\\
009898401\\
009899216\\
009906590\\
009909497\\
009934052\\
009935245\\
009935311\\
009944907\\
009947924\\
009948201\\
009953894\\
009956124\\
009957411\\
009970937\\
009991887\\
009994475\\
009995660\\
009995981\\
010004546\\
010007533\\
010014536\\
010014830\\
010020247\\
010024144\\
010030943\\
010032392\\
010032935\\
010074939\\
010084115\\
010090246\\
010090722\\
010092506\\
010096019\\
010096864\\
010119517\\
010123627\\
010128961\\
010135584\\
010148799\\
010149237\\
010149845\\
010154189\\
010155563\\
010159014\\
010162999\\
010198097\\
010206340\\
010216186\\
010221886\\
010226388\\
010228240\\
010229723\\
010253375\\
010253421\\
010255110\\
010259530\\
010267044\\
010274218\\
010275197\\
010275747\\
010280990\\
010285661\\
010288502\\
010291683\\
010292413\\
010322296\\
010322582\\
010350225\\
010355671\\
010357852\\
010383620\\
010388897\\
010389809\\
010389982\\
010395202\\
010395609\\
010417135\\
010417986\\
010447902\\
010454725\\
010481912\\
010485137\\
010528299\\
010547209\\
010556068\\
010557008\\
010586874\\
010596883\\
010600319\\
010611450\\
010618253\\
010619506\\
010661783\\
010679505\\
010680475\\
010684673\\
010711938\\
010723143\\
010724533\\
010727655\\
010737574\\
010753751\\
010789421\\
010794878\\
010796477\\
010797126\\
010799558\\
010801703\\
010802917\\
010809970\\
010815379\\
010818544\\
010844279\\
010848807\\
010854621\\
010855535\\
010858720\\
010861842\\
010863286\\
010873904\\
010877703\\
010880490\\
010905804\\
010905824\\
010916675\\
010919564\\
010920314\\
010934755\\
010965091\\
010979669\\
010991769\\
011012801\\
011017077\\
011036301\\
011036692\\
011042923\\
011046124\\
011071278\\
011083888\\
011084647\\
011084782\\
011091082\\
011097678\\
011122789\\
011127048\\
011133313\\
011135978\\
011137143\\
011144556\\
011151970\\
011153627\\
011154110\\
011175495\\
011179657\\
011190836\\
011198068\\
011244501\\
011245381\\
011246163\\
011247386\\
011255667\\
011284227\\
011284547\\
011288684\\
011289003\\
011295026\\
011295347\\
011303416\\
011303526\\
011305087\\
011336707\\
011338865\\
011341950\\
011347875\\
011352791\\
011395645\\
011402381\\
011403032\\
011403776\\
011404758\\
011405559\\
011408810\\
011409673\\
011410485\\
011413213\\
011442348\\
011444780\\
011447953\\
011460346\\
011494583\\
011495781\\
011496078\\
011502581\\
011509282\\
011515292\\
011559864\\
011566174\\
011568428\\
011568657\\
011572363\\
011572643\\
011604958\\
011612091\\
011616594\\
011618883\\
011649962\\
011652545\\
011671660\\
011672319\\
011703960\\
011704155\\
011716688\\
011717798\\
011722816\\
011751847\\
011769739\\
011774013\\
011805235\\
011825204\\
011859811\\
011875706\\
011904038\\
011910076\\
011920266\\
011923629\\
011924311\\
011973705\\
012016304\\
012019674\\
012055014\\
012055255\\
012055421\\
012055517\\
012059158\\
012066630\\
012071741\\
012104285\\
012108333\\
012109575\\
012153332\\
012157987\\
012216817\\
012218858\\
012255108\\
012257908\\
012267718\\
012305537\\
012350008\\
012352712\\
012418274\\
012418319\\
012458133\\
012508348\\
012554536\\
012598713\\
012602985\\
012785282\\


==> ephemmatch-full.tex <==
001295289-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002163326-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002166206-01 & 3735.01 & 1:1 & 8.3 & -1 & -2 & 17.64 & -4.34 & 3.4523E+02 & Direct-PRF & 0\\
002297793-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002305311-01 & 002305372-pri & 1:1 & 42.6 & 2 & 10 & 13.82 & 1.14 & 6.9390E+03 & Direct-PRF & 0\\
002308603-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002309585-01 & 5982.01 & 1:1 & 11.7 & -2 & 1 & 13.93 & 1.45 & 6.5525E+00 & Direct-PRF & 0\\
002437112-01 & 3598.01 & 1:1 & 19.7 & -5 & 1 & 17.63 & -1.48 & 7.0495E+02 & Direct-PRF & 0\\
002437112-02 & 3598.01 & 1:2 & 19.7 & -5 & 1 & 17.63 & -1.48 & 8.2520E+02 & Direct-PRF & 0\\
002437112-03 & 3712.01 & 1:1 & 15.1 & 4 & 1 & 16.99 & -0.84 & 7.6798E+02 & Direct-PRF & 0\\
002437488-01 & 002437452-pri & 1:1 & 10.6 & 0 & 3 & 16.98 & -2.02 & 9.3571E+01 & Direct-PRF & 0\\
002437488-02 & 002437452-01 & 2:1 & 10.6 & 0 & 3 & 16.98 & -2.02 & 1.3230E+02 & Direct-PRF & 0\\
002437804-01 & 002437783-01 & 1:1 & 14.4 & 4 & -1 & 17.30 & -3.14 & 2.5600E+02 & Direct-PRF & 0\\
002438062-01 & 002438061-01 & 1:1 & 3.5 & -1 & 1 & 0.00 & 16.39 & 1.7347E+00 & Direct-PRF & 0\\
002438070-01 & 002438061-01 & 1:1 & 6.3 & 2 & 0 & 0.00 & 13.77 & 4.2032E+01 & Direct-PRF & 0\\
002438517-01 & 3699.01 & 1:1 & 12.5 & -1 & 3 & 17.77 & -2.23 & 4.4492E+02 & Direct-PRF & 0\\
002439798-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002441151-01 & 002441161-01 & 1:1 & 10.6 & 2 & 1 & 16.65 & -1.97 & 1.3111E+02 & Direct-PRF & 0\\
002445154-01 & 5983.01 & 1:1 & 16.7 & 1 & 4 & 13.55 & 1.61 & 2.5523E+02 & Direct-PRF & 0\\
002449053-01 & 002449084-pri & 1:1 & 18.4 & 4 & 2 & 15.02 & 0.12 & 4.4483E+03 & Direct-PRF & 0\\
002449074-01 & 002449090-01 & 1:1 & 10.6 & -1 & 3 & 16.24 & -3.09 & 1.6632E+02 & Direct-PRF & 0\\
002449074-02 & 002449090-02 & 1:1 & 10.6 & -1 & 3 & 16.24 & -3.09 & 1.3216E+02 & Direct-PRF & 0\\
002449101-01 & 002449084-pri & 1:1 & 24.9 & 4 & -5 & 15.02 & 0.03 & 1.5926E+03 & Direct-PRF & 0\\
002452450-01 & 3687.01 & 1:1 & 7.4 & 0 & -2 & 16.47 & -3.36 & 7.6170E+01 & Direct-PRF & 0\\
002452450-02 & 002452440-02 & 1:1 & 7.4 & 0 & -2 & 16.47 & -3.36 & 5.3083E+01 & Direct-PRF & 0\\
002452920-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002558363-01 & 3855.01 & 1:1 & 6.9 & -1 & 1 & 18.55 & -2.55 & 7.2383E+02 & Direct-PRF & 0\\
002569488-01 & 3704.01 & 1:1 & 11.4 & -3 & 1 & 17.38 & -3.22 & 5.8470E+02 & Direct-PRF & 0\\
002570432-01 & 002708156-01 & 1:1 & 196.4 & 38 & -30 & 10.67 & 6.49 & 4.2670E+01 & Direct-PRF & 0\\
002570505-01 & UZ-Lyr-pri & 1:1 & 174.2 & 37 & -22 & 10.67 & 2.89 & 2.4497E+04 & Direct-PRF & 0\\
002570767-01 & UZ-Lyr-pri & 1:1 & 204.1 & 51 & 4 & 10.67 & 2.09 & 2.6538E+04 & Direct-PRF & 0\\
002570773-01 & UZ-Lyr-pri & 1:1 & 231.8 & 58 & 0 & 10.67 & 6.18 & 5.4765E+02 & Direct-PRF & 0\\
002571075-01 & UZ-Lyr-pri & 1:1 & 506.2 & 127 & 3 & 10.67 & 5.13 & 5.4438E+03 & Col-Anomaly & 0\\
002576224-01 & 489.01 & 1:1 & 15.7 & -1 & 3 & 14.61 & -1.88 & 1.8200E+01 & Direct-PRF & 0\\
002577952-01 & 002714932-02 & 1:2 & 284.6 & -71 & 7 & 14.61 & 0.39 & 1.7500E+00 & Direct-PRF & 1\\
002578072-01 & 002715113-01 & 1:1 & 82.3 & -19 & -7 & 15.60 & -1.68 & 3.6786E+00 & Direct-PRF & 1\\
002584908-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002707916-01 & UZ-Lyr-pri & 1:1 & 168.8 & 0 & -42 & 10.67 & 5.67 & 1.6416E+03 & Direct-PRF & 0\\
002707985-01 & UZ-Lyr-pri & 1:1 & 100.8 & -6 & -24 & 10.67 & 1.81 & 2.2747E+04 & Direct-PRF & 0\\
002708172-01 & UZ-Lyr-pri & 1:1 & 161.0 & -32 & 25 & 10.67 & 3.14 & 1.7214E+04 & Direct-PRF & 0\\
002708176-01 & UZ-Lyr-pri & 1:1 & 84.3 & 20 & -7 & 10.67 & 3.49 & 4.1629E+03 & Direct-PRF & 0\\
002708203-01 & UZ-Lyr-pri & 1:1 & 105.1 & 25 & -6 & 10.67 & 2.84 & 7.1564E+03 & Direct-PRF & 0\\
002708221-01 & UZ-Lyr-pri & 1:1 & 64.7 & 16 & 4 & 10.67 & 5.49 & 1.0759E+03 & Direct-PRF & 0\\
002708270-01 & UZ-Lyr-pri & 1:1 & 87.5 & 2 & 22 & 10.67 & 3.31 & 4.7889E+03 & Direct-PRF & 0\\
002708278-01 & UZ-Lyr-pri & 1:1 & 169.6 & -20 & 38 & 10.67 & 3.81 & 5.8974E+03 & Direct-PRF & 0\\
002708286-01 & UZ-Lyr-pri & 1:1 & 127.6 & 31 & 6 & 10.67 & 4.48 & 3.8139E+03 & Direct-PRF & 0\\
002708343-01 & UZ-Lyr-pri & 1:1 & 160.5 & 37 & 16 & 10.67 & 4.50 & 3.2006E+03 & Direct-PRF & 0\\
002708420-01 & UZ-Lyr-pri & 1:1 & 187.9 & 16 & 45 & 10.67 & 3.24 & 8.3806E+03 & Direct-PRF & 0\\
002708445-01 & UZ-Lyr-pri & 1:1 & 198.1 & 25 & 43 & 10.67 & 4.33 & 4.3926E+03 & Direct-PRF & 0\\
002711123-01 & 002711114-pri & 1:1 & 7.6 & 2 & 0 & 12.34 & 0.19 & 1.0398E+01 & Direct-PRF & 0\\
002711123-02 & 002711114-01 & 2:1 & 7.6 & 2 & 0 & 12.34 & 0.19 & 1.7695E+01 & Direct-PRF & 0\\
002711606-01 & 003339563-pri & 1:1 & 1990.0 & 501 & 0 & 14.18 & -0.41 & 2.8425E+04 & Col-Anomaly & 0\\
002714887-01 & 002714932-02 & 1:1 & 63.6 & -8 & 13 & 14.61 & -0.18 & 1.2963E+00 & Direct-PRF & 1\\
002714932-01 & 002715245-01 & 1:1 & 244.5 & -3 & 62 & 15.96 & -1.34 & 1.2059E+00 & Direct-PRF & 1\\
002714932-02 & 002714887-01 & 1:1 & 63.6 & 8 & -13 & 14.43 & 0.18 & 7.7143E-01 & Direct-PRF & 1\\
002714947-01 & 002715113-01 & 1:1 & 119.8 & 24 & 18 & 15.60 & -2.35 & 3.4333E+00 & Direct-PRF & 1\\
002714954-01 & 002714932-02 & 1:2 & 88.7 & -20 & 8 & 14.61 & -0.07 & 3.8889E+00 & Direct-PRF & 1\\
002715053-01 & 002715245-01 & 1:2 & 140.4 & 4 & 35 & 15.96 & -1.39 & 1.9070E+00 & Direct-PRF & 1\\
002715113-01 & 002715119-01 & 1:1 & 37.8 & -8 & 5 & 14.42 & 1.18 & 4.9515E-01 & Direct-PRF & 1\\
002715119-01 & 002715113-01 & 1:1 & 37.8 & 8 & -5 & 15.60 & -1.18 & 2.0196E+00 & Direct-PRF & 1\\
002715135-02 & 002715398-01 & 1:1 & 202.6 & 2 & 51 & 15.62 & -1.13 & 1.4894E+00 & Direct-PRF & 1\\
002715228-01 & 002715245-01 & 1:2 & 51.1 & -9 & 9 & 15.96 & -0.69 & 1.6735E+00 & Direct-PRF & 1\\
002715245-01 & 002715228-01 & 2:1 & 51.1 & 9 & -9 & 15.27 & 0.69 & 5.9756E-01 & Direct-PRF & 1\\
002715282-01 & 002715119-01 & 1:1 & 152.2 & 7 & -38 & 14.42 & 0.65 & 1.1087E+00 & Direct-PRF & 1\\
002715398-01 & 002715135-02 & 1:1 & 202.6 & -2 & -51 & 14.496 & 1.13 & 1.4894E+00 & Direct-PRF & 1\\
002830919-01 & 003836439-pri & 1:1 & 5110.8 & -763 & 6 & 7.57 & 7.18 & 6.5895E+02 & Col-Anomaly & 2\\
002852528-01 & 002852560-01 & 1:1 & 17.4 & 0 & -4 & 15.31 & 0.40 & 7.3918E+02 & Direct-PRF & 0\\
002860793-01 & 002860788-01 & 1:1 & 20.8 & -5 & 2 & 14.04 & -0.65 & 1.1929E+03 & Direct-PRF & 0\\
002860930-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002969628-02 & 002969638-01 & 1:1 & 6.1 & 0 & 2 & 13.95 & -2.26 & 5.7200E+00 & Direct-PRF & 0\\
002973800-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
002988768-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003003992-01 & 6099.01 & 1:1 & 19.8 & -5 & -2 & 13.93 & -2.77 & 1.8881E+03 & Direct-PRF & 0\\
003097346-01 & 3648.01 & 1:1 & 10.3 & 0 & 3 & 16.94 & -5.38 & 1.7813E+03 & Direct-PRF & 0\\
003098184-01 & 003098194-02 & 6:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 4.4830E+00 & Direct-PRF & 0\\
003098184-02 & 003098194-01 & 12:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 3.9917E+00 & Direct-PRF & 0\\
003098184-03 & 003098194-02 & 12:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 4.9720E+00 & Direct-PRF & 0\\
003098184-04 & 003098194-02 & 13:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 3.6455E+00 & Direct-PRF & 0\\
003098184-05 & 003098194-01 & 12:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 5.1240E+00 & Direct-PRF & 0\\
003098197-01 & 003098194-02 & 1:1 & 5.7 & 0 & -1 & 13.90 & 0.94 & 3.0656E+00 & Direct-PRF & 0\\
003098197-02 & 003098194-01 & 1:1 & 5.7 & 0 & -1 & 13.90 & 0.94 & 3.2466E+00 & Direct-PRF & 0\\
003109937-01 & 1112.01 & 1:1 & 4.8 & 1 & 2 & 14.63 & 1.12 & 1.4660E+00 & Direct-PRF & 0\\
003110937-01 & UZ-Lyr-pri & 1:1 & 1347.3 & -339 & 0 & 10.67 & 4.53 & 9.2308E+03 & Col-Anomaly & 0\\
003114661-01 & 3763.01 & 1:1 & 8.4 & -2 & 1 & 17.38 & -1.63 & 7.1141E+01 & Direct-PRF & 0\\
003117510-01 & 003117511-01 & 1:1 & 0.1 & 0 & 0 & 13.28 & -0.11 & 1.0741E+00 & Direct-PRF & 0\\
003119307-01 & 003119295-pri & 2:1 & 19.7 & -4 & 2 & 14.27 & 1.25 & 4.3061E+03 & Direct-PRF & 0\\
003120276-01 & 003120320-01 & 1:1 & 36.5 & 5 & 8 & 10.88 & 4.33 & 3.2659E+02 & Direct-PRF & 0\\
003120308-01 & 003120320-01 & 1:1 & 38.7 & -7 & 7 & 10.88 & 3.77 & 6.1585E+02 & Direct-PRF & 0\\
003120397-01 & 003120320-01 & 1:1 & 50.3 & -2 & -13 & 10.88 & 4.79 & 6.6468E+02 & Direct-PRF & 0\\
003120889-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003216838-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003218688-01 & 003218683-pri & 1:1 & 23.0 & 5 & 4 & 16.00 & -0.86 & 5.5459E+03 & Direct-PRF & 0\\
003228740-01 & V404-Lyr-pri & 1:1 & 94.1 & -18 & -16 & 11.82 & 1.89 & 2.7441E+04 & Direct-PRF & 0\\
003228804-01 & V404-Lyr-pri & 1:1 & 61.4 & 4 & -14 & 11.82 & 3.19 & 3.9201E+03 & Direct-PRF & 0\\
003228824-01 & V404-Lyr-pri & 1:1 & 59.1 & 7 & -13 & 11.82 & 3.92 & 3.0669E+04 & Direct-PRF & 0\\
003228825-01 & V404-Lyr-pri & 1:1 & 66.0 & -17 & 3 & 11.82 & 0.21 & 1.7379E+04 & Direct-PRF & 0\\
003228918-01 & V404-Lyr-pri & 1:1 & 31.9 & 2 & 8 & 11.82 & 3.38 & 2.3172E+03 & Direct-PRF & 0\\
003228945-01 & V404-Lyr-pri & 1:1 & 84.3 & -7 & 21 & 11.82 & 3.21 & 4.2388E+03 & Direct-PRF & 0\\
003228986-01 & V404-Lyr-pri & 1:1 & 80.4 & 11 & 17 & 11.82 & 2.37 & 7.4481E+03 & Direct-PRF & 0\\
003228988-01 & V404-Lyr-pri & 1:1 & 84.4 & 8 & 20 & 11.82 & 3.50 & 6.2068E+03 & Direct-PRF & 0\\
003229028-01 & V404-Lyr-pri & 1:1 & 182.9 & 46 & 1 & 11.82 & 1.22 & 1.9310E+04 & Direct-PRF & 0\\
003230206-01 & 003230227-pri & 1:1 & 92.9 & 17 & -16 & 9.00 & 6.58 & 2.6133E+02 & Direct-PRF & 0\\
003230227-02 & 965.01 & 1:1 & 17.8 & 2 & -4 & 13.36 & -4.36 & 9.0477E+02 & Direct-PRF & 0\\
003230753-01 & 6101.01 & 1:1 & 23.4 & -1 & -6 & 12.55 & 2.07 & 7.5519E+02 & Direct-PRF & 0\\
003231137-01 & 3643.01 & 1:1 & 8.7 & 1 & 2 & 16.60 & -3.04 & 1.9484E+02 & Direct-PRF & 0\\
003231137-02 & 3643.01 & 1:2 & 8.7 & 1 & 2 & 16.60 & -3.04 & 2.0246E+03 & Direct-PRF & 0\\
003231406-01 & 003231410-03 & 1:1 & 14.2 & -3 & 1 & 13.66 & -3.20 & 7.7965E+00 & Direct-PRF & 1\\
003231406-04 & 003231410-01 & 1:1 & 14.2 & -3 & 1 & 13.66 & -3.20 & 3.0361E+00 & Direct-PRF & 1\\
003231410-01 & 003231406-04 & 1:1 & 14.2 & 3 & -1 & 10.46 & 3.20 & 3.2937E-01 & Direct-PRF & 1\\
003231410-03 & 003231406-01 & 1:1 & 14.2 & 3 & -1 & 10.46 & 3.20 & 1.2826E-01 & Direct-PRF & 1\\
003238059-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003238686-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003241557-01 & 003241619-01 & 1:1 & 48.3 & 5 & 11 & 12.52 & 1.25 & 7.4194E+03 & Direct-PRF & 0\\
003241604-01 & 003241619-01 & 1:1 & 34.6 & -5 & 7 & 12.52 & 2.75 & 1.6434E+03 & Direct-PRF & 0\\
003241662-01 & 003241619-01 & 1:1 & 56.0 & 7 & -13 & 12.52 & 2.67 & 3.0031E+03 & Direct-PRF & 0\\
003247396-01 & 4035.01 & 1:1 & 6.8 & 2 & 0 & 18.53 & -5.77 & 6.0860E+01 & Direct-PRF & 0\\
003248033-01 & 1759.01 & 1:1 & 14.3 & -4 & 0 & 15.39 & -3.23 & 5.7517E+02 & Direct-PRF & 0\\
003324986-01 & 003836439-pri & 1:1 & 3214.5 & -286 & 6 & 7.57 & 7.42 & 4.8527E+02 & Col-Anomaly & 2\\
003327992-01 & 003327980-pri & 1:2 & 9.1 & -2 & -1 & 12.12 & 3.46 & 6.5756E+00 & Direct-PRF & 0\\
003327993-01 & 003327980-pri & 1:2 & 70.6 & 8 & -16 & 12.12 & 3.78 & 1.1872E+03 & Direct-PRF & 0\\
003328026-01 & 003327980-pri & 1:2 & 38.6 & -7 & -7 & 12.12 & 3.03 & 1.1678E+03 & Direct-PRF & 0\\
003328027-01 & 003327980-pri & 1:2 & 51.7 & -3 & -12 & 12.12 & 3.51 & 2.7397E+03 & Direct-PRF & 0\\
003328052-01 & 003327980-pri & 1:2 & 64.2 & -10 & -12 & 12.12 & 3.42 & 1.5656E+03 & Direct-PRF & 0\\
003329643-01 & 003431321-pri & 1:1 & 20.9 & 4 & -2 & 11.20 & 3.76 & 1.3676E+02 & Direct-PRF & 0\\
003329839-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003335813-01 & 003335816-01 & 1:1 & 8.3 & -2 & 1 & 12.08 & 1.71 & 2.7470E+00 & Direct-PRF & 0\\
003336476-01 & UZ-Lyr-pri & 1:1 & 2112.0 & -531 & 1 & 10.67 & 1.74 & 4.2461E+04 & Col-Anomaly & 0\\
003336937-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003337351-01 & 003230227-pri & 1:1 & 17.8 & -2 & 4 & 9.00 & 4.36 & 1.3488E+00 & Direct-PRF & 0\\
003337351-02 & 003230227-pri & 1:1 & 17.8 & -2 & 4 & 9.00 & 4.36 & 1.6894E+02 & Direct-PRF & 0\\
003337425-01 & 003230227-pri & 1:1 & 64.9 & 5 & 16 & 9.00 & 5.93 & 1.7936E+02 & Direct-PRF & 0\\
003337432-01 & 003439031-01 & 1:1 & 82.4 & 19 & -8 & 11.29 & 2.11 & 5.9767E+03 & Direct-PRF & 0\\
003337438-01 & 003439031-01 & 1:1 & 75.1 & 18 & -5 & 11.29 & 2.21 & 7.6423E+03 & Direct-PRF & 0\\
003337548-01 & 003439031-01 & 1:1 & 164.1 & 41 & 1 & 11.29 & 4.38 & 3.8211E+03 & Direct-PRF & 0\\
003338674-01 & 3795.01 & 1:1 & 8.5 & 2 & 1 & 14.81 & -2.10 & 1.0574E+02 & Direct-PRF & 0\\
003339823-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003340312-01 & 3677.01 & 1:1 & 11.0 & -2 & 1 & 16.25 & -1.71 & 9.6672E+01 & Direct-PRF & 0\\
003342628-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003344419-01 & 3764.01 & 1:2 & 11.4 & -3 & 0 & 15.83 & -0.84 & 1.2469E+03 & Direct-PRF & 0\\
003348082-01 & 003348093-01 & 1:1 & 15.2 & -2 & 3 & 16.20 & -1.16 & 9.6777E+02 & Direct-PRF & 0\\
003348533-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003431662-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003437739-01 & UZ-Lyr-pri & 1:1 & 2553.8 & -643 & 0 & 10.67 & 4.67 & 1.1580E+04 & Col-Anomaly & 0\\
003438975-01 & 003439031-01 & 1:1 & 38.3 & -2 & -10 & 11.29 & 1.01 & 4.3568E+03 & Direct-PRF & 0\\
003438976-01 & 003439031-01 & 1:1 & 83.8 & -21 & 3 & 11.29 & 2.82 & 9.7121E+03 & Direct-PRF & 0\\
003439096-01 & 003439031-01 & 1:1 & 45.4 & 6 & 9 & 11.29 & 2.51 & 2.1190E+03 & Direct-PRF & 0\\
003444699-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003445068-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003446451-01 & 3736.01 & 2:1 & 10.6 & 3 & 1 & 16.64 & -4.33 & 8.2250E+02 & Direct-PRF & 0\\
003448230-01 & 003448245-pri & 1:1 & 72.5 & -13 & 13 & 11.86 & 1.99 & 1.3424E+04 & Direct-PRF & 0\\
003448299-01 & 003448245-pri & 1:1 & 44.4 & -6 & -9 & 11.86 & 3.04 & 3.3228E+03 & Direct-PRF & 0\\
003448323-01 & 003448245-pri & 1:1 & 73.0 & -16 & -7 & 11.86 & 3.77 & 2.4319E+03 & Direct-PRF & 0\\
003454720-01 & 003454731-05 & 1:7 & 9.0 & 2 & 0 & 9.63 & 3.16 & 2.4690E+00 & Direct-PRF & 0\\
003542574-01 & 003542573-01 & 1:1 & 10.0 & -2 & 1 & 12.16 & 6.87 & 4.5403E-02 & Direct-PRF & 0\\
003542588-01 & 003542573-01 & 1:1 & 27.1 & -5 & 5 & 12.16 & 1.44 & 8.0782E+02 & Direct-PRF & 0\\
003544689-01 & 003544694-01 & 1:1 & 9.8 & 2 & 2 & 15.93 & -0.98 & 8.4126E+01 & Direct-PRF & 0\\
003546419-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003547178-02 & 003547187-01 & 1:1 & 5.8 & -1 & 1 & 13.05 & -0.64 & 3.4800E+00 & Direct-PRF & 0\\
003556220-01 & 3899.01 & 1:1 & 10.1 & -2 & -2 & 17.66 & -4.28 & 4.8971E+03 & Direct-PRF & 0\\
003557526-01 & 003557421-pri & 2:1 & 85.7 & -20 & 9 & 10.03 & 4.17 & 4.5660E+03 & Direct-PRF & 0\\
003558803-01 & 003558822-pri & 1:1 & 22.7 & 6 & 0 & 12.25 & 0.07 & 3.0466E+02 & Direct-PRF & 0\\
003629430-01 & 003629473-01 & 1:1 & 55.3 & -14 & -2 & 12.80 & 1.67 & 4.0000E-01 & Direct-PRF & 1\\
003629430-02 & 003629474-01 & 1:1 & 75.1 & -2 & 3 & 12.81 & 1.66 & 4.4186E-01 & Direct-PRF & 1\\
003629473-01 & 003629430-01 & 1:1 & 55.3 & 14 & 2 & 14.47 & -1.67 & 2.5000E+00 & Direct-PRF & 1\\
003629474-01 & 003629430-02 & 1:1 & 75.1 & 2 & -3 & 14.47 & -1.66 & 2.2632E+00 & Direct-PRF & 1\\
003644071-01 & 3511.01 & 3:1 & 447.0 & -6 & -1 & 8.35 & 5.86 & 5.7546E+01 & Direct-PRF & 0\\
003644071-02 & 003644542-01 & 3:1 & 447.0 & -6 & -1 & 8.35 & 5.86 & 5.1313E+01 & Direct-PRF & 1\\
003644505-01 & 3511.01 & 1:1 & 198.3 & 38 & 32 & 8.35 & 5.24 & 2.1206E+03 & Direct-PRF & 0\\
003644523-01 & 3511.01 & 1:1 & 55.0 & -13 & -5 & 8.35 & 7.58 & 7.9799E+01 & Direct-PRF & 0\\
003644523-02 & 003644542-01 & 1:1 & 55.0 & -13 & -5 & 8.35 & 7.58 & 8.1432E+01 & Direct-PRF & 0\\
003644602-01 & 003644542-02 & 3:1 & 133.3 & 33 & 5 & 8.35 & -6.79 & 4.7231E+02 & Direct-PRF & 0\\
003644653-01 & 3511.01 & 1:1 & 105.4 & 25 & -10 & 8.35 & 7.55 & 2.0678E+02 & Direct-PRF & 0\\
003644653-02 & 003644542-01 & 1:1 & 105.4 & 25 & -10 & 8.35 & 7.55 & 2.1439E+02 & Direct-PRF & 0\\
003655332-01 & 003655326-01 & 1:1 & 4.2 & -1 & 0 & 14.21 & -0.36 & 2.7662E+00 & Direct-PRF & 0\\
003732894-01 & 003836439-pri & 1:1 & 155.0 & 24 & -31 & 7.57 & 6.73 & 8.5753E+02 & Direct-PRF & 0\\
003735634-01 & 3544.01 & 1:1 & 6.8 & 0 & -2 & 16.14 & -2.23 & 5.4481E+01 & Direct-PRF & 0\\
003762553-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003834360-01 & 003834364-01 & 1:1 & 11.4 & 0 & -3 & 14.66 & 0.06 & 1.0125E+02 & Direct-PRF & 0\\
003836375-01 & 003836439-pri & 1:1 & 66.2 & 16 & 5 & 7.57 & 8.40 & 7.8446E+01 & Direct-PRF & 0\\
003836399-01 & 003836439-pri & 1:1 & 37.7 & 9 & 3 & 7.57 & 6.88 & 1.1060E+02 & Direct-PRF & 0\\
003836399-02 & 003836439-sec & 1:1 & 37.7 & 9 & 3 & 7.57 & 6.88 & 8.7097E+01 & Direct-PRF & 0\\
003836413-01 & 003836439-pri & 1:1 & 27.2 & 7 & 0 & 7.57 & 6.19 & 1.3467E+00 & Direct-PRF & 0\\
003836413-02 & 003836439-pri & 1:2 & 27.2 & 7 & 0 & 7.57 & 6.19 & 1.8849E+00 & Direct-PRF & 0\\
003836450-01 & 003836439-pri & 1:1 & 118.2 & -19 & 23 & 7.57 & 5.76 & 1.1382E+03 & Direct-PRF & 0\\
003836453-01 & 003836439-pri & 1:1 & 37.2 & 3 & -9 & 7.57 & 4.49 & 4.4714E+02 & Direct-PRF & 0\\
003836509-01 & 003836439-pri & 1:1 & 71.8 & -18 & -3 & 7.57 & 5.99 & 1.5048E+02 & Direct-PRF & 0\\
003836522-01 & 003836439-pri & 1:1 & 97.5 & -9 & -23 & 7.57 & 7.27 & 1.3973E+02 & Direct-PRF & 0\\
003836558-01 & 003836439-pri & 1:1 & 126.6 & -18 & -26 & 7.57 & 7.04 & 4.3776E+02 & Direct-PRF & 0\\
003838486-01 & 3700.01 & 1:1 & 10.1 & 2 & 1 & 17.90 & -2.06 & 7.7370E+02 & Direct-PRF & 0\\
003848665-01 & 003644542-01 & 3:1 & 993.1 & -250 & 2 & 8.35 & 6.61 & 6.6404E+01 & Direct-PRF & 0\\
003848948-01 & 5015.01 & 1:1 & 26.0 & 6 & -3 & 13.90 & -3.84 & 9.6882E+04 & Direct-PRF & 0\\
003849014-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
003851134-01 & 003954798-pri & 1:1 & 221.1 & 56 & -1 & 13.61 & -0.13 & 2.4326E+04 & Col-Anomaly & 0\\
003851194-01 & 003954798-pri & 1:1 & 317.7 & 80 & 1 & 13.61 & 0.21 & 4.4359E+04 & Col-Anomaly & 0\\
003858757-01 & 003858884-01 & 1:1 & 119.9 & -1 & -30 & 9.28 & 6.51 & 7.4108E+02 & Direct-PRF & 0\\
003858767-01 & 003352751-pri & 1:1 & 2253.1 & 566 & 1 & 13.44 & 0.80 & 2.3845E+03 & Col-Anomaly & 0\\
003858804-01 & 003858884-01 & 1:1 & 65.2 & 11 & -12 & 9.28 & 4.50 & 5.0783E+02 & Direct-PRF & 0\\
003858804-02 & 003858884-02 & 1:1 & 65.2 & 11 & -12 & 9.28 & 4.50 & 6.0288E+02 & Direct-PRF & 0\\
003858824-01 & 003858884-01 & 1:1 & 61.1 & 14 & -7 & 9.28 & 6.07 & 2.0419E+02 & Direct-PRF & 0\\
003858824-02 & 003858884-02 & 1:1 & 61.1 & 14 & -7 & 9.28 & 6.07 & 2.0430E+02 & Direct-PRF & 0\\
003858851-01 & 003858884-01 & 1:1 & 54.6 & 14 & -1 & 9.28 & 6.49 & 7.6061E+01 & Direct-PRF & 0\\
003858851-02 & 003858884-02 & 1:1 & 54.6 & 14 & -1 & 9.28 & 6.49 & 7.8259E+01 & Direct-PRF & 0\\
003858879-01 & 003858884-01 & 1:1 & 46.4 & 11 & 6 & 9.28 & 5.84 & 1.4180E+02 & Direct-PRF & 0\\
003858879-02 & 003858884-02 & 1:1 & 46.4 & 11 & 6 & 9.28 & 5.84 & 1.4021E+02 & Direct-PRF & 0\\
003858884-03 & 3293.01 & 1:1 & 54.6 & -14 & 1 & 15.77 & -6.49 & 3.5941E+01 & Direct-PRF & 1\\
003858917-01 & 003858884-01 & 1:1 & 33.0 & -8 & 1 & 9.28 & 5.41 & 1.1702E+02 & Direct-PRF & 0\\
003858917-02 & 003858884-02 & 1:1 & 33.0 & -8 & 1 & 9.28 & 5.41 & 1.1709E+02 & Direct-PRF & 0\\
003858919-01 & 003858884-02 & 1:1 & 97.7 & -23 & -7 & 9.28 & 6.72 & 6.9080E+02 & Direct-PRF & 0\\
003858919-02 & 003858884-01 & 1:1 & 97.7 & -23 & -7 & 9.28 & 6.72 & 7.5058E+02 & Direct-PRF & 0\\
003858949-01 & 003858884-01 & 1:1 & 43.0 & -5 & 10 & 9.28 & 5.30 & 3.6493E+02 & Direct-PRF & 0\\
003858949-02 & 003858884-02 & 1:1 & 43.0 & -5 & 10 & 9.28 & 5.30 & 3.5886E+02 & Direct-PRF & 0\\
003858988-01 & 003858884-01 & 1:1 & 90.4 & -20 & 11 & 9.28 & 5.72 & 3.0245E+02 & Direct-PRF & 0\\
003858988-02 & 003858884-02 & 1:1 & 90.4 & -20 & 11 & 9.28 & 5.72 & 2.8734E+02 & Direct-PRF & 0\\
003859151-01 & 003858884-01 & 1:1 & 194.1 & -11 & 48 & 9.28 & 5.60 & 2.6103E+03 & Direct-PRF & 0\\
003859151-02 & 003858884-02 & 1:1 & 194.1 & -11 & 48 & 9.28 & 5.60 & 2.2404E+03 & Direct-PRF & 0\\
003861611-01 & 4.01 & 1:1 & 11.7 & -1 & 3 & 11.43 & 4.42 & 2.6079E+00 & Direct-PRF & 0\\
003962684-01 & 003858884-01 & 1:1 & 108.6 & 27 & 6 & 9.28 & 4.68 & 2.6962E+03 & Direct-PRF & 0\\
003962684-02 & 003858884-02 & 1:1 & 108.6 & 27 & 6 & 9.28 & 4.68 & 2.2404E+03 & Direct-PRF & 0\\
003962728-01 & 003858884-01 & 1:1 & 141.9 & 32 & 17 & 9.28 & 6.47 & 1.3706E+03 & Direct-PRF & 0\\
003962728-02 & 003858884-02 & 1:1 & 141.9 & 32 & 17 & 9.28 & 6.47 & 1.2656E+03 & Direct-PRF & 0\\
003962872-01 & 003858884-02 & 1:1 & 213.5 & 31 & 45 & 9.28 & 4.87 & 3.1580E+03 & Direct-PRF & 0\\
003962872-02 & 003858884-01 & 1:1 & 213.5 & 31 & 45 & 9.28 & 4.87 & 3.5329E+03 & Direct-PRF & 0\\
003964562-01 & 3542.01 & 1:1 & 9.4 & -2 & 2 & 14.78 & -2.37 & 1.8614E+02 & Direct-PRF & 0\\
003964562-02 & 003964545-02 & 1:1 & 9.4 & -2 & 2 & 14.78 & -2.37 & 1.3930E+02 & Direct-PRF & 0\\
004035667-01 & 6107.01 & 1:1 & 13.7 & 1 & -3 & 12.70 & -2.67 & 2.7220E+02 & Direct-PRF & 0\\
004038095-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004043674-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004049108-01 & 5994.01 & 1:1 & 11.7 & 2 & -2 & 14.65 & 0.22 & 2.0476E+02 & Direct-PRF & 0\\
004055774-01 & 5025.01 & 1:1 & 19.6 & -4 & -3 & 14.04 & 1.54 & 4.2580E+02 & Direct-PRF & 0\\
004059887-01 & 5045.01 & 1:1 & 459.4 & 115 & 1 & 14.30 & -1.39 & 2.3604E+04 & Col-Anomaly & 0\\
004073730-01 & 004073707-01 & 1:1 & 9.9 & 0 & -3 & 14.12 & -3.06 & 1.3549E+02 & Direct-PRF & 0\\
004076976-01 & 004076952-pri & 1:2 & 19.5 & -3 & -3 & 13.77 & 0.43 & 2.2769E+03 & Direct-PRF & 0\\
004077006-02 & 004077032-02 & 1:1 & 17.6 & 4 & 1 & 9.69 & 3.69 & 3.8049E+00 & Direct-PRF & 0\\
004079535-01 & 3594.01 & 1:1 & 6.2 & 1 & -1 & 15.56 & -0.48 & 8.7852E+00 & Direct-PRF & 0\\
004079535-02 & 004079530-02 & 1:1 & 6.2 & 1 & -1 & 15.56 & -0.48 & 9.1567E+00 & Direct-PRF & 0\\
004136253-01 & 004136285-02 & 1:2 & 96.1 & 10 & -22 & 6.51 & 9.15 & 4.3182E-01 & Direct-PRF & 0\\
004136314-02 & 004136285-01 & 1:1 & 46.1 & 3 & 11 & 6.51 & 7.28 & 5.8824E-02 & Direct-PRF & 0\\
004136396-01 & 004136285-02 & 1:2 & 130.9 & 17 & 28 & 6.51 & 9.10 & 1.9000E-01 & Direct-PRF & 0\\
004136749-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004144231-01 & 6109.01 & 1:1 & 15.7 & -2 & 3 & 11.86 & 3.61 & 4.5641E+01 & Direct-PRF & 0\\
004144236-02 & 1791.01 & 1:1 & 15.7 & 2 & -3 & 15.47 & -3.61 & 9.6095E+00 & Direct-PRF & 1\\
004144238-01 & 6109.01 & 1:1 & 25.2 & 3 & -6 & 11.86 & 1.90 & 8.7732E+02 & Direct-PRF & 0\\
004150496-01 & 3156.03 & 1:1 & 98.0 & 24 & -7 & 7.90 & 7.64 & 1.3551E+02 & Direct-PRF & 0\\
004150496-02 & 004150611-sec & 1:1 & 98.0 & 24 & -7 & 7.90 & 7.64 & 1.3351E+02 & Direct-PRF & 0\\
004150496-03 & 004150611-03 & 1:1 & 98.0 & 24 & -7 & 7.90 & 7.64 & 1.1483E+02 & Direct-PRF & 0\\
004150539-01 & 3156.03 & 1:1 & 50.1 & 11 & -6 & 7.90 & 7.80 & 5.9596E+01 & Direct-PRF & 0\\
004150539-02 & 004150611-sec & 1:1 & 50.1 & 11 & -6 & 7.90 & 7.80 & 5.1710E+01 & Direct-PRF & 0\\
004150539-03 & 004150611-03 & 1:1 & 50.1 & 11 & -6 & 7.90 & 7.80 & 6.9785E+01 & Direct-PRF & 0\\
004150624-01 & 3156.03 & 1:1 & 69.4 & 14 & 11 & 7.90 & 7.56 & 1.0599E+02 & Direct-PRF & 0\\
004150624-02 & 004150611-sec & 1:1 & 69.4 & 14 & 11 & 7.90 & 7.56 & 8.6824E+01 & Direct-PRF & 0\\
004150624-03 & 004150611-03 & 1:1 & 69.4 & 14 & 11 & 7.90 & 7.56 & 1.3321E+02 & Direct-PRF & 0\\
004150701-01 & 004150611-sec & 1:1 & 97.5 & -24 & 1 & 7.90 & 7.96 & 1.0384E+02 & Direct-PRF & 0\\
004150701-02 & 3156.03 & 1:1 & 97.5 & -24 & 1 & 7.90 & 7.96 & 1.2373E+02 & Direct-PRF & 0\\
004150703-01 & 004150611-sec & 1:1 & 96.6 & -24 & 3 & 7.90 & 6.92 & 4.0472E+02 & Direct-PRF & 0\\
004160676-01 & 004160683-02 & 1:1 & 10.9 & -3 & -1 & 15.75 & -0.60 & 1.4941E+00 & Direct-PRF & 0\\
004160683-01 & 004160676-02 & 1:1 & 10.9 & 3 & 1 & 15.15 & 0.60 & 1.3431E+00 & Direct-PRF & 0\\
004245861-01 & 004245897-pri & 1:1 & 59.0 & 6 & -13 & 12.54 & 3.36 & 2.7471E+03 & Direct-PRF & 0\\
004245933-01 & 004245897-pri & 1:1 & 34.7 & -9 & 1 & 12.54 & 3.29 & 1.1319E+03 & Direct-PRF & 0\\
004247807-01 & 004247791-pri & 1:2 & 13.9 & -4 & -1 & 11.26 & 3.55 & 1.9552E+01 & Direct-PRF & 0\\
004247811-01 & 004247791-pri & 1:2 & 44.7 & -10 & -6 & 11.26 & 3.09 & 2.4440E+03 & Direct-PRF & 0\\
004285107-01 & 6112.01 & 1:1 & 19.0 & 2 & -4 & 12.79 & 1.20 & 1.1556E+03 & Direct-PRF & 0\\
004349442-02 & 004349452-01 & 1:1 & 8.4 & 1 & -1 & 10.73 & 2.53 & 4.7040E+00 & Direct-PRF & 0\\
004349442-03 & 244.02 & 1:1 & 8.4 & 1 & -1 & 10.73 & 2.53 & 3.9126E+00 & Direct-PRF & 0\\
004356621-01 & 004356766-01 & 1:1 & 251.7 & 63 & 1 & 15.45 & -0.43 & 9.9409E+02 & Col-Anomaly & 0\\
004357985-01 & 3156.03 & 1:1 & 712.6 & 180 & 0 & 7.90 & 7.52 & 1.5382E+02 & Direct-PRF & 0\\
004357985-02 & 004150611-sec & 1:1 & 712.6 & 180 & 0 & 7.90 & 7.52 & 1.9470E+02 & Direct-PRF & 0\\
004365442-01 & 5058.01 & 1:1 & 19.0 & -5 & 1 & 13.31 & -0.01 & 2.0846E+03 & Direct-PRF & 0\\
004372768-01 & 3698.01 & 1:1 & 9.1 & -1 & 1 & 18.23 & -2.32 & 1.7950E+02 & Direct-PRF & 0\\
004372768-02 & 004372765-sec & 1:1 & 9.1 & -1 & 1 & 18.23 & -2.32 & 1.2265E+02 & Direct-PRF & 0\\
004373195-01 & V1130-Cyg-pri & 1:1 & 1112.4 & 280 & 0 & 12.32 & -3.20 & 2.0063E+05 & Col-Anomaly & 0\\
004376629-01 & 397.01 & 1:1 & 9.5 & 1 & -2 & 13.77 & -0.09 & 6.1742E+01 & Direct-PRF & 0\\
004379599-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004384652-01 & 004482641-01 & 1:1 & 337.7 & -85 & 0 & 15.00 & -1.03 & 3.3756E+00 & Col-Anomaly & 0\\
004384652-02 & 004482641-01 & 1:1 & 337.7 & -85 & 0 & 15.00 & -1.03 & 4.1375E+00 & Col-Anomaly & 0\\
004384675-05 & 004482641-01 & 1:1 & 354.9 & -89 & 0 & 15.00 & -0.29 & 1.6627E+00 & Col-Anomaly & 0\\
004386059-01 & 3659.01 & 1:1 & 10.6 & -1 & -3 & 16.94 & -3.06 & 9.7201E+02 & Direct-PRF & 0\\
004386121-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004446299-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004458984-01 & 004458989-pri & 1:1 & 23.1 & -4 & -4 & 12.95 & 3.02 & 9.8500E+03 & Direct-PRF & 0\\
004474645-01 & 004474637-01 & 1:1 & 4.6 & 1 & 1 & 16.81 & -2.61 & 1.1122E+02 & Direct-PRF & 0\\
004474645-02 & 004474637-sec & 1:1 & 4.6 & 1 & 1 & 16.81 & -2.61 & 4.1707E+02 & Direct-PRF & 0\\
004482348-01 & 004482641-01 & 1:1 & 302.9 & 76 & 0 & 15.00 & -0.85 & 8.4347E+00 & Col-Anomaly & 0\\
004482738-01 & 004579598-01 & 1:1 & 136.2 & -34 & -2 & 13.79 & -0.84 & 3.7500E-01 & Direct-PRF & 1\\
004482738-02 & 004579598-01 & 1:1 & 136.2 & -34 & -2 & 13.79 & -0.84 & 4.4681E-01 & Direct-PRF & 1\\
004484251-01 & 004484252-01 & 1:1 & 1.7 & 0 & 0 & 11.75 & -0.11 & 1.0270E+00 & Direct-PRF & 0\\
004484312-01 & 6112.01 & 1:1 & 1125.9 & 284 & 1 & 12.79 & 0.40 & 1.0111E+04 & Col-Anomaly & 0\\
004544571-01 & 004544587-pri & 1:1 & 28.2 & 4 & -5 & 10.80 & 4.95 & 1.2342E+03 & Direct-PRF & 0\\
004544571-02 & 004544587-sec & 1:1 & 28.2 & 4 & -5 & 10.80 & 4.95 & 1.0668E+03 & Direct-PRF & 0\\
004544572-01 & 004544587-pri & 1:1 & 36.6 & 1 & -9 & 10.80 & 4.94 & 1.2176E+03 & Direct-PRF & 0\\
004544572-03 & 004544587-sec & 1:1 & 36.6 & 1 & -9 & 10.80 & 4.94 & 9.6608E+02 & Direct-PRF & 0\\
004544620-01 & 004544587-pri & 1:1 & 52.0 & -1 & 13 & 10.80 & 5.07 & 1.1376E+03 & Direct-PRF & 0\\
004544620-02 & 004544587-sec & 1:1 & 52.0 & -1 & 13 & 10.80 & 5.07 & 1.1572E+03 & Direct-PRF & 0\\
004544623-01 & 004544587-pri & 1:1 & 43.7 & -11 & 0 & 10.80 & 5.20 & 4.0696E+02 & Direct-PRF & 0\\
004544623-02 & 004544587-sec & 1:1 & 43.7 & -11 & 0 & 10.80 & 5.20 & 3.9939E+02 & Direct-PRF & 0\\
004544628-02 & 004544587-pri & 1:3 & 112.9 & 7 & 28 & 10.80 & 1.74 & 2.6500E+04 & Direct-PRF & 0\\
004544684-01 & 004544587-pri & 1:1 & 120.9 & -15 & 27 & 10.80 & 4.12 & 5.2384E+03 & Direct-PRF & 0\\
004547321-01 & 004547308-pri & 1:1 & 18.7 & -3 & 3 & 12.54 & 1.39 & 5.5563E+03 & Direct-PRF & 0\\
004555642-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004568117-01 & V1130-Cyg-pri & 1:1 & 88.9 & 2 & -22 & 12.32 & 1.22 & 2.5079E+04 & Direct-PRF & 0\\
004568298-01 & V1130-Cyg-pri & 1:1 & 99.0 & 25 & 3 & 12.32 & 3.63 & 1.9083E+02 & Direct-PRF & 0\\
004570931-01 & 1658.01 & 1:1 & 9.6 & 0 & -2 & 13.31 & 0.34 & 5.1886E+01 & Direct-PRF & 0\\
004579313-01 & 004579321-01 & 1:1 & 7.3 & -1 & 2 & 17.39 & -2.58 & 4.7318E+02 & Direct-PRF & 0\\
004579313-02 & 004579321-02 & 2:1 & 7.3 & -1 & 2 & 17.39 & -2.58 & 9.9284E+02 & Direct-PRF & 0\\
004579598-01 & 004482738-02 & 1:1 & 136.2 & 34 & 2 & 12.95 & 0.84 & 2.2381E+00 & Direct-PRF & 1\\
004584865-01 & 5335.01 & 1:1 & 10889.0 & -13 & 0 & 11.39 & 1.19 & 1.1915E+04 & Col-Anomaly & 2\\
004636565-01 & 004445630-01 & 1:1 & 1217.5 & 306 & 0 & 13.86 & -1.35 & 1.1943E+04 & Col-Anomaly & 0\\
004640983-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004645823-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004649173-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004659405-01 & 3691.01 & 1:1 & 9.9 & 2 & -1 & 16.03 & -2.10 & 1.7175E+02 & Direct-PRF & 0\\
004659405-02 & 004751083-02 & 1:1 & 9.9 & 2 & -1 & 16.03 & -2.10 & 1.7539E+02 & Direct-PRF & 0\\
004665991-01 & 004665989-pri & 1:2 & 35.6 & -8 & -4 & 13.02 & 1.65 & 6.3109E+03 & Direct-PRF & 0\\
004666008-01 & 004665989-pri & 1:1 & 19.3 & 4 & -3 & 13.02 & 1.42 & 1.3256E+03 & Direct-PRF & 0\\
004677282-01 & 004677321-pri & 1:1 & 19.3 & 4 & -3 & 13.48 & -0.32 & 8.9910E+02 & Direct-PRF & 0\\
004678873-01 & 004678875-01 & 1:1 & 4.9 & -1 & -1 & 13.24 & -0.52 & 7.8982E+00 & Direct-PRF & 0\\
004678919-01 & 004678875-01 & 1:1 & 29.3 & 2 & 7 & 13.24 & 0.45 & 9.2543E+03 & Direct-PRF & 0\\
004739565-01 & 004739791-pri & 1:1 & 353.3 & 89 & 0 & 14.70 & -0.53 & 6.8208E+03 & Col-Anomaly & 0\\
004740688-01 & 004740676-pri & 1:1 & 19.3 & 2 & 4 & 13.20 & 2.53 & 6.2353E+02 & Direct-PRF & 0\\
004743513-01 & 3572.01 & 1:1 & 4.3 & 0 & -1 & 14.55 & -1.59 & 1.6380E+01 & Direct-PRF & 0\\
004743513-02 & 004743508-02 & 1:1 & 4.3 & 0 & -1 & 14.55 & -1.59 & 4.9278E+00 & Direct-PRF & 0\\
004768756-01 & 6134.01 & 1:1 & 8066.6 & -2 & 11 & 11.94 & 0.69 & 1.3929E+04 & Cross-Talk & 0\\
004769824-01 & 5086.01 & 1:1 & 22.7 & -6 & 1 & 10.95 & 4.46 & 1.1195E+02 & Direct-PRF & 0\\
004769931-01 & 004678875-01 & 1:1 & 448.1 & 112 & 1 & 13.24 & 0.66 & 8.1939E+03 & Col-Anomaly & 0\\
004819950-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004831251-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004832175-01 & 004832197-pri & 1:2 & 18.2 & 3 & 4 & 11.51 & 4.25 & 4.7674E+01 & Direct-PRF & 0\\
004832225-01 & 004832197-pri & 1:1 & 39.0 & -10 & -1 & 11.51 & -2.44 & 4.5556E+02 & Direct-PRF & 1\\
004839411-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004842623-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004847782-01 & 004847832-01 & 1:1 & 34.8 & -6 & 7 & 12.45 & 2.63 & 1.2288E+03 & Direct-PRF & 0\\
004847782-02 & 004847832-02 & 1:1 & 34.8 & -6 & 7 & 12.45 & 2.63 & 8.9092E+02 & Direct-PRF & 0\\
004847843-01 & 004847832-02 & 1:1 & 17.4 & -2 & -3 & 12.45 & 0.96 & 7.8778E+02 & Direct-PRF & 0\\
004847843-02 & 004847832-01 & 1:1 & 17.4 & -2 & -3 & 12.45 & 0.96 & 9.4677E+02 & Direct-PRF & 0\\
004848321-01 & 3560.01 & 1:1 & 87.0 & -21 & 5 & 11.82 & 3.20 & 4.8130E+03 & Direct-PRF & 0\\
004848424-01 & 3560.01 & 1:1 & 83.1 & -18 & -11 & 11.82 & 2.94 & 4.1920E+03 & Direct-PRF & 0\\
004848532-01 & 3560.01 & 1:1 & 80.3 & 2 & -21 & 11.82 & 3.11 & 3.3321E+03 & Direct-PRF & 0\\
004850661-01 & 004850677-01 & 1:1 & 12.5 & 2 & 2 & 14.81 & 0.08 & 0.5778E-01 & Direct-PRF & 1\\
004850677-01 & 004850661-01 & 1:1 & 12.5 & -2 & -2 & 14.88 & -0.08 & 1.7308E+00 & Direct-PRF & 1\\
004850809-01 & 004851168-01 & 2:1 & 258.8 & -5 & 65 & 13.31 & 0.78 & 2.3214E+00 & Direct-PRF & 1\\
004851145-01 & 004851217-pri & 1:2 & 90.8 & 22 & -2 & 11.11 & 4.53 & 2.4825E+03 & Direct-PRF & 0\\
004851168-01 & 004850809-01 & 1:2 & 258.8 & 5 & -65 & 14.09 & -0.78 & 4.3077E-01 & Direct-PRF & 1\\
004851173-01 & 004482641-01 & 1:1 & 1641.9 & 413 & 0 & 15.00 & -1.52 & 1.0533E+00 & Col-Anomaly & 0\\
004851173-02 & 004482641-01 & 1:1 & 1641.9 & 413 & 0 & 15.00 & -1.52 & 1.2831E+00 & Col-Anomaly & 0\\
004851182-02 & 004482641-01 & 1:1 & 1635.5 & 411 & 0 & 15.00 & -0.15 & 1.9786E+00 & Col-Anomaly & 0\\
004851195-01 & 004482641-01 & 1:1 & 1618.1 & 407 & 1 & 15.00 & -0.49 & 5.9001E+00 & Col-Anomaly & 0\\
004851239-01 & 004851217-pri & 1:2 & 77.6 & -19 & 6 & 11.11 & 0.33 & 1.5277E+04 & Direct-PRF & 0\\
004851283-01 & 004851217-pri & 1:1 & 49.2 & -10 & -8 & 11.11 & 0.80 & 5.6102E+02 & Direct-PRF & 0\\
004851283-02 & 004851217-sec & 1:1 & 49.2 & -10 & -8 & 11.11 & 0.80 & 5.4685E+02 & Direct-PRF & 0\\
004851338-01 & 004851217-pri & 1:2 & 95.9 & 2 & -24 & 11.11 & 3.90 & 3.1524E+03 & Direct-PRF & 0\\
004851356-01 & 004851217-pri & 1:2 & 97.1 & -2 & -24 & 11.11 & 3.60 & 2.6480E+03 & Direct-PRF & 0\\
004861527-01 & 004773155-01 & 1:1 & 22.2 & 5 & 2 & 13.59 & 0.27 & 1.7332E+03 & Direct-PRF & 0\\
004861527-02 & 004773155-02 & 1:1 & 22.2 & 5 & 2 & 13.59 & 0.27 & 1.4940E+03 & Direct-PRF & 0\\
004861791-01 & 4278.01 & 1:2 & 16.5 & -4 & -1 & 15.99 & -0.04 & 2.1841E+00 & Direct-PRF & 1\\
004908774-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004913000-01 & 5997.01 & 1:1 & 9.3 & 2 & 0 & 11.30 & 0.37 & 6.0535E+01 & Direct-PRF & 0\\
004913858-01 & 005001655-01 & 1:1 & 241.3 & -4 & -60 & 15.08 & -0.19 & 0.6600E+00 & Direct-PRF & 1\\
004914399-01 & 004826439-01 & 1:1 & 255.5 & 64 & 0 & 13.82 & 0.64 & 3.1787E+03 & Col-Anomaly & 0\\
004914709-01 & 3156.03 & 1:1 & 3293.4 & 829 & 0 & 7.90 & 7.74 & 1.0292E+02 & Col-Anomaly & 0\\
004914709-02 & 004150611-sec & 1:1 & 3293.4 & 829 & 0 & 7.90 & 7.74 & 1.5815E+02 & Col-Anomaly & 0\\
004914737-01 & 004150611-sec & 1:1 & 3255.1 & 819 & 0 & 7.90 & 7.21 & 2.8398E+02 & Col-Anomaly & 0\\
004914737-02 & 3156.03 & 1:1 & 3255.1 & 819 & 0 & 7.90 & 7.21 & 2.2857E+02 & Col-Anomaly & 0\\
004914771-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004916845-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004929615-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004932689-01 & 004932691-01 & 1:1 & 16.9 & -4 & 2 & 13.63 & 1.93 & 4.8192E+02 & Direct-PRF & 0\\
004935198-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004936020-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004936284-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
004945547-01 & 004945588-sec & 1:2 & 52.9 & 13 & -1 & 11.15 & 3.31 & 1.1667E+03 & Direct-PRF & 0\\
004946049-01 & 004678875-01 & 1:1 & 1061.1 & 267 & 0 & 13.24 & -0.29 & 2.9134E+04 & Col-Anomaly & 0\\
004949027-01 & 005036538-01 & 1:1 & 43.2 & -11 & 0 & 13.35 & 1.79 & 4.3147E+03 & Direct-PRF & 0\\
004949769-01 & 004949770-pri & 1:1 & 13.7 & 3 & 2 & 12.57 & 2.35 & 9.4097E+02 & Direct-PRF & 0\\
004949769-02 & 004949770-pri & 1:1 & 13.7 & 3 & 2 & 12.57 & 2.35 & 1.3416E+03 & Direct-PRF & 0\\
004949795-01 & 004949770-pri & 1:1 & 23.9 & -6 & 1 & 12.57 & 2.34 & 2.4636E+03 & Direct-PRF & 0\\
004949801-01 & 004949770-pri & 1:1 & 40.8 & 6 & 8 & 12.57 & 3.04 & 1.7152E+03 & Direct-PRF & 0\\
004949825-01 & 004949770-pri & 1:1 & 30.0 & -4 & 7 & 12.57 & 2.54 & 2.0846E+03 & Direct-PRF & 0\\
005001655-01 & 004913858-01 & 1:1 & 241.3 & 4 & 60 & 14.89 & 0.19 & 1.5152E+00 & Direct-PRF & 1\\
005020044-01 & 3688.01 & 1:1 & 6.9 & 0 & -1 & 15.81 & -1.98 & 7.5579E+02 & Direct-PRF & 0\\
005020319-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005021176-01 & 3679.01 & 1:1 & 7.3 & 1 & 1 & 17.70 & -2.84 & 5.7568E+02 & Direct-PRF & 0\\
005021176-02 & 3679.01 & 1:2 & 7.3 & 1 & 1 & 17.70 & -2.84 & 3.5464E+03 & Direct-PRF & 0\\
005021737-01 & 005021732-01 & 1:1 & 4.5 & 0 & -1 & 13.62 & -1.63 & 1.1255E+01 & Direct-PRF & 0\\
005021737-02 & 005021732-02 & 1:1 & 4.5 & 0 & -1 & 13.62 & -1.63 & 1.1015E+01 & Direct-PRF & 0\\
005022943-01 & 005022908-pri & 1:1 & 42.6 & 11 & 0 & 14.31 & -0.44 & 6.6500E+03 & Direct-PRF & 0\\
005023956-01 & 3570.01 & 1:1 & 8.9 & 2 & 0 & 15.05 & -0.44 & 3.8377E+01 & Direct-PRF & 0\\
005024126-01 & 4286.01 & 1:1 & 20.5 & -3 & 4 & 14.96 & 0.66 & 2.0994E+00 & Direct-PRF & 1\\
005024252-01 & 005024292-01 & 1:1 & 19.0 & -2 & 5 & 14.57 & -1.25 & 2.5539E+03 & Direct-PRF & 0\\
005024268-01 & 005024292-01 & 1:1 & 16.5 & -4 & 2 & 14.57 & -3.21 & 3.9322E+03 & Direct-PRF & 0\\
005024414-01 & 1544.01 & 1:1 & 12.4 & -1 & 3 & 15.06 & -2.36 & 4.1745E+02 & Direct-PRF & 0\\
005024482-01 & 1544.01 & 1:1 & 11.7 & 1 & -2 & 15.06 & -2.86 & 9.2767E+01 & Direct-PRF & 0\\
005033298-01 & 006549623-01 & 1:2 & 7743.0 & 30 & 7 & 13.09 & 0.26 & 4.4000E+00 & Direct-PRF & 1\\
005036480-01 & 005036538-01 & 1:1 & 35.2 & -1 & -8 & 13.35 & 1.86 & 2.7072E+03 & Direct-PRF & 0\\
005036491-01 & 005036493-01 & 1:1 & 3.9 & 1 & 0 & 12.55 & 0.56 & 2.5600E+00 & Direct-PRF & 0\\
005036516-01 & 005036538-01 & 1:1 & 6.7 & 0 & -1 & 13.35 & 0.99 & 1.1004E+01 & Direct-PRF & 0\\
005036537-01 & 005036538-01 & 1:1 & 11.7 & -3 & -1 & 13.35 & 2.21 & 5.2806E+01 & Direct-PRF & 0\\
005078025-01 & 005077994-pri & 1:1 & 34.3 & 8 & -4 & 12.67 & 2.37 & 2.7023E+03 & Direct-PRF & 0\\
005078025-02 & 005077994-sec & 1:1 & 34.3 & 8 & -4 & 12.67 & 2.37 & 2.6814E+03 & Direct-PRF & 0\\
005097454-01 & 005097446-pri & 1:1 & 9.5 & 0 & -2 & 13.89 & 1.42 & 6.1743E+02 & Direct-PRF & 0\\
005097470-01 & 005097446-pri & 1:1 & 23.2 & -5 & -2 & 13.89 & 0.60 & 5.6873E+03 & Direct-PRF & 0\\
005108214-01 & 3688.01 & 1:1 & 89.7 & -22 & 1 & 15.81 & -7.97 & 4.9266E+03 & Col-Anomaly & 0\\
005111544-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005114470-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005114623-01 & 003858884-01 & 15:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 7.6802E+01 & Cross-Talk & 0\\
005123246-02 & 005123176-pri & 1:1 & 51.0 & -11 & 7 & 11.46 & 3.50 & 6.5512E+03 & Direct-PRF & 0\\
005130369-01 & 3707.01 & 1:1 & 5.9 & 0 & 1 & 16.30 & -2.45 & 3.6035E+01 & Direct-PRF & 0\\
005130369-02 & 005130380-02 & 1:1 & 5.9 & 0 & 1 & 16.30 & -2.45 & 3.0112E+01 & Direct-PRF & 0\\
005181817-01 & 3638.01 & 1:1 & 9.9 & 0 & -2 & 15.93 & -2.72 & 3.1447E+02 & Direct-PRF & 0\\
005193384-01 & 005193386-01 & 1:1 & 8.2 & 1 & -1 & 14.00 & 5.07 & 8.2260E-01 & Direct-PRF & 1\\
005193386-01 & 005193384-01 & 1:1 & 8.2 & -1 & 1 & 19.07 & -5.07 & 1.2157E+00 & Direct-PRF & 1\\
005193386-02 & 3637.01 & 1:1 & 8.2 & -1 & 1 & 19.07 & -5.07 & 3.7709E+00 & Direct-PRF & 0\\
005193400-01 & 3637.01 & 1:2 & 16.6 & 4 & 2 & 19.07 & -3.38 & 1.1867E+03 & Direct-PRF & 0\\
005201115-01 & 005288543-pri & 1:1 & 351.4 & 88 & 0 & 13.59 & -0.72 & 3.5230E+03 & Col-Anomaly & 0\\
005201115-02 & 005288543-pri & 1:2 & 351.4 & 88 & 0 & 13.59 & -0.72 & 9.5781E+03 & Col-Anomaly & 0\\
005201593-01 & 005201619-pri & 1:1 & 21.3 & 1 & 5 & 13.05 & 0.59 & 1.4239E+04 & Direct-PRF & 0\\
005201596-01 & 005201619-pri & 1:1 & 50.2 & 8 & 9 & 13.05 & 1.98 & 7.5226E+03 & Direct-PRF & 0\\
005201676-01 & 005201619-pri & 1:1 & 57.4 & 14 & -1 & 13.05 & 1.53 & 1.0776E+04 & Direct-PRF & 0\\
005201695-01 & 005201619-pri & 1:1 & 51.7 & 3 & -12 & 13.05 & 2.63 & 5.9507E+03 & Direct-PRF & 0\\
005215980-01 & 005215999-pri & 1:1 & 8.6 & 1 & 1 & 14.11 & 1.10 & 1.4541E+02 & Direct-PRF & 0\\
005217891-01 & 005217733-pri & 1:1 & 98.9 & -18 & -17 & 7.39 & 8.26 & 7.1006E+01 & Direct-PRF & 0\\
005264764-01 & 005264818-pri & 1:1 & 73.0 & 2 & -19 & 8.86 & 6.32 & 3.6027E+02 & Direct-PRF & 0\\
005264764-02 & 005264818-sec & 1:1 & 73.0 & 2 & -19 & 8.86 & 6.32 & 3.0641E+02 & Direct-PRF & 0\\
005264888-01 & 005264818-sec & 1:2 & 85.1 & 21 & 6 & 8.86 & 6.41 & 2.3900E+04 & Direct-PRF & 0\\
005272571-01 & 005097446-pri & 1:1 & 975.9 & 245 & 1 & 13.89 & -1.41 & 1.9229E+04 & Col-Anomaly & 0\\
005282049-02 & 502.01 & 1:2 & 8.3 & 2 & -1 & 14.28 & 0.89 & 1.2312E+00 & Direct-PRF & 0\\
005282051-01 & 1545.01 & 1:1 & 8.3 & -2 & 1 & 15.17 & -0.89 & 8.1026E+01 & Direct-PRF & 0\\
005288071-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005288570-01 & 005288543-pri & 1:2 & 23.9 & -1 & -6 & 13.59 & -0.60 & 1.3932E+03 & Direct-PRF & 0\\
005288577-01 & 005288543-pri & 1:2 & 25.8 & 0 & -7 & 13.59 & 0.01 & 2.0298E+03 & Direct-PRF & 0\\
005289959-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005298620-01 & V380-Cyg-pri & 1:1 & 396.0 & -82 & -56 & 5.77 & 9.93 & 9.2314E+02 & Direct-PRF & 0\\
005303551-01 & 3982.01 & 1:1 & 4.8 & 1 & 0 & 16.49 & -1.61 & 2.0935E+01 & Direct-PRF & 0\\
005305404-01 & 005217733-pri & 1:1 & 49.4 & 12 & -2 & 7.39 & 7.33 & 2.9694E+01 & Direct-PRF & 0\\
005305404-02 & 005217733-sec & 1:1 & 49.4 & 12 & -2 & 7.39 & 7.33 & 3.2497E+01 & Direct-PRF & 0\\
005305451-01 & 005217733-pri & 1:1 & 100.2 & 21 & -14 & 7.39 & 8.01 & 3.0530E+01 & Direct-PRF & 0\\
005305471-01 & 005217733-pri & 1:1 & 52.2 & 8 & -10 & 7.39 & 6.79 & 4.5512E+01 & Direct-PRF & 0\\
005306383-02 & 005306368-01 & 1:1 & 5.4 & -1 & -1 & 15.59 & -2.27 & 2.7273E+00 & Direct-PRF & 0\\
005308387-01 & 3887.01 & 1:2 & 13.8 & 4 & 1 & 13.48 & -0.60 & 4.4719E+00 & Direct-PRF & 0\\
005308419-01 & 2724.01 & 1:1 & 13.8 & -4 & -1 & 12.88 & 0.60 & 1.0928E+00 & Direct-PRF & 0\\
005308663-01 & 2718.01 & 1:1 & 13.5 & -3 & 1 & 13.82 & 1.77 & 1.2535E+00 & Direct-PRF & 0\\
005308666-01 & 1562.01 & 1:1 & 13.5 & 3 & -1 & 15.59 & -1.77 & 7.9579E+00 & Direct-PRF & 0\\
005371013-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005371090-01 & 005371109-pri & 1:1 & 13.6 & -1 & 3 & 13.97 & -0.47 & 3.2250E+03 & Direct-PRF & 0\\
005371796-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005373377-01 & 003973002-sec & 1:3 & 6413.6 & 283 & 0 & 14.98 & -1.03 & 6.2391E+02 & Col-Anomaly & 2\\
005376624-01 & 005376552-sec & 1:1 & 55.7 & 11 & -9 & 12.86 & 1.58 & 6.4957E+03 & Direct-PRF & 0\\
005376624-02 & 005376552-pri & 1:1 & 55.7 & 11 & -9 & 12.86 & 1.58 & 6.1392E+03 & Direct-PRF & 0\\
005376642-01 & 005376552-sec & 1:1 & 66.6 & 13 & -11 & 12.86 & 1.50 & 1.1742E+04 & Direct-PRF & 0\\
005385139-01 & V380-Cyg-pri & 1:1 & 372.1 & 32 & -87 & 5.77 & 10.07 & 6.3567E+02 & Direct-PRF & 0\\
005385139-02 & V380-Cyg-sec & 1:1 & 372.1 & 32 & -87 & 5.77 & 10.07 & 7.1687E+02 & Direct-PRF & 0\\
005385150-01 & V380-Cyg-pri & 1:1 & 368.9 & 28 & -88 & 5.77 & 9.70 & 8.4756E+02 & Direct-PRF & 0\\
005385150-02 & V380-Cyg-sec & 1:1 & 368.9 & 28 & -88 & 5.77 & 9.70 & 1.0003E+03 & Direct-PRF & 0\\
005385187-01 & V380-Cyg-sec & 1:1 & 340.4 & 36 & -77 & 5.77 & 10.08 & 4.4804E+02 & Direct-PRF & 0\\
005385187-02 & V380-Cyg-pri & 1:2 & 340.4 & 36 & -77 & 5.77 & 10.08 & 9.0583E+02 & Direct-PRF & 0\\
005385269-01 & V380-Cyg-pri & 1:1 & 323.9 & 0 & -81 & 5.77 & 8.56 & 1.2387E+03 & Direct-PRF & 0\\
005385269-02 & V380-Cyg-sec & 1:1 & 323.9 & 0 & -81 & 5.77 & 8.56 & 1.1521E+03 & Direct-PRF & 0\\
005385410-02 & V380-Cyg-pri & 1:1 & 318.2 & -31 & -74 & 5.77 & 7.81 & 2.1960E+03 & Direct-PRF & 0\\
005385410-03 & V380-Cyg-sec & 1:1 & 318.2 & -31 & -74 & 5.77 & 7.81 & 2.3461E+03 & Direct-PRF & 0\\
005385439-01 & V380-Cyg-pri & 1:1 & 200.5 & 4 & -50 & 5.77 & 8.38 & 6.6179E+02 & Direct-PRF & 0\\
005385439-02 & V380-Cyg-sec & 1:1 & 200.5 & 4 & -50 & 5.77 & 8.38 & 6.6513E+02 & Direct-PRF & 0\\
005385469-01 & V380-Cyg-pri & 1:1 & 355.9 & -50 & -74 & 5.77 & 7.32 & 2.6351E+03 & Direct-PRF & 0\\
005385471-01 & V380-Cyg-pri & 1:1 & 166.8 & 15 & -39 & 5.77 & 10.22 & 1.3686E+02 & Direct-PRF & 0\\
005385471-02 & V380-Cyg-sec & 1:1 & 166.8 & 15 & -39 & 5.77 & 10.22 & 1.3640E+02 & Direct-PRF & 0\\
005385491-01 & V380-Cyg-pri & 1:1 & 212.2 & -14 & -51 & 5.77 & 7.81 & 1.1978E+03 & Direct-PRF & 0\\
005385491-02 & V380-Cyg-sec & 1:1 & 212.2 & -14 & -51 & 5.77 & 7.81 & 9.8501E+02 & Direct-PRF & 0\\
005385509-01 & V380-Cyg-pri & 1:1 & 278.5 & -37 & -59 & 5.77 & 9.94 & 4.7209E+02 & Direct-PRF & 0\\
005385509-02 & V380-Cyg-sec & 1:1 & 278.5 & -37 & -59 & 5.77 & 9.94 & 4.2169E+02 & Direct-PRF & 0\\
005385548-01 & V380-Cyg-pri & 1:1 & 126.7 & 2 & -31 & 5.77 & 7.47 & 8.3295E+02 & Direct-PRF & 0\\
005385548-02 & V380-Cyg-sec & 1:1 & 126.7 & 2 & -31 & 5.77 & 7.47 & 1.0160E+03 & Direct-PRF & 0\\
005385566-01 & V380-Cyg-pri & 1:1 & 350.5 & -62 & -62 & 5.77 & 9.77 & 3.4344E+02 & Direct-PRF & 0\\
005385566-02 & V380-Cyg-sec & 1:2 & 350.5 & -62 & -62 & 5.77 & 9.77 & 5.0014E+02 & Direct-PRF & 0\\
005385575-01 & V380-Cyg-pri & 1:1 & 151.6 & -14 & -35 & 5.77 & 8.88 & 2.8643E+02 & Direct-PRF & 0\\
005385575-02 & V380-Cyg-sec & 1:1 & 151.6 & -14 & -35 & 5.77 & 8.88 & 1.9317E+02 & Direct-PRF & 0\\
005385647-01 & V380-Cyg-pri & 1:1 & 269.9 & -52 & -44 & 5.77 & 8.22 & 1.9586E+03 & Direct-PRF & 0\\
005385667-01 & V380-Cyg-pri & 1:1 & 247.5 & -49 & -38 & 5.77 & 7.45 & 2.1005E+03 & Direct-PRF & 0\\
005385667-02 & V380-Cyg-sec & 1:1 & 247.5 & -49 & -38 & 5.77 & 7.45 & 1.6130E+03 & Direct-PRF & 0\\
005385697-01 & V380-Cyg-pri & 1:1 & 229.0 & -48 & -32 & 5.77 & 9.83 & 3.2496E+02 & Direct-PRF & 0\\
005385697-02 & V380-Cyg-sec & 1:1 & 229.0 & -48 & -32 & 5.77 & 9.83 & 3.4781E+02 & Direct-PRF & 0\\
005385750-01 & V380-Cyg-pri & 1:1 & 88.6 & -21 & -7 & 5.77 & 8.71 & 1.1376E+02 & Direct-PRF & 1\\
005385750-02 & V380-Cyg-sec & 1:1 & 88.6 & -21 & -7 & 5.77 & 8.71 & 2.3984E+02 & Direct-PRF & 0\\
005385750-03 & V380-Cyg-sec & 3:1 & 88.6 & -21 & -7 & 5.77 & 8.71 & 5.1144E+01 & Direct-PRF & 0\\
005385773-01 & V380-Cyg-pri & 1:1 & 309.9 & -72 & -29 & 5.77 & 8.90 & 1.1235E+03 & Direct-PRF & 0\\
005385773-02 & V380-Cyg-sec & 1:1 & 309.9 & -72 & -29 & 5.77 & 8.90 & 9.9258E+02 & Direct-PRF & 0\\
005385778-01 & V380-Cyg-pri & 1:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 1.5754E+02 & Direct-PRF & 0\\
005385778-02 & V380-Cyg-pri & 1:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 1.2725E+02 & Direct-PRF & 0\\
005385778-03 & V380-Cyg-sec & 1:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 1.6780E+02 & Direct-PRF & 0\\
005385778-04 & V380-Cyg-sec & 3:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 1.0225E+02 & Direct-PRF & 0\\
005385778-05 & V380-Cyg-sec & 4:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 6.1475E+01 & Direct-PRF & 0\\
005385778-06 & V380-Cyg-sec & 2:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 6.7241E+01 & Direct-PRF & 0\\
005385792-01 & V380-Cyg-pri & 1:1 & 64.9 & -16 & 4 & 5.77 & 7.83 & 4.7364E+02 & Direct-PRF & 0\\
005385838-01 & V380-Cyg-pri & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 3.0257E+02 & Direct-PRF & 0\\
005385838-02 & V380-Cyg-sec & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 6.2336E+02 & Direct-PRF & 0\\
005385838-03 & V380-Cyg-sec & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 9.2169E+02 & Direct-PRF & 0\\
005385838-04 & V380-Cyg-pri & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 3.5178E+02 & Direct-PRF & 0\\
005385838-05 & V380-Cyg-sec & 1:3 & 81.2 & -15 & 15 & 5.77 & 7.20 & 6.7206E+02 & Direct-PRF & 0\\
005385838-06 & V380-Cyg-sec & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 3.8518E+02 & Direct-PRF & 0\\
005385838-07 & V380-Cyg-pri & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 1.4493E+03 & Direct-PRF & 0\\
005385838-08 & V380-Cyg-sec & 1:2 & 81.2 & -15 & 15 & 5.77 & 7.20 & 1.1028E+03 & Direct-PRF & 1\\
005386163-01 & V380-Cyg-pri & 1:1 & 317.3 & -70 & 40 & 5.77 & 7.49 & 3.0194E+03 & Direct-PRF & 0\\
005386163-02 & V380-Cyg-sec & 1:1 & 317.3 & -70 & 40 & 5.77 & 7.49 & 3.1472E+03 & Direct-PRF & 0\\
005386264-01 & V380-Cyg-sec & 1:1 & 323.2 & -47 & 67 & 5.77 & 9.07 & 1.0323E+03 & Direct-PRF & 0\\
005386264-02 & V380-Cyg-pri & 1:1 & 323.2 & -47 & 67 & 5.77 & 9.07 & 1.0135E+03 & Direct-PRF & 0\\
005386271-01 & V380-Cyg-pri & 1:1 & 403.4 & -91 & 45 & 5.77 & 9.75 & 1.1978E+03 & Direct-PRF & 0\\
005392871-01 & 3342.01 & 1:1 & 13.3 & 2 & 3 & 15.75 & -2.36 & 2.3497E+02 & Direct-PRF & 0\\
005392871-02 & 005392897-02 & 1:1 & 13.3 & 2 & 3 & 15.75 & -2.36 & 1.9953E+02 & Direct-PRF & 0\\
005428471-01 & 005513861-pri & 1:2 & 87.2 & -15 & -16 & 11.64 & 4.07 & 1.1824E+03 & Direct-PRF & 0\\
005443837-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005443980-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005444334-01 & 005444392-pri & 1:2 & 44.8 & 4 & 11 & 11.38 & 4.54 & 1.4262E+04 & Direct-PRF & 0\\
005444384-01 & 005444392-01 & 1:1 & 15.6 & -2 & 4 & 11.38 & 4.17 & 8.7963E+01 & Direct-PRF & 0\\
005444491-01 & 005444392-01 & 1:1 & 100.3 & -19 & -16 & 11.38 & 3.54 & 2.8038E+03 & Direct-PRF & 0\\
005458779-01 & 005458880-pri & 1:1 & 112.1 & 5 & 27 & 7.82 & 7.97 & 1.4235E+02 & Direct-PRF & 0\\
005458795-01 & 005458880-pri & 1:1 & 87.2 & 1 & 22 & 7.82 & 7.32 & 3.6667E+02 & Direct-PRF & 0\\
005458845-01 & 005458880-pri & 1:1 & 89.4 & 14 & 17 & 7.82 & 5.84 & 4.4815E+02 & Direct-PRF & 0\\
005458845-02 & 005458880-sec & 1:1 & 89.4 & 14 & 17 & 7.82 & 5.84 & 4.0000E+02 & Direct-PRF & 0\\
005458953-01 & 005458880-pri & 1:1 & 87.3 & 21 & -7 & 7.82 & 6.62 & 3.4571E+02 & Direct-PRF & 0\\
005467102-01 & 3825.01 & 1:1 & 7.5 & -1 & -1 & 15.83 & -0.47 & 2.6521E+01 & Direct-PRF & 0\\
005467102-02 & 005467113-sec & 1:1 & 7.5 & -1 & -1 & 15.83 & -0.47 & 5.5891E+01 & Direct-PRF & 0\\
005467124-01 & 3825.01 & 1:1 & 14.6 & -2 & 3 & 15.83 & -2.24 & 7.0762E+03 & Direct-PRF & 0\\
005467126-01 & 3825.01 & 1:1 & 8.4 & 2 & 1 & 15.83 & -3.47 & 2.2074E+02 & Direct-PRF & 0\\
005470851-01 & V380-Cyg-pri & 1:1 & 400.9 & 62 & -79 & 5.77 & 10.02 & 9.1153E+02 & Direct-PRF & 0\\
005470960-01 & V380-Cyg-pri & 1:1 & 383.4 & 82 & -50 & 5.77 & 10.18 & 6.8689E+02 & Direct-PRF & 0\\
005470960-02 & V380-Cyg-sec & 1:1 & 383.4 & 82 & -50 & 5.77 & 10.18 & 6.9374E+02 & Direct-PRF & 0\\
005471010-01 & V380-Cyg-pri & 1:1 & 301.9 & 48 & -58 & 5.77 & 9.87 & 6.8365E+02 & Direct-PRF & 0\\
005471010-02 & V380-Cyg-sec & 1:1 & 301.9 & 48 & -58 & 5.77 & 9.87 & 5.4217E+02 & Direct-PRF & 0\\
005471059-03 & V380-Cyg-pri & 1:1 & 293.2 & 59 & -43 & 5.77 & 8.95 & 9.9269E+02 & Direct-PRF & 0\\
005471059-04 & V380-Cyg-sec & 1:1 & 293.2 & 59 & -43 & 5.77 & 8.95 & 9.7020E+02 & Direct-PRF & 0\\
005471068-01 & V380-Cyg-pri & 1:1 & 298.8 & 63 & -41 & 5.77 & 9.41 & 8.3295E+02 & Direct-PRF & 0\\
005471068-02 & V380-Cyg-sec & 1:1 & 298.8 & 63 & -41 & 5.77 & 9.41 & 9.4187E+02 & Direct-PRF & 0\\
005471108-01 & V380-Cyg-pri & 1:1 & 246.3 & 44 & -43 & 5.77 & 5.83 & 3.2207E+03 & Direct-PRF & 0\\
005471108-02 & V380-Cyg-sec & 36:1 & 246.3 & 44 & -43 & 5.77 & 5.83 & 9.8501E+02 & Direct-PRF & 0\\
005471141-01 & V380-Cyg-pri & 1:1 & 223.0 & 37 & -42 & 5.77 & 8.08 & 1.2179E+03 & Direct-PRF & 0\\
005471141-02 & V380-Cyg-sec & 1:1 & 223.0 & 37 & -42 & 5.77 & 8.08 & 1.9259E+03 & Direct-PRF & 0\\
005471158-01 & V380-Cyg-pri & 1:1 & 207.3 & 27 & -44 & 5.77 & 9.95 & 3.0641E+02 & Direct-PRF & 0\\
005471158-02 & V380-Cyg-sec & 1:1 & 207.3 & 27 & -44 & 5.77 & 9.95 & 3.6044E+02 & Direct-PRF & 0\\
005471192-01 & V380-Cyg-pri & 1:1 & 218.9 & 48 & -27 & 5.77 & 8.51 & 1.0657E+03 & Direct-PRF & 0\\
005471192-02 & V380-Cyg-sec & 1:1 & 218.9 & 48 & -27 & 5.77 & 8.51 & 1.0241E+03 & Direct-PRF & 0\\
005471202-01 & V380-Cyg-pri & 1:1 & 179.6 & 23 & -38 & 5.77 & 9.09 & 4.4732E+02 & Direct-PRF & 0\\
005471202-02 & V380-Cyg-sec & 1:1 & 179.6 & 23 & -38 & 5.77 & 9.09 & 4.1491E+02 & Direct-PRF & 0\\
005471217-01 & V380-Cyg-pri & 1:1 & 274.3 & 68 & -10 & 5.77 & 8.65 & 1.0065E+03 & Direct-PRF & 0\\
005471217-02 & V380-Cyg-sec & 1:1 & 274.3 & 68 & -10 & 5.77 & 8.65 & 9.0870E+02 & Direct-PRF & 0\\
005471271-01 & V380-Cyg-pri & 1:1 & 243.8 & 61 & -5 & 5.77 & 7.83 & 1.2826E+03 & Direct-PRF & 0\\
005471271-02 & V380-Cyg-sec & 1:1 & 243.8 & 61 & -5 & 5.77 & 7.83 & 1.0160E+03 & Direct-PRF & 0\\
005471289-01 & V380-Cyg-pri & 1:1 & 220.1 & 55 & -5 & 5.77 & 9.16 & 4.7991E+02 & Direct-PRF & 0\\
005471289-02 & V380-Cyg-sec & 1:1 & 220.1 & 55 & -5 & 5.77 & 9.16 & 5.4676E+02 & Direct-PRF & 0\\
005471328-01 & V380-Cyg-pri & 1:1 & 93.6 & 14 & -18 & 5.77 & 10.13 & 1.6321E+02 & Direct-PRF & 0\\
005471328-02 & V380-Cyg-sec & 1:1 & 93.6 & 14 & -18 & 5.77 & 10.13 & 4.0450E+02 & Direct-PRF & 0\\
005471328-03 & V380-Cyg-sec & 1:6 & 93.6 & 14 & -18 & 5.77 & 10.13 & 5.4446E+02 & Direct-PRF & 0\\
005471328-04 & V380-Cyg-sec & 1:1 & 93.6 & 14 & -18 & 5.77 & 10.13 & 4.8656E+01 & Direct-PRF & 0\\
005471328-05 & V380-Cyg-sec & 1:1 & 93.6 & 14 & -18 & 5.77 & 10.13 & 2.4862E+02 & Direct-PRF & 0\\
005471328-06 & V380-Cyg-pri & 1:7 & 93.6 & 14 & -18 & 5.77 & 10.13 & 1.2691E+02 & Direct-PRF & 0\\
005471415-01 & V380-Cyg-pri & 1:1 & 88.4 & 22 & 3 & 5.77 & 6.85 & 2.3339E+02 & Direct-PRF & 0\\
005471415-02 & V380-Cyg-sec & 1:1 & 88.4 & 22 & 3 & 5.77 & 6.85 & 2.1797E+02 & Direct-PRF & 0\\
005471480-01 & V380-Cyg-pri & 1:1 & 317.3 & 68 & 42 & 5.77 & 9.94 & 4.0712E+02 & Direct-PRF & 0\\
005471480-02 & V380-Cyg-sec & 1:1 & 317.3 & 68 & 42 & 5.77 & 9.94 & 4.3301E+02 & Direct-PRF & 0\\
005471489-01 & V380-Cyg-pri & 1:1 & 297.2 & 62 & 41 & 5.77 & 7.27 & 1.7675E+03 & Direct-PRF & 0\\
005471489-02 & V380-Cyg-sec & 1:1 & 297.2 & 62 & 41 & 5.77 & 7.27 & 2.0162E+03 & Direct-PRF & 0\\
005471496-01 & V380-Cyg-pri & 1:1 & 198.2 & 39 & 30 & 5.77 & 10.12 & 1.1948E+02 & Direct-PRF & 0\\
005471496-02 & V380-Cyg-sec & 1:1 & 198.2 & 39 & 30 & 5.77 & 10.12 & 1.1289E+02 & Direct-PRF & 0\\
005471566-01 & 005471619-pri & 1:1 & 109.3 & 28 & 2 & 12.37 & 3.10 & 4.9222E+03 & Direct-PRF & 0\\
005471574-01 & 005471619-pri & 1:1 & 40.6 & 6 & -9 & 12.37 & 1.03 & 6.7121E+03 & Direct-PRF & 0\\
005471574-02 & V380-Cyg-pri & 1:1 & 182.4 & 24 & 39 & 5.77 & 7.63 & 4.6753E+02 & Direct-PRF & 0\\
005471574-03 & V380-Cyg-sec & 1:1 & 182.4 & 24 & 39 & 5.77 & 7.63 & 4.2307E+02 & Direct-PRF & 0\\
005471606-01 & 005471619-pri & 1:1 & 11.2 & 1 & -3 & 12.37 & -1.55 & 1.5329E+03 & Direct-PRF & 0\\
005471675-01 & 005471619-pri & 1:1 & 53.5 & 1 & 13 & 12.37 & 0.94 & 5.2738E+03 & Direct-PRF & 0\\
005471675-02 & V380-Cyg-pri & 1:1 & 253.7 & 19 & 61 & 5.77 & 7.53 & 1.1235E+03 & Direct-PRF & 0\\
005471688-01 & V380-Cyg-pri & 1:1 & 248.6 & 13 & 61 & 5.77 & 9.29 & 5.1578E+02 & Direct-PRF & 0\\
005471688-02 & V380-Cyg-sec & 1:1 & 248.6 & 13 & 61 & 5.77 & 9.29 & 3.8984E+02 & Direct-PRF & 0\\
005471688-03 & 005471619-pri & 1:1 & 58.9 & -5 & 13 & 12.37 & 2.69 & 5.4024E+03 & Direct-PRF & 0\\
005471690-01 & V380-Cyg-pri & 1:1 & 241.2 & 10 & 60 & 5.77 & 7.10 & 1.8346E+03 & Direct-PRF & 0\\
005471690-02 & V380-Cyg-sec & 1:1 & 241.2 & 10 & 60 & 5.77 & 7.10 & 1.4337E+03 & Direct-PRF & 0\\
005471690-03 & 005471619-pri & 1:1 & 59.6 & -8 & 12 & 12.37 & 0.51 & 2.6059E+04 & Direct-PRF & 0\\
005471769-01 & V380-Cyg-pri & 1:1 & 363.9 & 30 & 87 & 5.77 & 9.19 & 1.0816E+03 & Direct-PRF & 0\\
005471769-02 & V380-Cyg-sec & 1:1 & 363.9 & 30 & 87 & 5.77 & 9.19 & 1.0323E+03 & Direct-PRF & 0\\
005471770-01 & V380-Cyg-pri & 1:1 & 311.0 & 13 & 77 & 5.77 & 7.83 & 1.4493E+03 & Direct-PRF & 0\\
005471770-02 & V380-Cyg-sec & 1:1 & 311.0 & 13 & 77 & 5.77 & 7.83 & 1.7205E+03 & Direct-PRF & 0\\
005471792-01 & V380-Cyg-pri & 1:1 & 312.8 & 7 & 79 & 5.77 & 7.60 & 1.7051E+03 & Direct-PRF & 0\\
005471792-02 & V380-Cyg-sec & 1:1 & 312.8 & 7 & 79 & 5.77 & 7.60 & 2.3461E+03 & Direct-PRF & 0\\
005473087-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005475735-01 & 005475712-pri & 1:1 & 20.5 & 2 & -4 & 13.28 & 1.12 & 1.5356E+03 & Direct-PRF & 0\\
005475736-01 & 005475712-pri & 1:1 & 12.6 & -2 & -2 & 13.28 & 0.73 & 1.1152E+02 & Direct-PRF & 0\\
005475736-02 & 005475712-sec & 1:1 & 12.6 & -2 & -2 & 13.28 & 0.73 & 5.1212E+02 & Direct-PRF & 0\\
005475736-03 & 005475712-sec & 1:1 & 12.6 & -2 & -2 & 13.28 & 0.73 & 5.2812E+02 & Direct-PRF & 0\\
005478055-01 & 005478083-01 & 1:1 & 12.6 & 2 & 1 & 17.52 & -3.01 & 5.6727E+02 & Direct-PRF & 0\\
005479800-01 & 005479871-01 & 1:1 & 94.5 & -15 & 18 & 15.25 & -2.78 & 3.7778E-01 & Direct-PRF & 1\\
005479821-03 & 005479800-01 & 4:1 & 12.5 & -1 & -3 & 12.47 & -2.58 & 6.0000E+01 & Direct-PRF & 1\\
005479871-01 & 005479800-01 & 1:1 & 94.5 & 15 & -18 & 12.47 & 2.78 & 2.6471E+00 & Direct-PRF & 1\\
005479950-01 & 005479800-01 & 2:1 & 77.8 & -7 & -18 & 12.47 & 3.30 & 1.8182E+00 & Direct-PRF & 1\\
005480714-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005481416-01 & 3772.01 & 1:1 & 6.0 & 1 & 1 & 19.32 & -3.48 & 2.8690E+02 & Direct-PRF & 0\\
005513822-01 & 005513861-pri & 1:2 & 79.8 & -16 & 13 & 11.64 & 1.65 & 1.1104E+04 & Direct-PRF & 0\\
005513833-01 & 005513861-pri & 1:2 & 98.8 & 0 & 25 & 11.64 & 3.60 & 4.3288E+03 & Direct-PRF & 0\\
005513857-01 & 005513861-pri & 1:2 & 49.9 & 5 & 11 & 11.64 & 3.80 & 1.8113E+03 & Direct-PRF & 0\\
005513866-01 & 005513861-pri & 1:2 & 31.5 & 6 & 5 & 11.64 & 1.94 & 4.2567E+03 & Direct-PRF & 0\\
005513893-01 & 005513861-pri & 1:2 & 47.9 & 11 & -4 & 11.64 & 1.37 & 5.5522E+03 & Direct-PRF & 0\\
005513897-01 & 005513861-pri & 1:2 & 54.0 & 10 & -9 & 11.64 & 2.34 & 3.5472E+03 & Direct-PRF & 0\\
005521686-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005525655-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005529501-01 & 005444392-pri & 1:1 & 247.0 & 62 & 1 & 11.38 & 1.21 & 2.9543E+04 & Direct-PRF & 0\\
005529552-01 & 005444392-01 & 1:1 & 128.7 & 32 & 3 & 11.38 & 3.94 & 1.0942E+03 & Direct-PRF & 0\\
005529560-01 & 005444392-pri & 1:2 & 117.1 & 29 & 3 & 11.38 & 3.88 & 7.0102E+03 & Direct-PRF & 0\\
005529643-01 & 005444392-pri & 1:2 & 45.7 & 11 & -2 & 11.38 & 4.55 & 1.1178E+04 & Direct-PRF & 0\\
005529738-01 & 005444392-pri & 1:2 & 60.5 & 0 & -15 & 11.38 & 3.49 & 4.8659E+03 & Direct-PRF & 0\\
005530689-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005530882-01 & 005530881-01 & 1:1 & 22.8 & -5 & 3 & 13.51 & 0.94 & 3.1409E+03 & Direct-PRF & 0\\
005534476-02 & 005534702-pri & 1:1 & 360.2 & 90 & 0 & 13.82 & -1.41 & 6.3269E+03 & Col-Anomaly & 0\\
005542224-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005556726-01 & 005471619-pri & 1:1 & 489.4 & 123 & 1 & 12.37 & -0.20 & 6.1528E+03 & Col-Anomaly & 0\\
005556769-01 & V380-Cyg-pri & 1:1 & 421.9 & 101 & 32 & 5.77 & 8.70 & 2.8418E+03 & Direct-PRF & 0\\
005556804-01 & V380-Cyg-pri & 1:1 & 398.7 & 94 & 33 & 5.77 & 10.13 & 8.0968E+02 & Direct-PRF & 0\\
005556804-02 & V380-Cyg-sec & 1:1 & 398.7 & 94 & 33 & 5.77 & 10.13 & 7.0899E+02 & Direct-PRF & 0\\
005556830-01 & V380-Cyg-pri & 1:1 & 416.0 & 97 & 38 & 5.77 & 9.90 & 1.0207E+03 & Direct-PRF & 0\\
005558458-01 & 006543496-02 & 1:1 & 4685.4 & 640 & -3 & 13.64 & -2.24 & 4.3750E+00 & Col-Anomaly & 2\\
005565497-01 & 3742.01 & 1:1 & 11.3 & -1 & -3 & 14.96 & -3.44 & 4.9253E+02 & Direct-PRF & 0\\
005598595-01 & 005598639-sec & 1:2 & 67.8 & -13 & 11 & 10.20 & 5.20 & 4.3920E+02 & Direct-PRF & 0\\
005598645-01 & 005598639-sec & 1:2 & 84.0 & -11 & -18 & 10.20 & 1.49 & 5.4900E+03 & Direct-PRF & 0\\
005621299-01 & 005621294-pri & 1:1 & 27.8 & -7 & -3 & 13.61 & 0.30 & 6.6855E+03 & Direct-PRF & 0\\
005622812-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005623833-01 & RR-Lyr-pri & 1:1 & 8215.1 & -1 & -4 & 7.86 & 4.81 & 3.2805E+04 & Cross-Talk & 0\\
005632701-01 & 005632781-pri & 1:3 & 48.7 & -5 & 11 & 12.11 & 1.88 & 7.4528E+03 & Direct-PRF & 0\\
005636648-01 & 3817.01 & 1:1 & 6.3 & 1 & 2 & 16.43 & -1.10 & 6.0494E+01 & Direct-PRF & 0\\
005649215-01 & 3636.01 & 1:1 & 7.7 & -1 & -1 & 17.99 & -2.97 & 2.0065E+02 & Direct-PRF & 0\\
005649833-01 & 3831.01 & 1:1 & 12.0 & 3 & -1 & 16.38 & -3.01 & 5.1472E+03 & Direct-PRF & 0\\
005649837-01 & 3831.01 & 1:1 & 12.0 & -2 & 1 & 16.38 & -1.13 & 1.4843E+02 & Direct-PRF & 0\\
005652237-01 & 3703.01 & 1:1 & 9.4 & 0 & 2 & 17.30 & -3.79 & 3.8497E+02 & Direct-PRF & 0\\
005653163-01 & 6134.01 & 1:1 & 96.9 & -18 & 16 & 11.94 & -1.31 & 1.2044E+03 & Direct-PRF & 1\\
005686974-01 & 5206.01 & 1:1 & 771.4 & 194 & 1 & 14.74 & -1.01 & 3.0407E+03 & Col-Anomaly & 0\\
005687986-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005696918-01 & 005696909-pri & 1:1 & 8.6 & 2 & 0 & 14.98 & -0.18 & 5.0000E+01 & Direct-PRF & 0\\
005696918-02 & 005696909-sec & 1:1 & 8.6 & 2 & 0 & 14.98 & -0.18 & 3.1250E+01 & Direct-PRF & 0\\
005703256-01 & 005703230-pri & 1:1 & 27.9 & 0 & -7 & 11.79 & 1.45 & 2.3143E+03 & Direct-PRF & 0\\
005707308-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005724810-01 & 005724811-01 & 1:1 & 5.2 & 1 & -1 & 12.28 & -1.38 & 3.7407E+00 & Direct-PRF & 0\\
005725851-01 & 005725846-01 & 1:1 & 5.4 & 1 & 0 & 15.36 & -1.95 & 3.3056E+00 & Direct-PRF & 0\\
005730389-01 & 3603.01 & 1:2 & 12.8 & 3 & -1 & 16.12 & -1.50 & 1.0555E+03 & Direct-PRF & 0\\
005738496-01 & 005738506-01 & 1:1 & 11.2 & -1 & 2 & 18.35 & -3.55 & 1.0072E+03 & Direct-PRF & 0\\
005738496-02 & 3676.01 & 1:1 & 11.2 & -1 & 2 & 18.35 & -3.55 & 1.2248E+03 & Direct-PRF & 0\\
005738634-01 & 6134.01 & 1:1 & 72.0 & 18 & -1 & 11.94 & 1.31 & 4.1606E+03 & Direct-PRF & 0\\
005792102-01 & 005792093-pri & 1:1 & 12.4 & 2 & 3 & 13.91 & -0.13 & 4.0500E+04 & Direct-PRF & 0\\
005794339-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005796186-01 & 3369.01 & 1:1 & 8.5 & 2 & 1 & 15.83 & -1.92 & 6.4366E+01 & Direct-PRF & 0\\
005802478-01 & 005802470-01 & 1:1 & 17.5 & 4 & 1 & 13.76 & 0.63 & 5.2520E+02 & Direct-PRF & 0\\
005802478-02 & 005802470-01 & 1:2 & 17.5 & 4 & 1 & 13.76 & 0.63 & 1.6395E+03 & Direct-PRF & 0\\
005810197-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005816811-01 & 3645.01 & 1:2 & 7.0 & -2 & 0 & 17.05 & -2.20 & 2.6596E+02 & Direct-PRF & 0\\
005817533-01 & 005817566-sec & 1:2 & 51.4 & -9 & 9 & 11.68 & 3.63 & 9.1609E+02 & Direct-PRF & 0\\
005817553-01 & 005817566-sec & 1:2 & 15.3 & -3 & 3 & 11.68 & 2.40 & 2.5627E+02 & Direct-PRF & 0\\
005817613-01 & 005817566-sec & 1:2 & 44.5 & -11 & -1 & 11.68 & 4.21 & 6.5328E+02 & Direct-PRF & 0\\
005817712-01 & 005817566-sec & 1:2 & 74.3 & -8 & -17 & 11.68 & 3.77 & 1.3861E+03 & Direct-PRF & 0\\
005866099-01 & 005866104-01 & 1:1 & 5.5 & 0 & -1 & 17.07 & -3.37 & 2.0794E+02 & Direct-PRF & 0\\
005866099-02 & 005866104-02 & 1:1 & 5.5 & 0 & -1 & 17.07 & -3.37 & 1.8654E+02 & Direct-PRF & 0\\
005876368-01 & 4279.01 & 1:1 & 5.0 & -1 & 1 & 17.17 & -2.38 & 2.0002E+02 & Direct-PRF & 0\\
005903312-01 & 3692.01 & 1:1 & 8.0 & -2 & -1 & 15.15 & -2.70 & 9.5227E+01 & Direct-PRF & 0\\
005903453-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
005952309-01 & 6139.01 & 1:1 & 66.3 & -10 & 13 & 6.97 & 7.95 & 5.2556E+01 & Direct-PRF & 0\\
005952366-01 & 6139.01 & 1:1 & 34.5 & 0 & 9 & 6.97 & 6.41 & 2.8494E+00 & Direct-PRF & 0\\
005952403-01 & 3947.01 & 1:1 & 34.5 & 0 & -9 & 13.38 & -6.41 & 1.4920E+00 & Direct-PRF & 1\\
005952457-01 & 6139.01 & 1:1 & 60.3 & -6 & -14 & 6.97 & 8.32 & 4.9418E+01 & Direct-PRF & 0\\
005962509-01 & 005962514-pri & 1:2 & 18.6 & -3 & -4 & 14.84 & 0.69 & 5.1405E+03 & Direct-PRF & 0\\
005978295-01 & 006389755-01 & 1:3 & 5491.1 & -230 & -2 & 14.78 & -2.71 & 1.1200E+00 & Col-Anomaly & 2\\
005982368-01 & 005982353-pri & 1:1 & 11.0 & 3 & 1 & 11.12 & 2.92 & 2.2588E+00 & Direct-PRF & 0\\
006020898-01 & 006020929-01 & 1:1 & 87.6 & -21 & 8 & 13.61 & 0.05 & 9.2077E-02 & Direct-PRF & 1\\
006020929-01 & 006020898-01 & 1:1 & 87.6 & 21 & -8 & 13.66 & -0.05 & 1.0860E+01 & Direct-PRF & 1\\
006044188-01 & RR-Lyr-pri & 1:1 & 6300.0 & 565 & -132 & 7.86 & 1.80 & 8.2556E+02 & Col-Anomaly & 2\\
006044553-01 & 006044543-pri & 1:1 & 16.9 & -4 & -1 & 13.76 & 1.63 & 2.2734E+03 & Direct-PRF & 0\\
006044999-01 & RR-Lyr-pri & 1:1 & 6285.3 & 485 & 2 & 7.86 & 7.18 & 3.8956E+04 & Col-Anomaly & 2\\
006045250-01 & 006045264-pri & 1:1 & 9.0 & 2 & 0 & 13.44 & 1.53 & 2.7847E+03 & Direct-PRF & 0\\
006058896-01 & 3616.01 & 1:1 & 10.2 & 0 & 2 & 15.84 & -1.05 & 5.0851E+02 & Direct-PRF & 0\\
006065678-01 & 006065699-04 & 2:1 & 24.6 & 1 & 6 & 7.83 & 5.96 & 2.6316E-02 & Direct-PRF & 1\\
006065699-04 & 006065678-01 & 1:2 & 24.6 & -1 & -6 & 13.79 & -5.96 & 3.8000E+01 & Direct-PRF & 1\\
006066403-01 & 3649.01 & 1:1 & 12.2 & 3 & -1 & 15.47 & -1.92 & 2.2639E+03 & Direct-PRF & 0\\
006066416-01 & 3649.01 & 1:1 & 14.8 & 2 & -3 & 15.47 & -3.92 & 2.6190E+03 & Direct-PRF & 0\\
006113806-01 & V2083-Cyg-pri & 1:2 & 24193.4 & -3 & -52 & 6.90 & 7.61 & 8.2634E+03 & Reflection & 0\\
006124426-01 & 005878081-pri & 1:1 & 1472.4 & 370 & 0 & 14.37 & -0.49 & 5.5220E+03 & Col-Anomaly & 0\\
006125282-01 & 006044543-pri & 1:1 & 624.2 & 157 & 1 & 13.76 & 0.09 & 1.6255E+05 & Col-Anomaly & 0\\
006126076-01 & 006045264-pri & 1:1 & 432.0 & 109 & 1 & 13.44 & -0.71 & 3.6480E+04 & Col-Anomaly & 0\\
006126076-02 & 006045264-sec & 1:1 & 432.0 & 109 & 1 & 13.44 & -0.71 & 1.9811E+04 & Col-Anomaly & 0\\
006137681-01 & 3605.01 & 2:1 & 9.6 & -1 & -3 & 14.16 & 1.32 & 1.4848E+01 & Direct-PRF & 0\\
006145471-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006182846-01 & 3512.01 & 1:1 & 8.2 & -2 & 1 & 13.72 & 1.08 & 4.2487E+00 & Direct-PRF & 0\\
006182846-02 & 006182849-02 & 1:1 & 8.2 & -2 & 1 & 13.72 & 1.08 & 4.3646E+00 & Direct-PRF & 0\\
006185711-01 & 006185717-01 & 1:1 & 11.8 & 3 & -2 & 13.39 & 0.19 & 5.8152E+01 & Direct-PRF & 0\\
006199702-01 & 1812.01 & 1:1 & 6.1 & 2 & 1 & 13.74 & 0.89 & 6.0000E+00 & Direct-PRF & 0\\
006200715-01 & 3694.01 & 1:1 & 6.9 & 2 & -1 & 16.72 & -1.79 & 1.0069E+02 & Direct-PRF & 0\\
006205384-01 & 006205460-pri & 1:1 & 87.6 & 22 & -2 & 12.75 & 1.20 & 1.9481E+04 & Direct-PRF & 0\\
006205405-01 & 006205460-pri & 1:1 & 50.2 & -2 & -12 & 12.75 & 1.79 & 1.1132E+04 & Direct-PRF & 0\\
006205468-01 & 006205460-pri & 1:1 & 17.6 & -4 & 0 & 12.75 & 2.77 & 1.6109E+03 & Direct-PRF & 0\\
006205481-01 & 006205460-pri & 1:1 & 18.1 & -4 & 2 & 12.75 & 2.93 & 2.0642E+03 & Direct-PRF & 0\\
006205483-01 & 006205460-pri & 1:1 & 45.8 & 7 & 10 & 12.75 & 2.80 & 8.7803E+03 & Direct-PRF & 0\\
006205507-01 & 006205460-pri & 1:1 & 107.0 & 14 & 23 & 12.75 & -0.05 & 8.9057E+04 & Direct-PRF & 0\\
006206470-01 & 005962716-pri & 1:1 & 1510.3 & 380 & 0 & 13.88 & -0.15 & 4.3000E+03 & Col-Anomaly & 0\\
006206559-01 & 006206751-pri & 1:1 & 308.0 & 78 & -1 & 12.14 & 0.20 & 8.1567E+03 & Col-Anomaly & 0\\
006223877-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006233483-01 & 006233466-01 & 1:1 & 7.7 & 1 & -1 & 14.68 & -0.77 & 2.2325E+01 & Direct-PRF & 0\\
006233483-02 & 006233466-02 & 1:1 & 7.7 & 1 & -1 & 14.68 & -0.77 & 2.0868E+01 & Direct-PRF & 0\\
006233890-01 & 006233903-01 & 1:1 & 10.9 & 1 & 2 & 16.45 & -3.28 & 1.2103E+03 & Direct-PRF & 0\\
006263593-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006267414-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006277167-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006285094-01 & TT-Lyr-pri & 1:1 & 219.0 & -27 & -49 & 9.49 & 5.47 & 1.2379E+04 & Direct-PRF & 0\\
006285396-01 & TT-Lyr-pri & 1:1 & 283.6 & -42 & -26 & 9.49 & 6.30 & 7.7647E+03 & Direct-PRF & 0\\
006285397-01 & TT-Lyr-pri & 1:1 & 261.5 & -37 & -23 & 9.49 & 6.42 & 7.0010E+03 & Direct-PRF & 0\\
006285545-01 & TT-Lyr-pri & 1:1 & 326.3 & -57 & 4 & 9.49 & 5.31 & 2.0336E+04 & Direct-PRF & 0\\
006286155-01 & 006286161-01 & 1:1 & 7.5 & -1 & -2 & 16.71 & -2.95 & 2.3884E+02 & Direct-PRF & 0\\
006286155-02 & 3501.01 & 1:1 & 7.5 & -1 & -2 & 16.71 & -2.95 & 1.8104E+02 & Direct-PRF & 0\\
006289897-01 & 006048106-pri & 1:1 & 964.3 & 243 & -1 & 14.09 & -0.73 & 7.4949E+03 & Col-Anomaly & 0\\
006301035-01 & 006301030-02 & 1:1 & 8.8 & 3 & 1 & 17.78 & -2.80 & 1.5577E+02 & Direct-PRF & 0\\
006301035-02 & 6027.01 & 1:1 & 8.8 & 3 & 1 & 17.78 & -2.80 & 2.2072E+02 & Direct-PRF & 0\\
006307063-01 & 006307062-01 & 5:1 & 14.6 & 3 & 2 & 14.86 & -1.17 & 3.9211E+02 & Direct-PRF & 0\\
006307063-02 & 006307062-01 & 1:1 & 14.6 & 3 & 2 & 14.86 & -1.17 & 1.4418E+03 & Direct-PRF & 0\\
006307063-03 & 006307062-02 & 5:1 & 14.6 & 3 & 2 & 14.86 & -1.17 & 4.5101E+02 & Direct-PRF & 0\\
006307083-01 & 006307062-01 & 5:1 & 16.4 & 2 & -4 & 14.86 & -2.64 & 8.5169E+02 & Direct-PRF & 0\\
006307083-02 & 006307062-01 & 1:1 & 16.4 & 2 & -4 & 14.86 & -2.64 & 2.7605E+03 & Direct-PRF & 0\\
006307083-03 & 006307062-02 & 1:1 & 16.4 & 2 & -4 & 14.86 & -2.64 & 1.4553E+03 & Direct-PRF & 0\\
006307521-01 & 006307537-pri & 1:1 & 19.3 & 2 & 4 & 11.75 & 3.51 & 1.9637E+02 & Direct-PRF & 0\\
006312534-01 & 3656.01 & 1:2 & 6.2 & 1 & -1 & 17.36 & -1.77 & 4.0993E+01 & Direct-PRF & 0\\
006314185-01 & 3708.01 & 1:1 & 7.0 & 0 & -2 & 17.72 & -2.83 & 8.5391E+01 & Direct-PRF & 0\\
006314185-02 & 006314173-sec & 1:1 & 7.0 & 0 & -2 & 17.72 & -2.83 & 2.4601E+01 & Direct-PRF & 0\\
006343576-01 & 3512.01 & 1:1 & 1371.0 & 345 & 0 & 13.72 & -0.21 & 2.3404E+03 & Col-Anomaly & 0\\
006356627-01 & 005007640-01 & 2:1 & 6698.0 & -221 & 2 & 13.65 & -1.52 & 1.0444E+00 & Col-Anomaly & 2\\
006359802-01 & 1121.01 & 1:1 & 4.5 & 1 & -1 & 12.93 & 2.12 & 1.4285E+00 & Direct-PRF & 0\\
006359802-02 & 006359798-02 & 1:1 & 4.5 & 1 & -1 & 12.93 & 2.12 & 1.4863E+00 & Direct-PRF & 0\\
006363560-01 & 006363494-pri & 1:2 & 99.4 & 25 & -1 & 14.42 & -0.89 & 3.5600E+03 & Col-Anomaly & 0\\
006364064-01 & TT-Lyr-pri & 1:1 & 209.5 & -39 & -36 & 9.49 & 5.70 & 8.8054E+03 & Direct-PRF & 0\\
006364067-01 & TT-Lyr-pri & 1:1 & 202.3 & -33 & -39 & 9.49 & 6.07 & 6.3268E+03 & Direct-PRF & 0\\
006364126-01 & TT-Lyr-pri & 1:1 & 168.5 & -38 & -20 & 9.49 & 5.41 & 1.1092E+04 & Direct-PRF & 0\\
006364143-01 & TT-Lyr-pri & 1:1 & 258.7 & -65 & 3 & 9.49 & 5.09 & 1.4477E+04 & Direct-PRF & 0\\
006364162-01 & TT-Lyr-pri & 1:1 & 149.6 & -36 & -12 & 9.49 & 5.67 & 4.4954E+03 & Direct-PRF & 0\\
006364195-01 & TT-Lyr-pri & 1:1 & 253.4 & -62 & 14 & 9.49 & 6.43 & 6.6728E+03 & Direct-PRF & 0\\
006364200-01 & TT-Lyr-pri & 1:1 & 324.9 & -78 & 25 & 9.49 & 6.37 & 1.1863E+04 & Direct-PRF & 0\\
006364215-02 & TT-Lyr-pri & 1:1 & 252.8 & -61 & 19 & 9.49 & 6.16 & 6.6728E+03 & Direct-PRF & 0\\
006364247-01 & TT-Lyr-pri & 1:1 & 277.0 & -63 & 29 & 9.49 & 4.14 & 3.7136E+04 & Direct-PRF & 0\\
006364276-01 & TT-Lyr-pri & 1:1 & 154.7 & -34 & 19 & 9.49 & 5.80 & 3.8130E+03 & Direct-PRF & 0\\
006364294-01 & TT-Lyr-pri & 1:1 & 280.8 & -59 & 39 & 9.49 & 5.99 & 1.2202E+04 & Direct-PRF & 0\\
006364307-01 & TT-Lyr-pri & 1:1 & 179.7 & -35 & 29 & 9.49 & 6.34 & 4.6169E+03 & Direct-PRF & 0\\
006364327-01 & TT-Lyr-pri & 1:1 & 169.8 & -30 & 30 & 9.49 & 5.09 & 4.9658E+03 & Direct-PRF & 0\\
006367439-01 & 006367628-pri & 1:1 & 293.2 & 74 & 0 & 13.04 & 0.51 & 8.6136E+03 & Col-Anomaly & 0\\
006386784-01 & 006545018-pri & 1:2 & 692.6 & 175 & 1 & 13.75 & -1.80 & 1.6371E+04 & Col-Anomaly & 0\\
006390236-01 & 006390205-pri & 2:1 & 24.8 & 6 & -3 & 12.54 & -1.34 & 5.1818E+03 & Direct-PRF & 0\\
006390236-02 & 006390205-pri & 2:1 & 24.8 & 6 & -3 & 12.54 & -1.34 & 5.1818E+03 & Direct-PRF & 0\\
006421503-01 & 006421483-pri & 1:1 & 20.3 & 4 & 4 & 13.02 & 2.22 & 5.6636E+02 & Direct-PRF & 0\\
006422367-01 & 005343976-pri & 1:1 & 6526.0 & 0 & 1 & 12.61 & 2.18 & 1.0894E+03 & Cross-Talk & 0\\
006426592-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006438216-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006440528-01 & RR-Lyr-pri & 1:1 & 3336.1 & 546 & -636 & 7.86 & 7.55 & 1.1986E+04 & Col-Anomaly & 2\\
006442246-01 & 006521542-pri & 1:2 & 363.7 & 92 & 0 & 14.28 & -0.89 & 1.9310E+04 & Col-Anomaly & 0\\
006449291-01 & 006449358-pri & 1:1 & 100.8 & 25 & -2 & 11.61 & 2.10 & 2.2603E+03 & Direct-PRF & 0\\
006462874-01 & 94.01 & 17:1 & 7.3 & 1 & -1 & 12.21 & 3.51 & 2.9189E-01 & Direct-PRF & 0\\
006462874-02 & 94.01 & 8:1 & 7.3 & 1 & -1 & 12.21 & 3.51 & 3.2122E-01 & Direct-PRF & 0\\
006465159-01 & 006629588-pri & 1:1 & 634.1 & 160 & 0 & 13.98 & -0.61 & 9.5189E+02 & Col-Anomaly & 0\\
006470521-01 & 3705.01 & 1:1 & 6.6 & -1 & -1 & 16.45 & -2.59 & 5.8340E+01 & Direct-PRF & 0\\
006471229-01 & 5335.01 & 1:1 & 2138.2 & 538 & 1 & 11.39 & 2.59 & 3.0525E+03 & Col-Anomaly & 0\\
006471230-01 & 5335.01 & 1:1 & 2142.0 & 539 & 2 & 11.39 & 1.91 & 8.5897E+03 & Col-Anomaly & 0\\
006500714-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006507427-01 & 3815.01 & 1:1 & 4.3 & -1 & 0 & 15.43 & -1.02 & 1.3595E+01 & Direct-PRF & 0\\
006511799-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006520923-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006522745-01 & 006522750-01 & 1:1 & 43.5 & -9 & 5 & 11.23 & 4.72 & 9.8930E+02 & Direct-PRF & 0\\
006522824-01 & 006522750-01 & 1:1 & 64.5 & 6 & 15 & 11.23 & 4.58 & 9.2644E+02 & Direct-PRF & 0\\
006525106-01 & 5293.01 & 1:1 & 106.3 & -1 & -27 & 10.15 & 5.27 & 1.9212E+03 & Direct-PRF & 0\\
006525185-01 & 5293.01 & 1:1 & 76.3 & 17 & 8 & 10.15 & 5.71 & 7.4661E+02 & Direct-PRF & 0\\
006525193-01 & 5293.01 & 1:1 & 76.5 & -16 & -11 & 10.15 & 5.64 & 6.7323E+02 & Direct-PRF & 0\\
006525209-03 & 5293.01 & 1:1 & 63.8 & -15 & -7 & 10.15 & 4.50 & 1.2026E+03 & Direct-PRF & 0\\
006525249-01 & 5293.01 & 1:1 & 77.6 & -19 & 1 & 10.15 & 5.81 & 4.3160E+02 & Direct-PRF & 0\\
006525280-01 & 5293.01 & 1:1 & 84.8 & 0 & 21 & 10.15 & 3.23 & 4.6334E+03 & Direct-PRF & 0\\
006525462-01 & 006367628-pri & 1:1 & 912.2 & 230 & 1 & 13.04 & 1.11 & 8.0638E+03 & Col-Anomaly & 0\\
006531491-01 & 3646.01 & 1:1 & 8.3 & -1 & 1 & 16.09 & -0.49 & 7.0158E+01 & Direct-PRF & 0\\
006531491-02 & 006531496-02 & 2:1 & 8.3 & -1 & 1 & 16.09 & -0.49 & 4.1595E+01 & Direct-PRF & 0\\
006531496-03 & 006531491-03 & 1:1 & 8.3 & 1 & -1 & 15.61 & 0.49 & 4.0548E+00 & Direct-PRF & 0\\
006543645-01 & 006543682-01 & 1:1 & 45.0 & 7 & 9 & 13.91 & -0.46 & 2.3995E+04 & Direct-PRF & 0\\
006543674-01 & 006543682-01 & 1:1 & 5.6 & 0 & 1 & 13.91 & -0.37 & 2.1509E+00 & Direct-PRF & 0\\
006543683-01 & 006543682-01 & 1:1 & 13.6 & 3 & 1 & 13.91 & 0.09 & 9.1635E+01 & Direct-PRF & 0\\
006545051-01 & 006545018-pri & 1:2 & 22.8 & 0 & -6 & 13.75 & 1.99 & 1.3380E+03 & Direct-PRF & 0\\
006546528-01 & 006546508-01 & 1:1 & 10.3 & 1 & -2 & 15.74 & -1.14 & 1.2006E+02 & Direct-PRF & 0\\
006549623-01 & 005033298-01 & 2:1 & 7743.0 & -30 & -7 & 13.35 & -0.26 & 2.2727E-01 & Direct-PRF & 1\\
006584167-01 & 006669809-pri & 1:1 & 618.6 & 155 & -1 & 10.76 & 2.67 & 1.4406E+04 & Col-Anomaly & 0\\
006587796-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006612284-01 & 006206751-pri & 1:1 & 3776.4 & 0 & -2 & 12.14 & 3.75 & 1.5586E+03 & Cross-Talk & 0\\
006620691-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006634133-01 & 5308.01 & 1:1 & 12.7 & 3 & 0 & 14.10 & 0.03 & 8.7911E+01 & Direct-PRF & 0\\
006675056-01 & 3611.01 & 1:1 & 9.3 & 1 & 2 & 16.51 & -0.96 & 1.2620E+02 & Direct-PRF & 0\\
006676516-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006677256-01 & 006677267-01 & 1:1 & 19.5 & -4 & -3 & 12.77 & 1.75 & 2.8059E+01 & Direct-PRF & 0\\
006677256-02 & 006677267-02 & 1:1 & 19.5 & -4 & -3 & 12.77 & 1.75 & 2.5276E+01 & Direct-PRF & 0\\
006695801-01 & 006695889-pri & 1:1 & 117.2 & 30 & -1 & 15.41 & -0.83 & 3.3039E+03 & Col-Anomaly & 0\\
006699984-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006700200-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006705137-01 & 1758.01 & 1:1 & 5.1 & 0 & 2 & 15.97 & -1.34 & 9.1520E+00 & Direct-PRF & 0\\
006715577-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006778008-01 & 006778050-pri & 1:1 & 22.7 & -2 & -5 & 14.51 & 0.75 & 2.9959E+03 & Direct-PRF & 0\\
006778008-02 & 006778050-sec & 1:1 & 22.7 & -2 & -5 & 14.51 & 0.75 & 2.9349E+03 & Direct-PRF & 0\\
006778019-01 & 006778050-pri & 1:1 & 21.1 & 0 & -5 & 14.51 & 0.25 & 3.1934E+03 & Direct-PRF & 0\\
006778019-02 & 006778050-sec & 1:1 & 21.1 & 0 & -5 & 14.51 & 0.25 & 3.4800E+03 & Direct-PRF & 0\\
006781548-01 & 006781535-01 & 1:1 & 15.4 & 3 & -1 & 13.67 & 2.01 & 6.3816E+01 & Direct-PRF & 0\\
006781548-02 & 006781535-02 & 1:1 & 15.4 & 3 & -1 & 13.67 & 2.01 & 6.1063E+01 & Direct-PRF & 0\\
006792124-01 & 006791604-pri & 1:1 & 333.3 & 84 & 0 & 13.92 & -0.65 & 1.5830E+04 & Col-Anomaly & 0\\
006853248-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006859801-01 & 006859813-01 & 1:1 & 10.0 & -2 & -2 & 12.07 & 2.81 & 1.2539E+01 & Direct-PRF & 0\\
006859801-02 & 006859813-02 & 1:1 & 10.0 & -2 & -2 & 12.07 & 2.81 & 1.5543E+01 & Direct-PRF & 0\\
006861403-01 & RR-Lyr-pri & 1:1 & 1424.1 & 282 & -221 & 7.86 & 4.01 & 1.5582E+04 & Direct-PRF & 0\\
006861403-02 & RR-Lyr-pri & 1:1 & 1424.1 & 282 & -221 & 7.86 & 4.01 & 7.9910E+03 & Direct-PRF & 0\\
006862332-01 & 865.01 & 3:1 & 5.0 & 1 & 0 & 15.09 & 0.56 & 2.7838E+00 & Direct-PRF & 0\\
006863839-01 & 006863840-01 & 1:1 & 17.0 & 4 & -3 & 15.14 & -0.52 & 2.5384E+03 & Direct-PRF & 0\\
006864885-01 & 006864859-02 & 1:1 & 24.5 & 5 & 2 & 11.66 & 3.93 & 4.3972E+02 & Direct-PRF & 0\\
006864885-02 & 006864859-01 & 1:1 & 24.5 & 5 & 2 & 11.66 & 3.93 & 4.2462E+02 & Direct-PRF & 0\\
006864891-01 & 006864859-01 & 1:1 & 49.3 & 12 & 0 & 11.66 & 4.28 & 5.5760E+02 & Direct-PRF & 0\\
006864891-02 & 006864859-02 & 1:1 & 49.3 & 12 & 0 & 11.66 & 4.28 & 6.8374E+02 & Direct-PRF & 0\\
006864893-01 & 006864859-01 & 1:1 & 31.3 & 0 & 8 & 11.66 & 3.26 & 6.1763E+02 & Direct-PRF & 0\\
006864893-02 & 006864859-02 & 1:1 & 31.3 & 0 & 8 & 11.66 & 3.26 & 6.9682E+02 & Direct-PRF & 0\\
006869292-01 & 006869313-01 & 1:1 & 24.9 & 6 & 1 & 13.13 & 0.93 & 2.3261E+00 & Direct-PRF & 1\\
006869313-01 & 006869292-01 & 1:1 & 24.9 & -6 & -1 & 14.06 & -0.93 & 4.2991E-01 & Direct-PRF & 1\\
006891366-01 & 5335.01 & 1:1 & 63.9 & -9 & 13 & 11.39 & 2.22 & 3.1038E+03 & Direct-PRF & 0\\
006891543-01 & 5335.01 & 1:1 & 25.0 & -2 & -6 & 11.39 & 3.06 & 2.2522E+03 & Direct-PRF & 0\\
006891637-01 & 5335.01 & 1:1 & 63.4 & 5 & -15 & 11.39 & 4.44 & 5.5046E+02 & Direct-PRF & 0\\
006929016-01 & 006669809-pri & 1:1 & 1984.6 & -499 & 2 & 10.76 & 5.01 & 2.4010E+03 & Col-Anomaly & 0\\
006929841-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006936075-02 & FN-Lyr-pri & 1:1 & 57.3 & -1 & 15 & 12.88 & 2.64 & 1.6750E+04 & Direct-PRF & 0\\
006936075-03 & FN-Lyr-pri & 1:1 & 57.3 & -1 & 15 & 12.88 & 2.64 & 3.5001E+03 & Direct-PRF & 0\\
006937131-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006938584-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006946465-01 & RR-Lyr-pri & 1:1 & 1224.0 & 130 & -279 & 7.86 & 6.07 & 6.2330E+05 & Direct-PRF & 0\\
006946700-01 & RR-Lyr-pri & 1:1 & 1186.6 & 173 & -244 & 7.86 & 7.42 & 2.3973E+04 & Direct-PRF & 0\\
006947095-01 & RR-Lyr-pri & 1:1 & 1064.9 & 213 & -163 & 7.86 & 7.26 & 1.4166E+04 & Direct-PRF & 0\\
006947099-01 & RR-Lyr-pri & 1:1 & 1140.0 & 229 & -173 & 7.86 & 8.08 & 5.9932E+03 & Direct-PRF & 0\\
006947300-01 & RR-Lyr-pri & 1:1 & 1115.3 & 248 & -131 & 7.86 & 7.97 & 2.8178E+02 & Direct-PRF & 0\\
006947591-01 & RR-Lyr-pri & 1:1 & 1118.0 & 271 & -75 & 7.86 & 7.51 & 7.7912E+04 & Direct-PRF & 0\\
006948006-02 & RR-Lyr-pri & 1:1 & 1259.1 & 316 & 2 & 7.86 & 5.67 & 1.3290E+03 & Direct-PRF & 0\\
006950275-01 & 006864859-02 & 1:1 & 35.5 & -9 & 3 & 11.66 & 4.16 & 6.8929E+02 & Direct-PRF & 0\\
006950275-02 & 006864859-01 & 1:1 & 35.5 & -9 & 3 & 11.66 & 4.16 & 8.9954E+02 & Direct-PRF & 0\\
006951851-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006953219-01 & RR-Lyr-pri & 1:1 & 5133.8 & 922 & 0 & 7.86 & 7.04 & 5.1512E+03 & Col-Anomaly & 2\\
006953281-01 & RR-Lyr-pri & 1:1 & 5197.6 & 942 & -2 & 7.86 & 7.70 & 2.1493E+04 & Col-Anomaly & 2\\
006954721-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006956233-01 & 006956216-pri & 1:1 & 10.9 & 0 & -3 & 14.55 & 1.38 & 6.9268E+01 & Direct-PRF & 0\\
006956233-02 & 006956216-sec & 1:1 & 10.9 & 0 & -3 & 14.55 & 1.38 & 4.0884E+01 & Direct-PRF & 0\\
006960445-01 & 3654.01 & 1:2 & 6.7 & -1 & -1 & 16.80 & -2.96 & 2.2998E+02 & Direct-PRF & 0\\
006960456-01 & 3654.01 & 1:2 & 8.0 & 0 & -2 & 16.80 & -2.01 & 5.7003E+02 & Direct-PRF & 0\\
006962329-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
006967430-01 & 008504570-pri & 1:2 & 8373.6 & 1 & 2 & 13.25 & 1.22 & 3.1036E+03 & Cross-Talk & 0\\
007022432-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007023060-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007023872-02 & 007023917-sec & 1:1 & 52.0 & 5 & 12 & 10.12 & 4.81 & 1.9500E+03 & Direct-PRF & 0\\
007023973-01 & 007023917-pri & 1:1 & 47.9 & -11 & -3 & 10.12 & 1.65 & 8.2444E+03 & Direct-PRF & 0\\
007024511-01 & 007024530-01 & 6:1 & 12.7 & 1 & 4 & 15.52 & -2.87 & 2.7313E+01 & Direct-PRF & 0\\
007025526-01 & 3550.01 & 1:2 & 16.2 & 1 & 4 & 15.78 & -4.04 & 2.0389E+04 & Direct-PRF & 0\\
007025846-01 & 007025851-pri & 1:2 & 14.8 & 3 & -2 & 14.39 & -0.09 & 1.4476E+03 & Direct-PRF & 0\\
007030996-01 & RR-Lyr-pri & 1:1 & 1320.1 & -6 & -332 & 7.86 & 6.33 & 7.7912E+02 & Direct-PRF & 0\\
007031066-01 & RR-Lyr-pri & 1:1 & 1315.9 & 18 & -331 & 7.86 & 7.08 & 1.7314E+04 & Direct-PRF & 0\\
007031126-01 & RR-Lyr-pri & 1:1 & 1214.7 & 7 & -306 & 7.86 & 6.08 & 2.3973E+04 & Direct-PRF & 0\\
007031132-01 & RR-Lyr-pri & 1:1 & 1353.6 & 56 & -336 & 7.86 & 4.96 & 6.2330E+04 & Direct-PRF & 0\\
007031175-01 & RR-Lyr-pri & 1:1 & 1353.8 & 70 & -334 & 7.86 & 7.16 & 3.1165E+05 & Direct-PRF & 0\\
007031192-01 & RR-Lyr-pri & 1:1 & 1266.4 & 49 & -315 & 7.86 & 7.04 & 3.1165E+05 & Direct-PRF & 0\\
007031195-01 & RR-Lyr-pri & 1:1 & 1169.2 & 17 & -294 & 7.86 & 7.09 & 9.4439E+03 & Direct-PRF & 0\\
007031208-01 & RR-Lyr-pri & 1:1 & 1253.1 & 48 & -312 & 7.86 & 7.46 & 8.0948E+03 & Direct-PRF & 0\\
007031293-01 & RR-Lyr-pri & 1:1 & 1108.7 & 32 & -278 & 7.86 & 4.96 & 7.7912E+04 & Direct-PRF & 0\\
007031316-01 & RR-Lyr-pri & 1:1 & 1197.1 & 67 & -294 & 7.86 & 6.82 & 9.1661E+03 & Direct-PRF & 0\\
007031340-01 & RR-Lyr-pri & 1:1 & 1092.3 & 42 & -272 & 7.86 & 6.58 & 1.3851E+04 & Direct-PRF & 0\\
007031352-01 & RR-Lyr-pri & 1:1 & 1240.8 & 89 & -299 & 7.86 & 7.55 & 6.2330E+05 & Direct-PRF & 0\\
007031399-01 & RR-Lyr-pri & 1:1 & 1091.8 & 61 & -268 & 7.86 & 8.09 & 6.0514E+03 & Direct-PRF & 0\\
007031421-01 & RR-Lyr-pri & 1:1 & 1130.6 & 80 & -273 & 7.86 & 5.70 & 2.8332E+04 & Direct-PRF & 0\\
007031430-01 & RR-Lyr-pri & 1:1 & 1011.0 & 48 & -250 & 7.86 & 7.65 & 6.2330E+03 & Direct-PRF & 0\\
007031477-01 & RR-Lyr-pri & 1:1 & 1142.3 & 98 & -271 & 7.86 & 7.63 & 1.1130E+04 & Direct-PRF & 0\\
007031504-01 & RR-Lyr-pri & 1:1 & 1029.8 & 78 & -247 & 7.86 & 7.76 & 1.5982E+04 & Direct-PRF & 0\\
007031515-01 & RR-Lyr-pri & 1:1 & 1068.2 & 90 & -254 & 7.86 & 7.94 & 7.7912E+03 & Direct-PRF & 0\\
007031520-01 & RR-Lyr-pri & 1:1 & 1086.5 & 96 & -256 & 7.86 & 5.78 & 3.6664E+04 & Direct-PRF & 0\\
007031573-01 & RR-Lyr-pri & 1:1 & 924.4 & 65 & -224 & 7.86 & 7.32 & 1.0746E+04 & Direct-PRF & 0\\
007031638-01 & RR-Lyr-pri & 1:1 & 930.0 & 84 & -219 & 7.86 & 5.28 & 2.9681E+04 & Direct-PRF & 0\\
007031656-01 & RR-Lyr-pri & 1:1 & 926.9 & 87 & -217 & 7.86 & 6.42 & 1.1760E+04 & Direct-PRF & 0\\
007031659-01 & RR-Lyr-pri & 1:1 & 1124.8 & 137 & -248 & 7.86 & 4.47 & 1.2466E+05 & Direct-PRF & 0\\
007031716-02 & RR-Lyr-pri & 1:1 & 991.6 & 119 & -220 & 7.86 & 6.79 & 1.8332E+04 & Direct-PRF & 0\\
007031726-01 & RR-Lyr-pri & 1:1 & 842.6 & 83 & -195 & 7.86 & 3.61 & 1.8888E+04 & Direct-PRF & 0\\
007031732-01 & RR-Lyr-pri & 1:1 & 840.9 & 84 & -194 & 7.86 & 5.79 & 1.6846E+04 & Direct-PRF & 0\\
007031742-01 & RR-Lyr-pri & 1:1 & 939.7 & 112 & -209 & 7.86 & 7.47 & 6.2330E+05 & Direct-PRF & 0\\
007031753-01 & RR-Lyr-pri & 1:1 & 941.8 & 116 & -207 & 7.86 & 7.41 & 6.2330E+05 & Direct-PRF & 0\\
007031767-01 & RR-Lyr-pri & 1:1 & 1022.9 & 138 & -217 & 7.86 & 6.45 & 2.3973E+04 & Direct-PRF & 0\\
007031781-01 & RR-Lyr-pri & 1:1 & 960.1 & 127 & -206 & 7.86 & 7.96 & 5.4200E+03 & Direct-PRF & 0\\
007031824-01 & RR-Lyr-pri & 1:1 & 965.3 & 137 & -201 & 7.86 & 7.08 & 2.4932E+04 & Direct-PRF & 0\\
007031853-01 & RR-Lyr-pri & 1:1 & 960.8 & 141 & -196 & 7.86 & 7.70 & 8.9042E+03 & Direct-PRF & 0\\
007031872-01 & RR-Lyr-pri & 1:1 & 947.7 & 143 & -191 & 7.86 & 6.11 & 2.3973E+04 & Direct-PRF & 0\\
007031880-01 & RR-Lyr-pri & 1:1 & 756.8 & 100 & -162 & 7.86 & 7.87 & 6.2330E+05 & Direct-PRF & 0\\
007031898-01 & RR-Lyr-pri & 1:1 & 859.6 & 126 & -176 & 7.86 & 5.12 & 3.1165E+04 & Direct-PRF & 0\\
007031904-01 & RR-Lyr-pri & 1:1 & 982.7 & 155 & -193 & 7.86 & 5.47 & 4.1553E+04 & Direct-PRF & 0\\
007031914-01 & RR-Lyr-pri & 1:1 & 916.7 & 141 & -183 & 7.86 & 8.00 & 3.1165E+05 & Direct-PRF & 0\\
007031942-01 & RR-Lyr-pri & 1:1 & 789.3 & 117 & -161 & 7.86 & 6.01 & 1.8332E+04 & Direct-PRF & 0\\
007031948-01 & RR-Lyr-pri & 1:1 & 774.0 & 115 & -158 & 7.86 & 7.90 & 6.4257E+03 & Direct-PRF & 0\\
007031956-01 & RR-Lyr-pri & 1:1 & 857.5 & 135 & -168 & 7.86 & 6.34 & 2.7100E+04 & Direct-PRF & 0\\
007031992-01 & RR-Lyr-pri & 1:1 & 727.3 & 113 & -144 & 7.86 & 7.93 & 1.2221E+04 & Direct-PRF & 0\\
007032001-01 & RR-Lyr-pri & 1:1 & 919.0 & 157 & -170 & 7.86 & 6.98 & 2.2261E+04 & Direct-PRF & 0\\
007032116-01 & RR-Lyr-pri & 1:1 & 830.2 & 157 & -138 & 7.86 & 6.58 & 6.2330E+05 & Direct-PRF & 0\\
007032116-02 & RR-Lyr-pri & 1:1 & 830.2 & 157 & -138 & 7.86 & 6.58 & 2.0777E+04 & Direct-PRF & 0\\
007032117-01 & RR-Lyr-pri & 1:1 & 854.6 & 162 & -141 & 7.86 & 7.01 & 8.3106E+03 & Direct-PRF & 0\\
007032132-01 & RR-Lyr-pri & 1:1 & 989.5 & 194 & -156 & 7.86 & 5.83 & 2.8332E+04 & Direct-PRF & 0\\
007032174-01 & RR-Lyr-pri & 1:1 & 903.2 & 180 & -139 & 7.86 & 4.12 & 4.1553E+04 & Direct-PRF & 0\\
007032274-01 & RR-Lyr-pri & 1:1 & 841.6 & 180 & -112 & 7.86 & 7.70 & 2.0777E+05 & Direct-PRF & 0\\
007032365-01 & RR-Lyr-pri & 1:1 & 791.9 & 179 & -87 & 7.86 & 7.32 & 1.8888E+04 & Direct-PRF & 0\\
007032369-01 & RR-Lyr-pri & 1:1 & 1018.9 & 228 & -117 & 7.86 & 7.42 & 2.0777E+05 & Direct-PRF & 0\\
007032383-01 & RR-Lyr-pri & 1:1 & 735.5 & 169 & -76 & 7.86 & 7.49 & 8.7788E+03 & Direct-PRF & 0\\
007032388-01 & RR-Lyr-pri & 1:1 & 900.7 & 204 & -98 & 7.86 & 5.98 & 6.2330E+05 & Direct-PRF & 0\\
007032388-02 & RR-Lyr-pri & 1:1 & 900.7 & 204 & -98 & 7.86 & 5.98 & 6.2330E+05 & Direct-PRF & 0\\
007032421-02 & RR-Lyr-pri & 1:1 & 749.1 & 175 & -71 & 7.86 & 6.93 & 1.6846E+04 & Direct-PRF & 0\\
007032429-01 & RR-Lyr-pri & 1:1 & 955.1 & 219 & -98 & 7.86 & 7.76 & 3.4570E+02 & Direct-PRF & 0\\
007032438-01 & RR-Lyr-pri & 1:1 & 782.4 & 183 & -73 & 7.86 & 7.88 & 8.3106E+03 & Direct-PRF & 0\\
007032456-01 & RR-Lyr-pri & 1:1 & 772.3 & 182 & -68 & 7.86 & 8.01 & 1.9478E+04 & Direct-PRF & 0\\
007032481-01 & RR-Lyr-pri & 1:1 & 746.4 & 178 & -59 & 7.86 & 7.17 & 7.7912E+04 & Direct-PRF & 0\\
007032524-01 & RR-Lyr-pri & 1:1 & 919.9 & 219 & -74 & 7.86 & 7.76 & 6.2330E+05 & Direct-PRF & 0\\
007032568-01 & RR-Lyr-pri & 1:1 & 772.4 & 189 & -46 & 7.86 & 5.97 & 2.8332E+04 & Direct-PRF & 0\\
007032687-01 & RR-Lyr-pri & 1:1 & 965.8 & 238 & -50 & 7.86 & 7.91 & 9.1661E+03 & Direct-PRF & 0\\
007032807-01 & RR-Lyr-pri & 1:1 & 1072.4 & 266 & -43 & 7.86 & 7.97 & 2.3102E+02 & Direct-PRF & 0\\
007032833-01 & RR-Lyr-pri & 1:1 & 1001.3 & 250 & -26 & 7.86 & 6.80 & 6.2330E+05 & Direct-PRF & 0\\
007032891-01 & RR-Lyr-pri & 1:1 & 1027.9 & 258 & -15 & 7.86 & 7.25 & 6.2330E+05 & Direct-PRF & 0\\
007032923-01 & RR-Lyr-pri & 1:1 & 1093.7 & 275 & -14 & 7.86 & 6.72 & 3.1165E+04 & Direct-PRF & 0\\
007032938-01 & RR-Lyr-pri & 1:1 & 1135.4 & 285 & -17 & 7.86 & 8.06 & 2.0680E+02 & Direct-PRF & 0\\
007032968-01 & RR-Lyr-pri & 1:1 & 1146.9 & 288 & -10 & 7.86 & 3.92 & 8.9042E+04 & Direct-PRF & 0\\
007032999-01 & RR-Lyr-pri & 1:1 & 945.6 & 236 & 30 & 7.86 & 8.12 & 2.0777E+05 & Direct-PRF & 0\\
007033044-01 & RR-Lyr-pri & 1:1 & 1026.8 & 257 & 28 & 7.86 & 7.50 & 6.2330E+05 & Direct-PRF & 0\\
007033067-01 & RR-Lyr-pri & 1:1 & 1015.6 & 252 & 38 & 7.86 & 6.48 & 2.7100E+04 & Direct-PRF & 0\\
007033421-01 & RR-Lyr-pri & 1:1 & 1232.1 & 289 & 110 & 7.86 & 6.69 & 2.5971E+04 & Direct-PRF & 0\\
007033713-01 & 007033748-pri & 1:2 & 30.6 & -8 & -2 & 13.69 & 2.13 & 3.1055E+03 & Direct-PRF & 0\\
007038096-01 & RR-Lyr-pri & 1:1 & 4900.3 & 836 & -1 & 7.86 & 6.79 & 7.1643E+03 & Col-Anomaly & 2\\
007038372-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007041882-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007049849-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007091610-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007097534-01 & 007097571-pri & 1:1 & 39.6 & 5 & -8 & 11.27 & 3.19 & 1.9485E+03 & Direct-PRF & 0\\
007102615-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007107561-01 & 5353.01 & 1:1 & 13.0 & 3 & -1 & 14.23 & -0.81 & 1.5166E+02 & Direct-PRF & 0\\
007115085-01 & RR-Lyr-pri & 1:1 & 1305.1 & -24 & -328 & 7.86 & 7.38 & 1.1130E+04 & Direct-PRF & 0\\
007115200-01 & RR-Lyr-pri & 1:1 & 1207.5 & -17 & -304 & 7.86 & 4.90 & 5.1941E+04 & Direct-PRF & 0\\
007115237-01 & RR-Lyr-pri & 1:1 & 1196.1 & -2 & -301 & 7.86 & 7.17 & 1.9478E+04 & Direct-PRF & 0\\
007115249-01 & RR-Lyr-pri & 1:1 & 1165.0 & -9 & -293 & 7.86 & 7.16 & 6.2330E+05 & Direct-PRF & 0\\
007115291-02 & RR-Lyr-pri & 1:1 & 1129.1 & -8 & -284 & 7.86 & 7.33 & 8.5383E+03 & Direct-PRF & 0\\
007115308-01 & RR-Lyr-pri & 1:1 & 1123.8 & -2 & -283 & 7.86 & 6.95 & 5.4868E+02 & Direct-PRF & 0\\
007115323-01 & RR-Lyr-pri & 1:1 & 1066.9 & -22 & -268 & 7.86 & 6.65 & 6.2330E+05 & Direct-PRF & 0\\
007115323-02 & RR-Lyr-pri & 1:1 & 1066.9 & -22 & -268 & 7.86 & 6.65 & 2.8332E+04 & Direct-PRF & 0\\
007115323-03 & RR-Lyr-pri & 1:1 & 1066.9 & -22 & -268 & 7.86 & 6.65 & 7.8898E+03 & Direct-PRF & 0\\
007115332-01 & RR-Lyr-pri & 1:1 & 1042.7 & -26 & -261 & 7.86 & 7.08 & 1.1333E+04 & Direct-PRF & 0\\
007115366-01 & RR-Lyr-pri & 1:1 & 1064.6 & -1 & -268 & 7.86 & 7.88 & 8.5383E+03 & Direct-PRF & 0\\
007115384-01 & RR-Lyr-pri & 1:1 & 1006.4 & -18 & -253 & 7.86 & 2.77 & 5.6663E+04 & Direct-PRF & 0\\
007115390-01 & RR-Lyr-pri & 1:1 & 983.9 & -26 & -247 & 7.86 & 8.10 & 5.4200E+03 & Direct-PRF & 0\\
007115427-01 & RR-Lyr-pri & 1:1 & 1002.4 & 5 & -253 & 7.86 & 7.21 & 2.0777E+05 & Direct-PRF & 0\\
007115450-01 & RR-Lyr-pri & 1:1 & 1034.4 & 26 & -259 & 7.86 & 2.15 & 2.0777E+05 & Direct-PRF & 0\\
007115463-01 & RR-Lyr-pri & 1:1 & 958.1 & 4 & -241 & 7.86 & 7.26 & 1.5582E+04 & Direct-PRF & 0\\
007115499-01 & RR-Lyr-pri & 1:1 & 863.4 & -19 & -217 & 7.86 & 7.78 & 3.2096E+02 & Direct-PRF & 0\\
007115530-01 & RR-Lyr-pri & 1:1 & 927.5 & 16 & -233 & 7.86 & 7.67 & 1.5582E+05 & Direct-PRF & 0\\
007115550-01 & RR-Lyr-pri & 1:1 & 956.7 & 30 & -239 & 7.86 & 6.36 & 1.8332E+04 & Direct-PRF & 0\\
007115597-01 & RR-Lyr-pri & 1:1 & 854.0 & 12 & -215 & 7.86 & 8.05 & 3.9449E+03 & Direct-PRF & 0\\
007115661-01 & RR-Lyr-pri & 1:1 & 775.8 & 5 & -136 & 7.86 & 2.76 & 6.2330E+05 & Direct-PRF & 0\\
007115671-01 & RR-Lyr-pri & 1:1 & 855.9 & 36 & -213 & 7.86 & 5.99 & 1.5982E+04 & Direct-PRF & 0\\
007115733-01 & RR-Lyr-pri & 1:1 & 811.1 & 43 & -200 & 7.86 & 6.71 & 1.4495E+04 & Direct-PRF & 0\\
007115785-03 & RR-Lyr-pri & 1:1 & 733.4 & 39 & -181 & 7.86 & 6.14 & 1.5982E+04 & Direct-PRF & 0\\
007115816-01 & RR-Lyr-pri & 1:1 & 749.2 & 52 & -181 & 7.86 & 7.19 & 1.3550E+04 & Direct-PRF & 0\\
007115842-01 & RR-Lyr-pri & 1:1 & 687.3 & 41 & -168 & 7.86 & 6.25 & 2.0777E+04 & Direct-PRF & 0\\
007115869-01 & RR-Lyr-pri & 1:1 & 791.2 & 77 & -184 & 7.86 & 5.55 & 1.5582E+05 & Direct-PRF & 0\\
007115878-01 & RR-Lyr-pri & 1:1 & 563.9 & 15 & -142 & 7.86 & 7.04 & 1.1760E+04 & Direct-PRF & 0\\
007115879-01 & RR-Lyr-pri & 1:1 & 543.6 & 8 & -137 & 7.86 & 6.68 & 3.2805E+04 & Direct-PRF & 0\\
007115923-01 & RR-Lyr-pri & 1:1 & 578.5 & 33 & -142 & 7.86 & 5.93 & 1.0201E+03 & Direct-PRF & 0\\
007115925-01 & RR-Lyr-pri & 1:1 & 700.2 & 66 & -164 & 7.86 & 4.67 & 3.8956E+04 & Direct-PRF & 0\\
007116043-01 & RR-Lyr-pri & 1:1 & 650.3 & 78 & -144 & 7.86 & 6.67 & 9.0333E+03 & Direct-PRF & 0\\
007116046-01 & RR-Lyr-pri & 1:1 & 690.5 & 88 & -150 & 7.86 & 7.95 & 2.8332E+04 & Direct-PRF & 0\\
007116072-01 & RR-Lyr-pri & 1:1 & 591.7 & 70 & -132 & 7.86 & 5.77 & 3.8956E+04 & Direct-PRF & 0\\
007116117-01 & RR-Lyr-pri & 2:1 & 418.9 & 36 & -99 & 7.86 & 2.38 & 1.2466E+05 & Direct-PRF & 0\\
007116166-01 & RR-Lyr-pri & 1:1 & 522.9 & 73 & -110 & 7.86 & 7.88 & 1.2466E+05 & Direct-PRF & 0\\
007116217-01 & RR-Lyr-pri & 1:1 & 539.5 & 87 & -105 & 7.86 & 7.59 & 2.0777E+04 & Direct-PRF & 0\\
007116226-01 & RR-Lyr-pri & 1:1 & 622.6 & 108 & -114 & 7.86 & 7.56 & 5.2290E+02 & Direct-PRF & 0\\
007116236-01 & RR-Lyr-pri & 1:1 & 615.6 & 108 & -112 & 7.86 & 7.81 & 7.6012E+03 & Direct-PRF & 0\\
007116282-01 & RR-Lyr-pri & 1:1 & 518.6 & 94 & -90 & 7.86 & 7.73 & 1.1986E+04 & Direct-PRF & 0\\
007116382-01 & RR-Lyr-pri & 1:1 & 307.9 & 63 & -45 & 7.86 & 7.91 & 5.3732E+03 & Direct-PRF & 0\\
007116466-01 & RR-Lyr-pri & 1:1 & 635.1 & 140 & -76 & 7.86 & 8.06 & 7.9910E+03 & Direct-PRF & 0\\
007116519-01 & RR-Lyr-pri & 1:1 & 608.1 & 139 & -64 & 7.86 & 7.91 & 6.2330E+05 & Direct-PRF & 0\\
007116561-01 & RR-Lyr-pri & 1:1 & 371.3 & 90 & -25 & 7.86 & 7.96 & 8.4229E+03 & Direct-PRF & 0\\
007116632-01 & RR-Lyr-pri & 1:1 & 378.1 & 94 & -13 & 7.86 & 8.04 & 5.4675E+03 & Direct-PRF & 0\\
007116670-01 & RR-Lyr-pri & 1:1 & 384.7 & 96 & -6 & 7.86 & 8.14 & 1.2985E+04 & Direct-PRF & 0\\
007116766-01 & RR-Lyr-pri & 1:1 & 603.5 & 151 & -17 & 7.86 & 7.30 & 8.9042E+04 & Direct-PRF & 0\\
007116842-01 & RR-Lyr-pri & 1:1 & 718.8 & 180 & -15 & 7.86 & 6.19 & 2.5971E+04 & Direct-PRF & 0\\
007116851-01 & RR-Lyr-pri & 1:1 & 684.9 & 172 & -8 & 7.86 & 7.69 & 5.7183E+03 & Direct-PRF & 0\\
007116859-01 & RR-Lyr-pri & 1:1 & 691.3 & 174 & -8 & 7.86 & 7.30 & 1.1986E+04 & Direct-PRF & 0\\
007117003-03 & RR-Lyr-pri & 1:1 & 703.3 & 174 & 29 & 7.86 & 6.31 & 2.7100E+04 & Direct-PRF & 0\\
007117020-01 & RR-Lyr-pri & 1:1 & 692.4 & 171 & 33 & 7.86 & 7.43 & 1.0746E+04 & Direct-PRF & 0\\
007117126-01 & RR-Lyr-pri & 1:1 & 820.3 & 202 & 43 & 7.86 & 5.86 & 7.7912E+04 & Direct-PRF & 0\\
007117147-01 & RR-Lyr-pri & 1:1 & 722.6 & 167 & 70 & 7.86 & 4.89 & 3.4628E+04 & Direct-PRF & 0\\
007117178-01 & RR-Lyr-pri & 1:1 & 802.9 & 191 & 64 & 7.86 & 6.09 & 4.7946E+04 & Direct-PRF & 0\\
007117226-01 & RR-Lyr-pri & 1:1 & 779.9 & 177 & 84 & 7.86 & 7.14 & 6.2330E+05 & Direct-PRF & 0\\
007117270-01 & RR-Lyr-pri & 1:1 & 841.2 & 193 & 85 & 7.86 & 7.52 & 1.5582E+05 & Direct-PRF & 0\\
007117284-01 & RR-Lyr-pri & 1:1 & 868.7 & 201 & 85 & 7.86 & 5.57 & 6.2330E+04 & Direct-PRF & 0\\
007117348-01 & RR-Lyr-pri & 1:1 & 994.2 & 237 & 78 & 7.86 & 7.34 & 8.7788E+03 & Direct-PRF & 0\\
007117355-01 & RR-Lyr-pri & 1:1 & 946.7 & 220 & 90 & 7.86 & 7.03 & 7.2392E+02 & Direct-PRF & 0\\
007117413-01 & RR-Lyr-pri & 1:1 & 1050.7 & 249 & 87 & 7.86 & 7.52 & 3.1165E+05 & Direct-PRF & 0\\
007117436-01 & RR-Lyr-pri & 1:1 & 1054.7 & 247 & 95 & 7.86 & 7.22 & 5.9080E+02 & Direct-PRF & 0\\
007117457-01 & RR-Lyr-pri & 1:1 & 1069.3 & 248 & 103 & 7.86 & 7.92 & 9.0333E+03 & Direct-PRF & 0\\
007117485-01 & RR-Lyr-pri & 1:1 & 1092.1 & 252 & 108 & 7.86 & 7.59 & 5.1941E+04 & Direct-PRF & 0\\
007117491-01 & RR-Lyr-pri & 1:1 & 979.6 & 201 & 141 & 7.86 & 8.06 & 8.6569E+03 & Direct-PRF & 0\\
007117492-01 & RR-Lyr-pri & 1:1 & 966.9 & 194 & 146 & 7.86 & 6.44 & 1.7808E+04 & Direct-PRF & 0\\
007117513-01 & RR-Lyr-pri & 1:1 & 987.0 & 198 & 149 & 7.86 & 8.05 & 6.4927E+03 & Direct-PRF & 0\\
007117549-01 & RR-Lyr-pri & 1:1 & 1027.3 & 208 & 152 & 7.86 & 7.20 & 4.2575E+02 & Direct-PRF & 0\\
007117561-01 & RR-Lyr-pri & 1:1 & 1043.5 & 216 & 149 & 7.86 & 7.95 & 6.2330E+05 & Direct-PRF & 0\\
007117568-01 & RR-Lyr-pri & 1:1 & 1064.2 & 225 & 145 & 7.86 & 6.67 & 2.3085E+04 & Direct-PRF & 0\\
007117585-01 & RR-Lyr-pri & 1:1 & 1043.4 & 208 & 160 & 7.86 & 7.16 & 3.8835E+02 & Direct-PRF & 0\\
007117610-01 & RR-Lyr-pri & 1:1 & 1081.2 & 223 & 155 & 7.86 & 7.99 & 6.9255E+04 & Direct-PRF & 0\\
007117710-01 & RR-Lyr-pri & 1:1 & 1146.0 & 231 & 172 & 7.86 & 5.82 & 2.0777E+04 & Direct-PRF & 0\\
007117723-01 & RR-Lyr-pri & 1:1 & 1125.2 & 210 & 189 & 7.86 & 7.82 & 2.3646E+02 & Direct-PRF & 0\\
007137725-01 & 007137798-pri & 1:1 & 48.7 & 12 & 0 & 13.45 & -0.33 & 2.2884E+03 & Direct-PRF & 0\\
007174351-01 & 3844.01 & 1:2 & 7.4 & -1 & -2 & 19.29 & -3.77 & 7.0737E+02 & Direct-PRF & 0\\
007177555-01 & 007177553-01 & 1:1 & 8.8 & -1 & 2 & 11.51 & 3.33 & 1.8871E+00 & Direct-PRF & 0\\
007177555-02 & 007177553-02 & 1:1 & 8.8 & -1 & 2 & 11.51 & 3.33 & 1.9464E+00 & Direct-PRF & 0\\
007177766-02 & 007259917-pri & 2:1 & 494.9 & 124 & 0 & 12.13 & -0.08 & 1.8545E+04 & Col-Anomaly & 0\\
007198648-01 & RR-Lyr-pri & 1:1 & 267.9 & 2 & -68 & 7.86 & 7.66 & 4.2692E+03 & Direct-PRF & 0\\
007198734-01 & RR-Lyr-pri & 1:1 & 194.5 & 0 & -49 & 7.86 & 5.83 & 1.5582E+05 & Direct-PRF & 0\\
007198769-01 & RR-Lyr-pri & 1:1 & 184.7 & 9 & -46 & 7.86 & 7.93 & 5.9932E+03 & Direct-PRF & 0\\
007198791-01 & RR-Lyr-pri & 1:1 & 233.3 & 25 & -53 & 7.86 & 7.96 & 6.2330E+05 & Direct-PRF & 0\\
007198817-01 & RR-Lyr-pri & 1:1 & 237.7 & 31 & -51 & 7.86 & 4.41 & 2.3085E+04 & Direct-PRF & 0\\
007198906-02 & 007198959-01 & 1:1 & 92.4 & 13 & -19 & 7.86 & 4.75 & 1.1765E+03 & Direct-PRF & 0\\
007198941-01 & RR-Lyr-pri & 1:1 & 273.0 & 56 & -40 & 7.86 & 7.93 & 1.0388E+05 & Direct-PRF & 0\\
007198941-02 & RR-Lyr-pri & 1:1 & 273.0 & 56 & -40 & 7.86 & 7.93 & 5.4675E+03 & Direct-PRF & 0\\
007199013-01 & 007198959-01 & 2:1 & 37.1 & -3 & 8 & 7.86 & 6.30 & 5.0066E+02 & Direct-PRF & 0\\
007199037-01 & RR-Lyr-pri & 1:1 & 63.2 & 16 & 0 & 7.86 & 6.95 & 4.3284E+03 & Direct-PRF & 0\\
007199060-01 & RR-Lyr-pri & 1:1 & 275.8 & 64 & -26 & 7.86 & 5.11 & 2.0777E+04 & Direct-PRF & 0\\
007199168-01 & RR-Lyr-pri & 1:1 & 284.0 & 71 & 1 & 7.86 & 7.84 & 5.4993E+01 & Direct-PRF & 0\\
007199203-01 & RR-Lyr-pri & 1:1 & 220.2 & 50 & 22 & 7.86 & 3.36 & 6.2330E+04 & Direct-PRF & 0\\
007199203-02 & RR-Lyr-pri & 1:1 & 220.2 & 50 & 22 & 7.86 & 3.36 & 7.7912E+04 & Direct-PRF & 0\\
007199225-01 & RR-Lyr-pri & 1:1 & 211.0 & 18 & 49 & 7.86 & 3.81 & 1.5582E+04 & Direct-PRF & 0\\
007199272-01 & RR-Lyr-pri & 1:1 & 264.1 & 53 & 39 & 7.86 & 5.47 & 8.7788E+03 & Direct-PRF & 0\\
007199343-01 & RR-Lyr-pri & 1:1 & 369.4 & 85 & 37 & 7.86 & 7.70 & 6.2330E+05 & Direct-PRF & 0\\
007199343-02 & RR-Lyr-pri & 1:1 & 369.4 & 85 & 37 & 7.86 & 7.70 & 6.6308E+03 & Direct-PRF & 0\\
007199351-01 & RR-Lyr-pri & 1:1 & 382.3 & 89 & 36 & 7.86 & 5.41 & 2.4932E+04 & Direct-PRF & 0\\
007199418-01 & RR-Lyr-pri & 1:1 & 374.4 & 72 & 60 & 7.86 & 7.59 & 4.7946E+04 & Direct-PRF & 0\\
007199724-01 & RR-Lyr-pri & 1:1 & 644.9 & 131 & 95 & 7.86 & 6.69 & 8.2229E+02 & Direct-PRF & 0\\
007199756-01 & RR-Lyr-pri & 1:1 & 697.1 & 147 & 95 & 7.86 & 7.88 & 6.4257E+03 & Direct-PRF & 0\\
007199814-01 & RR-Lyr-pri & 1:1 & 725.8 & 148 & 106 & 7.86 & 7.42 & 1.2466E+04 & Direct-PRF & 0\\
007199883-01 & RR-Lyr-pri & 1:1 & 768.8 & 146 & 126 & 7.86 & 5.71 & 6.2330E+04 & Direct-PRF & 0\\
007199884-01 & RR-Lyr-pri & 1:1 & 743.4 & 122 & 141 & 7.86 & 5.18 & 6.9255E+04 & Direct-PRF & 0\\
007199906-01 & RR-Lyr-pri & 1:1 & 808.4 & 165 & 118 & 7.86 & 7.27 & 5.1898E+02 & Direct-PRF & 0\\
007199917-01 & RR-Lyr-pri & 1:1 & 781.9 & 142 & 136 & 7.86 & 4.92 & 1.5582E+05 & Direct-PRF & 0\\
007199935-01 & RR-Lyr-pri & 1:1 & 794.7 & 145 & 136 & 7.86 & 5.52 & 1.8332E+04 & Direct-PRF & 0\\
007199989-01 & RR-Lyr-pri & 1:1 & 808.6 & 111 & 170 & 7.86 & 4.50 & 5.1941E+04 & Direct-PRF & 0\\
007200001-01 & RR-Lyr-pri & 1:1 & 824.9 & 132 & 159 & 7.86 & 6.93 & 2.0106E+04 & Direct-PRF & 0\\
007200012-01 & RR-Lyr-pri & 1:1 & 827.8 & 109 & 177 & 7.86 & 7.88 & 1.2466E+05 & Direct-PRF & 0\\
007200013-01 & RR-Lyr-pri & 1:1 & 842.9 & 142 & 157 & 7.86 & 7.61 & 6.5610E+03 & Direct-PRF & 0\\
007200050-01 & RR-Lyr-pri & 1:1 & 868.0 & 145 & 163 & 7.86 & 7.48 & 1.4495E+04 & Direct-PRF & 0\\
007200111-01 & RR-Lyr-pri & 1:1 & 941.2 & 170 & 164 & 7.86 & 4.29 & 4.1553E+04 & Direct-PRF & 0\\
007200148-01 & RR-Lyr-pri & 1:1 & 965.9 & 165 & 178 & 7.86 & 7.73 & 8.9042E+04 & Direct-PRF & 0\\
007200156-01 & RR-Lyr-pri & 1:1 & 974.0 & 167 & 178 & 7.86 & 6.94 & 6.2330E+05 & Direct-PRF & 0\\
007200225-01 & RR-Lyr-pri & 1:1 & 997.8 & 145 & 204 & 7.86 & 7.47 & 5.5159E+03 & Direct-PRF & 0\\
007200299-01 & RR-Lyr-pri & 1:1 & 1076.7 & 180 & 201 & 7.86 & 6.31 & 2.0777E+04 & Direct-PRF & 0\\
007200301-01 & RR-Lyr-pri & 1:1 & 1066.9 & 164 & 212 & 7.86 & 6.84 & 1.0388E+04 & Direct-PRF & 0\\
007200303-01 & RR-Lyr-pri & 1:1 & 1063.4 & 151 & 220 & 7.86 & 7.83 & 4.2750E+02 & Direct-PRF & 0\\
007200359-01 & RR-Lyr-pri & 1:1 & 1116.2 & 141 & 242 & 7.86 & 7.27 & 3.1165E+05 & Direct-PRF & 0\\
007200463-01 & RR-Lyr-pri & 1:1 & 1228.9 & 212 & 224 & 7.86 & 7.96 & 5.7713E+03 & Direct-PRF & 0\\
007203194-01 & 007203179-pri & 1:1 & 48.2 & -8 & -9 & 13.43 & 0.81 & 1.1632E+04 & Direct-PRF & 0\\
007204073-01 & RR-Lyr-pri & 1:1 & 4208.6 & 549 & -1 & 7.86 & 4.80 & 2.2261E+04 & Col-Anomaly & 2\\
007220322-01 & 3775.01 & 1:1 & 4.5 & 0 & -1 & 14.08 & -2.20 & 8.3291E+01 & Direct-PRF & 0\\
007257363-01 & 007257373-01 & 1:1 & 24.9 & 1 & 6 & 13.42 & 2.09 & 1.6069E+03 & Direct-PRF & 0\\
007258902-01 & 007258889-pri & 1:1 & 20.8 & 0 & -5 & 13.67 & 1.98 & 1.0918E+03 & Direct-PRF & 0\\
007266266-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007280944-01 & RR-Lyr-pri & 1:1 & 237.1 & 14 & 57 & 7.86 & 4.87 & 6.2330E+05 & Direct-PRF & 0\\
007280953-01 & RR-Lyr-pri & 1:1 & 332.4 & -20 & 81 & 7.86 & 5.21 & 1.3262E+04 & Direct-PRF & 0\\
007281217-01 & RR-Lyr-pri & 1:1 & 521.8 & -5 & 131 & 7.86 & 7.78 & 4.3526E+02 & Direct-PRF & 0\\
007281229-01 & RR-Lyr-pri & 1:1 & 481.6 & 18 & 119 & 7.86 & 8.11 & 2.7714E+02 & Direct-PRF & 0\\
007281301-01 & RR-Lyr-pri & 1:1 & 505.4 & 50 & 116 & 7.86 & 5.80 & 9.8623E+02 & Direct-PRF & 0\\
007281311-01 & RR-Lyr-pri & 1:1 & 513.6 & 44 & 121 & 7.86 & 7.98 & 9.5892E+03 & Direct-PRF & 0\\
007281356-01 & RR-Lyr-pri & 1:1 & 590.8 & 17 & 147 & 7.86 & 7.17 & 2.0777E+05 & Direct-PRF & 0\\
007281357-01 & RR-Lyr-pri & 1:1 & 640.1 & -3 & 160 & 7.86 & 8.13 & 6.2330E+05 & Direct-PRF & 0\\
007281372-01 & RR-Lyr-pri & 1:1 & 565.8 & 50 & 133 & 7.86 & 7.79 & 6.2330E+05 & Direct-PRF & 0\\
007281399-01 & RR-Lyr-pri & 1:1 & 596.7 & 42 & 143 & 7.86 & 8.13 & 5.1090E+03 & Direct-PRF & 0\\
007281410-01 & RR-Lyr-pri & 1:1 & 695.6 & -2 & 174 & 7.86 & 3.72 & 3.8956E+04 & Direct-PRF & 0\\
007281411-01 & RR-Lyr-pri & 1:1 & 602.9 & 45 & 144 & 7.86 & 7.91 & 5.9362E+03 & Direct-PRF & 0\\
007281454-01 & RR-Lyr-pri & 1:1 & 684.5 & 23 & 170 & 7.86 & 6.79 & 1.2466E+05 & Direct-PRF & 0\\
007281468-01 & RR-Lyr-pri & 1:1 & 652.0 & 55 & 154 & 7.86 & 7.26 & 1.0388E+04 & Direct-PRF & 0\\
007281484-01 & RR-Lyr-pri & 1:1 & 650.9 & 67 & 149 & 7.86 & 4.46 & 4.1553E+04 & Direct-PRF & 0\\
007281503-01 & RR-Lyr-pri & 1:1 & 664.8 & 76 & 148 & 7.86 & 7.93 & 7.8898E+03 & Direct-PRF & 0\\
007281615-01 & RR-Lyr-pri & 1:1 & 764.1 & 61 & 182 & 7.86 & 7.98 & 6.2330E+05 & Direct-PRF & 0\\
007281616-01 & RR-Lyr-pri & 1:1 & 791.7 & 41 & 194 & 7.86 & 8.03 & 4.9864E+03 & Direct-PRF & 0\\
007281644-01 & RR-Lyr-pri & 1:1 & 814.2 & 53 & 197 & 7.86 & 8.06 & 1.2466E+05 & Direct-PRF & 0\\
007281664-01 & RR-Lyr-pri & 1:1 & 805.1 & 85 & 183 & 7.86 & 7.98 & 8.7788E+03 & Direct-PRF & 0\\
007281668-01 & RR-Lyr-pri & 1:1 & 811.8 & 87 & 184 & 7.86 & 5.66 & 2.3973E+04 & Direct-PRF & 0\\
007281694-01 & RR-Lyr-pri & 1:1 & 837.9 & 93 & 189 & 7.86 & 6.04 & 2.0777E+04 & Direct-PRF & 0\\
007281699-01 & RR-Lyr-pri & 1:1 & 910.7 & 36 & 226 & 7.86 & 7.91 & 3.9201E+03 & Direct-PRF & 0\\
007281825-01 & RR-Lyr-pri & 2:1 & 1010.2 & 53 & 248 & 7.86 & 6.78 & 1.7808E+04 & Direct-PRF & 0\\
007281838-01 & RR-Lyr-pri & 1:1 & 958.6 & 113 & 212 & 7.86 & 8.10 & 5.2822E+03 & Direct-PRF & 0\\
007281856-01 & RR-Lyr-pri & 1:1 & 1011.4 & 72 & 243 & 7.86 & 5.97 & 2.4932E+04 & Direct-PRF & 0\\
007281864-02 & RR-Lyr-pri & 1:1 & 985.2 & 107 & 223 & 7.86 & 6.55 & 2.0106E+04 & Direct-PRF & 0\\
007281947-01 & RR-Lyr-pri & 1:1 & 1059.7 & 98 & 247 & 7.86 & 7.41 & 3.2805E+04 & Direct-PRF & 0\\
007281951-01 & RR-Lyr-pri & 1:1 & 1059.5 & 101 & 246 & 7.86 & 7.80 & 1.0218E+04 & Direct-PRF & 0\\
007281979-01 & RR-Lyr-pri & 1:1 & 1091.7 & 93 & 258 & 7.86 & 5.24 & 5.6663E+04 & Direct-PRF & 0\\
007281980-01 & RR-Lyr-pri & 1:1 & 1108.7 & 79 & 267 & 7.86 & 7.52 & 1.5582E+05 & Direct-PRF & 0\\
007282008-01 & RR-Lyr-pri & 1:1 & 1107.3 & 99 & 260 & 7.86 & 8.02 & 6.4257E+03 & Direct-PRF & 0\\
007282028-01 & RR-Lyr-pri & 1:1 & 1125.2 & 100 & 264 & 7.86 & 5.84 & 1.5582E+05 & Direct-PRF & 0\\
007282042-01 & RR-Lyr-pri & 1:1 & 1127.9 & 112 & 260 & 7.86 & 5.59 & 3.8956E+04 & Direct-PRF & 0\\
007282154-01 & RR-Lyr-pri & 1:1 & 1246.8 & 100 & 297 & 7.86 & 7.96 & 5.6663E+04 & Direct-PRF & 0\\
007282158-01 & RR-Lyr-pri & 1:1 & 1279.5 & 77 & 312 & 7.86 & 6.69 & 2.9681E+04 & Direct-PRF & 0\\
007282162-01 & RR-Lyr-pri & 1:1 & 1249.2 & 107 & 295 & 7.86 & 3.99 & 8.9042E+04 & Direct-PRF & 0\\
007282168-01 & RR-Lyr-pri & 1:1 & 1261.9 & 101 & 300 & 7.86 & 7.05 & 6.2330E+05 & Direct-PRF & 0\\
007285616-01 & RR-Lyr-pri & 1:1 & 4106.4 & 495 & -2 & 7.86 & 5.12 & 2.3085E+04 & Col-Anomaly & 2\\
007285673-01 & RR-Lyr-pri & 1:1 & 4147.3 & 521 & 0 & 7.86 & 6.64 & 8.6569E+03 & Col-Anomaly & 2\\
007289162-01 & 399.01 & 1:1 & 16.8 & -3 & -3 & 12.95 & 0.70 & 8.6475E+02 & Direct-PRF & 0\\
007289165-01 & 399.01 & 1:1 & 14.7 & 4 & 1 & 12.95 & -0.09 & 3.5328E+02 & Direct-PRF & 0\\
007289165-02 & 007289157-03 & 1:2 & 14.7 & 4 & 1 & 12.95 & -0.09 & 1.3622E+02 & Direct-PRF & 0\\
007293937-01 & 007374746-01 & 1:1 & 14.1 & -2 & -2 & 15.00 & -3.05 & 3.8767E+03 & Direct-PRF & 0\\
007296086-01 & 007296094-01 & 1:1 & 9.4 & -2 & -1 & 18.59 & -3.97 & 1.6102E+03 & Direct-PRF & 0\\
007302940-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007303287-03 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007304121-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007362073-01 & RR-Lyr-pri & 1:1 & 678.8 & -25 & 168 & 7.86 & 5.82 & 1.8332E+04 & Direct-PRF & 0\\
007362301-01 & RR-Lyr-pri & 1:1 & 848.7 & -6 & 213 & 7.86 & 6.85 & 1.8332E+04 & Direct-PRF & 0\\
007362355-01 & RR-Lyr-pri & 1:1 & 868.4 & 10 & 218 & 7.86 & 6.45 & 1.0388E+05 & Direct-PRF & 0\\
007362364-01 & RR-Lyr-pri & 1:1 & 873.8 & 11 & 219 & 7.86 & 6.56 & 2.0777E+05 & Direct-PRF & 0\\
007362391-01 & RR-Lyr-pri & 1:1 & 903.1 & 9 & 226 & 7.86 & 6.53 & 1.6403E+04 & Direct-PRF & 0\\
007362420-01 & RR-Lyr-pri & 1:1 & 966.7 & -3 & 243 & 7.86 & 7.38 & 5.7183E+02 & Direct-PRF & 0\\
007362434-01 & RR-Lyr-pri & 1:1 & 971.0 & 2 & 244 & 7.86 & 7.90 & 7.9910E+03 & Direct-PRF & 0\\
007362450-01 & RR-Lyr-pri & 1:1 & 991.7 & -1 & 249 & 7.86 & 5.04 & 3.1165E+04 & Direct-PRF & 0\\
007362501-01 & RR-Lyr-pri & 1:1 & 1060.1 & -11 & 266 & 7.86 & 7.10 & 1.2466E+04 & Direct-PRF & 0\\
007362534-01 & RR-Lyr-pri & 1:1 & 1121.2 & -20 & 281 & 7.86 & 5.90 & 1.9478E+04 & Direct-PRF & 0\\
007362573-01 & RR-Lyr-pri & 1:1 & 1147.3 & -15 & 288 & 7.86 & 7.33 & 6.0338E+02 & Direct-PRF & 0\\
007362579-01 & RR-Lyr-pri & 1:1 & 1074.0 & 19 & 269 & 7.86 & 7.49 & 6.2330E+05 & Direct-PRF & 0\\
007362579-02 & RR-Lyr-pri & 1:1 & 1074.0 & 19 & 269 & 7.86 & 7.49 & 8.5383E+03 & Direct-PRF & 0\\
007362587-01 & RR-Lyr-pri & 1:1 & 1053.3 & 33 & 262 & 7.86 & 4.18 & 1.0388E+05 & Direct-PRF & 0\\
007362592-01 & RR-Lyr-pri & 1:1 & 1122.7 & 3 & 282 & 7.86 & 5.80 & 2.1493E+04 & Direct-PRF & 0\\
007362631-01 & RR-Lyr-pri & 1:1 & 1190.1 & -7 & 299 & 7.86 & 6.79 & 1.5202E+04 & Direct-PRF & 0\\
007362632-01 & RR-Lyr-pri & 1:1 & 1172.3 & 0 & 294 & 7.86 & 7.58 & 1.2221E+04 & Direct-PRF & 0\\
007362695-01 & RR-Lyr-pri & 1:1 & 1147.1 & 36 & 286 & 7.86 & 6.99 & 3.1165E+05 & Direct-PRF & 0\\
007362696-03 & RR-Lyr-pri & 1:1 & 1155.4 & 33 & 288 & 7.86 & 7.67 & 7.7912E+03 & Direct-PRF & 0\\
007362865-01 & RR-Lyr-pri & 1:1 & 1307.3 & 41 & 326 & 7.86 & 6.74 & 3.2805E+04 & Direct-PRF & 0\\
007365557-01 & 007365569-01 & 1:1 & 65.7 & -16 & -6 & 15.63 & -1.02 & 5.9375E+01 & Direct-PRF & 1\\
007365569-01 & 007365557-01 & 1:1 & 65.7 & 16 & 6 & 14.61 & 1.02 & 1.6842E-02 & Direct-PRF & 1\\
007366036-01 & RR-Lyr-pri & 1:1 & 3852.6 & 346 & -1 & 7.86 & 3.79 & 2.8332E+04 & Col-Anomaly & 2\\
007366065-01 & RR-Lyr-pri & 1:1 & 3866.0 & 360 & 1 & 7.86 & 6.45 & 1.4166E+04 & Col-Anomaly & 2\\
007368137-01 & 007368103-pri & 1:1 & 21.7 & 3 & -5 & 13.42 & 1.48 & 1.7586E+03 & Direct-PRF & 0\\
007376490-01 & 3535.01 & 1:1 & 5.4 & -1 & 0 & 15.18 & -2.03 & 2.2134E+01 & Direct-PRF & 0\\
007376490-02 & 007376500-sec & 1:1 & 5.4 & -1 & 0 & 15.18 & -2.03 & 1.0376E+01 & Direct-PRF & 0\\
007376982-01 & 007212722-01 & 1:1 & 1367.4 & 344 & 1 & 13.97 & -0.36 & 1.1902E+04 & Col-Anomaly & 0\\
007378049-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007385387-01 & 007385478-pri & 1:1 & 66.0 & 16 & 2 & 11.47 & 4.40 & 1.6652E+03 & Direct-PRF & 0\\
007385509-01 & 007385478-pri & 1:1 & 18.4 & -4 & -3 & 11.47 & 2.37 & 1.9927E+02 & Direct-PRF & 0\\
007387593-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007429256-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007431709-01 & 007431703-pri & 1:1 & 65.4 & 8 & 15 & 12.25 & 2.83 & 6.0128E+03 & Direct-PRF & 0\\
007435780-01 & 007518816-pri & 2:1 & 40.3 & -1 & -10 & 12.85 & 2.17 & 5.5667E+03 & Direct-PRF & 0\\
007435780-02 & 007518816-pri & 2:1 & 40.3 & -1 & -10 & 12.85 & 2.17 & 5.9868E+03 & Direct-PRF & 0\\
007447200-03 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007448023-01 & RR-Lyr-pri & 1:1 & 3776.6 & 295 & 1 & 7.86 & 7.82 & 3.8956E+04 & Col-Anomaly & 2\\
007458309-01 & 007458285-pri & 1:1 & 18.4 & 3 & -3 & 13.52 & 0.35 & 6.6094E+03 & Direct-PRF & 0\\
007458433-01 & 007458285-pri & 1:1 & 109.4 & 27 & -1 & 13.52 & 0.64 & 6.4870E+03 & Direct-PRF & 0\\
007461314-01 & 2909.01 & 1:1 & 27.8 & 5 & 6 & 14.62 & 0.27 & 1.8140E+00 & Direct-PRF & 1\\
007464386-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007501194-01 & 007501230-pri & 1:1 & 44.6 & -10 & -6 & 12.45 & -3.14 & 6.7140E+04 & Direct-PRF & 0\\
007501194-02 & 007501230-sec & 2:1 & 44.6 & -10 & -6 & 12.45 & -3.14 & 6.4675E+04 & Direct-PRF & 0\\
007514582-01 & 007431703-pri & 1:1 & 79.0 & -2 & -20 & 12.25 & 3.08 & 5.8875E+03 & Direct-PRF & 0\\
007515964-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007516379-01 & 007516345-pri & 2:1 & 71.2 & 0 & -18 & 12.32 & 2.51 & 6.8732E+03 & Direct-PRF & 0\\
007530196-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007584778-01 & 007584826-pri & 1:1 & 105.1 & 27 & 1 & 15.19 & -0.67 & 4.6807E+03 & Col-Anomaly & 0\\
007598111-01 & 007598128-pri & 1:1 & 16.8 & 0 & 4 & 13.20 & 0.14 & 3.3116E+00 & Direct-PRF & 0\\
007620660-02 & 007620664-pri & 1:1 & 10.5 & -2 & -2 & 13.11 & 2.37 & 8.4182E+02 & Direct-PRF & 0\\
007622059-02 & 007622072-01 & 1:1 & 16.5 & -3 & -2 & 13.58 & -0.31 & 2.5855E+02 & Direct-PRF & 0\\
007622473-01 & 1447.01 & 1:1 & 14.1 & -4 & 1 & 13.09 & -0.78 & 8.0926E+02 & Direct-PRF & 0\\
007625221-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007662697-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007671974-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007672453-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007680114-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007695087-01 & 6041.01 & 1:1 & 8.5 & -1 & 2 & 13.86 & 0.87 & 2.3807E+01 & Direct-PRF & 0\\
007695087-02 & 6041.01 & 1:2 & 8.5 & -1 & 2 & 13.86 & 0.87 & 4.6737E+02 & Direct-PRF & 0\\
007699298-01 & 3706.01 & 1:1 & 617.8 & 155 & -1 & 14.62 & -1.07 & 2.1259E+04 & Col-Anomaly & 0\\
007700561-01 & 007700578-pri & 1:1 & 16.9 & 2 & 3 & 14.15 & 1.39 & 1.4932E+03 & Direct-PRF & 0\\
007700590-01 & 007700578-pri & 1:1 & 9.2 & -1 & -3 & 14.15 & 0.70 & 2.2326E+01 & Direct-PRF & 0\\
007707736-01 & 007707742-pri & 1:1 & 6.5 & -2 & 0 & 16.98 & -1.36 & 6.0889E+02 & Direct-PRF & 0\\
007708215-01 & 3666.01 & 1:1 & 11.1 & 3 & 0 & 15.99 & -0.73 & 1.0039E+02 & Direct-PRF & 0\\
007708215-02 & 007708193-02 & 2:1 & 11.1 & 3 & 0 & 15.99 & -0.73 & 6.2271E+01 & Direct-PRF & 0\\
007739152-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007751571-01 & 007751562-01 & 1:1 & 6.1 & 0 & -1 & 15.25 & 0.32 & 1.5856E+01 & Direct-PRF & 0\\
007751571-02 & 007751562-sec & 1:1 & 6.1 & 0 & -1 & 15.25 & 0.32 & 8.4337E+00 & Direct-PRF & 0\\
007766113-01 & 007766185-pri & 1:1 & 57.7 & -15 & 1 & 12.11 & 1.61 & 2.8821E+04 & Direct-PRF & 0\\
007766113-02 & 007766185-sec & 1:1 & 57.7 & -15 & 1 & 12.11 & 1.61 & 2.1600E+04 & Direct-PRF & 0\\
007766209-01 & 007766185-pri & 1:1 & 28.1 & 6 & 3 & 12.11 & 2.70 & 8.7717E+03 & Direct-PRF & 0\\
007770450-01 & 3706.01 & 1:1 & 17.7 & 3 & 3 & 14.62 & 1.22 & 1.9385E+03 & Direct-PRF & 0\\
007777365-01 & 007777443-pri & 1:1 & 74.7 & -17 & -6 & 11.91 & 3.96 & 2.3656E+03 & Direct-PRF & 0\\
007777372-01 & 007777443-pri & 1:1 & 53.7 & -7 & 12 & 11.91 & 2.24 & 4.9436E+03 & Direct-PRF & 0\\
007777397-01 & 007777416-02 & 2:1 & 9.7 & -3 & 0 & 15.30 & -3.71 & 7.5294E+00 & Direct-PRF & 0\\
007777397-02 & 007777416-02 & 2:1 & 9.7 & -3 & 0 & 15.30 & -3.71 & 8.6292E+00 & Direct-PRF & 0\\
007777471-01 & 007777443-pri & 1:1 & 64.8 & -3 & -16 & 11.91 & 2.63 & 4.4322E+03 & Direct-PRF & 0\\
007777522-01 & 007777443-pri & 1:1 & 56.9 & 15 & -1 & 11.91 & 3.85 & 2.8992E+03 & Direct-PRF & 0\\
007800750-01 & 007938870-pri & 1:1 & 682.7 & 172 & -1 & 12.29 & 1.11 & 1.4392E+04 & Col-Anomaly & 0\\
007808747-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007812167-01 & 3665.01 & 1:1 & 9.4 & 0 & -2 & 16.33 & -0.95 & 1.6571E+02 & Direct-PRF & 0\\
007812167-02 & 007812175-sec & 1:1 & 9.4 & 0 & -2 & 16.33 & -0.95 & 3.0128E+01 & Direct-PRF & 0\\
007812179-01 & 3665.01 & 1:1 & 5.1 & 1 & 1 & 16.33 & -1.90 & 7.0257E+01 & Direct-PRF & 0\\
007812179-02 & 007812175-sec & 1:1 & 5.1 & 1 & 1 & 16.33 & -1.90 & 2.9102E+01 & Direct-PRF & 0\\
007813370-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007816137-01 & 007816201-sec & 1:1 & 75.0 & -9 & 17 & 12.02 & 3.00 & 3.4667E+03 & Direct-PRF & 0\\
007816137-02 & 007816201-pri & 1:1 & 75.0 & -9 & 17 & 12.02 & 3.00 & 2.4778E+03 & Direct-PRF & 0\\
007816665-01 & 007816680-01 & 1:1 & 13.2 & -3 & 2 & 15.57 & 0.31 & 5.1492E+02 & Direct-PRF & 0\\
007838214-01 & 007838213-01 & 1:1 & 4.4 & -1 & 1 & 14.40 & -0.59 & 1.4528E+00 & Direct-PRF & 0\\
007838655-01 & 007838639-pri & 1:2 & 10.0 & -1 & -3 & 13.77 & 1.69 & 1.2239E+01 & Direct-PRF & 0\\
007840044-01 & 3758.01 & 1:1 & 6.8 & 0 & -2 & 16.90 & -2.37 & 1.3094E+02 & Direct-PRF & 0\\
007840145-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007870250-01 & 007938870-pri & 1:1 & 91.5 & 23 & 2 & 12.29 & 2.27 & 8.7756E+03 & Direct-PRF & 0\\
007870306-01 & 007938870-pri & 1:1 & 61.5 & 8 & 13 & 12.29 & 2.82 & 9.7243E+03 & Direct-PRF & 0\\
007877818-01 & 3530.01 & 1:1 & 8.2 & -1 & -2 & 15.65 & -1.83 & 3.3495E+02 & Direct-PRF & 0\\
007877818-02 & 007877824-02 & 1:1 & 8.2 & -1 & -2 & 15.65 & -1.83 & 2.9905E+02 & Direct-PRF & 0\\
007877820-01 & 3530.01 & 1:1 & 4.7 & -1 & 0 & 15.65 & -2.55 & 4.0038E+01 & Direct-PRF & 0\\
007877820-02 & 007877824-02 & 1:1 & 4.7 & -1 & 0 & 15.65 & -2.55 & 3.8615E+01 & Direct-PRF & 0\\
007881228-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007884866-01 & 007884842-pri & 1:1 & 20.6 & 3 & -4 & 9.60 & 5.64 & 1.6471E+02 & Direct-PRF & 0\\
007885518-01 & 007885570-pri & 1:1 & 44.4 & -8 & 9 & 11.68 & 1.39 & 6.6040E+03 & Direct-PRF & 0\\
007885518-02 & 007885570-sec & 1:1 & 44.4 & -8 & 9 & 11.68 & 1.39 & 4.6471E+03 & Direct-PRF & 0\\
007885558-01 & 007885570-pri & 1:1 & 31.4 & 2 & 8 & 11.68 & 3.22 & 1.3103E+03 & Direct-PRF & 0\\
007889486-01 & 007821010-01 & 1:1 & 106.6 & -14 & 23 & 10.82 & 4.94 & 8.2619E+02 & Direct-PRF & 0\\
007889486-02 & 007821010-02 & 1:1 & 106.6 & -14 & 23 & 10.82 & 4.94 & 1.1667E+03 & Direct-PRF & 0\\
007900450-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007906865-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007908633-01 & 008111622-03 & 1:5 & 2398.0 & -361 & 4 & 15.49 & -4.27 & 1.3503E+03 & Col-Anomaly & 2\\
007918172-02 & 007918217-01 & 9:1 & 25.6 & -7 & 1 & 10.88 & 3.46 & 2.4903E-01 & Direct-PRF & 1\\
007918217-01 & 007918172-02 & 1:9 & 25.6 & 7 & -1 & 14.34 & -3.46 & 4.0155E+00 & Direct-PRF & 1\\
007938180-01 & 007938179-02 & 1:1 & 5.3 & 0 & 1 & 11.45 & 2.17 & 2.3529E+00 & Direct-PRF & 0\\
007938499-01 & V481-Lyr-pri & 1:1 & 71.3 & -1 & 18 & 13.27 & 1.67 & 4.5382E+03 & Direct-PRF & 0\\
007948779-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007970283-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007974626-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
007985134-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008009496-01 & 008009500-01 & 9:1 & 15.3 & 2 & 3 & 14.58 & -1.18 & 2.3656E+02 & Direct-PRF & 0\\
008017379-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008023848-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008029197-01 & 008098300-pri & 1:2 & 293.3 & 74 & -1 & 12.82 & -0.17 & 1.0053E+04 & Col-Anomaly & 0\\
008035802-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008038388-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008043721-01 & 008043961-pri & 1:2 & 209.6 & 53 & 2 & 10.74 & 4.97 & 3.7328E+03 & Direct-PRF & 0\\
008043882-01 & 008043961-pri & 1:2 & 80.2 & 4 & -19 & 10.74 & 4.47 & 2.8111E+03 & Direct-PRF & 0\\
008043968-01 & 008043961-pri & 1:2 & 83.8 & -11 & -17 & 10.74 & 4.56 & 2.9192E+03 & Direct-PRF & 0\\
008044008-01 & 008043961-pri & 1:2 & 79.0 & -16 & -10 & 10.74 & 4.21 & 3.7950E+04 & Direct-PRF & 0\\
008044016-01 & 008043961-pri & 1:2 & 44.0 & -10 & 3 & 10.74 & 3.01 & 7.8517E+03 & Direct-PRF & 0\\
008058135-01 & 008058127-01 & 1:1 & 5.8 & 1 & -1 & 13.47 & 0.45 & 5.3077E+00 & Direct-PRF & 0\\
008059291-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008075991-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008086600-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008087887-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008094120-02 & 008094140-pri & 1:1 & 30.1 & 0 & 8 & 15.16 & -2.27 & 9.5681E+02 & Direct-PRF & 0\\
008095110-01 & 6171.01 & 1:1 & 5.4 & 2 & 0 & 14.17 & -1.00 & 1.2061E+01 & Direct-PRF & 0\\
008104436-01 & 006706287-pri & 1:1 & 7756.9 & -2 & 1 & 13.62 & 1.94 & 2.1029E+03 & Cross-Talk & 0\\
008108997-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008111716-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008123628-02 & 009304367-02 & 3:1 & 6571.1 & -177 & 8 & 13.25 & 0.38 & 3.7586E+00 & Col-Anomaly & 2\\
008127586-01 & 008127607-pri & 1:1 & 19.7 & 3 & 3 & 14.66 & 0.27 & 1.9886E+00 & Direct-PRF & 1\\
008127639-01 & 3713.01 & 1:1 & 10.0 & 3 & 0 & 17.51 & -2.12 & 4.0658E+02 & Direct-PRF & 0\\
008128247-01 & 008128965-pri & 1:2 & 486.9 & 122 & 0 & 13.23 & 0.10 & 3.1132E+03 & Col-Anomaly & 0\\
008129005-01 & 008128965-pri & 1:2 & 27.9 & -7 & -3 & 13.23 & 1.51 & 3.0681E+03 & Direct-PRF & 0\\
008149350-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008149484-01 & 008081389-pri & 1:1 & 229.3 & 58 & 0 & 13.99 & -0.90 & 1.0587E+04 & Col-Anomaly & 0\\
008161715-02 & 008161816-01 & 1:1 & 131.9 & -33 & -3 & 15.54 & -2.01 & 4.7647E+00 & Direct-PRF & 1\\
008161816-01 & 008161830-01 & 1:1 & 24.2 & 0 & 6 & 13.31 & 2.23 & 3.0864E-01 & Direct-PRF & 1\\
008161816-02 & 008161830-02 & 1:1 & 24.2 & 0 & 6 & 13.31 & 2.23 & 3.4444E-01 & Direct-PRF & 1\\
008161825-01 & 008161830-02 & 1:4 & 43.5 & 5 & 10 & 13.31 & -1.79 & 4.4286E+00 & Direct-PRF & 1\\
008161830-01 & 008161816-01 & 1:1 & 24.2 & 0 & -6 & 15.54 & -2.23 & 3.2400E+00 & Direct-PRF & 1\\
008161830-02 & 008161816-02 & 1:1 & 24.2 & 0 & -6 & 15.54 & -2.23 & 2.9032E+00 & Direct-PRF & 1\\
008162376-01 & 008094140-pri & 1:1 & 102.9 & 26 & 0 & 15.16 & -1.16 & 7.5959E+03 & Col-Anomaly & 0\\
008162790-01 & 521.01 & 1:1 & 3.4 & 0 & -1 & 14.63 & 0.41 & 1.7020E+00 & Direct-PRF & 0\\
008166912-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008178616-01 & 008380743-pri & 1:2 & 2477.1 & 622 & 0 & 14.04 & -0.09 & 1.3765E+04 & Col-Anomaly & 0\\
008217331-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008240123-01 & 008240109-pri & 1:1 & 11.7 & 2 & 2 & 13.49 & 2.33 & 1.2577E+02 & Direct-PRF & 0\\
008243283-01 & 008243263-pri & 1:2 & 16.1 & 3 & 2 & 12.98 & 2.24 & 1.7879E+02 & Direct-PRF & 0\\
008244190-01 & 3545.01 & 1:1 & 13.7 & 3 & 3 & 15.90 & -1.40 & 4.7792E+03 & Direct-PRF & 0\\
008244295-01 & 3545.01 & 1:1 & 111.4 & 28 & 0 & 15.90 & 0.03 & 6.1067E+03 & Col-Anomaly & 0\\
008256049-01 & 3652.01 & 1:1 & 7.9 & 2 & -1 & 15.88 & -0.22 & 2.2558E+01 & Direct-PRF & 0\\
008256643-01 & 008456151-01 & 1:1 & 2163.7 & -544 & -3 & 11.44 & 2.25 & 1.6238E+00 & Col-Anomaly & 0\\
008258171-01 & 008258160-01 & 1:1 & 9.3 & 2 & -2 & 16.38 & -4.73 & 9.3553E+01 & Direct-PRF & 0\\
008258171-02 & 008258160-02 & 1:1 & 9.3 & 2 & -2 & 16.38 & -4.73 & 9.3620E+01 & Direct-PRF & 0\\
008260234-01 & 1066.01 & 1:1 & 9.6 & 3 & 0 & 15.62 & -1.46 & 4.9236E+01 & Direct-PRF & 0\\
008262210-01 & 008262223-pri & 1:1 & 26.7 & -1 & 6 & 12.15 & 1.80 & 1.4422E+03 & Direct-PRF & 0\\
008263752-01 & 3581.01 & 1:1 & 7.4 & 0 & -1 & 16.75 & -3.32 & 1.0079E+02 & Direct-PRF & 0\\
008263752-02 & 008263746-02 & 2:1 & 7.4 & 0 & -1 & 16.75 & -3.32 & 9.1053E+01 & Direct-PRF & 0\\
008264070-01 & 3655.01 & 1:1 & 14.0 & 3 & 2 & 17.69 & -2.65 & 3.5340E+02 & Direct-PRF & 0\\
008264543-01 & 008264588-01 & 1:1 & 139.1 & -7 & 35 & 10.74 & 0.68 & 3.2143E+00 & Direct-PRF & 1\\
008264588-01 & 008264543-01 & 1:1 & 139.1 & 7 & -35 & 11.42 & -0.68 & 3.1111E-01 & Direct-PRF & 1\\
008265921-01 & 008265951-pri & 1:1 & 53.1 & 10 & -9 & 12.73 & 1.19 & 1.0944E+04 & Direct-PRF & 0\\
008265921-02 & 008265951-sec & 1:1 & 53.1 & 10 & -9 & 12.73 & 1.19 & 1.0533E+04 & Direct-PRF & 0\\
008265953-01 & 008265951-pri & 1:1 & 34.6 & -4 & 8 & 12.73 & 2.57 & 3.3580E+03 & Direct-PRF & 0\\
008265953-02 & 008265951-sec & 1:1 & 34.6 & -4 & 8 & 12.73 & 2.57 & 4.7698E+03 & Direct-PRF & 0\\
008265990-01 & 008265951-pri & 1:1 & 63.5 & -3 & -16 & 12.73 & 0.68 & 1.4071E+04 & Direct-PRF & 0\\
008265993-01 & 008265951-pri & 1:1 & 38.7 & -8 & -5 & 12.73 & 0.30 & 1.4775E+04 & Direct-PRF & 0\\
008265993-02 & 008265951-sec & 1:1 & 38.7 & -8 & -5 & 12.73 & 0.30 & 1.6853E+04 & Direct-PRF & 0\\
008266004-01 & 008265951-pri & 1:1 & 58.3 & -15 & 2 & 12.73 & 2.73 & 3.4360E+03 & Direct-PRF & 0\\
008285787-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008299955-01 & 3631.01 & 1:1 & 11.2 & -2 & -2 & 17.74 & -4.27 & 4.2627E+03 & Direct-PRF & 0\\
008302450-01 & 008302455-01 & 1:1 & 73.9 & 11 & -15 & 11.54 & 3.75 & 4.1056E+02 & Direct-PRF & 0\\
008302473-01 & 008302455-01 & 1:1 & 56.4 & -10 & 9 & 11.54 & 4.08 & 7.5055E+02 & Direct-PRF & 0\\
008323753-01 & 3767.01 & 1:1 & 7.7 & -2 & 0 & 17.38 & -3.89 & 9.4100E+01 & Direct-PRF & 0\\
008330548-01 & 008330575-01 & 1:1 & 12.3 & 2 & 3 & 13.48 & 0.96 & 6.4971E+00 & Direct-PRF & 0\\
008358012-01 & 008358008-01 & 1:1 & 10.9 & 3 & 0 & 14.67 & 0.22 & 2.8341E+01 & Direct-PRF & 0\\
008364115-01 & 008364119-01 & 1:1 & 19.3 & -2 & 4 & 12.41 & 0.83 & 4.5978E+02 & Direct-PRF & 0\\
008364115-02 & 008364119-02 & 1:1 & 19.3 & -2 & 4 & 12.41 & 0.83 & 4.6772E+02 & Direct-PRF & 0\\
008374494-01 & 008374499-01 & 1:1 & 8.3 & -1 & -2 & 14.91 & 0.84 & 1.4312E+01 & Direct-PRF & 0\\
008374494-02 & 008374499-02 & 2:1 & 8.3 & -1 & -2 & 14.91 & 0.84 & 3.3476E+01 & Direct-PRF & 0\\
008378634-01 & 008378656-pri & 1:1 & 14.2 & 3 & -1 & 12.79 & 0.27 & 5.0641E+02 & Direct-PRF & 0\\
008378634-02 & 008378656-pri & 1:2 & 14.2 & 3 & -1 & 12.79 & 0.27 & 3.2341E+03 & Direct-PRF & 0\\
008379705-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008379965-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008382075-01 & 008382182-pri & 1:1 & 82.7 & 14 & -16 & 8.18 & 6.78 & 2.7736E+02 & Direct-PRF & 0\\
008382114-01 & 008382182-pri & 2:1 & 57.8 & 7 & -13 & 8.18 & 7.10 & 2.4915E+02 & Direct-PRF & 0\\
008382223-01 & 008382182-pri & 1:1 & 82.9 & 5 & 20 & 8.18 & 7.81 & 1.3009E+02 & Direct-PRF & 0\\
008414216-01 & 008414159-01 & 1:1 & 111.1 & 28 & 0 & 14.38 & -0.38 & 2.6882E+03 & Col-Anomaly & 0\\
008414907-01 & 5513.01 & 4:1 & 5.2 & -1 & -1 & 17.91 & -2.13 & 2.6654E+01 & Direct-PRF & 0\\
008414907-03 & 008414914-02 & 4:1 & 5.2 & -1 & -1 & 17.91 & -2.13 & 2.2875E+01 & Direct-PRF & 0\\
008414907-04 & 5513.01 & 2:1 & 5.2 & -1 & -1 & 17.91 & -2.13 & 8.8578E+01 & Direct-PRF & 0\\
008414907-05 & 008414914-02 & 2:1 & 5.2 & -1 & -1 & 17.91 & -2.13 & 7.1988E+01 & Direct-PRF & 0\\
008416925-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008429415-01 & 008429450-pri & 1:2 & 28.6 & 7 & -1 & 13.11 & -0.40 & 1.3048E+04 & Direct-PRF & 0\\
008453211-01 & 008453191-01 & 1:1 & 14.4 & 3 & 0 & 13.36 & 1.22 & 1.2514E+02 & Direct-PRF & 0\\
008453214-01 & 008453191-01 & 1:1 & 15.8 & 3 & -2 & 13.36 & 2.11 & 9.5019E+01 & Direct-PRF & 0\\
008474898-01 & 5520.01 & 1:1 & 7.5 & -1 & 2 & 14.37 & 0.17 & 7.9970E+00 & Direct-PRF & 0\\
008487748-01 & V2277-Cyg-pri & 1:1 & 102.6 & -3 & 25 & 10.29 & 5.16 & 1.1664E+03 & Direct-PRF & 0\\
008487805-01 & V2277-Cyg-pri & 1:2 & 154.7 & 16 & 35 & 10.29 & 4.76 & 7.0760E+04 & Direct-PRF & 0\\
008487838-01 & V2277-Cyg-pri & 1:2 & 223.6 & 17 & 54 & 10.29 & 3.88 & 2.1228E+04 & Direct-PRF & 0\\
008488876-01 & 1248.01 & 1:1 & 5.5 & -1 & 1 & 15.36 & -2.99 & 1.2921E+00 & Direct-PRF & 0\\
008492101-01 & 008621026-pri & 1:1 & 951.1 & 0 & 239 & 13.37 & 0.14 & 2.2964E+03 & Col-Anomaly & 0\\
008509361-01 & 008509346-01 & 1:1 & 12.2 & -3 & -1 & 13.74 & 0.21 & 2.4462E+02 & Direct-PRF & 0\\
008509694-02 & 008509703-01 & 1:1 & 7.5 & 0 & -2 & 15.74 & -3.29 & 2.1207E+00 & Direct-PRF & 0\\
008524110-01 & 6060.01 & 1:2 & 1544.2 & 389 & -4 & 14.59 & -1.19 & 1.0205E+03 & Col-Anomaly & 0\\
008524346-01 & 3518.01 & 1:2 & 487.5 & 123 & 0 & 14.00 & -0.28 & 1.9235E+03 & Col-Anomaly & 0\\
008543102-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008543279-01 & 008543278-01 & 1:1 & 5.7 & 1 & 1 & 14.61 & 1.38 & 4.4340E+00 & Direct-PRF & 0\\
008543279-02 & 008543278-01 & 1:2 & 5.7 & 1 & 1 & 14.61 & 1.38 & 1.3113E+01 & Direct-PRF & 0\\
008552498-01 & V2277-Cyg-pri & 1:1 & 59.3 & -13 & -8 & 10.29 & 3.29 & 5.8967E+03 & Direct-PRF & 0\\
008552500-01 & V2277-Cyg-pri & 1:2 & 125.9 & 4 & -32 & 10.29 & 4.72 & 9.0332E+03 & Direct-PRF & 0\\
008552565-01 & V2277-Cyg-pri & 1:1 & 65.4 & 15 & -8 & 10.29 & 2.66 & 6.4327E+03 & Direct-PRF & 0\\
008552583-01 & V2277-Cyg-pri & 1:1 & 102.6 & 23 & -13 & 10.29 & 4.77 & 2.8117E+03 & Direct-PRF & 0\\
008552587-01 & V2277-Cyg-pri & 1:1 & 58.7 & 6 & 13 & 10.29 & 3.83 & 4.2885E+03 & Direct-PRF & 0\\
008552607-01 & V2277-Cyg-pri & 1:1 & 103.0 & 26 & -3 & 10.29 & 3.99 & 3.9311E+03 & Direct-PRF & 0\\
008555360-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008559962-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008560804-01 & 008560861-01 & 1:1 & 73.8 & 18 & -5 & 8.50 & 4.07 & 6.9336E+02 & Direct-PRF & 0\\
008560804-02 & 008560861-02 & 2:1 & 73.8 & 18 & -5 & 8.50 & 4.07 & 4.9828E+02 & Direct-PRF & 0\\
008560840-01 & 008560861-01 & 1:1 & 61.0 & 10 & -11 & 8.50 & 7.03 & 5.5941E+01 & Direct-PRF & 0\\
008560840-02 & 008560861-02 & 2:1 & 61.0 & 10 & -11 & 8.50 & 7.03 & 6.4870E+01 & Direct-PRF & 0\\
008560940-01 & 008560861-01 & 1:1 & 94.7 & -14 & -20 & 8.50 & 6.04 & 4.4720E+02 & Direct-PRF & 0\\
008589731-01 & 3518.01 & 1:2 & 19.9 & 4 & 4 & 14.00 & -0.76 & 1.0423E+02 & Direct-PRF & 0\\
008618728-01 & 008554005-pri & 1:1 & 68.2 & 16 & -6 & 12.71 & 2.34 & 3.0046E+02 & Direct-PRF & 0\\
008619448-01 & 008619436-01 & 1:1 & 15.5 & 4 & 1 & 11.81 & 0.61 & 1.2667E+00 & Direct-PRF & 0\\
008620565-01 & 008620561-01 & 1:1 & 5.2 & 0 & -1 & 16.78 & -1.87 & 2.5463E+02 & Direct-PRF & 0\\
008621348-01 & 3682.01 & 1:1 & 7.3 & 1 & -2 & 17.95 & -3.54 & 5.5096E+02 & Direct-PRF & 0\\
008621348-02 & 008621353-02 & 1:1 & 7.3 & 1 & -2 & 17.95 & -3.54 & 3.9330E+02 & Direct-PRF & 0\\
008625732-01 & 008560861-01 & 1:1 & 115.2 & -20 & 21 & 8.50 & 6.32 & 6.7479E+02 & Direct-PRF & 0\\
008625813-01 & 1859.01 & 1:1 & 10.8 & 3 & -1 & 15.02 & 0.96 & 1.4775E+00 & Direct-PRF & 0\\
008635938-01 & 008700506-01 & 1:1 & 313.4 & 79 & 0 & 13.48 & -0.52 & 2.0945E+03 & Col-Anomaly & 0\\
008638036-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008682015-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008700529-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008700537-01 & 008700506-02 & 1:1 & 21.8 & -5 & 4 & 13.48 & 0.89 & 2.5117E+03 & Direct-PRF & 0\\
008700537-02 & 008700506-01 & 1:1 & 21.8 & -5 & 4 & 13.48 & 0.89 & 3.0091E+03 & Direct-PRF & 0\\
008701276-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008703884-01 & 008703887-pri & 1:1 & 12.4 & -1 & -3 & 11.05 & 4.32 & 5.3993E+00 & Direct-PRF & 0\\
008703887-03 & 1262.01 & 1:1 & 12.4 & 1 & 3 & 15.38 & -4.32 & 2.0887E+01 & Direct-PRF & 0\\
008746295-01 & 008746310-01 & 1:1 & 12.4 & -3 & -2 & 14.77 & -0.03 & 3.4904E+02 & Direct-PRF & 0\\
008747904-01 & V2277-Cyg-pri & 1:2 & 2256.5 & 568 & 2 & 10.29 & 5.57 & 5.4431E+03 & Col-Anomaly & 0\\
008752817-01 & 008817929-01 & 2:1 & 349.5 & -2 & 88 & 14.12 & -0.45 & 1.0476E+00 & Direct-PRF & 1\\
008758136-01 & 008758161-01 & 1:1 & 34.5 & 0 & 8 & 12.46 & 3.09 & 1.6164E+03 & Direct-PRF & 0\\
008766285-01 & 1260.01 & 1:1 & 102.7 & -26 & -4 & 13.85 & -3.60 & 5.7949E+00 & Direct-PRF & 1\\
008780959-01 & 008780968-01 & 1:1 & 8.1 & 2 & 1 & 16.30 & -3.00 & 8.8425E+01 & Direct-PRF & 0\\
008817759-01 & 008817929-01 & 3:1 & 219.8 & 55 & 4 & 14.12 & 0.50 & 0.6111E-01 & Direct-PRF & 1\\
008817929-01 & 008817759-01 & 1:3 & 219.8 & -55 & -4 & 14.62 & -0.50 & 1.6364E+00 & Direct-PRF & 1\\
008818050-01 & 008752817-02 & 1:4 & 160.4 & 1 & -40 & 13.67 & -0.83 & 8.0000E+00 & Direct-PRF & 1\\
008818095-01 & 008817929-01 & 1:2 & 254.3 & -4 & 64 & 14.12 & -0.71 & 1.5714E+00 & Direct-PRF & 1\\
008823426-01 & 008823397-pri & 1:1 & 20.5 & 3 & -4 & 13.25 & 2.34 & 1.3587E+03 & Direct-PRF & 0\\
008823833-01 & 008823397-pri & 1:1 & 487.8 & 123 & 0 & 13.25 & -0.35 & 1.0072E+04 & Col-Anomaly & 0\\
008823893-01 & 008823397-pri & 1:1 & 552.0 & 139 & 2 & 13.25 & 0.66 & 1.3237E+04 & Col-Anomaly & 0\\
008848115-01 & 008454553-04 & 1:1 & 5253.6 & -414 & -4 & 11.51 & 1.21 & 1.2593E+00 & Col-Anomaly & 2\\
008868649-01 & 008868650-pri & 1:1 & 25.8 & 3 & -6 & 11.94 & 2.08 & 2.9141E+03 & Direct-PRF & 0\\
008868657-01 & 008868650-pri & 1:1 & 74.2 & 13 & -14 & 11.94 & 4.05 & 2.0138E+03 & Direct-PRF & 0\\
008868686-01 & 008868650-pri & 1:1 & 60.0 & 15 & 0 & 11.94 & 1.57 & 1.1795E+04 & Direct-PRF & 0\\
008885841-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008890996-01 & 008823397-pri & 1:1 & 627.1 & 158 & 0 & 13.25 & -0.76 & 2.5739E+04 & Col-Anomaly & 0\\
008892721-01 & 3336.01 & 1:1 & 7.4 & -1 & -2 & 15.52 & 0.42 & 1.7794E+01 & Direct-PRF & 0\\
008894646-02 & 008894630-pri & 1:2 & 30.9 & 1 & -8 & 11.54 & 2.30 & 2.3412E+03 & Direct-PRF & 0\\
008906045-01 & 008906039-pri & 1:1 & 3.9 & 1 & -1 & 12.62 & 1.55 & 1.1062E+02 & Direct-PRF & 0\\
008906045-02 & 008906039-pri & 1:1 & 3.9 & 1 & -1 & 12.62 & 1.55 & 2.0065E+01 & Direct-PRF & 0\\
008937021-01 & 008937019-01 & 1:1 & 4.2 & 0 & 1 & 17.93 & -2.49 & 3.5711E+02 & Direct-PRF & 0\\
008937021-02 & 008937019-02 & 1:1 & 4.2 & 0 & 1 & 17.93 & -2.49 & 2.0297E+02 & Direct-PRF & 0\\
008953281-01 & 008953296-pri & 1:1 & 21.9 & 5 & -1 & 13.90 & 1.26 & 1.0442E+03 & Direct-PRF & 0\\
008953414-01 & 008953426-pri & 1:2 & 82.8 & 13 & 16 & 12.16 & 3.23 & 9.8537E+02 & Direct-PRF & 0\\
008953475-01 & 008953426-pri & 1:2 & 118.5 & 0 & 30 & 12.16 & 1.41 & 4.4889E+03 & Direct-PRF & 0\\
008955889-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
008963721-01 & 5614.01 & 1:1 & 1527.8 & 384 & 0 & 13.95 & 0.73 & 8.2887E+03 & Col-Anomaly & 0\\
009005042-01 & 009005043-pri & 2:1 & 13.3 & -2 & 2 & 15.78 & -0.23 & 1.8710E+04 & Direct-PRF & 0\\
009007953-01 & 009007918-pri & 1:1 & 55.1 & 0 & -14 & 11.66 & 3.06 & 3.2000E+03 & Direct-PRF & 0\\
009009211-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009025922-01 & 3596.01 & 1:1 & 8.4 & 2 & 1 & 16.76 & -3.47 & 1.1903E+02 & Direct-PRF & 0\\
009025922-02 & 009025914-02 & 1:1 & 8.4 & 2 & 1 & 16.76 & -3.47 & 5.9789E+01 & Direct-PRF & 0\\
009047284-01 & 008977390-pri & 1:1 & 610.2 & 154 & 0 & 13.11 & -0.25 & 1.0129E+04 & Col-Anomaly & 0\\
009048161-01 & 6063.01 & 1:1 & 9.0 & 0 & 2 & 13.09 & -0.06 & 1.7053E+01 & Direct-PRF & 0\\
009048161-02 & 009048145-sec & 1:1 & 9.0 & 0 & 2 & 13.09 & -0.06 & 2.0290E+01 & Direct-PRF & 0\\
009049697-01 & 3799.01 & 1:1 & 19.4 & -4 & 1 & 15.82 & -0.66 & 5.4359E+01 & Direct-PRF & 0\\
009053086-01 & 702.01 & 1:1 & 14.3 & 3 & -2 & 13.76 & 0.28 & 1.0514E+00 & Direct-PRF & 0\\
009053112-01 & 3751.01 & 1:1 & 14.3 & -3 & 2 & 14.03 & -0.28 & 4.5346E+02 & Direct-PRF & 0\\
009071343-01 & 009071373-pri & 2:1 & 27.5 & -5 & -5 & 13.07 & 1.54 & 3.3600E+03 & Direct-PRF & 0\\
009071343-02 & 009071373-pri & 2:1 & 27.5 & -5 & -5 & 13.07 & 1.54 & 4.3077E+03 & Direct-PRF & 0\\
009074955-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009083470-01 & 009083523-pri & 1:1 & 80.2 & -18 & 7 & 12.71 & 3.19 & 2.8119E+03 & Direct-PRF & 0\\
009083564-01 & 009083523-pri & 1:1 & 54.5 & 10 & 9 & 12.71 & -0.28 & 1.8746E+04 & Direct-PRF & 0\\
009099950-01 & 009164694-pri & 1:1 & 163.6 & 41 & 0 & 14.18 & -1.33 & 9.7050E+03 & Col-Anomaly & 0\\
009101208-01 & 5614.01 & 1:1 & 69.8 & 17 & 2 & 13.95 & 1.43 & 1.8490E+04 & Direct-PRF & 0\\
009108085-01 & 5615.01 & 1:1 & 28.0 & 0 & 7 & 14.28 & -0.63 & 8.1511E+03 & Direct-PRF & 0\\
009110357-01 & 3607.01 & 1:1 & 9.9 & 2 & -2 & 16.40 & -2.82 & 2.3755E+03 & Direct-PRF & 0\\
009137728-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009142974-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009159242-01 & 009159301-pri & 1:1 & 48.2 & -10 & 7 & 12.15 & 1.88 & 7.5462E+03 & Direct-PRF & 0\\
009159265-01 & 009159301-pri & 1:1 & 34.5 & -9 & -1 & 12.15 & 2.36 & 2.5284E+03 & Direct-PRF & 0\\
009159275-01 & 009159301-pri & 1:1 & 21.2 & -5 & 3 & 12.15 & 3.47 & 1.6972E+03 & Direct-PRF & 0\\
009162224-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009166870-01 & 931.01 & 1:1 & 7.5 & -2 & 1 & 15.27 & -0.22 & 1.8726E+01 & Direct-PRF & 0\\
009210823-01 & 009210828-pri & 1:2 & 15.2 & -2 & -3 & 13.22 & -1.48 & 1.0481E+03 & Direct-PRF & 0\\
009214712-02 & 6065.01 & 1:1 & 4.1 & 1 & 0 & 15.28 & 0.24 & 5.6633E+00 & Direct-PRF & 0\\
009214715-02 & 6064.01 & 1:1 & 4.1 & -1 & 0 & 15.52 & -0.24 & 4.8120E+00 & Direct-PRF & 0\\
009214715-03 & 6064.01 & 1:1 & 4.1 & -1 & 0 & 15.52 & -0.24 & 7.6256E+01 & Direct-PRF & 0\\
009220612-01 & 009220600-pri & 1:1 & 21.2 & 4 & 4 & 12.26 & 3.01 & 5.5378E+02 & Direct-PRF & 0\\
009282762-01 & BR-Cyg-pri & 1:1 & 7602.3 & -2 & 7 & 10.03 & 5.68 & 5.7168E+03 & Cross-Talk & 0\\
009282769-01 & BR-Cyg-pri & 1:1 & 7582.2 & 3 & 2 & 10.03 & 3.38 & 1.7150E+04 & Cross-Talk & 0\\
009286728-01 & 009159301-pri & 1:1 & 1349.3 & 339 & -1 & 12.15 & 2.42 & 1.2262E+04 & Col-Anomaly & 0\\
009291039-02 & 009291368-pri & 1:1 & 304.5 & 77 & 1 & 14.01 & -1.77 & 2.6660E+04 & Col-Anomaly & 0\\
009291378-01 & 009291368-pri & 1:1 & 12.6 & -3 & 0 & 14.01 & 1.53 & 1.3609E+02 & Direct-PRF & 0\\
009304561-01 & 3597.01 & 1:1 & 810.8 & 204 & 0 & 14.37 & -0.45 & 2.6534E+03 & Col-Anomaly & 0\\
009304907-01 & 009304976-03 & 1:2 & 113.8 & 2 & -29 & 13.82 & 2.09 & 1.3446E+00 & Direct-PRF & 1\\
009304955-01 & 009305157-01 & 2:1 & 207.2 & 49 & -17 & 15.70 & -3.69 & 7.0909E+00 & Direct-PRF & 1\\
009304976-03 & 009304907-01 & 2:1 & 113.8 & -2 & 29 & 15.91 & -2.09 & 7.4372E-01 & Direct-PRF & 1\\
009305136-02 & 009304976-01 & 1:2 & 184.6 & -47 & 1 & 13.82 & 1.17 & 2.8356E+00 & Direct-PRF & 1\\
009305157-01 & 009304907-01 & 2:1 & 113.8 & -2 & 29 & 15.91 & -2.09 & 7.1498E-01 & Direct-PRF & 1\\
009328864-01 & 009328852-pri & 1:1 & 16.6 & -4 & 1 & 15.33 & -1.22 & 6.7000E+03 & Direct-PRF & 0\\
009335664-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009340980-01 & V2281-Cyg-pri & 1:2 & 123.9 & 18 & 26 & 11.82 & 3.46 & 9.2261E+04 & Direct-PRF & 0\\
009345771-01 & 009345819-01 & 1:1 & 86.9 & 0 & -22 & 15.80 & -0.10 & 1.0357E+00 & Direct-PRF & 1\\
009345819-01 & 009345771-01 & 1:1 & 86.9 & 0 & 22 & 15.70 & 0.10 & 0.9655E+00 & Direct-PRF & 1\\
009357375-01 & 009357275-pri & 1:1 & 81.5 & 15 & -15 & 12.19 & 3.27 & 2.0864E+03 & Direct-PRF & 0\\
009366989-01 & 3597.01 & 1:1 & 7.9 & 1 & 2 & 14.37 & 0.54 & 2.0101E+01 & Direct-PRF & 0\\
009366989-02 & 3597.01 & 1:2 & 7.9 & 1 & 2 & 14.37 & 0.54 & 6.8177E+01 & Direct-PRF & 0\\
009390655-01 & 249.01 & 1:1 & 4.3 & -1 & 0 & 14.49 & 0.98 & 2.8006E+00 & Direct-PRF & 0\\
009392668-02 & 009392682-sec & 1:1 & 49.3 & -3 & -12 & 11.50 & 4.20 & 2.8000E+03 & Direct-PRF & 0\\
009394605-01 & 009394601-pri & 1:1 & 18.1 & -4 & -1 & 12.29 & 3.11 & 4.7012E+02 & Direct-PRF & 0\\
009396760-01 & FL-Lyr-pri & 1:1 & 1783.6 & -448 & 3 & 9.18 & 5.38 & 6.7979E+03 & Col-Anomaly & 0\\
009402583-01 & V2281-Cyg-pri & 1:2 & 86.9 & 22 & 0 & 11.82 & 4.07 & 3.3431E+03 & Direct-PRF & 0\\
009402649-01 & V2281-Cyg-pri & 1:2 & 74.5 & 11 & 16 & 11.82 & -0.76 & 3.6904E+04 & Direct-PRF & 0\\
009402670-01 & V2281-Cyg-pri & 1:2 & 72.2 & -13 & -12 & 11.82 & 3.84 & 3.7277E+03 & Direct-PRF & 0\\
009402709-01 & V2281-Cyg-pri & 1:2 & 74.5 & -18 & 0 & 11.82 & 1.62 & 1.8452E+04 & Direct-PRF & 0\\
009412445-01 & 009412462-01 & 1:2 & 15.4 & 4 & 0 & 14.85 & -0.20 & 2.1042E+03 & Direct-PRF & 0\\
009430371-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009456165-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009457541-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009468382-01 & 3466.01 & 1:1 & 9.4 & -1 & 2 & 16.41 & -2.85 & 3.1805E+02 & Direct-PRF & 0\\
009468382-02 & 009468384-02 & 1:1 & 9.4 & -1 & 2 & 16.41 & -2.85 & 2.5074E+02 & Direct-PRF & 0\\
009474232-01 & 009474232-pri & 1:1 & 18.2 & -3 & 3 & 13.28 & 1.29 & 9.6697E+02 & Direct-PRF & 0\\
009474239-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009474483-01 & 5683.01 & 1:1 & 20.9 & 3 & -4 & 14.88 & 0.60 & 2.2180E+02 & Direct-PRF & 0\\
009474493-02 & 5683.01 & 1:1 & 17.3 & 1 & -4 & 14.88 & 0.45 & 2.8724E+03 & Direct-PRF & 0\\
009474995-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009489348-01 & 009489411-pri & 1:2 & 43.7 & 11 & 1 & 13.96 & -0.36 & 8.0984E+03 & Direct-PRF & 0\\
009509223-01 & 009509207-sec & 1:1 & 34.4 & -8 & 0 & 13.13 & 0.46 & 2.6725E+03 & Direct-PRF & 0\\
009509223-02 & 009509207-pri & 1:1 & 34.4 & -8 & 0 & 13.13 & 0.46 & 2.3866E+03 & Direct-PRF & 0\\
009518651-01 & FL-Lyr-pri & 1:1 & 771.8 & -194 & 2 & 9.18 & 4.93 & 7.9102E+03 & Direct-PRF & 0\\
009529744-01 & 3600.01 & 1:2 & 14.0 & 4 & 0 & 14.04 & -0.56 & 9.5460E+02 & Direct-PRF & 0\\
009532117-01 & 6069.01 & 1:1 & 12.1 & -1 & -3 & 16.36 & -4.01 & 1.5658E+03 & Direct-PRF & 0\\
009532117-02 & 009532123-02 & 1:1 & 12.1 & -1 & -3 & 16.36 & -4.01 & 1.3531E+03 & Direct-PRF & 0\\
009532424-01 & 3710.01 & 1:1 & 9.4 & 1 & 3 & 16.77 & -2.21 & 2.0576E+02 & Direct-PRF & 0\\
009535876-01 & 4228.01 & 1:1 & 21.5 & 4 & -4 & 13.40 & 1.52 & 3.3126E+01 & Direct-PRF & 0\\
009540675-01 & V995-Cyg-pri & 1:1 & 119.4 & -1 & -30 & 11.88 & 1.99 & 1.7521E+04 & Direct-PRF & 0\\
009541089-01 & 009541127-pri & 1:1 & 23.4 & -6 & 2 & 12.56 & 1.40 & 7.7163E+03 & Direct-PRF & 0\\
009541094-01 & 009541127-pri & 1:1 & 56.6 & 1 & 14 & 12.56 & 1.25 & 1.6439E+04 & Direct-PRF & 0\\
009541144-01 & 009541127-pri & 1:1 & 78.7 & 10 & 16 & 12.56 & 1.36 & 1.2197E+04 & Direct-PRF & 0\\
009541163-01 & 009541127-pri & 1:1 & 61.9 & -2 & -16 & 12.56 & 2.89 & 4.1098E+03 & Direct-PRF & 0\\
009541223-01 & 009541127-pri & 1:1 & 102.0 & 24 & 8 & 12.56 & 1.10 & 6.3017E+04 & Direct-PRF & 0\\
009541295-01 & 009541127-pri & 1:1 & 131.5 & 33 & 0 & 12.56 & 0.09 & 3.7810E+04 & Direct-PRF & 0\\
009549471-01 & 6206.01 & 1:1 & 9.3 & 1 & 2 & 14.05 & 0.24 & 1.6199E+01 & Direct-PRF & 0\\
009549471-02 & 009549472-02 & 1:1 & 9.3 & 1 & 2 & 14.05 & 0.24 & 1.4465E+01 & Direct-PRF & 0\\
009579266-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009579789-01 & FL-Lyr-pri & 1:1 & 166.9 & -9 & -41 & 9.18 & 6.28 & 3.9551E+03 & Direct-PRF & 0\\
009592579-01 & 3565.01 & 1:1 & 6.7 & 0 & 1 & 15.90 & -0.80 & 3.3254E+01 & Direct-PRF & 0\\
009592831-01 & 009592855-01 & 1:2 & 30.2 & -7 & 1 & 12.22 & 4.46 & 1.3692E+01 & Direct-PRF & 0\\
009592850-01 & 009592855-pri & 1:2 & 6.9 & 0 & -1 & 12.22 & 4.18 & 7.1206E+00 & Direct-PRF & 0\\
009592918-01 & 009592855-pri & 1:2 & 83.9 & 21 & -1 & 12.22 & 2.80 & 5.2419E+03 & Direct-PRF & 0\\
009593757-01 & 009593759-01 & 1:1 & 6.2 & 0 & -2 & 17.47 & 0.22 & 4.3027E+01 & Direct-PRF & 0\\
009593757-02 & 3800.01 & 2:1 & 6.2 & 0 & -2 & 17.47 & 0.22 & 1.0398E+02 & Direct-PRF & 0\\
009597042-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009602421-01 & V995-Cyg-pri & 1:1 & 134.2 & -34 & 1 & 11.88 & 0.96 & 4.0574E+04 & Direct-PRF & 0\\
009602431-01 & V995-Cyg-pri & 1:1 & 123.0 & -18 & 25 & 11.88 & 3.31 & 1.2849E+04 & Direct-PRF & 0\\
009602514-01 & V995-Cyg-pri & 1:1 & 58.7 & -15 & 1 & 11.88 & 2.24 & 4.7295E+03 & Direct-PRF & 0\\
009602538-01 & V995-Cyg-pri & 1:1 & 197.3 & 14 & 48 & 11.88 & 2.73 & 1.3766E+04 & Direct-PRF & 0\\
009602562-01 & V995-Cyg-pri & 1:1 & 104.7 & 5 & 26 & 11.88 & 2.50 & 4.0789E+03 & Direct-PRF & 0\\
009602775-01 & V995-Cyg-pri & 1:1 & 134.2 & 29 & -16 & 11.88 & 4.04 & 6.3712E+03 & Direct-PRF & 0\\
009632007-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009635510-01 & 009635529-pri & 1:2 & 33.1 & 8 & 1 & 12.23 & 3.12 & 1.0345E+03 & Direct-PRF & 0\\
009636563-01 & 3618.01 & 1:1 & 10.2 & -2 & -1 & 17.04 & -1.94 & 1.0670E+03 & Direct-PRF & 0\\
009636569-01 & 3618.01 & 1:1 & 10.1 & -2 & 2 & 17.04 & -2.60 & 1.1762E+03 & Direct-PRF & 0\\
009640907-01 & FL-Lyr-pri & 1:2 & 170.1 & 30 & -30 & 9.18 & 6.52 & 2.3265E+03 & Direct-PRF & 0\\
009640921-03 & FL-Lyr-pri & 1:1 & 153.6 & 8 & -38 & 9.18 & 6.22 & 3.7832E+03 & Direct-PRF & 0\\
009640924-01 & FL-Lyr-pri & 1:2 & 143.3 & 30 & -20 & 9.18 & 5.80 & 5.3056E+03 & Direct-PRF & 0\\
009640931-01 & FL-Lyr-pri & 1:1 & 151.6 & 2 & -38 & 9.18 & 6.74 & 1.7472E+03 & Direct-PRF & 0\\
009640946-01 & FL-Lyr-pri & 1:1 & 153.8 & 38 & -8 & 9.18 & 5.78 & 3.5661E+03 & Direct-PRF & 0\\
009640962-01 & FL-Lyr-pri & 1:1 & 122.6 & 31 & -5 & 9.18 & 6.29 & 1.8513E+03 & Direct-PRF & 0\\
009640976-01 & FL-Lyr-pri & 1:1 & 138.2 & 35 & 2 & 9.18 & 4.54 & 2.7362E+03 & Direct-PRF & 0\\
009640976-02 & 009641031-01 & 2:1 & 138.2 & 35 & 2 & 9.18 & 4.54 & 5.9944E+03 & Direct-PRF & 0\\
009640985-01 & FL-Lyr-pri & 1:1 & 63.1 & 13 & -9 & 9.18 & 4.66 & 2.0619E+03 & Direct-PRF & 0\\
009641008-01 & FL-Lyr-pri & 1:1 & 70.0 & -10 & -14 & 9.18 & 5.31 & 1.3900E+03 & Direct-PRF & 0\\
009641018-01 & FL-Lyr-pri & 1:1 & 90.3 & 21 & 10 & 9.18 & 4.89 & 1.9957E+03 & Direct-PRF & 0\\
009641041-01 & FL-Lyr-pri & 1:1 & 66.6 & -15 & -7 & 9.18 & 3.04 & 4.6781E+03 & Direct-PRF & 0\\
009641076-01 & FL-Lyr-pri & 1:1 & 143.3 & 15 & 33 & 9.18 & 5.95 & 3.9195E+03 & Direct-PRF & 0\\
009641103-01 & FL-Lyr-pri & 1:2 & 230.9 & 25 & 53 & 9.18 & 4.95 & 1.2796E+04 & Direct-PRF & 0\\
009641144-01 & FL-Lyr-pri & 1:2 & 173.5 & -26 & 35 & 9.18 & 4.76 & 9.4579E+03 & Direct-PRF & 0\\
009644683-01 & 009644680-pri & 1:1 & 16.0 & 2 & -4 & 13.44 & 2.48 & 1.5933E+03 & Direct-PRF & 0\\
009652649-01 & 009652632-01 & 1:1 & 31.7 & 4 & 7 & 11.58 & 2.53 & 2.7426E+03 & Direct-PRF & 0\\
009652655-01 & 009652632-01 & 1:1 & 38.5 & 8 & 6 & 11.58 & 3.19 & 1.4165E+03 & Direct-PRF & 0\\
009661877-01 & 3647.01 & 1:1 & 7.8 & 2 & 0 & 16.68 & -1.51 & 1.0724E+02 & Direct-PRF & 0\\
009674564-01 & 009674592-01 & 1:1 & 16.5 & 4 & 0 & 15.93 & -1.89 & 6.4200E+01 & Direct-PRF & 0\\
009674564-02 & 3729.01 & 1:1 & 16.5 & 4 & 0 & 15.93 & -1.89 & 5.9861E+01 & Direct-PRF & 0\\
009691284-01 & 009691311-01 & 1:1 & 69.6 & 17 & -5 & 12.93 & 2.27 & 2.2892E-01 & Direct-PRF & 1\\
009691311-01 & 009691284-01 & 1:1 & 69.6 & -17 & 5 & 15.20 & -2.27 & 4.3684E+00 & Direct-PRF & 1\\
009692128-01 & 009569866-pri & 1:1 & 845.0 & 212 & 0 & 13.98 & -0.32 & 4.0061E+03 & Col-Anomaly & 0\\
009692345-01 & 3859.01 & 1:1 & 13.3 & -2 & 3 & 17.49 & -1.83 & 1.9572E+03 & Direct-PRF & 0\\
009704377-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009716262-01 & BR-Cyg-pri & 1:1 & 2691.0 & 676 & 7 & 10.03 & 7.56 & 7.0112E+02 & Col-Anomaly & 0\\
009716262-02 & BR-Cyg-pri & 1:1 & 2691.0 & 676 & 7 & 10.03 & 7.56 & 5.9455E+02 & Col-Anomaly & 0\\
009716302-01 & BR-Cyg-pri & 1:1 & 2638.5 & 663 & 5 & 10.03 & 6.46 & 1.8683E+03 & Col-Anomaly & 0\\
009716955-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009719634-01 & 3686.01 & 1:1 & 8.6 & 0 & 2 & 17.28 & -2.46 & 1.3587E+02 & Direct-PRF & 0\\
009724984-01 & 009724993-01 & 1:1 & 9.7 & -1 & 2 & 12.52 & 0.42 & 4.0425E+01 & Direct-PRF & 0\\
009752973-01 & 3871.01 & 1:1 & 13.0 & 3 & 0 & 12.22 & -2.18 & 1.5069E+01 & Direct-PRF & 0\\
009762514-01 & 009762519-01 & 1:1 & 18.1 & 1 & -4 & 13.71 & 1.81 & 6.4120E+02 & Direct-PRF & 0\\
009764489-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009764868-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009773869-03 & 3457.01 & 1:1 & 7.0 & 0 & 1 & 12.43 & 4.24 & 3.4390E+03 & Direct-PRF & 0\\
009776692-01 & 009776718-sec & 1:1 & 22.4 & 6 & -1 & 15.04 & 0.92 & 1.5230E+02 & Direct-PRF & 0\\
009777087-01 & 009777090-01 & 1:1 & 4.1 & 1 & 0 & 17.78 & -0.71 & 1.0317E+01 & Direct-PRF & 0\\
009777087-02 & 009777090-02 & 2:1 & 4.1 & 1 & 0 & 17.78 & -0.71 & 1.0425E+01 & Direct-PRF & 0\\
009777087-03 & 009777062-01 & 1:1 & 22.8 & -5 & 3 & 12.24 & 4.82 & 7.9196E+01 & Direct-PRF & 0\\
009777200-01 & BR-Cyg-pri & 1:1 & 2041.8 & 513 & 1 & 10.03 & 3.89 & 1.8078E+04 & Col-Anomaly & 0\\
009777251-01 & BR-Cyg-pri & 1:1 & 1984.9 & 499 & 3 & 10.03 & 5.03 & 5.4380E+03 & Col-Anomaly & 0\\
009777256-01 & BR-Cyg-pri & 1:1 & 1975.9 & 496 & 1 & 10.03 & 5.23 & 5.6684E+03 & Col-Anomaly & 0\\
009777290-01 & BR-Cyg-pri & 1:1 & 1957.7 & 492 & 5 & 10.03 & 6.31 & 2.8247E+03 & Col-Anomaly & 0\\
009777453-01 & BR-Cyg-pri & 1:1 & 1839.7 & 462 & 15 & 10.03 & 8.73 & 3.8956E+02 & Col-Anomaly & 0\\
009777556-01 & BR-Cyg-pri & 1:1 & 1676.0 & 421 & 3 & 10.03 & 6.04 & 1.7107E+03 & Col-Anomaly & 0\\
009777724-01 & BR-Cyg-pri & 1:1 & 1509.7 & 379 & 3 & 10.03 & 5.84 & 5.6684E+03 & Col-Anomaly & 0\\
009777757-01 & BR-Cyg-pri & 1:1 & 1477.6 & 371 & 4 & 10.03 & 2.97 & 1.5555E+04 & Col-Anomaly & 0\\
009821151-01 & 009821078-01 & 1:2 & 173.3 & 44 & -1 & 14.12 & -1.73 & 7.5647E+03 & Col-Anomaly & 0\\
009827596-01 & 6211.01 & 1:1 & 529.6 & 133 & -1 & 14.71 & -0.15 & 6.8087E+03 & Col-Anomaly & 0\\
009833599-01 & 009833618-pri & 1:1 & 29.0 & -3 & -7 & 13.68 & 1.74 & 7.5333E+03 & Direct-PRF & 0\\
009834257-01 & 009773869-01 & 1:1 & 7.0 & 0 & -1 & 16.67 & -4.24 & 1.0848E+02 & Direct-PRF & 0\\
009834257-02 & 3568.01 & 1:1 & 7.0 & 0 & -1 & 16.67 & -4.24 & 1.3008E+02 & Direct-PRF & 0\\
009835505-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009837586-01 & 009837578-01 & 1:2 & 5.4 & -1 & -1 & 15.73 & 1.75 & 7.2012E+00 & Direct-PRF & 0\\
009838537-01 & BR-Cyg-pri & 1:1 & 1056.9 & 265 & 3 & 10.03 & 3.43 & 1.6722E+05 & Col-Anomaly & 0\\
009838608-01 & BR-Cyg-pri & 1:1 & 982.9 & 247 & 2 & 10.03 & 5.14 & 7.4319E+03 & Col-Anomaly & 0\\
009838804-01 & BR-Cyg-pri & 1:1 & 763.2 & 191 & 3 & 10.03 & 5.96 & 3.6155E+03 & Col-Anomaly & 0\\
009842906-01 & 009842890-pri & 1:1 & 10.3 & 3 & -1 & 15.75 & -0.31 & 1.6598E+00 & Direct-PRF & 0\\
009842937-01 & 009842890-pri & 1:1 & 40.0 & 9 & 3 & 15.75 & -0.42 & 3.9801E+00 & Direct-PRF & 1\\
009849884-01 & 009971475-01 & 1:1 & 1507.6 & 379 & 0 & 13.17 & -0.57 & 2.8102E+03 & Col-Anomaly & 0\\
009850843-01 & 009851142-pri & 1:1 & 218.0 & 53 & 12 & 7.63 & 7.23 & 7.4545E+02 & Direct-PRF & 0\\
009850893-01 & 009851142-pri & 1:1 & 192.2 & 29 & 39 & 7.63 & 7.04 & 2.8276E+02 & Direct-PRF & 0\\
009850912-01 & 009851142-pri & 1:1 & 202.8 & 22 & 46 & 7.63 & 8.16 & 3.1103E+02 & Direct-PRF & 0\\
009850957-01 & 009851142-pri & 1:1 & 138.4 & 22 & 27 & 7.63 & 5.49 & 6.0537E+02 & Direct-PRF & 0\\
009850966-01 & 009851142-pri & 1:1 & 160.5 & 39 & -10 & 7.63 & 8.23 & 2.6297E+02 & Direct-PRF & 0\\
009851021-01 & 009851142-pri & 1:1 & 113.1 & 10 & 27 & 7.63 & 2.63 & 1.0612E+03 & Direct-PRF & 0\\
009851123-01 & 009851142-pri & 1:1 & 56.7 & -3 & 14 & 7.63 & 8.11 & 3.4025E+01 & Direct-PRF & 0\\
009851123-02 & 009851142-02 & 1:1 & 56.7 & -3 & 14 & 7.63 & 8.11 & 1.3534E+00 & Direct-PRF & 0\\
009851126-01 & 009851142-pri & 1:1 & 21.4 & 1 & 5 & 7.63 & 5.55 & 1.1128E+00 & Direct-PRF & 0\\
009851126-02 & 009851142-02 & 1:1 & 21.4 & 1 & 5 & 7.63 & 5.55 & 1.3588E-01 & Direct-PRF & 0\\
009851226-01 & 009851142-pri & 1:1 & 77.9 & -6 & -19 & 7.63 & 7.63 & 6.4108E+01 & Direct-PRF & 0\\
009851226-02 & 009851142-02 & 1:1 & 77.9 & -6 & -19 & 7.63 & 7.63 & 6.9511E+00 & Direct-PRF & 0\\
009851271-01 & 009851142-pri & 1:1 & 91.0 & -14 & -18 & 7.63 & 6.98 & 2.3429E+02 & Direct-PRF & 0\\
009851360-01 & 009851142-pri & 1:1 & 184.5 & -45 & 9 & 7.63 & 7.68 & 5.0111E+02 & Direct-PRF & 0\\
009851845-01 & 009851944-pri & 1:2 & 113.9 & 7 & 27 & 11.25 & 2.63 & 5.7778E+03 & Direct-PRF & 0\\
009851943-01 & 009851944-pri & 1:2 & 33.2 & -4 & 7 & 11.25 & 4.00 & 1.1304E+03 & Direct-PRF & 0\\
009851970-01 & 009851944-pri & 1:2 & 89.4 & -14 & 17 & 11.25 & 4.22 & 1.7190E+03 & Direct-PRF & 0\\
009873759-01 & 009873869-01 & 1:1 & 324.1 & 82 & 1 & 13.04 & 0.78 & 2.8364E+03 & Col-Anomaly & 0\\
009886221-01 & 3614.01 & 1:1 & 13.4 & -1 & 3 & 16.33 & -1.93 & 1.2108E+03 & Direct-PRF & 0\\
009893365-01 & 009953894-sec & 1:2 & 93.4 & -23 & 0 & 11.08 & 3.26 & 6.7850E+03 & Direct-PRF & 0\\
009893463-01 & 009953894-sec & 1:2 & 77.5 & -6 & 19 & 11.08 & 4.48 & 2.2617E+03 & Direct-PRF & 0\\
009896438-01 & 3755.01 & 1:1 & 6.2 & -1 & 1 & 16.64 & 0.03 & 2.5173E+00 & Direct-PRF & 0\\
009899065-01 & BR-Cyg-pri & 1:1 & 361.9 & 91 & 2 & 10.03 & 5.83 & 5.2667E+03 & Direct-PRF & 0\\
009899141-01 & BR-Cyg-pri & 1:1 & 236.5 & 57 & -17 & 10.03 & 2.47 & 4.7776E+04 & Direct-PRF & 0\\
009899153-01 & BR-Cyg-pri & 1:1 & 215.8 & 42 & -34 & 10.03 & 4.85 & 1.1944E+04 & Direct-PRF & 0\\
009899181-01 & BR-Cyg-pri & 1:1 & 196.6 & 47 & -14 & 10.03 & 2.88 & 2.4773E+04 & Direct-PRF & 0\\
009899193-01 & BR-Cyg-pri & 1:1 & 250.7 & 61 & 15 & 10.03 & 3.16 & 2.1576E+04 & Direct-PRF & 0\\
009899217-01 & BR-Cyg-pri & 1:1 & 181.5 & 45 & -3 & 10.03 & 5.24 & 6.8956E+03 & Direct-PRF & 0\\
009899233-01 & BR-Cyg-pri & 1:1 & 186.6 & 46 & 5 & 10.03 & 5.14 & 4.1035E+03 & Direct-PRF & 0\\
009899256-01 & BR-Cyg-pri & 1:1 & 261.3 & 56 & 34 & 10.03 & 4.25 & 2.7870E+04 & Direct-PRF & 0\\
009899280-01 & BR-Cyg-pri & 1:1 & 104.9 & 22 & -15 & 10.03 & 5.01 & 4.2876E+03 & Direct-PRF & 0\\
009899315-01 & BR-Cyg-pri & 1:1 & 203.7 & 41 & -8 & 15.92 & -0.54 & 1.9254E+00 & Col-Anomaly & 0\\
009899352-01 & BR-Cyg-pri & 1:1 & 135.3 & 25 & 22 & 10.03 & 5.82 & 4.0052E+03 & Direct-PRF & 0\\
009899355-01 & BR-Cyg-pri & 1:1 & 108.1 & 21 & 16 & 10.03 & 5.84 & 1.1532E+04 & Direct-PRF & 0\\
009899410-01 & BR-Cyg-pri & 1:1 & 89.5 & 12 & 18 & 10.03 & 3.48 & 6.9674E+03 & Direct-PRF & 0\\
009899414-01 & BR-Cyg-pri & 1:1 & 43.4 & 6 & 9 & 10.03 & 4.89 & 3.9814E+03 & Direct-PRF & 0\\
009899421-01 & BR-Cyg-pri & 1:1 & 53.4 & 4 & 12 & 10.03 & 2.27 & 7.5154E+03 & Direct-PRF & 0\\
009899449-01 & BR-Cyg-pri & 1:1 & 51.9 & -13 & -3 & 10.03 & 5.60 & 5.2255E+03 & Direct-PRF & 0\\
009899483-01 & BR-Cyg-pri & 1:1 & 105.9 & -4 & 26 & 10.03 & 3.59 & 9.4207E+03 & Direct-PRF & 0\\
009899505-01 & BR-Cyg-pri & 1:1 & 85.2 & -17 & 13 & 10.03 & 5.92 & 3.0129E+03 & Direct-PRF & 0\\
009899514-01 & BR-Cyg-pri & 1:1 & 166.0 & -2 & 41 & 10.03 & 5.89 & 5.1850E+03 & Direct-PRF & 0\\
009899538-01 & BR-Cyg-pri & 1:1 & 215.6 & -1 & 54 & 10.03 & 4.00 & 3.9345E+04 & Direct-PRF & 0\\
009899577-01 & BR-Cyg-pri & 1:1 & 149.9 & -25 & 28 & 10.03 & 4.79 & 9.8363E+03 & Direct-PRF & 0\\
009899583-01 & BR-Cyg-pri & 1:1 & 182.5 & -19 & 42 & 10.03 & 4.81 & 1.4864E+04 & Direct-PRF & 0\\
009899607-01 & BR-Cyg-pri & 1:1 & 168.4 & -32 & 27 & 10.03 & 5.27 & 7.9627E+03 & Direct-PRF & 0\\
009899630-01 & BR-Cyg-pri & 1:1 & 189.7 & -35 & 33 & 10.03 & 5.53 & 5.3510E+03 & Direct-PRF & 0\\
009910828-01 & 009851142-pri & 1:1 & 206.6 & -21 & 47 & 7.63 & 7.25 & 3.7119E+02 & Direct-PRF & 0\\
009910942-01 & 009851142-pri & 1:1 & 183.3 & -33 & 32 & 7.63 & 5.17 & 2.2000E+03 & Direct-PRF & 0\\
009934274-01 & 009873869-01 & 1:1 & 458.1 & 116 & -1 & 13.04 & 0.31 & 5.2190E+03 & Col-Anomaly & 0\\
009944356-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009953851-01 & 009953894-sec & 1:2 & 61.7 & -7 & -14 & 11.08 & 4.23 & 2.2246E+03 & Direct-PRF & 0\\
009957659-01 & 5744.01 & 2:1 & 9.6 & 2 & 1 & 12.51 & 2.99 & 4.4578E+00 & Direct-PRF & 0\\
009959492-01 & BR-Cyg-pri & 1:1 & 184.6 & -6 & -46 & 10.03 & 5.25 & 9.1626E+03 & Direct-PRF & 0\\
009959494-01 & BR-Cyg-pri & 1:1 & 127.6 & 1 & -32 & 10.03 & 1.81 & 4.4591E+04 & Direct-PRF & 0\\
009959545-01 & BR-Cyg-pri & 1:1 & 141.5 & -14 & -33 & 10.03 & 4.12 & 1.6314E+04 & Direct-PRF & 0\\
009959589-01 & BR-Cyg-pri & 1:1 & 127.2 & -21 & -25 & 10.03 & 5.76 & 4.0293E+03 & Direct-PRF & 0\\
009965184-01 & 009965206-02 & 1:1 & 12.5 & -3 & 0 & 15.90 & -0.51 & 3.3103E+02 & Direct-PRF & 0\\
009965184-02 & 3558.01 & 1:1 & 12.5 & -3 & 0 & 15.90 & -0.51 & 3.8237E+02 & Direct-PRF & 0\\
009995753-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
009995942-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010002266-01 & 010002261-pri & 1:1 & 22.4 & 5 & -2 & 13.10 & 2.03 & 2.3064E+02 & Direct-PRF & 0\\
010014702-01 & 5742.01 & 1:1 & 157.5 & 40 & 1 & 14.56 & 0.57 & 1.4798E+04 & Col-Anomaly & 0\\
010016317-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010026458-01 & 010026457-01 & 1:1 & 7.4 & -1 & -2 & 15.39 & 0.39 & 1.5673E+01 & Direct-PRF & 0\\
010026458-02 & 010026457-02 & 1:1 & 7.4 & -1 & -2 & 15.39 & 0.39 & 1.8149E+01 & Direct-PRF & 0\\
010031500-01 & 010031808-01 & 1:1 & 228.3 & 58 & 2 & 9.56 & 5.66 & 8.8592E+02 & Direct-PRF & 0\\
010031526-01 & 010031808-01 & 1:1 & 188.8 & 41 & 25 & 9.56 & 6.13 & 1.3053E+03 & Direct-PRF & 0\\
010031656-01 & 010031808-01 & 1:1 & 112.5 & 19 & 21 & 9.56 & 5.85 & 9.2220E+02 & Direct-PRF & 0\\
010031707-01 & 010031808-01 & 1:1 & 68.7 & 18 & 0 & 9.56 & 4.31 & 6.7048E+02 & Direct-PRF & 0\\
010031707-02 & 010031808-02 & 1:1 & 68.7 & 18 & 0 & 9.56 & 4.31 & 6.4979E+02 & Direct-PRF & 0\\
010031885-01 & 010031808-01 & 1:1 & 62.5 & -15 & 2 & 9.56 & 3.92 & 1.1120E+03 & Direct-PRF & 0\\
010031885-02 & 010031808-02 & 1:1 & 62.5 & -15 & 2 & 9.56 & 3.92 & 1.2496E+03 & Direct-PRF & 0\\
010031907-01 & 010031808-01 & 1:1 & 69.4 & -17 & 0 & 9.56 & 5.09 & 2.7914E+02 & Direct-PRF & 0\\
010031907-02 & 010031808-01 & 1:2 & 69.4 & -17 & 0 & 9.56 & 5.09 & 1.5095E+03 & Direct-PRF & 0\\
010031918-01 & 010031808-01 & 1:1 & 117.8 & -26 & 13 & 9.56 & 5.28 & 1.9439E+03 & Direct-PRF & 0\\
010068024-01 & 529.01 & 1:1 & 5.8 & 2 & 1 & 14.98 & -1.85 & 2.1387E+01 & Direct-PRF & 0\\
010068030-03 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010082556-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010090219-01 & 010090246-pri & 1:1 & 16.7 & -3 & 2 & 13.57 & 1.55 & 8.6351E+02 & Direct-PRF & 0\\
010090257-01 & 010090246-pri & 1:1 & 15.3 & 2 & -4 & 13.57 & 1.98 & 5.5808E+02 & Direct-PRF & 0\\
010092312-02 & 1080.01 & 1:1 & 9.9 & -1 & -2 & 14.87 & -0.91 & 2.9640E+00 & Direct-PRF & 0\\
010130057-01 & FL-Lyr-pri & 1:1 & 3770.8 & -384 & 5 & 9.18 & 6.44 & 4.5319E+03 & Col-Anomaly & 2\\
010156055-01 & 010156064-pri & 1:2 & 58.1 & -8 & 12 & 10.37 & 3.68 & 1.7411E+03 & Direct-PRF & 0\\
010158990-01 & 1823.02 & 1:1 & 9.9 & 1 & 2 & 13.95 & 0.91 & 3.9812E+00 & Direct-PRF & 0\\
010189542-01 & 427.01 & 1:1 & 6.4 & 0 & 1 & 14.62 & -0.28 & 7.8571E+00 & Direct-PRF & 0\\
010191036-01 & T-Lyr1-00687-sec & 1:2 & 66.2 & 17 & -2 & 10.81 & 1.30 & 8.6436E+03 & Direct-PRF & 0\\
010191070-01 & T-Lyr1-00687-sec & 1:2 & 26.5 & -1 & -7 & 10.81 & 5.01 & 4.4223E+03 & Direct-PRF & 0\\
010191142-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010195926-01 & 010195933-02 & 1:1 & 16.2 & -4 & -1 & 15.67 & -5.10 & 3.6579E+00 & Direct-PRF & 1\\
010195926-02 & 010195933-02 & 1:1 & 16.2 & -4 & -1 & 15.67 & -5.10 & 6.0435E+00 & Direct-PRF & 1\\
010195926-04 & 010195933-01 & 1:1 & 16.2 & -4 & -1 & 15.67 & -5.10 & 8.8947E+00 & Direct-PRF & 1\\
010195933-01 & 010195926-04 & 1:1 & 16.2 & 4 & 1 & 10.57 & 5.10 & 1.1243E-01 & Direct-PRF & 1\\
010195933-02 & 010195926-02 & 1:1 & 16.2 & 4 & 1 & 10.57 & 5.10 & 1.6547E-01 & Direct-PRF & 1\\
010196750-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010201143-02 & 1783.01 & 1:13 & 1311.6 & 170 & -9 & 13.93 & -0.67 & 1.7878E+02 & Col-Anomaly & 2\\
010215584-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010226343-01 & 010226388-pri & 1:1 & 72.3 & 14 & -12 & 10.77 & 4.89 & 2.3880E+03 & Direct-PRF & 0\\
010226448-01 & 010226388-pri & 1:1 & 53.1 & -4 & -13 & 10.77 & 3.23 & 8.5967E+03 & Direct-PRF & 0\\
010226451-01 & 010226388-pri & 1:1 & 66.5 & -15 & 8 & 10.77 & 4.17 & 1.9838E+04 & Direct-PRF & 0\\
010226451-02 & 010226388-sec & 1:1 & 66.5 & -15 & 8 & 10.77 & 4.17 & 2.1180E+05 & Direct-PRF & 0\\
010226487-01 & 010226388-pri & 1:1 & 78.8 & -19 & 4 & 10.77 & 4.06 & 6.4475E+04 & Direct-PRF & 0\\
010226488-01 & 010226388-pri & 1:1 & 99.1 & -23 & 10 & 10.77 & 3.46 & 6.6128E+03 & Direct-PRF & 0\\
010226498-01 & 010226388-pri & 1:1 & 81.4 & -21 & 1 & 10.77 & 4.16 & 5.4872E+03 & Direct-PRF & 0\\
010227863-01 & 5780.01 & 1:1 & 20.2 & 4 & -3 & 15.53 & -1.77 & 8.1228E+00 & Direct-PRF & 1\\
010256023-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010259031-01 & 3630.01 & 1:1 & 6.1 & -2 & 1 & 17.11 & -1.52 & 9.2524E+01 & Direct-PRF & 0\\
010259031-02 & 010259029-02 & 1:1 & 6.1 & -2 & 1 & 17.11 & -1.52 & 5.0247E+01 & Direct-PRF & 0\\
010262272-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010268907-01 & 3773.01 & 1:1 & 6.0 & -1 & 0 & 17.36 & -1.63 & 3.5975E+02 & Direct-PRF & 0\\
010268907-02 & 3773.01 & 1:2 & 6.0 & -1 & 0 & 17.36 & -1.63 & 5.4576E+02 & Direct-PRF & 0\\
010272389-01 & V850-Cyg-pri & 1:1 & 311.7 & 78 & 1 & 11.20 & 3.14 & 3.3625E+03 & Direct-PRF & 0\\
010275284-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010275420-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010275766-01 & 010275747-pri & 1:1 & 31.0 & 4 & 6 & 12.80 & 2.60 & 3.5252E+03 & Direct-PRF & 0\\
010275880-01 & 010275887-pri & 1:1 & 10.0 & 2 & -1 & 13.04 & 0.17 & 6.2096E+01 & Direct-PRF & 0\\
010275880-02 & 010275887-sec & 1:1 & 10.0 & 2 & -1 & 13.04 & 0.17 & 1.1430E+02 & Direct-PRF & 0\\
010294509-01 & 010294608-pri & 1:2 & 67.8 & 17 & 1 & 13.34 & 2.36 & 1.4739E+03 & Direct-PRF & 0\\
010294613-01 & 010294608-pri & 1:1 & 16.1 & -3 & 3 & 13.34 & 1.55 & 7.1598E+02 & Direct-PRF & 0\\
010294613-02 & 010294608-01 & 2:1 & 16.1 & -3 & 3 & 13.34 & 1.55 & 2.3926E+03 & Direct-PRF & 0\\
010322797-01 & T-Lyr1-00687-sec & 1:2 & 793.5 & 200 & 1 & 10.81 & 2.39 & 1.0008E+04 & Col-Anomaly & 0\\
010337035-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010340212-01 & V2083-Cyg-pri & 1:2 & 1723.9 & 206 & -382 & 6.90 & 6.91 & 3.3054E+03 & Direct-PRF & 0\\
010340228-01 & V2083-Cyg-pri & 1:2 & 1699.4 & 228 & -362 & 6.90 & 8.89 & 2.6443E+03 & Direct-PRF & 0\\
010341755-01 & V2083-Cyg-pri & 1:2 & 267.2 & 24 & -63 & 6.90 & 8.77 & 2.2283E+03 & Direct-PRF & 0\\
010341777-01 & V2083-Cyg-pri & 1:2 & 246.8 & 24 & -58 & 6.90 & 6.18 & 6.6107E+04 & Direct-PRF & 0\\
010341781-01 & V2083-Cyg-pri & 1:2 & 244.5 & 24 & -57 & 6.90 & 8.49 & 1.8710E+03 & Direct-PRF & 0\\
010341787-01 & V2083-Cyg-pri & 1:2 & 252.8 & 11 & -63 & 6.90 & 9.02 & 1.6807E+03 & Direct-PRF & 0\\
010341831-01 & V2083-Cyg-pri & 1:2 & 195.9 & 33 & -37 & 6.90 & 8.06 & 1.7867E+03 & Direct-PRF & 0\\
010341905-01 & V2083-Cyg-pri & 1:2 & 151.2 & -9 & -37 & 6.90 & 8.34 & 1.6666E+03 & Direct-PRF & 0\\
010341913-01 & V2083-Cyg-pri & 1:2 & 124.6 & -1 & -31 & 6.90 & 6.18 & 7.9329E+03 & Direct-PRF & 0\\
010341917-01 & V2083-Cyg-pri & 1:2 & 140.7 & -10 & -34 & 6.90 & 8.91 & 1.2713E+03 & Direct-PRF & 0\\
010342097-01 & V2083-Cyg-pri & 1:2 & 102.9 & 3 & -25 & 6.90 & 6.60 & 1.9832E+03 & Direct-PRF & 0\\
010342248-01 & V2083-Cyg-pri & 1:2 & 229.2 & -34 & -45 & 6.90 & 7.86 & 3.5415E+03 & Direct-PRF & 0\\
010342316-01 & V2083-Cyg-pri & 1:2 & 295.8 & -23 & -69 & 6.90 & 8.42 & 4.3113E+03 & Direct-PRF & 0\\
010352945-01 & 3756.01 & 1:1 & 7.3 & 2 & 2 & 14.35 & 1.05 & 1.3113E+01 & Direct-PRF & 0\\
010363281-01 & 010363300-pri & 1:1 & 15.2 & 2 & 3 & 14.68 & -2.37 & 2.4140E+03 & Direct-PRF & 0\\
010383687-01 & 3671.01 & 1:1 & 10.9 & -1 & -3 & 16.95 & -3.65 & 4.9294E+02 & Direct-PRF & 0\\
010383687-02 & 010383696-02 & 1:1 & 10.9 & -1 & -3 & 16.95 & -3.65 & 4.1142E+02 & Direct-PRF & 0\\
010394802-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010405470-01 & V2083-Cyg-pri & 1:2 & 1712.0 & 295 & -314 & 6.90 & 8.39 & 3.9664E+03 & Direct-PRF & 0\\
010407020-01 & V2083-Cyg-pri & 1:2 & 170.4 & 41 & -13 & 6.90 & 6.47 & 7.0829E+03 & Direct-PRF & 0\\
010407047-01 & V2083-Cyg-pri & 1:2 & 232.4 & 59 & -5 & 6.90 & 6.42 & 2.9165E+03 & Direct-PRF & 0\\
010407054-01 & V2083-Cyg-pri & 1:2 & 272.9 & 68 & -12 & 6.90 & 6.44 & 2.2537E+03 & Direct-PRF & 0\\
010407086-01 & V2083-Cyg-pri & 1:1 & 349.6 & 82 & -31 & 6.90 & 5.98 & 2.4790E+04 & Direct-PRF & 0\\
010407210-01 & V2083-Cyg-pri & 1:1 & 265.9 & 65 & 19 & 6.90 & 4.06 & 1.3221E+04 & Direct-PRF & 0\\
010407221-01 & V2083-Cyg-pri & 1:2 & 257.3 & 46 & -45 & 6.90 & 8.75 & 1.3221E+03 & Direct-PRF & 0\\
010407271-01 & V2083-Cyg-pri & 1:2 & 351.8 & 59 & -65 & 6.90 & 8.08 & 7.6278E+03 & Direct-PRF & 0\\
010407430-01 & V2083-Cyg-pri & 1:2 & 306.4 & -11 & -75 & 6.90 & 8.72 & 2.0237E+03 & Direct-PRF & 0\\
010407464-01 & V2083-Cyg-pri & 1:2 & 352.3 & -3 & -87 & 6.90 & 5.82 & 1.5256E+04 & Direct-PRF & 0\\
010470882-01 & V2083-Cyg-pri & 1:2 & 1853.6 & 339 & -320 & 6.90 & 9.06 & 3.5415E+03 & Direct-PRF & 0\\
010470968-01 & V2083-Cyg-pri & 1:2 & 1835.5 & 369 & -278 & 6.90 & 8.05 & 6.8387E+03 & Direct-PRF & 0\\
010471055-01 & V2083-Cyg-pri & 1:2 & 1726.2 & 330 & -283 & 6.90 & 8.12 & 4.4072E+03 & Direct-PRF & 0\\
010471113-01 & V2083-Cyg-pri & 1:2 & 1653.3 & 311 & -277 & 6.90 & 8.41 & 3.6726E+03 & Direct-PRF & 0\\
010471167-01 & V2083-Cyg-pri & 1:2 & 1696.6 & 362 & -226 & 6.90 & 6.10 & 1.7867E+03 & Direct-PRF & 0\\
010471174-01 & V2083-Cyg-pri & 1:2 & 1645.2 & 339 & -238 & 6.90 & 9.08 & 1.9069E+03 & Direct-PRF & 0\\
010471204-01 & V2083-Cyg-pri & 1:2 & 1605.9 & 326 & -239 & 6.90 & 8.92 & 9.9161E+03 & Direct-PRF & 0\\
010471345-01 & V2083-Cyg-pri & 1:2 & 1469.3 & 303 & -212 & 6.90 & 8.86 & 3.3054E+03 & Direct-PRF & 0\\
010480921-01 & 5797.01 & 1:1 & 33.7 & -8 & 3 & 12.22 & 1.97 & 2.7480E+03 & Direct-PRF & 0\\
010480982-02 & 5797.01 & 1:1 & 74.0 & 14 & -12 & 12.22 & 3.12 & 2.0356E+03 & Direct-PRF & 0\\
010481045-01 & 5797.01 & 1:1 & 96.7 & 24 & 2 & 12.22 & 2.83 & 2.9183E+03 & Direct-PRF & 0\\
010481054-01 & 5797.01 & 1:1 & 118.0 & 13 & 27 & 12.22 & 1.71 & 9.6989E+03 & Direct-PRF & 0\\
010485035-01 & 010485137-pri & 2:1 & 64.9 & -16 & -2 & 11.88 & 1.61 & 1.0788E+04 & Direct-PRF & 0\\
010485047-01 & 010485137-pri & 2:1 & 62.2 & -8 & -14 & 11.88 & 3.89 & 5.1662E+03 & Direct-PRF & 0\\
010485069-01 & 010485137-pri & 2:1 & 80.9 & 0 & -21 & 11.88 & 3.46 & 1.0480E+04 & Direct-PRF & 0\\
010485165-01 & 010485137-pri & 2:1 & 66.5 & 13 & -10 & 11.88 & 2.63 & 8.1511E+03 & Direct-PRF & 0\\
010485179-01 & 010485137-pri & 2:1 & 37.0 & 9 & 0 & 11.88 & 2.62 & 5.8222E+03 & Direct-PRF & 0\\
010485179-02 & 010485137-pri & 2:1 & 37.0 & 9 & 0 & 11.88 & 2.62 & 1.0189E+04 & Direct-PRF & 0\\
010489525-01 & 3625.01 & 1:1 & 11.8 & -2 & -2 & 16.17 & -3.39 & 1.7668E+03 & Direct-PRF & 0\\
010489525-02 & 010489521-01 & 2:1 & 11.8 & -2 & -2 & 16.17 & -3.39 & 3.1333E+03 & Direct-PRF & 0\\
010491044-01 & 010491031-sec & 1:2 & 21.0 & -4 & 3 & 13.24 & 2.71 & 5.5106E+02 & Direct-PRF & 0\\
010491062-01 & 010491031-sec & 1:2 & 16.9 & -4 & -2 & 13.24 & 2.09 & 3.9542E+02 & Direct-PRF & 0\\
010491544-01 & 010491554-01 & 1:1 & 4.4 & 1 & 1 & 15.02 & -1.58 & 8.3394E+00 & Direct-PRF & 0\\
010491544-02 & 010491554-sec & 1:1 & 4.4 & 1 & 1 & 15.02 & -1.58 & 6.3636E+00 & Direct-PRF & 0\\
010514430-01 & 010514429-01 & 1:1 & 2.1 & 1 & 1 & 11.41 & -0.59 & 1.3874E+00 & Direct-PRF & 0\\
010517437-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010518399-01 & 010583181-pri & 1:1 & 106.1 & -4 & 26 & 11.01 & 3.51 & 2.4794E+03 & Direct-PRF & 0\\
010518424-01 & 010583181-pri & 1:1 & 85.0 & -11 & 19 & 11.01 & 4.31 & 1.2397E+03 & Direct-PRF & 0\\
010518424-02 & 010583181-sec & 1:1 & 85.0 & -11 & 19 & 11.01 & 4.31 & 9.8261E+02 & Direct-PRF & 0\\
010518725-01 & 3612.01 & 1:1 & 14.6 & 4 & 1 & 16.74 & -3.62 & 1.5073E+03 & Direct-PRF & 0\\
010518725-02 & 010518735-02 & 1:1 & 14.6 & 4 & 1 & 16.74 & -3.62 & 1.0775E+03 & Direct-PRF & 0\\
010528093-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010532030-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010533906-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010535708-01 & V2083-Cyg-pri & 1:2 & 1927.9 & 417 & -248 & 6.90 & 8.71 & 2.8742E+03 & Direct-PRF & 0\\
010535858-01 & V2083-Cyg-pri & 1:2 & 1863.9 & 421 & -208 & 6.90 & 8.53 & 2.5756E+03 & Direct-PRF & 0\\
010535867-01 & V2083-Cyg-pri & 1:2 & 1856.7 & 420 & -206 & 6.90 & 8.49 & 3.7419E+03 & Direct-PRF & 0\\
010535897-01 & V2083-Cyg-pri & 1:2 & 1768.7 & 390 & -215 & 6.90 & 6.89 & 1.0438E+04 & Direct-PRF & 0\\
010549562-01 & 010549576-pri & 1:1 & 14.3 & -3 & 3 & 13.02 & 1.39 & 1.1247E+02 & Direct-PRF & 0\\
010549562-02 & 010549576-sec & 1:1 & 14.3 & -3 & 3 & 13.02 & 1.39 & 1.5963E+02 & Direct-PRF & 0\\
010555375-01 & 3771.01 & 1:1 & 6.7 & -2 & 0 & 16.61 & -2.85 & 3.1284E+01 & Direct-PRF & 0\\
010582569-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010583180-01 & 010583181-pri & 1:1 & 52.9 & -10 & 9 & 11.01 & 4.26 & 7.4164E+02 & Direct-PRF & 0\\
010583180-02 & 010583181-sec & 1:1 & 52.9 & -10 & 9 & 11.01 & 4.26 & 1.1300E+03 & Direct-PRF & 0\\
010583225-01 & 010583181-pri & 1:1 & 71.8 & -17 & -4 & 11.01 & 3.54 & 1.3452E+03 & Direct-PRF & 0\\
010583225-02 & 010583181-sec & 1:1 & 71.8 & -17 & -4 & 11.01 & 3.54 & 1.4349E+03 & Direct-PRF & 0\\
010590285-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010593761-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010597164-01 & V850-Cyg-pri & 1:1 & 2549.0 & 641 & 1 & 11.20 & 2.78 & 8.9835E+03 & Col-Anomaly & 0\\
010598279-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010601538-01 & 010601549-pri & 1:1 & 19.1 & 5 & 1 & 13.32 & -0.15 & 1.8297E+03 & Direct-PRF & 0\\
010618236-01 & 010618253-pri & 2:1 & 44.4 & 8 & 8 & 12.81 & 2.72 & 5.8240E+03 & Direct-PRF & 0\\
010619142-01 & 010619109-pri & 1:1 & 83.0 & -14 & -16 & 11.70 & 3.27 & 1.9838E+03 & Direct-PRF & 0\\
010621666-01 & 010686876-01 & 1:1 & 56.6 & 0 & 14 & 11.73 & 2.87 & 1.1570E+03 & Direct-PRF & 0\\
010661718-01 & 010661783-pri & 1:1 & 66.9 & -15 & -9 & 9.59 & 5.69 & 1.6969E+03 & Direct-PRF & 0\\
010661778-01 & 010661783-pri & 1:1 & 42.6 & -10 & 5 & 9.59 & 8.08 & 2.6958E+02 & Direct-PRF & 0\\
010661913-01 & 010661783-pri & 1:1 & 124.7 & 27 & 16 & 9.59 & 5.29 & 3.5306E+03 & Direct-PRF & 0\\
010661917-01 & 010661783-pri & 1:1 & 129.0 & 26 & 19 & 9.59 & 3.39 & 1.3681E+04 & Direct-PRF & 0\\
010662021-01 & 010661783-pri & 1:1 & 237.3 & 17 & 57 & 9.59 & 5.56 & 4.7587E+03 & Direct-PRF & 0\\
010676923-01 & 3830.01 & 1:1 & 10.8 & -2 & 2 & 17.02 & -1.89 & 1.1656E+03 & Direct-PRF & 0\\
010686814-01 & 010686876-01 & 1:1 & 56.1 & 14 & -3 & 11.73 & 3.87 & 8.2284E+02 & Direct-PRF & 0\\
010686930-01 & 010686876-01 & 1:1 & 61.3 & -15 & -4 & 11.73 & 0.66 & 5.1801E+03 & Direct-PRF & 0\\
010724372-01 & 010724533-pri & 1:1 & 188.2 & -10 & 46 & 9.04 & 5.58 & 6.7263E+03 & Direct-PRF & 0\\
010724379-01 & 010724533-pri & 1:1 & 195.8 & -2 & 49 & 9.04 & 6.32 & 3.6514E+03 & Direct-PRF & 0\\
010724450-01 & 010724533-pri & 1:1 & 206.4 & 26 & 45 & 9.04 & 4.56 & 1.2780E+04 & Direct-PRF & 0\\
010724544-01 & 010724533-pri & 1:1 & 88.7 & 20 & 11 & 9.04 & 5.97 & 1.7040E+03 & Direct-PRF & 0\\
010724551-01 & 010724533-pri & 1:1 & 179.6 & 40 & 22 & 9.04 & 6.84 & 3.9938E+03 & Direct-PRF & 0\\
010724569-01 & 010724533-pri & 1:1 & 112.7 & 27 & 10 & 9.04 & 6.45 & 1.5585E+03 & Direct-PRF & 0\\
010724619-01 & 010724533-pri & 1:1 & 108.3 & 27 & -4 & 9.04 & 6.25 & 4.7333E+03 & Direct-PRF & 0\\
010724621-01 & 010724533-pri & 1:1 & 152.9 & 39 & 3 & 9.04 & 5.58 & 3.4541E+03 & Direct-PRF & 0\\
010724635-01 & 010724533-pri & 1:1 & 84.7 & 16 & -15 & 9.04 & 5.51 & 3.8727E+03 & Direct-PRF & 0\\
010730571-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010732401-01 & V2083-Cyg-pri & 1:2 & 2277.7 & 573 & -1 & 6.90 & 7.84 & 3.5415E+03 & Direct-PRF & 0\\
010732407-01 & V2083-Cyg-pri & 1:2 & 2242.3 & 564 & -1 & 6.90 & 7.71 & 2.3894E+03 & Direct-PRF & 0\\
010736179-01 & V2290-Cyg-pri & 1:1 & 46.5 & 9 & 7 & 13.65 & 2.16 & 7.2631E+03 & Direct-PRF & 0\\
010743597-03 & 010743600-01 & 1:1 & 5.6 & 0 & -1 & 17.21 & -1.72 & 4.9254E+02 & Direct-PRF & 0\\
010747439-01 & 2673.01 & 1:1 & 5.8 & 1 & 1 & 16.44 & -1.99 & 3.8608E+01 & Direct-PRF & 0\\
010748393-01 & 010748390-01 & 1:1 & 11.0 & -2 & -2 & 9.17 & 6.22 & 3.4130E-01 & Direct-PRF & 0\\
010749745-01 & 010815379-pri & 1:1 & 80.2 & 20 & 3 & 11.24 & 2.80 & 2.8714E+03 & Direct-PRF & 0\\
010749766-01 & 010815379-pri & 1:1 & 59.9 & 15 & 3 & 11.24 & 3.40 & 2.2333E+03 & Direct-PRF & 0\\
010794405-01 & 010858720-pri & 1:1 & 22.8 & 1 & -6 & 10.97 & 3.74 & 3.8134E+03 & Direct-PRF & 0\\
010794509-01 & 010858720-pri & 1:1 & 169.4 & 43 & 0 & 10.97 & 1.65 & 3.4593E+04 & Direct-PRF & 0\\
010794509-02 & 010858720-sec & 1:1 & 169.4 & 43 & 0 & 10.97 & 1.65 & 2.2152E+04 & Direct-PRF & 0\\
010796473-01 & 010796477-pri & 2:1 & 22.6 & 6 & 1 & 14.11 & 0.91 & 6.5397E+03 & Direct-PRF & 0\\
010796473-02 & 010796477-pri & 2:1 & 22.6 & 6 & 1 & 14.11 & 0.91 & 6.8964E+03 & Direct-PRF & 0\\
010797123-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010801249-01 & 3617.01 & 1:1 & 498.2 & 125 & 0 & 14.57 & -1.20 & 7.0954E+03 & Col-Anomaly & 0\\
010801951-01 & V2290-Cyg-pri & 1:1 & 399.6 & 101 & 0 & 13.65 & 0.86 & 2.5070E+04 & Col-Anomaly & 0\\
010847907-01 & 010586874-pri & 1:1 & 2114.9 & 532 & 1 & 14.10 & -0.71 & 1.5439E+04 & Col-Anomaly & 0\\
010847907-02 & 010586874-sec & 1:1 & 2114.9 & 532 & 1 & 14.10 & -0.71 & 1.0684E+04 & Col-Anomaly & 0\\
010858737-01 & 010858720-sec & 1:1 & 88.3 & -14 & 17 & 10.97 & 2.57 & 2.3260E+04 & Direct-PRF & 0\\
010858737-02 & 010858720-pri & 1:1 & 88.3 & -14 & 17 & 10.97 & 2.57 & 1.5623E+04 & Direct-PRF & 0\\
010858785-01 & 010858720-pri & 1:1 & 74.4 & 4 & 18 & 10.97 & 4.90 & 6.2896E+03 & Direct-PRF & 0\\
010858785-02 & 010858720-sec & 1:1 & 74.4 & 4 & 18 & 10.97 & 4.90 & 6.2027E+03 & Direct-PRF & 0\\
010858803-01 & 010858720-pri & 1:1 & 91.1 & 9 & 21 & 10.97 & 4.64 & 4.0025E+03 & Direct-PRF & 0\\
010858803-02 & 010858720-sec & 1:1 & 91.1 & 9 & 21 & 10.97 & 4.64 & 3.9092E+03 & Direct-PRF & 0\\
010877024-01 & 010934755-pri & 1:1 & 382.1 & 96 & 0 & 14.40 & -0.89 & 2.2959E+04 & Col-Anomaly & 0\\
010877669-01 & 010877703-pri & 2:1 & 29.5 & 7 & -1 & 14.34 & 0.09 & 5.4576E+03 & Direct-PRF & 0\\
010879208-01 & 010879213-01 & 2:1 & 7.3 & 1 & 1 & 18.79 & -2.89 & 5.4577E+02 & Direct-PRF & 0\\
010919230-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010922610-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010924340-01 & 010924400-01 & 1:1 & 86.7 & 22 & -1 & 12.31 & 1.64 & 5.5000E-01 & Direct-PRF & 1\\
010924400-01 & 010924340-01 & 1:1 & 86.7 & -22 & 1 & 13.94 & -1.64 & 1.8182E+00 & Direct-PRF & 1\\
010924400-02 & 4326.01 & 1:1 & 86.7 & -22 & 1 & 13.94 & -1.64 & 9.3333E+00 & Direct-PRF & 1\\
010925113-01 & 010925104-01 & 1:1 & 6.2 & -1 & -1 & 13.74 & 1.27 & 5.3593E+00 & Direct-PRF & 0\\
010960993-01 & 3564.01 & 1:1 & 4.8 & -1 & 0 & 14.50 & -3.10 & 2.3647E+01 & Direct-PRF & 0\\
010972902-01 & 4673.01 & 1:1 & 1281.8 & -323 & 1 & 12.62 & 2.15 & 8.0645E-01 & Direct-PRF & 1\\
010979139-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010982884-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
010989166-01 & 009851142-pri & 1:1 & 7066.1 & 5 & 3 & 7.63 & 6.52 & 6.6716E+01 & Cross-Talk & 0\\
010992011-01 & 010991989-pri & 1:1 & 20.3 & -4 & 1 & 10.28 & 4.37 & 4.7120E+01 & Direct-PRF & 0\\
011017070-01 & 011017077-pri & 1:1 & 26.2 & -4 & -6 & 13.45 & 1.97 & 3.3706E+03 & Direct-PRF & 0\\
011017094-01 & 011017077-pri & 1:1 & 24.0 & -5 & 4 & 13.45 & 1.57 & 1.2733E+04 & Direct-PRF & 0\\
011044770-01 & 3327.01 & 1:1 & 11.0 & 2 & 0 & 15.47 & -2.09 & 1.0494E+02 & Direct-PRF & 0\\
011044770-02 & 011044779-02 & 1:1 & 11.0 & 2 & 0 & 15.47 & -2.09 & 9.5739E+01 & Direct-PRF & 0\\
011046870-01 & 1418.01 & 1:1 & 10.2 & 2 & 1 & 15.73 & -0.67 & 4.0215E+01 & Direct-PRF & 0\\
011076276-01 & 011076279-pri & 1:1 & 28.5 & -6 & 5 & 14.21 & 0.91 & 3.3290E+03 & Direct-PRF & 0\\
011080961-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011134682-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011137065-01 & V2083-Cyg-pri & 1:2 & 5482.1 & 677 & 0 & 6.90 & 7.91 & 2.3332E+03 & Col-Anomaly & 2\\
011137913-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011186929-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011200415-01 & 3724.01 & 1:1 & 7.6 & 1 & -1 & 16.80 & -4.75 & 3.1747E+02 & Direct-PRF & 0\\
011200767-01 & 011200773-01 & 1:1 & 6.3 & -2 & 1 & 13.67 & -0.30 & 8.2268E+00 & Direct-PRF & 0\\
011243547-01 & 011401845-pri & 1:1 & 1079.4 & 271 & 1 & 14.36 & 0.40 & 5.3506E+03 & Col-Anomaly & 0\\
011251058-01 & 011250867-01 & 1:1 & 226.8 & 57 & 1 & 13.39 & -0.21 & 5.5154E+03 & Col-Anomaly & 0\\
011303815-01 & 3744.01 & 1:1 & 10.0 & 1 & 2 & 15.77 & -0.50 & 9.0647E+01 & Direct-PRF & 0\\
011341314-01 & 011235323-pri & 1:2 & 866.0 & 218 & 0 & 13.49 & -0.69 & 7.7000E+03 & Col-Anomaly & 0\\
011401822-01 & 011401845-pri & 1:1 & 25.7 & -3 & 6 & 14.36 & 1.63 & 1.2523E+03 & Direct-PRF & 0\\
011401869-01 & 011401845-pri & 1:1 & 30.3 & 5 & -5 & 14.36 & 1.18 & 5.2152E+03 & Direct-PRF & 0\\
011446254-01 & 011904038-pri & 1:1 & 4120.9 & 755 & 0 & 12.78 & 2.53 & 7.1212E+01 & Col-Anomaly & 2\\
011454341-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011454525-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011455491-01 & 011455484-01 & 1:1 & 6.9 & 0 & -2 & 16.15 & -2.70 & 8.6159E+02 & Direct-PRF & 0\\
011455491-02 & 011455484-sec & 1:1 & 6.9 & 0 & -2 & 16.15 & -2.70 & 5.0256E+02 & Direct-PRF & 0\\
011456382-01 & 4845.01 & 1:1 & 21.0 & 0 & 5 & 15.37 & -3.62 & 2.1316E+00 & Direct-PRF & 1\\
011456405-01 & 2771.01 & 1:1 & 21.0 & 0 & -5 & 11.75 & 3.62 & 8.2963E+00 & Direct-PRF & 0\\
011502179-01 & 970.01 & 1:1 & 32.4 & 1 & -8 & 6.97 & 6.06 & 4.2312E+00 & Direct-PRF & 0\\
011516242-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011520793-01 & 011520787-01 & 1:2 & 8.2 & 0 & -2 & 14.00 & -4.23 & 2.0833E+01 & Direct-PRF & 0\\
011560382-01 & 011560447-pri & 1:1 & 99.0 & -22 & 12 & 10.83 & 4.52 & 3.1349E+03 & Direct-PRF & 0\\
011560431-01 & 011560447-pri & 1:1 & 43.1 & -11 & 0 & 10.83 & -1.14 & 7.9294E+03 & Direct-PRF & 0\\
011567149-01 & 011618883-sec & 1:1 & 72.8 & -14 & -11 & 13.38 & 0.78 & 6.7778E+03 & Direct-PRF & 0\\
011616596-01 & 011616594-pri & 1:2 & 28.4 & 4 & -6 & 11.17 & 1.45 & 4.3284E+03 & Direct-PRF & 0\\
011616631-01 & 011616594-pri & 1:2 & 50.2 & 12 & -2 & 11.17 & 4.68 & 2.0145E+03 & Direct-PRF & 0\\
011616663-01 & 011616594-pri & 1:2 & 63.0 & 14 & 8 & 11.17 & 3.80 & 3.3716E+03 & Direct-PRF & 0\\
011673674-01 & 011673686-pri & 1:1 & 16.5 & 4 & -1 & 11.69 & 1.97 & 7.8188E+00 & Direct-PRF & 0\\
011673674-02 & 011673686-pri & 1:2 & 16.5 & 4 & -1 & 11.69 & 1.97 & 3.9468E+02 & Direct-PRF & 0\\
011673686-02 & 133.01 & 1:2 & 16.5 & -4 & 1 & 13.65 & -1.97 & 4.0983E+00 & Direct-PRF & 1\\
011752908-01 & 253.01 & 1:1 & 5.1 & 1 & 1 & 15.25 & 0.30 & 2.6813E+00 & Direct-PRF & 0\\
011824218-01 & 437.01 & 1:1 & 6.3 & 2 & 0 & 14.50 & -0.77 & 1.3767E+01 & Direct-PRF & 0\\
011855538-01 & 012004679-pri & 1:2 & 1115.0 & 280 & 1 & 13.23 & -1.00 & 1.3217E+04 & Col-Anomaly & 0\\
011858748-01 & 011858741-01 & 1:1 & 11.6 & -3 & 0 & 16.48 & -0.97 & 7.0648E+02 & Direct-PRF & 0\\
011869257-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
011872139-01 & 011922782-pri & 1:2 & 609.0 & 153 & 2 & 10.46 & 2.85 & 7.7267E+03 & Col-Anomaly & 0\\
011873171-01 & 011873166-pri & 1:2 & 26.1 & -4 & -4 & 13.47 & 2.12 & 1.8059E+03 & Direct-PRF & 0\\
011911580-01 & 003644542-01 & 3:1 & 41461.2 & -18 & 44 & 8.35 & 5.55 & 2.4046E+02 & Reflection & 0\\
011911580-02 & 3511.01 & 3:1 & 41461.2 & -18 & 44 & 8.35 & 5.55 & 2.8076E+02 & Reflection & 0\\
011912911-01 & 011913071-pri & 1:1 & 255.6 & 54 & 35 & 9.53 & 5.99 & 1.3593E+03 & Direct-PRF & 0\\
011912916-01 & 011913071-pri & 1:1 & 236.0 & 44 & 39 & 9.53 & 6.29 & 7.8636E+02 & Direct-PRF & 0\\
011912932-01 & 011913071-pri & 1:1 & 209.5 & 37 & 37 & 9.53 & 4.79 & 2.1874E+03 & Direct-PRF & 0\\
011912941-01 & 011913071-pri & 1:1 & 189.7 & 28 & 38 & 9.53 & 5.60 & 1.6127E+03 & Direct-PRF & 0\\
011912987-01 & 011913071-pri & 1:1 & 122.5 & 17 & 26 & 9.53 & 4.04 & 2.5716E+03 & Direct-PRF & 0\\
011913012-01 & 011913071-pri & 1:1 & 90.4 & 15 & 17 & 9.53 & 5.23 & 5.4684E+02 & Direct-PRF & 0\\
011913012-02 & 011913071-sec & 1:1 & 90.4 & 15 & 17 & 9.53 & 5.23 & 7.5968E+02 & Direct-PRF & 0\\
011913013-01 & 011913071-pri & 1:1 & 91.7 & 17 & 15 & 9.53 & 7.91 & 3.9945E+01 & Direct-PRF & 0\\
011913013-02 & 011913071-sec & 1:1 & 91.7 & 17 & 15 & 9.53 & 7.91 & 6.1892E+01 & Direct-PRF & 0\\
011913052-01 & 011913071-pri & 1:1 & 103.7 & 25 & -5 & 9.53 & 4.31 & 1.5347E+03 & Direct-PRF & 0\\
011913072-01 & 011913071-pri & 1:1 & 102.6 & -22 & 14 & 9.53 & 4.88 & 2.6431E+03 & Direct-PRF & 0\\
011913073-01 & 011913071-pri & 1:1 & 34.9 & 7 & -5 & 9.53 & 3.96 & 2.9504E+02 & Direct-PRF & 0\\
011922648-01 & 011922782-pri & 1:2 & 158.8 & 40 & 3 & 10.46 & 4.07 & 2.9718E+03 & Direct-PRF & 0\\
011922678-01 & 011922782-pri & 1:2 & 106.3 & 20 & -18 & 10.46 & 3.05 & 3.7387E+03 & Direct-PRF & 0\\
011922722-01 & 011922782-pri & 1:2 & 76.8 & 5 & -18 & 10.46 & 3.30 & 2.3414E+03 & Direct-PRF & 0\\
011968514-01 & 3587.01 & 1:1 & 8.4 & 1 & -2 & 14.44 & -2.99 & 3.4221E+02 & Direct-PRF & 0\\
012004680-01 & 012004679-pri & 1:2 & 38.7 & 8 & 5 & 13.23 & 2.07 & 4.1304E+03 & Direct-PRF & 0\\
012004689-01 & 012004679-pri & 1:2 & 57.6 & 13 & 6 & 13.23 & 2.66 & 2.2456E+03 & Direct-PRF & 0\\
012023078-01 & 012023089-01 & 1:1 & 9.8 & 1 & -2 & 15.63 & -2.98 & 4.3732E+02 & Direct-PRF & 0\\
012062667-01 & 3746.01 & 1:1 & 6.8 & 1 & -2 & 17.38 & -4.71 & 4.6402E+02 & Direct-PRF & 0\\
012066629-01 & 012066630-pri & 1:1 & 42.3 & -5 & 10 & 11.01 & 4.06 & 1.0744E+03 & Direct-PRF & 0\\
012066629-02 & 012066630-sec & 1:1 & 42.3 & -5 & 10 & 11.01 & 4.06 & 1.0561E+03 & Direct-PRF & 0\\
012071037-01 & 012071006-pri & 1:1 & 30.7 & -6 & 6 & 13.53 & 0.57 & 7.0984E+03 & Direct-PRF & 0\\
012106875-01 & 3895.01 & 1:1 & 96.3 & -5 & -23 & 18.36 & -2.98 & 2.8319E+02 & Direct-PRF & 1\\
012106929-01 & 3895.01 & 1:1 & 12.0 & -1 & -2 & 18.36 & -4.56 & 1.0440E+02 & Direct-PRF & 1\\
012106934-01 & 359.01 & 1:1 & 12.0 & 1 & 2 & 13.80 & 4.56 & 1.8762E-02 & Direct-PRF & 1\\
012107008-01 & 3895.01 & 1:1 & 96.9 & -22 & 10 & 18.36 & -3.66 & 4.2745E+02 & Direct-PRF & 1\\
012107021-01 & 3895.01 & 1:1 & 121.0 & 2 & 31 & 18.36 & -5.34 & 2.1889E+02 & Direct-PRF & 1\\
012108293-01 & 012108333-pri & 1:1 & 50.3 & -1 & 13 & 13.23 & 1.61 & 1.3704E+04 & Direct-PRF & 0\\
012108293-02 & 012108333-sec & 1:1 & 50.3 & -1 & 13 & 13.23 & 1.61 & 9.2548E+03 & Direct-PRF & 0\\
012108312-01 & 012108333-pri & 1:1 & 21.4 & -1 & 5 & 13.23 & 1.12 & 4.6882E+03 & Direct-PRF & 0\\
012108364-01 & 012108333-pri & 1:1 & 52.4 & -1 & -13 & 13.23 & 2.60 & 1.4914E+02 & Direct-PRF & 0\\
012109421-01 & 012157987-pri & 1:1 & 67.5 & 1 & 17 & 12.21 & 1.25 & 7.4286E+03 & Direct-PRF & 0\\
012117945-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
012157971-01 & 012157987-pri & 1:1 & 26.5 & -1 & 7 & 12.21 & 1.45 & 3.4098E+03 & Direct-PRF & 0\\
012157983-01 & 012157987-pri & 1:1 & 25.1 & 6 & -1 & 12.21 & 1.56 & 2.1443E+03 & Direct-PRF & 0\\
012158032-01 & 012157987-pri & 1:1 & 61.9 & -8 & -13 & 12.21 & 3.70 & 1.8087E+03 & Direct-PRF & 0\\
012164770-01 & 012164751-pri & 1:1 & 20.6 & 5 & 1 & 14.19 & 0.46 & 2.5705E+03 & Direct-PRF & 0\\
012218917-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
012257851-01 & 012257908-pri & 1:2 & 99.2 & -2 & 25 & 10.43 & 4.94 & 2.2250E+03 & Direct-PRF & 0\\
012257886-01 & 012257908-pri & 1:1 & 53.4 & -4 & 12 & 10.43 & 4.75 & 1.0430E+03 & Direct-PRF & 0\\
012267759-01 & 012267718-sec & 1:1 & 37.8 & -7 & 6 & 13.38 & -0.09 & 2.6720E+05 & Direct-PRF & 0\\
012316431-01 & 3575.01 & 1:1 & 14.4 & 4 & 0 & 16.11 & -1.94 & 2.9210E+02 & Direct-PRF & 0\\
012353501-01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
012353633-01 & 012554536-pri & 1:1 & 1587.3 & 399 & 0 & 12.82 & 0.36 & 1.6930E+04 & Col-Anomaly & 0\\
012404890-02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & Systematic & 0\\
012418795-01 & 012418816-pri & 1:2 & 63.8 & 12 & 10 & 12.40 & 1.24 & 9.4051E+03 & Direct-PRF & 0\\
012418891-01 & 012418816-pri & 1:2 & 73.4 & -11 & 15 & 12.40 & 3.45 & 3.0314E+03 & Direct-PRF & 0\\
012506342-01 & 012506351-pri & 1:2 & 15.9 & 0 & 4 & 13.18 & 2.53 & 1.7516E+02 & Direct-PRF & 0\\
012554510-01 & 012554536-pri & 1:1 & 45.3 & -6 & 9 & 12.82 & 0.84 & 3.0782E+04 & Direct-PRF & 0\\
012643589-01 & 3626.01 & 1:1 & 7.5 & -1 & 2 & 16.44 & -2.69 & 6.1460E+01 & Direct-PRF & 0\\
012644774-01 & 1611.01 & 10:1 & 16.1 & -3 & -3 & 11.76 & 3.14 & 2.0434E+01 & Direct-PRF & 0\\
012644774-02 & 1611.01 & 10:1 & 16.1 & -3 & -3 & 11.76 & 3.14 & 2.0122E+01 & Direct-PRF & 0\\
012644774-03 & 1611.01 & 10:1 & 16.1 & -3 & -3 & 11.76 & 3.14 & 2.0766E+01 & Direct-PRF & 0\\
012644774-04 & 1611.01 & 2:1 & 16.1 & -3 & -3 & 11.76 & 3.14 & 1.0905E+02 & Direct-PRF & 0\\
\nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata\\

==> robodisps-full.tex <==
000757450-01 & 0889.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
000892667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
000892772-01 & 1009.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
001026032-01 & 6252.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
001026032-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
001026133-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001026133-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001026957-01 & 0958.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
001028018-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001160891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001160891-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001160891-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001161345-01 & 0984.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
001162150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
001162150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001162150-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001162345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001162345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001162345-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF\\
001164109-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
001292087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
001292087-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001293031-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001293031-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001293379-01 & 6253.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
001294670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001294670-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001294756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001295289-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
001295546-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
001295546-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
001296164-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
001296164-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
001296164-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001296721-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
001429120-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001429120-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001429589-01 & 4923.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001429653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
001429653-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
001430207-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
001430590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001430590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001430741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001430741-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001431122-01 & 0994.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
001431794-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001431794-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001431794-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001432149-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001432214-01 & 0998.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
001432214-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
001432789-01 & 0992.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001432789-02 & 0992.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
001433399-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001433399-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001433399-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001433531-01 & 6254.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
001433899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
001433962-01 & 0982.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
001433980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001433980-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001433980-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001434660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
001434660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001434800-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
001434800-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
001434800-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
001570924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
001571088-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001571511-01 & 0362.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
001571511-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
001571717-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001571717-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001572948-01 & 4924.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
001573174-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001573174-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001574792-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001575690-01 & 3658.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
001575873-01 & 4359.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
001575977-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001575977-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001575977-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
001576115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001576115-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001576115-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001576115-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
001576141-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
001576144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001576144-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001576144-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
001576144-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001576144-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
001576558-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
001577039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001577039-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001577039-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001577039-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001577912-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001577912-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001717528-01 & 6255.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
001717722-01 & 3145.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
001717722-02 & 3145.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
001718189-01 & 0993.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001718189-02 & 0993.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
001718189-03 & 0993.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
001718290-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001718290-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001718290-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001718594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001718594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001718594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001718958-01 & 4053.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001719308-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
001720673-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
001721157-01 & 4644.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001721361-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
001721795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001724222-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001724222-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001724513-01 & 4224.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
001724719-01 & 4212.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001724719-02 & 4212.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
001724961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001724961-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001724961-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001725016-01 & 1007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001725193-01 & 4925.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
001849235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001849235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001849235-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
001849555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001849702-01 & 2538.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001865042-01 & 1002.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001865567-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001865567-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001865567-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001866252-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
001867078-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
001867630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001868918-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
001869607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001869607-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001870398-01 & 4927.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001870849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001870849-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001870849-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
001870849-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
001871056-01 & 1001.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001871056-02 & 1001.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
001871483-01 & 6256.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
001872262-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
001872262-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
001872821-01 & 2351.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001872948-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
001872948-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001872948-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
001873030-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
001873513-01 & 4928.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
001995519-01 & 2634.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001995732-01 & 3351.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
001995732-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
001996180-01 & 2534.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
001996180-02 & 2534.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
001996456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
001996679-01 & 0147.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
001996679-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
001996773-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002010191-01 & 3999.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002010414-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002010414-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002010414-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002010414-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002010607-01 & 4929.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
002011424-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002011424-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002011424-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002012722-01 & 6257.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002012722-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002013883-01 & 6258.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
002014991-01 & 2178.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002015013-01 & 4930.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002016979-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
002016979-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
002018261-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002018685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002018685-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002018685-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002018906-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
002019076-01 & 3585.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
002019227-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
002019297-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002019477-01 & 6093.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002019477-02 & 6093.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002019477-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
002019477-04 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
002020444-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002021099-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
002021100-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002021100-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
002021440-01 & 1987.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
002021440-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
002140360-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002141783-01 & 2201.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002141938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002141938-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002142522-01 & 2403.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002156514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002157247-01 & \nodata & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
002157247-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
002157489-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002157489-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002158190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002158208-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
002158208-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002158208-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002159700-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
002159852-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002159852-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002159852-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002159852-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
002161536-01 & 2130.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002161623-01 & 6094.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002161623-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002161949-01 & 6259.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002161949-02 & 6259.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002162635-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002162635-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
002162904-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
002162904-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002162904-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002162994-01 & 6260.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
002163326-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002164165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
002164169-01 & 1029.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002164726-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002164884-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
002165002-01 & 0999.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002165002-02 & 0999.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002165188-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002165352-01 & 4934.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
002166200-01 & 3735.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002166206-01 & 1028.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3735.01\\
002166218-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
002166218-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002167183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
002167444-01 & 6261.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002167600-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002167600-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002167600-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002167783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002167783-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002167890-01 & 3670.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
002167890-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
002168333-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
002168333-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002168333-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002168420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002168420-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
002282763-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002282763-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002282763-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002283124-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002283124-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002283124-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002283362-01 & 6262.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002283362-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002297728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002297728-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002297729-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002297739-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
002297739-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
002297793-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002300319-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002300529-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002300529-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002300529-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002300603-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002300603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002300603-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002300603-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002301068-01 & 6263.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002302548-01 & 0988.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002302548-02 & 0988.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002303102-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002303304-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002303365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002303365-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002303365-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002303903-01 & 4709.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
002304168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002304168-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002304235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
002304235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002304235-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002304320-01 & 2033.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002304566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002304655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002305255-01 & 4935.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002305311-01 & 4434.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_002305372-pri\\
002305372-01 & 6264.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
002305543-01 & 4936.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002305866-01 & 2610.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002305866-02 & 2610.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002305866-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002305866-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002306740-01 & 6265.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002306740-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002306740-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
002307197-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002307199-01 & 0151.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002307199-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE\\
002307206-01 & 3549.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002307206-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002307415-01 & 2053.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002307415-02 & 2053.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002307533-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002307533-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002307533-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002308603-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002308957-01 & 6266.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
002309568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
002309568-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002309579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002309579-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002309585-01 & 1004.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED---PARENT\_IS\_5982.01\\
002309587-01 & 5982.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002309587-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002309719-01 & 1020.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002309910-01 & 4937.01 & FP & 1 & 0 & 1 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
002310284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002310284-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002310586-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002422539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
002422820-01 & 6267.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
002436378-01 & 2682.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
002436421-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002436635-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002437060-01 & 3712.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
002437112-01 & 3461.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3598.01\\
002437112-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3598.01\\
002437112-03 & 3461.02 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3712.01\\
002437149-01 & 3598.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002437149-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002437340-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002437452-01 & 6268.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
002437488-01 & 3920.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_002437452-pri\\
002437488-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_002437452-01\\
002437505-01 & 2671.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002437505-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
002437762-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
002437783-01 & 3745.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002437783-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002437804-01 & 6269.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_002437783-01\\
002437897-01 & 4909.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002438061-01 & 6270.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
002438062-01 & 6271.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_002438061-01\\
002438070-01 & 0363.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_002438061-01\\
002438249-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002438264-01 & 0440.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002438264-02 & 0440.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002438490-01 & 3699.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
002438490-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
002438502-01 & 1003.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
002438502-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
002438513-01 & 1944.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002438517-01 & 6272.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3699.01\\
002439211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002439211-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002439243-01 & 2280.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002439469-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002439660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002439798-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002440757-01 & 0792.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002440757-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002441151-01 & 0603.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_002441161-01\\
002441161-01 & 3642.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
002441470-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
002441495-01 & 0166.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002441728-01 & 1000.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002442084-01 & 6273.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002442084-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002442118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002442118-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002442359-01 & 3997.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002442448-01 & 2812.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002442551-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002443393-01 & 2603.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002443753-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002444412-01 & 0103.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002444769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002445129-01 & 0793.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
002445129-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
002445134-01 & 5983.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002445134-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
002445154-01 & 1023.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5983.01\\
002445298-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002445975-01 & 0053.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002445975-02 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
002445975-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
002446113-01 & 0379.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002446113-02 & 0379.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002446623-01 & 3674.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002447832-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002447832-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002448113-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002448307-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002449053-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_002449084-pri\\
002449074-01 & 0378.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_002449090-01\\
002449074-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_002449090-02\\
002449090-01 & 3702.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002449090-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002449101-01 & 4236.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_002449084-pri\\
002449245-01 & 6274.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002449383-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002449431-01 & 2009.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002450716-01 & 6275.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
002450944-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
002451696-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002452185-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002452289-01 & 4942.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002452440-01 & 3687.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
002452440-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
002452450-01 & 0380.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3687.01\\
002452450-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_002452440-02\\
002452920-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002554853-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002554853-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
002554867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002554867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002554867-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002556639-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
002556650-01 & 2156.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002557335-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
002557335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
002557350-01 & 6276.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002557430-01 & 6277.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
002557555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002557816-01 & 0488.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002558163-01 & 4655.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002558363-01 & 1021.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3855.01\\
002558370-01 & 3855.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002558488-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002568519-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002568971-01 & 6278.01 & FP & 0 & 1 & 1 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
002568971-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
002568971-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE\\
002568971-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
002569488-01 & 4944.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3704.01\\
002569494-01 & 3704.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---KIC\_OFFSET\\
002569516-01 & 4945.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002570281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002570281-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002570432-01 & 4946.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---KIC\_OFFSET---PARENT\_IS\_002708156-01\\
002570505-01 & 6279.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_UZ-Lyr-pri\\
002570760-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002570767-01 & 6280.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CROWDED\_DIFF---PARENT\_IS\_UZ-Lyr-pri\\
002570773-01 & 4376.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_UZ-Lyr-pri\\
002571075-01 & 6281.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_UZ-Lyr-pri\\
002571238-01 & 0084.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002571417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002571417-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002571417-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002571417-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
002571868-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002571868-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002571868-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002572029-01 & 4581.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002573056-01 & 2648.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002574201-01 & 1025.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002574338-01 & 1030.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002574543-01 & 4947.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
002574960-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002574960-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002575161-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002575952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002575964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002575964-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
002575964-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
002576107-01 & 3709.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
002576197-01 & 0489.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002576224-01 & 4465.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_489.01\\
002576224-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
002576692-01 & 6282.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002576692-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002577952-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_002714932-02\\
002578072-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_002715113-01\\
002578077-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
002578077-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002578404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002578404-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002578404-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
002578811-01 & 4948.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002578891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002578901-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
002578901-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
002578901-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
002579043-01 & 2064.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002579147-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002579147-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002579147-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002579147-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
002579814-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002579906-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002580613-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002580872-01 & 6283.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002580872-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002580872-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002580882-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
002581191-01 & 2203.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002581316-01 & 3681.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002581316-02 & 3681.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002581452-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
002581457-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
002581457-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002581457-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002581554-01 & 3835.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002581674-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002581674-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002581674-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002582539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002582800-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002583153-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002583153-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002583234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002583234-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
002583667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002583669-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
002583777-01 & 6284.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
002583777-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002584115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002584118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002584163-01 & 1031.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002584879-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002584879-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002584908-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
002585092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002585092-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002585092-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002585092-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002692377-01 & 0299.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002692377-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
002692377-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
002693092-01 & 6285.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
002693092-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
002693097-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002693097-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002693097-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002693450-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002693450-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002693736-01 & 1976.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002694337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002694337-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002695030-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002695030-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002695110-01 & 0400.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002696703-01 & 3161.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
002696938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
002697935-01 & 3853.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
002706947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002707097-01 & 6095.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
002707479-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002707479-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002707479-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002707916-01 & 4950.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_UZ-Lyr-pri\\
002707985-01 & 3253.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_UZ-Lyr-pri\\
002708156-01 & 6286.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
002708156-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
002708172-01 & 6287.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_UZ-Lyr-pri\\
002708176-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_UZ-Lyr-pri\\
002708203-01 & 4045.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CROWDED\_DIFF---PARENT\_IS\_UZ-Lyr-pri\\
002708221-01 & 4352.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_UZ-Lyr-pri\\
002708270-01 & 4951.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_UZ-Lyr-pri\\
002708270-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
002708278-01 & 4102.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_UZ-Lyr-pri\\
002708286-01 & 4071.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_UZ-Lyr-pri\\
002708343-01 & 4111.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_UZ-Lyr-pri\\
002708420-01 & 4003.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_UZ-Lyr-pri\\
002708445-01 & 6288.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_UZ-Lyr-pri\\
002708614-01 & 6289.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
002708787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
002708885-01 & 2907.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002710327-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002710406-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002710406-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002710406-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002710623-01 & 4532.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
002711114-01 & 6290.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002711123-01 & 4953.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_002711114-pri\\
002711123-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_002711114-01\\
002711597-01 & 4746.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
002711597-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002711606-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_003339563-pri\\
002712582-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002712821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002713049-01 & 0794.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002714707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002714707-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002714707-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002714807-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002714831-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002714887-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_002714932-02\\
002714932-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_002715245-01\\
002714932-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_002714887-01\\
002714947-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_002715113-01\\
002714954-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_002714932-02\\
002714955-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002715053-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_002715245-01\\
002715113-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_002715119-01\\
002715119-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_002715113-01\\
002715135-01 & 1024.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002715135-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_002715398-01\\
002715228-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_002715245-01\\
002715245-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_002715228-01\\
002715282-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_002715119-01\\
002715398-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_002715135-02\\
002715487-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002715487-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002715695-01 & 3077.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
002715695-02 & 3077.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002716801-01 & 3053.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002716801-02 & 3053.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
002716853-01 & 1022.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002716979-01 & 6291.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002717158-01 & 3459.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002717483-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002717483-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002717483-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002718630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002718630-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002718630-03 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002718672-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002718778-01 & 2489.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002718944-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002718944-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CENTROID\_SIGNIF\_UNCERTAIN\\
002719125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002719125-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002719436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
002719873-01 & 6096.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002719873-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002719928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002719928-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002719928-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002720354-01 & 6292.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002720354-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002720354-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
002720514-01 & 2979.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002720582-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002720582-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002720582-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
002720594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
002720594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002720594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
002720828-01 & 4669.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002721030-01 & 1094.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002721129-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002721129-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---TOO\_FEW\_QUARTERS\\
002721835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002722074-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
002830919-01 & 4387.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_003836439-pri\\
002831048-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002831055-01 & 4400.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002831097-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002831251-01 & 4702.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002832589-01 & 1942.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002832753-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002832753-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002833554-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002833554-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002834463-01 & 6293.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002835657-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002837111-01 & 1110.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002837111-02 & 1110.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002846358-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
002846358-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002846358-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002847816-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
002849140-01 & 3416.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002849805-01 & 1116.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002850321-01 & 4956.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002851014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
002851100-01 & 1104.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
002851100-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
002852528-01 & 3446.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_002852560-01\\
002852560-01 & 6294.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
002852560-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002852560-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
002852560-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
002852810-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
002852941-01 & 4298.02 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002852941-02 & 4298.01 & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
002853029-01 & 3259.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002853093-01 & 1099.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002853280-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002853280-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002853280-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002853280-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002853280-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002853320-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002853320-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002853320-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002853320-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
002853446-01 & 1118.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002853780-01 & 2081.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002853828-01 & 2896.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002853828-02 & 2896.02 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002853889-01 & 4604.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002854181-01 & 2232.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002854181-02 & 2232.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002854698-01 & 0986.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002854698-02 & 0986.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002854914-01 & 1113.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002854914-02 & 1113.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002854927-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CENTROID\_SIGNIF\_UNCERTAIN\\
002854948-01 & 3786.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
002854953-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002854953-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002854953-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
002855415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002855603-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002855603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002855680-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002855680-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002856756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002856756-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002856756-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002856960-01 & 6295.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002857323-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002857323-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002857607-01 & 4659.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002857722-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---LARGE\_RM\\
002857722-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
002857722-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
002858134-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002859299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002859299-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
002860114-01 & 2170.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
002860594-01 & 6296.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002860594-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002860594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002860594-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002860656-01 & 4857.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002860788-01 & 6297.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
002860793-01 & 2277.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_002860788-01\\
002860793-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
002860851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002860851-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002860866-01 & 1103.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002860930-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002861126-01 & 4957.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
002864938-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002969628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002969628-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_002969638-01\\
002969628-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002969638-01 & 6298.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002969638-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002969991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002969991-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002970670-01 & 6299.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002970804-01 & 3993.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
002970804-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
002970836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002970836-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002971415-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
002971415-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002971415-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
002972005-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002972005-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002973386-01 & 3034.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002973509-01 & 6300.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002973509-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
002973800-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002974815-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002974858-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
002975770-01 & 1788.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002975770-02 & 1788.02 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL\\
002975832-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002975832-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002976017-01 & 4849.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002984505-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002985022-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002985022-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002985022-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
002985054-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002985396-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
002985396-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
002985398-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002985398-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002985587-01 & 2807.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002985767-01 & 2032.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002986506-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
002986833-01 & 4875.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002987027-01 & 0197.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002987433-01 & 4959.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
002987660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002987660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
002988145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
002988145-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
002988145-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002988768-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
002988783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002989404-01 & 1824.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002989404-02 & 1824.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
002989706-01 & 2692.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002990873-01 & 2335.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002992648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002992648-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002992648-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002993038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
002993589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002993589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002994092-01 & 6301.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002994888-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002994888-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
002995392-01 & 3379.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
002995823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
002995823-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
002995931-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002996015-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
002996015-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
002997178-01 & 3814.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
002997455-01 & 6098.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
002997455-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
002997459-01 & 4389.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
002998070-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
002998070-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
002998124-01 & 6302.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
002998124-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
002998561-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
002998561-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003001885-01 & 2540.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003002336-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003002478-01 & 2380.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003003019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003003991-01 & 6099.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
003003992-01 & 1119.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---SATURATED---PARENT\_IS\_6099.01\\
003003992-02 & 1119.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003097346-01 & 0264.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3648.01\\
003097352-01 & 3648.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_CENTROIDS\\
003097352-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
003097912-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
003097912-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003097926-01 & 2186.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003098015-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003098015-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003098015-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003098184-01 & \nodata & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_6:1---CLEAR\_APO---PARENT\_IS\_003098194-02\\
003098184-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003098194-01\\
003098184-03 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003098194-02\\
003098184-04 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_003098194-02\\
003098184-05 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003098194-01\\
003098194-01 & 6303.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
003098194-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
003098194-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003098194-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003098197-01 & 3362.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_003098194-02\\
003098197-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003098194-01\\
003098605-01 & 4844.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003098810-01 & 1878.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003098843-01 & 3376.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003101178-01 & 4963.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003101923-01 & 3483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003102000-01 & 3373.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003102000-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003102024-01 & 6304.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
003102024-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
003102384-01 & 0273.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003103212-01 & 4145.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003103227-01 & 4091.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003103473-01 & 4395.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003109550-01 & 3225.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003109924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003109930-01 & 1112.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003109937-01 & 4720.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_1112.01\\
003110937-01 & 6305.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_UZ-Lyr-pri\\
003112129-01 & 4144.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003112129-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003113266-01 & 1088.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003113266-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003114167-01 & 0795.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003114661-01 & 0796.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3763.01\\
003114667-01 & 3763.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
003114811-01 & 1117.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003115272-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003115435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003115480-01 & 6306.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
003115728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003115728-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003115728-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003115833-01 & 0797.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003116412-01 & 1115.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
003116989-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003117510-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_003117511-01\\
003117510-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
003117511-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003117511-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
003117514-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003118797-01 & 1950.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003119256-01 & 2784.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003119256-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003119256-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003119307-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_003119295-pri\\
003119307-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003119604-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003119604-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003120057-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003120057-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003120057-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003120276-01 & 1111.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003120320-01\\
003120308-01 & 3380.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003120320-01\\
003120320-01 & 6307.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
003120355-01 & 2099.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003120397-01 & 4965.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003120320-01\\
003120431-01 & 0798.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003120650-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003120889-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
003120889-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003120889-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003120904-01 & 3277.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003121340-01 & 3945.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003121407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003122188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003122188-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003122872-01 & 3203.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003122913-01 & 2490.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003122985-01 & 1949.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
003123418-01 & 7542.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
003124598-01 & 4187.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003127817-01 & 6308.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
003128325-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003128325-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
003128552-01 & 2055.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003128552-02 & 2055.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003128552-03 & 2055.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003128793-01 & 1786.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003128853-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003130300-01 & 1105.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003130548-01 & 2773.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003130548-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003216518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003216518-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003216518-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
003216838-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003217264-01 & 0401.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003217264-02 & 0401.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003217264-03 & 0401.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003217554-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003217554-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003217554-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003217554-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003218308-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003218637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003218688-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_003218683-pri\\
003218908-01 & 1108.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003218908-02 & 1108.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003218908-03 & 1108.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003219037-01 & 3395.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003219037-02 & 3395.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003219256-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003219256-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003219643-01 & 3072.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003219995-01 & 2314.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003221077-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003221272-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
003221310-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003222104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003222183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
003222183-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003222183-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003222680-01 & 4966.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003223460-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003228740-01 & 6309.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V404-Lyr-pri\\
003228804-01 & 3996.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_V404-Lyr-pri\\
003228824-01 & 1100.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V404-Lyr-pri\\
003228825-01 & 4055.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V404-Lyr-pri\\
003228918-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_V404-Lyr-pri\\
003228945-01 & 2917.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_V404-Lyr-pri\\
003228959-01 & 1107.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---CLEAR\_APO\\
003228959-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
003228986-01 & 4031.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_V404-Lyr-pri\\
003228988-01 & 3992.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_V404-Lyr-pri\\
003229028-01 & 6100.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V404-Lyr-pri\\
003229150-01 & 2150.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003229150-02 & 2150.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003230206-01 & 6310.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003230227-pri\\
003230227-01 & 6311.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003230227-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED---PARENT\_IS\_965.01\\
003230578-01 & 0381.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003230578-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003230578-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003230578-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003230753-01 & 2928.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_6101.01\\
003230787-01 & 6101.01 & PC & 0 & 0 & 0 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT\\
003230805-01 & 3068.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003230805-02 & 3068.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003231120-01 & 3643.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
003231120-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
003231137-01 & 0382.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3643.01\\
003231137-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3643.01\\
003231341-01 & 1102.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003231341-02 & 1102.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003231341-03 & 1102.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003231341-04 & 1102.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
003231406-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_003231410-03\\
003231406-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003231406-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003231406-04 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_003231410-01\\
003231410-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_003231406-04\\
003231410-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003231410-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED---PARENT\_IS\_003231406-01\\
003231950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003232859-01 & 1090.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003232859-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003233043-01 & 0966.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
003233043-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003233302-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003233302-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003234598-01 & 2413.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003234598-02 & 2413.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003234843-01 & 3057.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003234843-02 & 3057.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003236705-01 & 3343.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003238010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003238059-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003238073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003238073-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003238245-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003238245-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003238686-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003238787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
003239171-01 & 4967.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003239636-01 & 1093.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
003239671-01 & 2066.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003239926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003239945-01 & 0490.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003239945-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
003239945-03 & 0490.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003239945-04 & 0490.04 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
003240049-01 & 4968.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003240158-01 & 1106.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003240158-02 & 1106.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003240158-03 & 1106.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003240159-01 & 3515.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003240231-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003240231-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003240406-01 & 3185.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003240406-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003240411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003240411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003240411-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003240556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003240556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003240556-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003240556-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003240556-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003240706-01 & 1098.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003240706-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003241199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003241199-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003241199-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003241248-01 & 4141.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003241248-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003241344-01 & 5984.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003241344-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003241557-01 & 2863.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_003241619-01\\
003241604-01 & 2824.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_003241619-01\\
003241619-01 & 6312.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
003241619-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003241662-01 & 6313.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_003241619-01\\
003241685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003241685-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003244792-01 & 4347.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003245000-01 & 6314.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003245420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003245420-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003245420-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003245638-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003245969-01 & 1101.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003246083-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003246083-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
003246782-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---LARGE\_RM\\
003246867-01 & 6315.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003246890-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
003246890-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003246890-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003246890-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003246890-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003246984-01 & 0799.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
003246984-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
003246984-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
003247039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003247039-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003247268-01 & 1089.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003247268-02 & 1089.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003247294-01 & 6316.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003247294-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
003247306-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003247306-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003247396-01 & 0121.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_4035.01\\
003247404-01 & 4035.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003247503-01 & 4397.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003247503-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003247616-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003247616-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003247616-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003248019-01 & 1759.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003248019-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
003248033-01 & 0006.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1759.01\\
003248332-01 & 6317.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
003248501-01 & 2052.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003249334-01 & 6318.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003323168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003323168-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003323289-01 & 6319.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
003323289-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
003323887-01 & 0377.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
003323887-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003324069-01 & 6320.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003324644-01 & 3781.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003324644-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003324986-01 & 3084.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_003836439-pri\\
003326377-01 & 1830.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003326377-02 & 1830.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003326428-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003326428-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003326428-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003326428-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
003327980-01 & 6321.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
003327992-01 & 3635.01 & FP & 0 & 1 & 1 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003327980-pri\\
003327992-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
003327993-01 & 2157.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_003327980-pri\\
003328026-01 & 1994.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003327980-pri\\
003328027-01 & 4174.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003327980-pri\\
003328052-01 & 3011.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---LARGE\_RM---PARENT\_IS\_003327980-pri\\
003328080-01 & 3075.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003329204-01 & 1095.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003329643-01 & 6322.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_003431321-pri\\
003329839-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003330684-01 & 4533.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003330688-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003335813-01 & 3632.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003335816-01\\
003335816-01 & 6323.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
003336055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003336283-01 & 2974.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
003336283-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003336283-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003336283-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003336476-01 & 3247.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_UZ-Lyr-pri\\
003336765-01 & 2740.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
003336845-01 & 4275.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003336845-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003336937-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003337002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003337002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003337061-01 & 3172.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
003337351-01 & 0965.01 & FP & 0 & 1 & 1 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003230227-pri\\
003337351-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_003230227-pri\\
003337351-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
003337351-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003337425-01 & 1114.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003230227-pri\\
003337432-01 & 2265.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_003439031-01\\
003337438-01 & 6324.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003439031-01\\
003337548-01 & 6325.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_003439031-01\\
003338608-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003338608-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003338608-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003338660-01 & 3795.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
003338674-01 & 3796.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3795.01\\
003338680-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003338885-01 & 1845.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003338885-02 & 1845.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003339538-01 & 6326.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003339823-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003340165-01 & 4972.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003340312-01 & 0441.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3677.01\\
003340313-01 & 3677.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
003340313-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
003340360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003340360-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003340360-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003340593-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003341760-01 & 4973.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
003341760-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
003341934-01 & 6327.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003341934-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003342467-01 & 3278.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003342592-01 & 0402.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
003342592-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003342628-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003342779-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003342794-01 & 2278.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003342794-02 & 2278.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003342952-01 & 3215.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003342970-01 & 0800.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003342970-02 & 0800.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003343281-01 & 4860.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003343854-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003343866-01 & 6328.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003344419-01 & 1181.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3764.01\\
003344427-01 & 3764.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
003345675-01 & 1772.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003346027-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003346027-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003346027-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003346154-01 & 2723.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003346195-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003346195-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003346195-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
003346543-01 & 6329.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003347258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003347307-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003347337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003347395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003347395-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003347485-01 & 5985.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003347485-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003347485-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003347485-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003347643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003347643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003348082-01 & 1196.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003348093-01\\
003348082-02 & 1196.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003348082-03 & 1196.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003348090-01 & 4112.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003348093-01 & 3590.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
003348216-01 & 3448.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003348285-01 & 3021.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
003348288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003348288-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003348288-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003348533-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003348714-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003351888-01 & 0801.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003351945-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003351945-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003351945-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003351945-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003352122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003352122-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003352751-01 & 6330.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003352751-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003353050-01 & 0384.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003353454-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
003354846-01 & 2444.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003354855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003355104-01 & 4975.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003356155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003356193-01 & 6331.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
003356799-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003356799-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
003356839-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003425758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
003425802-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003425802-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003425851-01 & 0268.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003426367-01 & 2662.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003426991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003427727-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003427727-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003427759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
003427776-01 & 6332.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003427776-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003428013-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003428013-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003428468-01 & 3582.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003428468-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003429637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003429637-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003429973-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003429973-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
003431662-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003433668-01 & 3415.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003437557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003437557-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003437557-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
003437739-01 & 6333.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_UZ-Lyr-pri\\
003437776-01 & 0549.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003437776-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003437940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003437940-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003437940-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003438507-01 & 1204.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003438975-01 & 0300.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CROWDED\_DIFF---PARENT\_IS\_003439031-01\\
003438976-01 & 4527.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_003439031-01\\
003439031-01 & 4980.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003439096-01 & 3509.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003439031-01\\
003439374-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003439374-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003440074-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003440074-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003440074-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003440118-01 & 3876.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
003440230-01 & 6334.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
003440230-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003440429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003440710-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003440840-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003440840-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003440978-01 & 2288.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003440985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003441159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003441159-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003441159-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003441159-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003441340-01 & 6335.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003441340-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003441784-01 & 0976.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003441784-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003441784-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003441864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003441864-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003442006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003442006-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003442006-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003442006-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
003442054-01 & 3593.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003442054-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003442055-01 & 1218.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003442058-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003442058-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003442058-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003442058-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003443127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003443127-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003443582-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003443790-01 & 1185.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003443790-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003444098-01 & 4042.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
003444588-01 & 1202.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003444699-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003445068-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003445406-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003445443-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003445812-01 & 4802.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003446451-01 & 1735.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3736.01\\
003446471-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003446471-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003446471-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003446746-01 & 0385.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003446837-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003446837-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003446837-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003446996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003446996-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003447701-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003447722-01 & 1198.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003447722-02 & 1198.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003447722-03 & 1198.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003448130-01 & 2043.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003448230-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_003448245-pri\\
003448299-01 & \nodata & FP & 1 & 0 & 1 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_003448245-pri\\
003448323-01 & 6336.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_003448245-pri\\
003448456-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
003448456-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
003448777-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003448777-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003448777-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003448777-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003448817-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003449540-01 & 4982.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
003450040-01 & 4205.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003453026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003453026-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF\\
003453214-01 & 0802.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003453272-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003453272-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003453272-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003453494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003453494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003454720-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_003454731-05\\
003454731-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003454731-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003454731-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003454731-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003454731-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003454941-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003455863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003455863-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003455863-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003456198-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003456198-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003456198-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003456605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003456780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003456780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003456945-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
003456945-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003456945-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003457172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
003457192-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003457192-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003458028-01 & 2276.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003458318-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003458687-01 & 7543.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003458919-01 & 6337.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
003458990-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003459199-01 & 3725.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
003459226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
003459261-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003459261-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003526331-01 & 4800.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003529147-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003529242-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003529242-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003529290-01 & 3340.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003529290-02 & 3340.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003530245-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
003530668-01 & 5986.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003530668-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003531558-01 & 0118.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003532510-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003532510-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003532982-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003532982-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003532985-01 & 5987.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
003532985-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
003533469-01 & 2430.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003534118-01 & 3641.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003534192-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003534192-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003539231-01 & 4626.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003539331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003539521-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
003539521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
003539521-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
003539632-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003539869-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003539869-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003540153-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003541800-01 & 0491.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003541946-01 & 0624.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003541946-02 & 0624.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003541946-03 & 0624.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003542119-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003542167-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003542222-01 & 4137.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003542345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003542345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003542345-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003542566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003542573-01 & 6338.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003542574-01 & 3628.01 & FP & 0 & 0 & 0 & 1 & FIT\_FAILED---PARENT\_IS\_003542573-01\\
003542588-01 & 1217.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003542573-01\\
003543070-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003543070-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003543070-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003543270-01 & 6339.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003543270-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
003543433-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003543931-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003543931-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003544595-01 & 0069.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003544640-01 & 3279.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003544653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003544678-01 & 6340.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003544678-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003544689-01 & 1183.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003544694-01\\
003544694-01 & 3629.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
003544878-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
003544878-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003544900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003545038-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003545038-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003545135-01 & 2755.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003545457-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003545457-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003545457-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003545457-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003545478-01 & 0366.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003545626-01 & 6341.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003545840-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003545840-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003546060-01 & 2126.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003546419-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003546765-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003546765-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003546765-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003547014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003547014-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003547014-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003547091-01 & 1177.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
003547091-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003547178-01 & 6342.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET---CENTROID\_SIGNIF\_UNCERTAIN\\
003547178-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_003547187-01\\
003547178-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003547187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
003547187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003547315-01 & 3736.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003547523-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003547523-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003547692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003547760-01 & 4535.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003547760-02 & 4535.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003548044-01 & 2194.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003548044-02 & 2194.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003548369-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
003548369-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003548449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003548622-01 & 6343.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
003548639-01 & 4191.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003548639-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003548900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003548900-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003548900-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003550372-01 & 4357.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003550434-01 & 3854.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003553413-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003553413-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003553900-01 & 4992.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003554031-01 & 1194.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003554031-02 & 1194.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003554031-03 & 1194.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003554600-01 & 0803.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003554600-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003555191-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003555191-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003556220-01 & 1213.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3899.01\\
003556742-01 & 6344.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003556847-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
003557043-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003557273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003557273-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003557283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003557526-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_003557421-pri\\
003557560-01 & 4456.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003558145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003558145-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003558803-01 & 6345.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_003558822-pri\\
003558849-01 & 4307.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003558981-01 & 0052.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003558981-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003559860-01 & 3440.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003559860-02 & 3440.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003559933-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003559933-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003559933-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003559935-01 & 0492.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003560301-01 & 0968.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003560301-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003560301-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003560660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003560660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003560871-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003560871-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003561464-01 & 3398.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003561464-02 & 3398.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003561656-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
003561656-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003561656-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003561656-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003561700-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003561700-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003626325-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
003629100-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003629330-01 & 3418.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003629430-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_003629473-01\\
003629430-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_003629474-01\\
003629473-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_003629430-01\\
003629474-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_003629430-02\\
003629967-01 & 1901.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003632089-01 & 3308.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003632089-02 & 3308.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003632418-01 & 0975.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
003632418-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003633806-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003633889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003634051-01 & 6103.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
003634051-02 & 6103.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003634169-01 & 6346.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003634384-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003634384-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003634981-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003635233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
003635233-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
003635233-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
003635233-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003640832-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003640832-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003640905-01 & 1221.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003640905-02 & 1221.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003641023-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
003641023-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003641023-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003641023-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003641702-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003641726-01 & 0804.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003642289-01 & 0301.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003642289-02 & 0301.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003642324-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003642335-01 & 3010.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003642335-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
003642713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003642713-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003642741-01 & 0242.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003643155-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
003644071-01 & 1192.02 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_3511.01\\
003644071-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003644542-01\\
003644116-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003644116-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003644128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003644174-01 & 6347.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003644505-01 & 4641.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_3511.01\\
003644523-01 & 1195.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---PARENT\_IS\_3511.01\\
003644523-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_003644542-01\\
003644542-01 & 3511.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
003644542-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
003644602-01 & 4479.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003644542-02\\
003644653-01 & 2596.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_3511.01\\
003644653-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_003644542-01\\
003645438-01 & 4385.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003645438-02 & 4385.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
003645438-03 & 4385.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003645863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
003645863-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003646449-01 & 4999.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
003647291-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003648000-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
003648131-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
003648289-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003648437-01 & 1861.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003649426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003650040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003650040-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003650049-01 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003650057-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
003650111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003650111-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003654095-01 & 2667.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003654515-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003654515-02 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003654719-01 & 3081.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003654950-01 & 1766.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
003655115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
003655115-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003655115-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003655326-01 & 6348.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
003655326-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
003655332-01 & 1179.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED---PARENT\_IS\_003655326-01\\
003655513-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003655513-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003655513-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003656121-01 & 0386.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003656121-02 & 0386.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003656322-01 & 6349.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
003656648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CENTROID\_SIGNIF\_UNCERTAIN\\
003656700-01 & 6350.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003656905-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003656913-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
003657176-01 & 2903.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003657547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003657758-01 & 2034.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003657758-02 & 2034.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
003658906-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003659012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003659186-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003659940-01 & 6351.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
003660006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003660006-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003660392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003660392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003660476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003660476-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
003660828-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
003660924-01 & 1214.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003660943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003661206-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003661361-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003661361-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003661886-01 & 2279.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003661886-02 & 2279.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003662635-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003662838-01 & 0302.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003662838-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003662838-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003663141-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003663141-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
003663173-01 & 2750.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
003663494-01 & 6352.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
003663904-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003663904-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003728432-01 & 3893.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003728701-01 & 2536.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003730335-01 & 2808.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003730390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003730390-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003732035-01 & 3966.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003732821-01 & 1207.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003732894-01 & 4476.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_003836439-pri\\
003733346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003733346-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003733628-01 & 0387.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003733638-01 & 6353.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003733693-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003734418-01 & 2261.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003734868-01 & 0805.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003734868-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003735629-01 & 3544.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
003735634-01 & 3615.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3544.01\\
003742855-01 & 0045.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003742855-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003743511-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
003744309-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003744309-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003745559-01 & 3423.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003745690-01 & 0442.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003745690-02 & 0442.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003745690-03 & 0442.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003746248-01 & 6354.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003746248-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003747118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003747262-01 & 3005.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003747373-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003747641-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003747641-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003747817-01 & 4103.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003747817-02 & 4103.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
003748172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003748250-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003748250-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003748250-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
003748855-01 & 6355.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003748855-02 & 6355.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
003749134-01 & 1212.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003749348-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
003749365-01 & 1176.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
003749389-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003749389-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003749508-01 & 7544.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003749833-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003749833-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003749833-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003749978-01 & 2308.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003749989-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003749989-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003752110-01 & 3142.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003756264-01 & 3108.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003756613-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003757407-01 & 4057.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003757407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003757407-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003757521-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003757521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003757588-01 & 6356.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
003757588-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
003757590-01 & 3520.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
003757590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
003757778-01 & 3402.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003757778-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003757814-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003757814-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003758403-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003758403-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003758443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003758499-01 & 5007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003758922-01 & 4853.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003759974-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003760002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003760002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003760002-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003761175-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003761175-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003761319-01 & 6104.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003761641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003761641-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003761788-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
003762468-01 & 0208.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003762553-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003762553-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
003762741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003762741-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003763579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003763579-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003763579-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003763579-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003764025-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003764411-01 & 6357.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
003764428-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
003764714-01 & 3963.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003764714-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
003764714-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003764879-01 & 2141.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003765054-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003765692-01 & 6358.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003765771-01 & 1189.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003765917-01 & 4526.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003765917-02 & 4526.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003766353-01 & 6359.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003766353-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003766353-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003830820-01 & 6360.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003830820-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003831053-01 & 0388.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003831523-01 & 6361.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003831523-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003831523-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003831746-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003831746-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003831911-01 & 5988.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
003831911-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003831911-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003832474-01 & 0806.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003832474-02 & 0806.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003832716-01 & 0027.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003832716-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
003833007-01 & 0443.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003834317-01 & 4203.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
003834317-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003834317-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
003834322-01 & 2763.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003834322-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003834360-01 & 0493.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_003834364-01\\
003834364-01 & 6362.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003834364-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003835670-01 & 0149.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003836375-01 & 0807.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_003836439-pri\\
003836399-01 & 3834.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003836439-pri\\
003836399-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003836439-sec\\
003836399-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
003836413-01 & 6363.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003836439-pri\\
003836413-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED---PARENT\_IS\_003836439-pri\\
003836439-01 & 6364.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
003836439-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
003836450-01 & 5010.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_003836439-pri\\
003836453-01 & 1903.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_003836439-pri\\
003836509-01 & 5011.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_003836439-pri\\
003836522-01 & 5012.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_003836439-pri\\
003836558-01 & 4086.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_003836439-pri\\
003836727-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003836727-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
003836772-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003837702-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003837702-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003838004-01 & 6365.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
003838486-01 & 0808.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3700.01\\
003838496-01 & 3700.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
003839488-01 & 1216.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003839488-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003839928-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003839928-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003846515-01 & 5013.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003847138-01 & 0444.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003847563-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003847660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003847660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003847678-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
003847708-01 & 0389.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003847907-01 & 0229.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
003848275-01 & 2995.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003848572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
003848645-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003848665-01 & 5014.01 & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003644542-01\\
003848919-01 & 5015.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
003848948-01 & 5016.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---SATURATED---PARENT\_IS\_5015.01\\
003848966-01 & 3389.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003848972-01 & 1187.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003848972-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003849014-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
003849155-01 & 0390.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
003849187-01 & 4780.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003849354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003849354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003849354-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003849414-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
003849415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003849415-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
003849795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003850331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003850331-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003850551-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003850810-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003850810-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003851130-01 & 2284.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
003851134-01 & 6366.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_003954798-pri\\
003851151-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003851193-01 & 6367.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
003851194-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_003954798-pri\\
003851949-01 & 3808.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003851949-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003852258-01 & 5989.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003852258-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003852644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003852644-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003852655-01 & 3002.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003852712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003852712-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003853654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003853654-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003853654-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003853673-01 & 1197.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003854101-01 & 5018.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003854437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003854437-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003854496-01 & 6368.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
003855001-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003855001-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003855001-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003858704-01 & 1211.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003858757-01 & 6369.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-01\\
003858767-01 & 6370.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_003352751-pri\\
003858804-01 & 0391.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003858804-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_003858884-02\\
003858824-01 & 0996.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-01\\
003858824-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-02\\
003858851-01 & 3293.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003858851-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003858884-02\\
003858879-01 & 3276.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003858879-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_003858884-02\\
003858884-01 & 6371.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
003858884-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
003858884-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED---PARENT\_IS\_3293.01\\
003858884-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003858917-01 & 3294.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003858917-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003858884-02\\
003858919-01 & 5990.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-02\\
003858919-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-01\\
003858926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003858926-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003858949-01 & 0995.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003858949-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003858884-02\\
003858988-01 & 3388.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003858988-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003858884-02\\
003859079-01 & 1199.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003859151-01 & 4761.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_003858884-01\\
003859151-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-02\\
003859363-01 & 2887.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003859628-01 & 1191.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003859890-01 & 5020.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003860441-01 & 1188.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003861139-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003861139-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003861414-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003861414-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003861595-01 & 0004.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
003861595-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
003861611-01 & 2932.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_4.01\\
003862244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
003862246-01 & 0230.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
003862246-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
003862353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
003862354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003863594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003863594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003863594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003864417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003864417-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003864417-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003864443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003865298-01 & 3540.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
003865298-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
003865358-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---LARGE\_RM\\
003865567-01 & 1182.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
003865567-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003865595-01 & 3938.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
003865991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003865991-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003866099-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003866536-01 & 4423.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003866552-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
003866552-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003866552-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003866714-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003866714-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
003867256-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003867256-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003867256-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003867299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
003867593-01 & 5023.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003867615-01 & 2289.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003867615-02 & 2289.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
003867794-01 & 4685.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
003867794-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
003868284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003868284-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003868420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003868420-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003868420-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003868442-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003868442-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003868759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003869014-01 & 1205.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003869322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003869322-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
003869326-01 & 5991.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003869326-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003869794-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003869794-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003869825-01 & 1178.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003869825-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003869825-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003869825-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
003869825-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
003870389-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003935200-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003935914-01 & 0809.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003936061-01 & 6372.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003936965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003937519-01 & 0221.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003937519-02 & 0221.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003937814-01 & 4084.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003937814-02 & 4084.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003937814-03 & 4084.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003938073-01 & 6373.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003938073-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003939069-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003939150-01 & 1215.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003939150-02 & 1215.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003940372-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003940418-01 & 0810.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003941283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003941283-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003941283-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003941581-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
003942392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003942446-01 & 1193.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003942571-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003942571-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003942670-01 & 0392.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003942670-02 & 0392.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003942911-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
003942911-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003942911-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003943223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
003945791-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003945791-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003945791-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003945802-01 & 3435.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003945818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003945818-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003945818-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003945892-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003945892-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003945892-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003945892-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003946023-01 & 2447.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
003951334-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003951334-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003951622-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003952431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003952623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003952623-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003952651-01 & 1912.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003952852-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
003953106-01 & 5025.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
003953173-01 & 4493.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003954112-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
003954136-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
003954136-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003954227-01 & 3766.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
003954227-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
003954798-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003954798-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003955026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003955817-01 & 4117.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003955867-01 & 7545.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003955867-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003955867-03 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003956238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003957082-01 & 2864.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
003957270-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
003957477-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
003957477-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003957477-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
003957584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003957584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003957584-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003957622-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003957739-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003957739-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
003958707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003962243-01 & 1203.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003962243-02 & 1203.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003962243-03 & 1203.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
003962357-01 & 1210.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003962684-01 & 4908.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_003858884-01\\
003962684-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_003858884-02\\
003962728-01 & 5028.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-01\\
003962728-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_003858884-02\\
003962872-01 & 4539.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_003858884-02\\
003962872-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_003858884-01\\
003963203-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003963203-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003963203-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003964082-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003964109-01 & 0393.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003964128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003964128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003964128-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003964318-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
003964545-01 & 3542.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
003964545-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
003964562-01 & 0015.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3542.01\\
003964562-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_003964545-02\\
003965201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003965201-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003965201-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003965201-04 & 7546.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003965242-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003965242-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003965242-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003965879-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
003965879-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003965879-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003966262-01 & 1811.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
003966262-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
003966273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003966273-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003966273-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003966273-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003966491-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003966801-01 & 0494.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003966912-01 & 1186.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
003966912-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003967018-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
003967085-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003967085-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003967219-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
003967268-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003967268-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
003967268-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003967326-01 & 2084.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003967333-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003967333-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003967333-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
003967760-01 & 1760.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003967760-02 & 1760.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
003968961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003968961-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003968961-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003969604-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
003969604-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
003969687-01 & 2904.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003969800-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
003969800-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003969800-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
003969803-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
003970117-01 & 3556.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003970117-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003970233-01 & 0604.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003970233-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003970233-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003970621-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003970621-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003970621-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
003970729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003971315-01 & 5992.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
003971315-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
003972120-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
003972123-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
003972391-01 & 6374.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CROWDED\_DIFF\\
003972432-01 & 6375.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
003972517-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
003973002-01 & 6376.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
003973504-01 & 6377.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
003973504-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
003973549-01 & 5032.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
003974401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
003975085-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
003975085-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
003975085-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004035640-01 & 1881.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004035667-01 & 2684.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_6107.01\\
004035667-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004035675-01 & 6107.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
004035675-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004037428-01 & 5993.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004037428-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004037476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004038095-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004038095-02 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004038095-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004039966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004040636-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004042026-01 & 1180.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
004042026-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
004042088-01 & 6378.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
004042590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004042590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004043190-01 & 1220.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004043227-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
004043443-01 & 0231.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004043443-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004043674-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004044005-01 & 0969.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004044353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004044353-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004047631-01 & 2519.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004047900-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004047915-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
004048168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004048168-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004048494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004048494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004048494-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004048769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004048769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004049108-01 & 0495.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5994.01\\
004049124-01 & 5994.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004049124-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004049131-01 & 0811.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004049901-01 & 2295.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004050017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004050017-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004050017-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004050047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004054968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004054968-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004054968-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004055092-01 & 6379.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004055092-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004055304-01 & 2119.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004055765-01 & 0100.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004055765-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004055765-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004055774-01 & 2381.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5025.01\\
004056616-01 & 2013.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004058169-01 & 5034.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004058206-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004058206-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004058681-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004058881-01 & 3912.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004059007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004059043-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004059416-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004059887-01 & 4887.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_5045.01\\
004060229-01 & 4570.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004060976-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004061149-01 & 1201.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004064365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004064365-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004064365-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004064365-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004064365-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004066066-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004066066-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004066281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004066898-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004067110-01 & 4026.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004067336-01 & 1761.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004067549-01 & 6380.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004067549-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004067925-01 & 3066.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004068256-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004068256-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004068256-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004069039-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
004069063-01 & 6381.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004069213-01 & 6382.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
004069213-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
004069477-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004070376-01 & 1318.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004072333-01 & 2731.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004072526-01 & 1329.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004072582-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004072582-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004072582-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004072750-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004072750-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004072955-01 & 3041.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004073707-01 & 3525.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
004073730-01 & 3785.01 & FP & 0 & 0 & 0 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---SATURATED---PARENT\_IS\_004073707-01\\
004073730-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004073730-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004073730-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004074294-01 & 7547.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004074294-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004074388-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004074388-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004074640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004074640-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004074736-01 & 1328.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004075015-01 & 2850.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004075064-01 & 6383.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004075064-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004075064-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
004075067-01 & 3777.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
004075067-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
004075067-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004075067-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004075067-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004075172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004075172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004075172-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004075685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004075685-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004076061-01 & 6384.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004076098-01 & 1323.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004076952-01 & 6385.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004076976-01 & 3124.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004076952-pri\\
004077006-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004077006-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_004077032-02\\
004077006-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004077032-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004077032-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004077252-01 & 5038.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004077252-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004077275-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004077526-01 & 1336.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004077526-02 & 1336.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004077526-03 & 1336.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004077526-04 & 1336.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
004077558-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004077901-01 & 2239.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004078157-01 & 1319.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
004078157-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004078311-01 & 4166.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004078620-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004078693-01 & 6386.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004078693-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004078743-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004078743-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004078743-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004079482-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004079482-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004079482-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004079530-01 & 3594.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
004079530-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004079535-01 & 1322.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3594.01\\
004079535-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004079530-02\\
004135516-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
004135665-01 & 1339.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004135912-01 & 5040.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004136253-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_004136285-02\\
004136285-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004136285-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004136285-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004136285-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004136314-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004136314-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_004136285-01\\
004136396-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_004136285-02\\
004136396-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004136466-01 & 1344.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004136749-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004137903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
004137903-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004138008-01 & 4742.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004138848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004138848-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004138848-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004138951-01 & 2866.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004139254-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
004139254-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004139254-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004139351-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004139351-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004139673-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
004139673-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS\\
004139816-01 & 0812.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004139816-02 & 0812.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004139816-03 & 0812.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004139816-04 & 0812.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
004140813-01 & 2117.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004141376-01 & 0280.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004141464-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004141464-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004141670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004141670-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004141760-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004142768-01 & 6387.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004142768-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
004142768-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
004142768-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004142789-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004142789-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004142789-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004142847-01 & 2210.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004142847-02 & 2210.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004143755-01 & 0281.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004144231-01 & 1791.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_6109.01\\
004144236-01 & 6109.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004144236-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---PARENT\_IS\_1791.01\\
004144236-03 & 6109.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004144238-01 & 5041.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_6109.01\\
004144576-01 & 2202.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004147444-01 & 3880.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004149412-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004149450-01 & 1864.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004149684-01 & 6388.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004150390-01 & 1768.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004150390-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004150496-01 & 4046.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_3156.03\\
004150496-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_004150611-sec\\
004150496-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_004150611-03\\
004150539-01 & 1330.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3156.03\\
004150539-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004150611-sec\\
004150539-03 & 1330.02 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_004150611-03\\
004150611-01 & 3156.03 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
004150611-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
004150611-03 & 3156.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004150611-04 & 3156.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004150611-05 & 3156.02 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
004150624-01 & 1334.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3156.03\\
004150624-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_004150611-sec\\
004150624-03 & 1334.02 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_004150611-03\\
004150701-01 & 6110.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_004150611-sec\\
004150701-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_3156.03\\
004150703-01 & 6389.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004150611-sec\\
004150804-01 & 3678.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004155328-01 & 1335.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004156254-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004156254-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004156309-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004157325-01 & 1860.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004157325-02 & 1860.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004157325-03 & 1860.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004157325-04 & 1860.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
004157488-01 & 6390.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
004157849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004158822-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004158822-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004158876-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004158876-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004158876-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004159347-01 & 0394.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004159347-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004160006-01 & 5045.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004160235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004160235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004160669-01 & 6391.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004160676-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_004160683-02\\
004160676-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004160676-03 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004160683-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_004160676-02\\
004160683-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004160876-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004160876-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004164393-01 & 3413.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004164922-01 & 3864.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004164994-01 & 1320.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
004165473-01 & 0550.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004165739-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004165903-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
004165960-01 & 0395.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004168490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004168574-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004168574-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004168579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004168579-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004170511-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004170511-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004170631-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004170631-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004171302-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
004171302-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
004171302-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004171302-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004171302-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004171441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004171955-01 & 6392.01 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004172013-01 & 2386.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004172746-01 & 2531.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004172805-01 & 4427.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004173026-01 & 2172.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004173026-02 & 2172.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004174472-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004174472-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004174507-01 & 6393.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
004174754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004174754-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004174754-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004175105-01 & 4836.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004175630-01 & 2998.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004175706-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004176455-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004177905-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004177905-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004177905-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
004178173-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004178376-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004178389-01 & 0185.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004178606-01 & 2728.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004178606-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004178654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
004178654-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004179599-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004180099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004180099-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004180099-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004180199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004180199-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004180199-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004180280-01 & 0144.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004180346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004180375-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004180375-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004180375-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004180375-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004180396-01 & 6394.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
004180396-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
004180396-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004180396-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED\\
004180396-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004180401-01 & 2709.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004180401-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004181421-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004181421-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004181749-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
004242147-01 & 1934.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004242315-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
004242315-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004242575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004242692-01 & 3928.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004243461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004243461-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004243911-01 & 1337.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004243984-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004243984-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
004243984-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004244642-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004244642-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004245701-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004245701-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004245701-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004245861-01 & 5050.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_004245897-pri\\
004245897-01 & 6395.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004245933-01 & 2190.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004245897-pri\\
004247023-01 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
004247092-01 & 0403.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004247092-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004247791-01 & 0028.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
004247807-01 & 3748.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004247791-pri\\
004247811-01 & 4678.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_004247791-pri\\
004247991-01 & 2311.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004248120-01 & 2216.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004249611-01 & 2821.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
004249725-01 & 0222.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004249725-02 & 0222.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004252226-01 & 6396.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004252226-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004252322-01 & 0396.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004252716-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004252716-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004252757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004252757-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004253413-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004253413-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004253413-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
004253860-01 & 5052.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
004253860-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004253860-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004254466-01 & 2134.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004254741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004254741-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004254741-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004254741-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004255422-01 & 3528.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004255944-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004255944-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
004255944-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004261149-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004261960-01 & 6397.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004262040-01 & 3202.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004262581-01 & 2122.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004263127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004263127-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004263127-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
004263293-01 & 1895.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004263293-02 & 1895.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004263293-03 & 1895.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004263529-01 & 3358.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004263932-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004264365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004264365-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004264365-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004264546-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004269252-01 & 6398.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004269329-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004269329-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004269329-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004269337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004269337-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004269337-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004269337-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004270253-01 & 0551.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004270253-02 & 0551.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004270565-01 & 2819.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004270799-01 & 4810.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004270987-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004270987-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004270987-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004271063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004271063-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004271474-01 & 3324.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004271930-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004271930-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004271930-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004273425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004273425-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004274071-01 & 6399.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004274252-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004274480-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004274480-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004274517-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004274548-01 & 1331.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004274730-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004274730-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004274748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004275117-01 & 2776.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004275186-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004275191-01 & 0813.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
004275328-01 & 5995.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004275328-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004275721-01 & 1342.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004275721-02 & 1342.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004275739-01 & 1317.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
004276002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004276002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004276114-01 & 5054.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004276114-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004276716-01 & 1619.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004276821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004276821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004276892-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004277242-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004277304-01 & 4774.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004277581-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004278221-01 & 1615.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004279066-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004279066-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004279066-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004281581-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004281895-01 & 6400.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004282191-01 & 3439.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004282390-01 & 6401.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004282390-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
004282872-01 & 1325.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004283612-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004283747-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004283747-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004284125-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004284147-01 & 6402.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
004284959-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004285040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004285087-01 & 6112.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004285107-01 & 1333.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_6112.01\\
004285359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004285359-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004285359-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004346178-01 & 2652.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004346875-01 & 6113.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004346875-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004348313-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004348313-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004348313-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS\\
004349442-01 & 1803.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004349442-02 & 1803.02 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004349452-01\\
004349442-03 & 1803.03 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_244.02\\
004349452-01 & 0244.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004349452-02 & 0244.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004349452-03 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004349612-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004349612-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004349935-01 & 6403.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
004350501-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004351367-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004351414-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004352168-01 & 6404.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004352168-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004355012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004355012-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004355012-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004355012-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004356621-01 & 6405.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_004356766-01\\
004356766-01 & 3669.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004357960-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004357960-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004357960-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004357967-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004357967-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004357985-01 & 6406.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_3156.03\\
004357985-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_CENTROIDS---PARENT\_IS\_004150611-sec\\
004358206-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004358206-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004358355-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004358355-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004358571-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004358571-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004365442-01 & 2787.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5058.01\\
004365461-01 & 5058.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004365645-01 & 1738.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004366323-01 & 3258.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004366913-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004366913-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004366913-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004366913-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004367544-01 & 6407.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
004367616-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
004367854-01 & 2876.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004370527-01 & 2166.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004370956-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004370956-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004371947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004372213-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004372282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004372410-01 & 6408.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004372410-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004372410-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004372620-01 & 6409.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004372765-01 & 3698.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
004372768-01 & 1327.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3698.01\\
004372768-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004372765-sec\\
004372961-01 & 6410.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004373195-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_V1130-Cyg-pri\\
004374122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004374339-01 & 2987.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004374610-01 & 4712.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004374812-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004374812-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004374812-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004375101-01 & 6411.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004375101-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004375408-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004376559-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
004376629-01 & 3378.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_397.01\\
004376644-01 & 0397.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004377638-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004377638-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004378863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004378863-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004379599-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004379925-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
004380283-01 & 6412.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
004380558-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
004380558-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004380560-01 & 7548.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004380775-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004380834-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004380834-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004380951-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004380951-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004380951-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004381016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004381016-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004381016-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004381221-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004381221-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004381282-01 & 2922.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004381282-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004381429-01 & 4474.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004381649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004381649-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004382014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004382014-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004382014-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004382143-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004382143-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004382785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004383117-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004383270-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004383955-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004383955-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004383955-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004383955-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004384398-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004384398-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004384398-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004384652-01 & 7549.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004384652-02 & \nodata & FP & 1 & 0 & 0 & 1 & RESID\_OF\_PREV\_TCE---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004384652-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004384675-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
004384675-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---FIT\_FAILED\\
004384675-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
004384675-04 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
004384675-05 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004384793-01 & 6413.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004384793-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004384793-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004385148-01 & 2942.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004385148-02 & 2942.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004386047-01 & 3659.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
004386059-01 & 1340.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3659.01\\
004386091-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004386091-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004386121-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004386947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004390625-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004390625-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004390899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004390902-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004390912-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004391348-01 & 2514.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004391466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004391466-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
004445630-01 & 6414.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004446044-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004446135-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004446135-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004446181-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004446299-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004446411-01 & 6415.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
004447461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004448848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004449034-01 & 0625.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004450028-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004450028-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004450844-01 & 3168.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004451755-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004454219-01 & 6416.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
004454752-01 & 0496.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004454906-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004454934-01 & 2245.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004454980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004455231-01 & 1332.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004455231-02 & 1332.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004455231-03 & 1332.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004455314-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004455763-01 & 5061.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004456107-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004456107-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004456107-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004456622-01 & 6417.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004456622-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
004456940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004456940-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004457122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004458082-01 & 2303.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004458082-02 & 2303.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004458109-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004458109-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004458172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004458172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004458172-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004458346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004458346-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004458918-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004458918-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004458984-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_004458989-pri\\
004459068-01 & 6114.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
004459068-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
004459285-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004459924-01 & 2441.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004459939-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004459939-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004464287-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004464287-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004464287-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004464394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004464394-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004464394-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
004464689-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004465188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004465188-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004465188-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004466180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004466180-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004466356-01 & 3295.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004466677-01 & 1338.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004466677-02 & 1338.02 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004466677-03 & 1338.03 & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004470141-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
004470415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004471379-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004471379-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004471379-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004471747-01 & 1656.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004472465-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004472465-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004472818-01 & 3878.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004472818-02 & 3878.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004473083-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004473083-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004473083-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004473226-01 & 2229.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004473450-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004473450-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004473613-01 & 4803.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004473933-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004473933-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004474407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004474407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004474462-01 & 4452.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004474462-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004474484-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004474637-01 & 3829.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004474637-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
004474645-01 & 1657.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_004474637-01\\
004474645-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004474637-sec\\
004476011-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
004476011-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004476013-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004476123-01 & 0814.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004476186-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004476186-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004476186-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004476186-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004476392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004477104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004477170-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004477747-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004477747-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004477871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004478168-01 & 0626.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004478168-02 & 0626.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004479633-01 & 2814.01 & FP & 0 & 0 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004479633-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004479949-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004479949-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004480321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004480676-01 & 1321.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004481004-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004481426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004481426-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004481426-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004481700-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004481700-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004481700-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004482231-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004482231-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
004482231-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004482348-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004482348-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004482641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
004482738-01 & 6418.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_004579598-01\\
004482738-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_004579598-01\\
004483138-01 & 2910.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
004483235-01 & 7550.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004483235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004483235-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004483262-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004483262-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004483262-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004483691-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004483781-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004483781-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004484128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004484128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004484128-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004484251-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_004484252-01\\
004484251-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004484251-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
004484252-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004484252-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
004484252-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004484271-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004484271-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004484271-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004484312-01 & 6419.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_6112.01\\
004484336-01 & 2547.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004484356-01 & 6420.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004488796-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004488796-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004488796-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004488840-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
004488840-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004488840-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004489387-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
004489829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004489844-01 & 6421.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004540632-01 & 6422.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004540632-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004540632-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
004544571-01 & 3976.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_004544587-pri\\
004544571-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004544587-sec\\
004544571-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004544571-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004544572-01 & 3950.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_004544587-pri\\
004544572-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
004544572-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_004544587-sec\\
004544587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004544620-01 & 3915.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_004544587-pri\\
004544620-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004544587-sec\\
004544620-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004544623-01 & 6423.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_004544587-pri\\
004544623-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_004544587-sec\\
004544628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004544628-02 & 4753.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_004544587-pri\\
004544670-01 & 0815.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004544684-01 & 4847.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_004544587-pri\\
004544757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
004544907-01 & 2024.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004545187-01 & 0223.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004545187-02 & 0223.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004545570-01 & 4506.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004545926-01 & 4787.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004547321-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_004547308-pri\\
004547480-01 & 6116.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004547480-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004547603-01 & 2855.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004547830-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004547830-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004548011-01 & 4288.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004548011-02 & 4288.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004548011-03 & 4288.03 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
004548098-01 & 4157.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004548098-02 & 4157.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004550962-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004551328-01 & 1324.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
004551563-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004551663-01 & 2576.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004552374-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004552395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004552395-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004552514-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
004552729-01 & 2691.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004555642-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004555954-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004556345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004556345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004556345-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004556468-01 & 4491.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004557777-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004562317-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004562615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004562615-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004562615-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004563268-01 & 0627.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004563268-02 & 0627.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004565985-01 & 6424.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
004565985-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
004566740-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004566740-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004566848-01 & 5071.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004567118-01 & 6425.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
004567400-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004567531-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004568117-01 & 4248.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V1130-Cyg-pri\\
004568298-01 & 2986.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED---PARENT\_IS\_V1130-Cyg-pri\\
004568729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004569150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004569150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004569150-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004569150-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004569590-01 & 6426.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004569590-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004570555-01 & 5072.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004570931-01 & 1343.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1658.01\\
004570949-01 & 1658.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004570949-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004570949-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004570949-04 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
004571004-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004571004-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004571536-01 & 2954.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_CENTROIDS\\
004571780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004571780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004571780-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004571844-01 & 4353.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
004572605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004574142-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004574310-01 & 6427.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004574310-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004575824-01 & 6428.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
004575908-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
004576280-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004576968-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---CLEAR\_APO\\
004577324-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004577647-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
004577860-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004577969-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004577969-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004577969-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004578594-01 & 6429.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
004578644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004579313-01 & 3884.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_004579321-01\\
004579313-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004579321-02\\
004579321-01 & 3657.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004579321-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
004579598-01 & 4414.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_004482738-02\\
004579651-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004579651-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CENTROID\_SIGNIF\_UNCERTAIN\\
004580484-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
004580484-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004584664-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004584865-01 & 4429.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5335.01\\
004585982-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004586468-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004586482-01 & 5073.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CENTROID\_SIGNIF\_UNCERTAIN\\
004586482-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
004587135-01 & 4680.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004587448-01 & 6430.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004587448-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004587528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004587528-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004588073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004588115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004588115-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004588115-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004633434-01 & 6431.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004633434-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004633454-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004633454-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004633570-01 & 0446.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004633570-02 & 0446.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004634135-01 & 3328.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
004634135-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
004636464-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004636464-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004636464-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004636565-01 & 4138.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_004445630-01\\
004636578-01 & 2025.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004636578-02 & 2025.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004636578-03 & 2025.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004638237-01 & 3811.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004639291-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004639868-01 & 1326.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004640914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004640914-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004640983-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004641419-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004641519-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004641555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004644277-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
004644604-01 & 0628.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004644922-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004644952-01 & 1805.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004644952-02 & 1805.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004644952-03 & 1805.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004645174-01 & 3437.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004645174-02 & 3437.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004645626-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004645823-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004645833-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004645833-02 & 4783.01 & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004647715-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004647715-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004647715-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004647763-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004647763-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004647763-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004648848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004648848-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004649173-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004649238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004649238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004649238-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004649238-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004649305-01 & 0143.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004649305-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
004649305-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004649339-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004649339-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004649440-01 & 3919.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004649440-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004649462-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004649462-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004649476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
004649476-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004649476-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004650137-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004650327-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004650674-01 & 1341.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004650686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004650733-01 & 1659.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004650995-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004650995-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004656049-01 & 0629.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004656194-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004658336-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004658336-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004658336-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004659094-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004659255-01 & 3580.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004659405-01 & 0630.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3691.01\\
004659405-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004751083-02\\
004660027-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004661634-01 & 6432.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004661634-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004661660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004661660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004661660-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004661914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004661980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004662336-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004662336-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004662336-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004662336-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004662363-01 & 7551.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
004663148-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004663185-01 & 3805.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004663658-01 & 3187.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004664046-01 & 2930.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004664466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004664743-01 & 4642.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004664743-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004664754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
004664847-01 & 0816.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004665571-01 & 2393.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004665571-02 & 2393.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004665989-01 & 6433.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
004665991-01 & 4870.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_004665989-pri\\
004666008-01 & 3872.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_004665989-pri\\
004667875-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004667989-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004667989-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004667989-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004668393-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004668393-02 & \nodata & FP & 1 & 0 & 1 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004669058-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004669402-01 & 4128.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004669402-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004669402-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004670217-01 & 2560.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004670267-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004670267-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004670267-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004670388-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004670388-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004670388-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004670846-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004670846-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004670846-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004671225-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004671225-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
004671225-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004671584-01 & 6434.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
004672045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004672045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004672512-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004673628-01 & 4056.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004676964-01 & 3069.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004677140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004677282-01 & 2766.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_004677321-pri\\
004677446-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004677446-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004677684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004678171-01 & 6435.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004678171-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
004678171-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
004678171-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
004678171-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
004678171-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004678873-01 & 5075.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_004678875-01\\
004678875-01 & 3664.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004678875-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004678919-01 & 4219.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004678875-01\\
004679104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004679242-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004679242-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004679314-01 & 4425.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004679369-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004679369-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004679528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004679528-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004679528-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004679562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004679562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
004679687-01 & 4049.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004679687-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
004679769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004679769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004679988-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004679988-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004679988-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004679988-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004680002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
004680002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004680002-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004680543-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004680543-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
004680597-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004680597-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004680745-01 & 7552.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004680772-01 & 4707.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
004681152-01 & 6436.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
004725292-01 & 6437.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004725681-01 & 0817.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004725681-02 & 0817.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004725737-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004725882-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004726268-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004726268-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004726268-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004729553-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004729553-02 & 6438.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004729553-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004731303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004731916-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004731916-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004732015-01 & 5076.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
004732015-02 & 5076.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED\\
004733003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004733003-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004733318-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004733318-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004733344-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004733344-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004735826-01 & 3184.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004735826-02 & 3184.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004736208-01 & 6439.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004736208-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
004736561-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004736562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004736562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004736562-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004736569-01 & 1996.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004736569-02 & 1996.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004736644-01 & 3330.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004737267-01 & 6117.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
004737302-01 & 6441.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004737720-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004737720-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004737720-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004738155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004739194-01 & 6442.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004739229-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004739565-01 & 6443.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_004739791-pri\\
004739791-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004739791-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004740125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004740125-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004740287-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004740676-01 & 6119.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004740688-01 & 6444.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004740676-pri\\
004741126-01 & 1534.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004741126-02 & 1534.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004742414-01 & 0631.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004742436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004742461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004742461-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004743125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004743188-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004743188-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004743189-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004743189-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004743189-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004743508-01 & 3572.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
004743508-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004743513-01 & 0024.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM---PARENT\_IS\_3572.01\\
004743513-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_004743508-02\\
004749989-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004749989-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004750341-01 & 4884.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
004750669-01 & 4649.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
004751083-01 & 3691.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
004751083-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004752451-01 & 0109.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004752451-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004752731-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004753561-01 & 5996.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004753561-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004753988-01 & 6445.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004754310-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004754831-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004754831-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004754831-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
004755450-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004755450-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004755510-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004755510-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004755510-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004755510-04 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004756040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004756040-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004756040-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004756092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004756171-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004756171-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004756243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004756243-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004756335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004756725-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004756725-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004756776-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004756776-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004757331-01 & 6446.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
004757437-01 & 0497.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004757437-02 & 0497.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004757997-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
004757997-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004757997-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004758350-01 & 6447.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
004758350-02 & 6447.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004758368-01 & 6448.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
004758368-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED\\
004760478-01 & 5084.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
004760746-01 & 1455.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004760946-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004760946-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004760946-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004760959-01 & 6449.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
004761060-01 & 2249.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004761060-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004761060-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004761183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004761269-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004762283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
004763381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004763381-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004763776-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004764008-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004764523-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004764523-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004764523-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004764774-01 & 4825.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004764969-01 & 6450.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
004768668-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
004768668-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004768668-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004768677-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004768731-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
004768756-01 & 6451.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_6134.01\\
004768846-01 & 2077.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004768846-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004768919-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004768919-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004769007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004769007-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004769007-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004769505-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004769505-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004769505-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004769799-01 & 5086.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
004769824-01 & 6452.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5086.01\\
004769931-01 & 4058.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_004678875-01\\
004770092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004770092-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004770174-01 & 2971.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004770365-01 & 1475.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004770365-02 & 1475.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004770365-03 & 1475.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004770617-01 & 2243.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004770617-02 & 2243.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004771707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004773133-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004773155-01 & 6453.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004773155-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
004773155-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004773155-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
004773155-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004773392-01 & 4367.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004773851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004773851-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
004773851-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004773851-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004774194-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004774194-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004774194-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004774208-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004774208-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
004774321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004774321-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004813563-01 & 1959.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004813750-01 & 5088.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004814502-01 & 4004.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004815520-01 & 0367.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004815612-01 & 5090.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
004816098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004819564-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004819950-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004820550-01 & 3823.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004820642-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004824268-01 & 3533.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004824268-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004825872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004825872-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004825872-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004826031-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004826031-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004826031-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
004826110-01 & 1524.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004826439-01 & 6121.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004827662-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004827662-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004827723-01 & 0632.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004828341-01 & 1496.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004829243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004829935-01 & 2395.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004830605-01 & 1660.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004830859-01 & 6454.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004831251-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004831616-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---KIC\_OFFSET\\
004831616-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004831728-01 & 2739.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004831728-02 & 2739.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
004831769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004832175-01 & 2846.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004832197-pri\\
004832197-01 & 1661.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004832225-01 & 4013.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_004832197-pri\\
004832225-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004832273-01 & 6455.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
004832837-01 & 0605.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004832837-02 & 0605.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004833050-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004833050-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004833421-01 & 0232.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004833421-02 & 0232.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004833421-03 & 0232.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
004833421-04 & 0232.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004833421-05 & 0232.05 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
004839180-01 & 6456.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
004839411-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004839494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
004840263-01 & 6457.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
004840327-01 & 5093.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004840401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004840513-01 & 1541.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004840513-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004840675-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004840675-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004840818-01 & 6458.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
004841314-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004841314-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004841374-01 & 0633.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004842166-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004842166-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004842166-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004842623-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004842790-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004843037-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004843037-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004843592-01 & 4683.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
004843592-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
004844004-01 & 1662.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004844367-01 & 4498.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004844470-01 & 3469.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004845003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
004845555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004845555-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004845555-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004845590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004845862-01 & 4606.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004846150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
004846373-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004846856-01 & 2900.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004846926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004846926-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004847078-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004847371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004847371-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004847411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004847411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004847534-01 & 0499.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004847691-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004847782-01 & 3067.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_004847832-01\\
004847782-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004847832-02\\
004847832-01 & 6459.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
004847832-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
004847832-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
004847843-01 & 3505.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_004847832-02\\
004847843-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004847832-01\\
004848115-01 & 4537.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004848216-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004848321-01 & 4573.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3560.01\\
004848423-01 & 3560.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
004848424-01 & 2991.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_3560.01\\
004848532-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_3560.01\\
004848695-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
004848695-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004848695-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004850046-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004850661-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_004850677-01\\
004850677-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_004850661-01\\
004850763-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
004850809-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_004851168-01\\
004850961-01 & 4092.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004850965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004851145-01 & 4688.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004851217-pri\\
004851168-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_004850809-01\\
004851173-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004851173-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004851182-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004851182-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004851182-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004851182-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
004851195-01 & 7553.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---FIT\_FAILED---PARENT\_IS\_004482641-01\\
004851195-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004851195-03 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
004851217-01 & 6460.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004851239-01 & 4851.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_004851217-pri\\
004851283-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_004851217-pri\\
004851283-02 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_004851217-sec\\
004851304-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004851338-01 & 6461.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_004851217-pri\\
004851356-01 & 6462.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_004851217-pri\\
004851457-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004851464-01 & 1757.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004851464-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004851530-01 & 1884.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
004851530-02 & 1884.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004852055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004852297-01 & 4695.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004852455-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004852528-01 & 0500.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004852528-02 & 0500.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004852528-03 & 0500.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
004852528-04 & 0500.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
004852528-05 & 0500.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
004856549-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
004856630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004856630-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
004857058-01 & 3061.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004857058-02 & 3061.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004857213-01 & 2120.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004857734-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
004858525-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004858525-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004858610-01 & 2844.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004859418-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004859557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004859557-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004859559-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004860300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004860444-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004860444-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004860678-01 & 1602.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004860678-02 & 1602.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004860686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004860932-01 & 1600.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004860932-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004861364-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004861527-01 & 2727.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_004773155-01\\
004861527-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_004773155-02\\
004861736-01 & 0634.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
004861736-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004861784-01 & 4278.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004861791-01 & 2870.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_4278.01\\
004862155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004862332-01 & 6463.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004862625-01 & 6464.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004862625-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004862625-03 & 6464.03 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
004862625-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004862625-05 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004862625-06 & 6464.02 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
004862625-07 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004862730-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004862730-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004862924-01 & 7554.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004862968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004862968-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004862968-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004863077-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004863077-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004863260-01 & 5096.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004863369-01 & 6465.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004863614-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004863614-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004863753-01 & 6466.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004863836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004863956-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004863956-02 & 4344.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004864734-01 & 3944.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004902030-01 & 6467.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
004902475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004902475-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004907266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004908495-01 & 6468.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
004908774-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004909697-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004909697-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004909707-01 & 3175.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004909707-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004909707-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004912589-01 & 6469.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004912650-01 & 5098.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004912991-01 & 5997.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
004913000-01 & 1775.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_5997.01\\
004913852-01 & 0818.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004913858-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_005001655-01\\
004914032-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
004914399-01 & 5100.01 & FP & 0 & 0 & 0 & 1 & TOO\_FEW\_QUARTERS---PARENT\_IS\_004826439-01\\
004914423-01 & 0108.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004914423-02 & 0108.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004914490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004914566-01 & 2635.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004914709-01 & 6470.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_3156.03\\
004914709-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_004150611-sec\\
004914737-01 & 6471.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_004150611-sec\\
004914737-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_3156.03\\
004914771-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004915638-01 & 2617.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004915765-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004916395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
004916845-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004917014-01 & 6472.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004917014-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004917596-01 & 1973.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004918303-01 & 5104.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004918309-01 & 1582.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004918925-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004918972-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004919550-01 & 4766.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004919550-02 & 4766.02 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
004919814-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004919818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004919818-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004919818-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004920125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004920125-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004920125-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004920125-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004922612-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
004927192-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004927192-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004927192-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004927315-01 & 1663.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004927315-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004927495-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004927495-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004927495-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004927734-01 & 3212.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004927985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004927985-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
004928119-01 & 1664.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004928235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004929092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004929299-01 & 4018.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
004929299-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
004929615-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004930578-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004930578-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004930578-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004930913-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
004930913-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF\\
004930913-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004931073-01 & 6473.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004931073-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004931073-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004931073-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004931390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004931390-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004931864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
004932348-01 & 0819.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004932348-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004932417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004932417-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004932417-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004932442-01 & 1665.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004932657-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004932657-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
004932689-01 & 3453.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_004932691-01\\
004932691-01 & 6474.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004932691-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004933476-01 & 6122.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
004934347-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004934893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004934893-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004934893-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004935172-01 & 2962.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004935198-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004935594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
004935594-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004935606-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004935813-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004935813-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004935914-01 & 3743.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004935914-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---CENTROID\_SIGNIF\_UNCERTAIN\\
004936020-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004936180-01 & 0820.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004936284-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
004936524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004936990-01 & 3290.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
004936990-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
004937143-01 & 3715.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004937143-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004937340-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004937340-02 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004937379-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004937379-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004937435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004937435-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004937872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004937872-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004937872-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004938281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004938281-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004938281-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004938893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004939265-01 & 6475.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
004939281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004939304-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
004939346-01 & 1873.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004939346-02 & 1873.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004939533-01 & 2899.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
004940092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004940201-01 & 6476.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
004940217-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004940226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
004940438-01 & 1561.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004940438-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004944828-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
004945035-01 & 5108.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
004945107-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004945107-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
004945266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004945285-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004945346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
004945346-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004945547-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_004945588-sec\\
004945764-01 & 4377.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004945764-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
004945764-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004945764-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004945877-01 & 1936.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
004946049-01 & 4658.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_004678875-01\\
004946581-01 & 5109.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004946627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004946680-01 & 6477.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
004946680-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
004946956-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004946956-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004947130-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004947130-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004947130-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004947556-01 & 3936.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004947556-02 & 3936.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
004947726-01 & 6478.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004947726-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004948730-01 & 3272.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
004948730-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
004948863-01 & 6479.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
004949027-01 & 6480.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005036538-01\\
004949187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004949187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004949187-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004949214-01 & 6481.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
004949524-01 & 3852.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
004949751-01 & 0404.01 & FP & 0 & 0 & 1 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
004949769-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_004949770-pri\\
004949769-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_004949770-pri\\
004949795-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_004949770-pri\\
004949801-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_004949770-pri\\
004949825-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_004949770-pri\\
004950232-01 & 1753.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004950341-01 & 6482.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
004950557-01 & 6483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004950985-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
004951030-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004951030-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004951030-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
004951249-01 & 2258.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
004951447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004951447-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004951711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
004951877-01 & 0501.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004952226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004952259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004952259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
004952259-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
004952341-01 & 2818.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
004952341-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
004952341-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004952608-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004952608-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004953173-01 & 4676.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
004953372-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
004953696-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
004954074-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
004954074-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
004989057-01 & 1923.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004989879-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004989879-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
004990101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
004990637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004990977-01 & 6123.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
004990977-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
004991208-01 & 2951.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
004994971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
004995716-01 & 6484.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
004995948-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
004995948-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
004995953-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
004996558-01 & 5111.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005000179-01 & 6485.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005000179-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005000179-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
005000179-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005001655-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_004913858-01\\
005002361-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005002361-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005002557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005003117-01 & 0405.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005003117-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005003342-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005003342-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005003670-01 & 4524.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005003670-02 & 4524.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005004705-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005004909-01 & 3421.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005005121-01 & 2237.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005005618-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005007345-01 & 2406.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005007640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005007640-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005008211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005008245-01 & 3770.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005008501-01 & 1666.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005008689-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005008954-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005008954-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005008954-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005008954-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005008954-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005008966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005009189-01 & 1605.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005009189-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005009743-01 & 1609.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005010302-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005010302-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005014753-01 & 0606.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005014753-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005014903-01 & 2966.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005015459-01 & 3923.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005015913-01 & 1667.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005016163-01 & 5115.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005017058-01 & 6486.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---SEASONAL\_DEPTH\_DIFFS\_IN\_DV\\
005018711-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005018787-01 & 6487.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005019101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005019101-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005019101-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005019234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005019234-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005019567-01 & 6488.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005019567-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005019587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005020034-01 & 3688.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
005020044-01 & 3802.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3688.01\\
005020065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005020065-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005020319-01 & 0635.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005020319-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005021024-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005021174-01 & 3679.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005021174-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005021176-01 & 0447.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3679.01\\
005021176-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3679.01\\
005021286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005021329-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005021432-01 & 6489.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005021732-01 & 6490.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005021732-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005021737-01 & 0026.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_005021732-01\\
005021737-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_005021732-02\\
005021899-01 & 0821.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005022440-01 & 6491.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005022440-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005022535-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005022828-01 & 2138.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005022900-01 & 6492.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
005022943-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005022908-pri\\
005023338-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---KIC\_OFFSET\\
005023338-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005023338-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005023948-01 & 3570.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005023956-01 & 0233.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3570.01\\
005024126-01 & 6493.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_4286.01\\
005024138-01 & 4819.01 & FP & 0 & 0 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005024138-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005024177-01 & 4286.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005024177-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005024252-01 & 4682.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005024292-01\\
005024268-01 & 6494.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_005024292-01\\
005024292-01 & 3579.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
005024372-01 & 6495.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005024414-01 & 7555.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1544.01\\
005024450-01 & 1544.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005024455-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005024482-01 & 2041.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1544.01\\
005025217-01 & 6496.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005025217-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005025234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005025234-02 & 6497.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005025294-01 & 6498.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005025294-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005025294-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005025464-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005025692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005026187-01 & 6499.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005026326-01 & 4280.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
005027441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005027441-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
005027859-01 & 5117.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005031804-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005031804-02 & 6500.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005031804-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005031857-01 & 1573.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005031857-02 & 1573.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005031882-01 & 6501.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005033298-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_006549623-01\\
005033823-01 & 4546.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005034039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005034039-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
005034333-01 & 6124.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005034333-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
005034333-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE\\
005034333-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
005034333-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
005035237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005035849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005035972-01 & 0406.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005035972-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005036037-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005036037-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005036037-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005036480-01 & 4080.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005036538-01\\
005036491-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_005036493-01\\
005036491-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005036491-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005036493-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---KIC\_OFFSET\\
005036493-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005036516-01 & 6502.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_005036538-01\\
005036530-01 & 6503.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005036530-02 & 6503.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
005036537-01 & 3718.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005036538-01\\
005036538-01 & 6504.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
005036705-01 & 2437.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005036761-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005036761-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005036966-01 & 5998.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
005036966-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
005037068-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005037568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005037568-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005038228-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005038228-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005038443-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005038469-01 & 6505.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
005038469-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---KIC\_OFFSET\\
005038469-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005038493-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005038493-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005039129-01 & 2546.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005039228-01 & 1597.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CROWDED\_DIFF\\
005039441-01 & 6125.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005039441-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005039687-01 & 6506.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005040077-01 & 3065.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005040223-01 & 4354.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005041569-01 & 2795.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---TOO\_FEW\_QUARTERS\\
005042210-01 & 2462.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005042785-01 & 6507.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005042785-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005077629-01 & 0822.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005077629-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005078025-01 & 4211.02 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_005077994-pri\\
005078025-02 & 4211.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_005077994-sec\\
005078879-01 & 6508.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005078939-01 & 2438.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005078939-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005080346-01 & 6509.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
005080346-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005080636-01 & 1843.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005080636-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005080636-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
005080652-01 & 6510.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
005083138-01 & 6511.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005083252-01 & 6512.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005084171-01 & 4202.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005084289-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005084942-01 & 0161.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005087223-01 & 6513.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005088308-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005088308-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005088400-01 & 4127.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005088536-01 & 0282.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005088536-02 & 0282.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005088536-03 & 0282.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005088591-01 & 1801.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005089498-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005089498-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005089498-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005090286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005090690-01 & 0636.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005090937-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005091016-01 & 2973.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005091075-01 & 6514.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
005091614-01 & 6515.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005091614-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005092266-01 & 3045.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005092655-01 & 4116.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005092799-01 & 6516.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005092799-02 & 6516.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005093168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005093223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005094301-01 & 6517.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005094301-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005094412-01 & 5124.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005094751-01 & 0123.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005094751-02 & 0123.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005094751-03 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT\\
005094944-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005094944-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005095082-01 & 4320.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005095098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005095232-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005095269-01 & 6518.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005095635-01 & 2607.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005096053-01 & 4331.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005096095-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005096590-01 & 3093.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005097278-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
005097278-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005097278-03 & 6519.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005097454-01 & 4244.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_005097446-pri\\
005097470-01 & 2767.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_005097446-pri\\
005097868-01 & 2435.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005098444-01 & 0637.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005098444-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
005098757-01 & 6520.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005098757-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005103942-01 & 1668.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005103942-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005103998-01 & 3660.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005104153-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005106292-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005106313-01 & 2878.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005108214-01 & 1924.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_3688.01\\
005108514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005108514-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005108514-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005108946-01 & 2955.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005110034-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005110034-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005110038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005110038-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005110423-01 & 1777.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005111544-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005111801-01 & 6521.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005112198-01 & 6522.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
005112567-01 & 4043.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005113053-01 & 3571.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005113146-01 & 5127.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005113557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005113557-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005113794-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005113809-01 & 6523.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
005113809-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005113822-01 & 0638.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005113822-02 & 0638.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005114470-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005114623-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003858884-01\\
005115178-01 & 6524.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005115178-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005115379-01 & 6525.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
005115607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005115607-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005115637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005115637-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005115688-01 & 6526.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005115778-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005119143-01 & 6527.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005119143-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005119143-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005119619-01 & 4789.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005120087-01 & 0639.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005120165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005120165-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005120225-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005120225-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005120225-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005120689-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005120689-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005121044-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005121511-01 & 0640.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005122112-01 & 0552.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005122112-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005123145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005123246-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005123246-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_005123176-pri\\
005123624-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005123624-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005124254-01 & 3099.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005124667-01 & 1822.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005125048-01 & 6528.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005125048-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005125347-01 & 2241.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005126182-01 & 4428.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005126627-01 & 6529.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005128673-01 & 2698.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005128931-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005129453-01 & 4208.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005129738-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005129738-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CENTROID\_SIGNIF\_UNCERTAIN\\
005130005-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005130369-01 & 0140.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3707.01\\
005130369-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005130380-02\\
005130380-01 & 3707.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005130380-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005130472-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005130563-01 & 5128.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005130740-01 & 3583.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005130890-01 & 6530.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005130890-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005130983-01 & 3325.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005130983-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
005131180-01 & 0641.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005131276-01 & 5129.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005164255-01 & 0824.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005164458-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005164794-01 & 6531.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005167392-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005167392-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005167392-03 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005167392-04 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005171493-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005171493-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
005171493-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005171707-01 & 6532.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005172274-01 & 6533.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005174492-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005174492-02 & 6534.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
005174492-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
005174677-01 & 5131.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
005174858-01 & 2532.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005174920-01 & 6535.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005174920-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005175024-01 & 2563.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005175986-01 & 2708.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005176531-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005176531-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005177020-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005177065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005177065-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005177065-03 & 7556.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
005177104-01 & 1603.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005177593-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005177859-01 & 4246.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005179328-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005179609-01 & 5132.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005179979-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005179979-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005179979-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005180524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005180796-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005180796-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005180796-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005181100-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005181455-01 & 6536.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005181455-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005181804-01 & 3638.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005181804-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005181817-01 & 0642.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3638.01\\
005181845-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005182131-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005182451-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005183357-01 & 1669.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005184472-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005184584-01 & 1564.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005184709-01 & 1670.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005184863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005184863-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005184911-01 & 2719.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005184911-02 & 2719.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005185032-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005185032-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005185153-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005185153-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
005185321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005185321-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005185897-01 & 2693.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005185897-02 & 2693.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005185897-03 & 2693.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005192090-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005192090-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005193077-01 & 3492.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005193384-01 & 3637.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED---PARENT\_IS\_005193386-01\\
005193384-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005193386-01 & 6537.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_005193384-01\\
005193386-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_3637.01\\
005193400-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_3637.01\\
005193439-01 & 6538.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005193659-01 & 3323.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005193735-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005195172-01 & 1671.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005195945-01 & 3940.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005196646-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005196646-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
005196787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005196787-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005196787-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005196851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
005196851-02 & 6539.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005196864-01 & 2695.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005197233-01 & 4178.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005198168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005198246-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005198390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005199426-01 & 5138.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005199772-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005199978-01 & 6540.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005200084-01 & 3159.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005200521-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005200521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005200521-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005201115-01 & 4044.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET---PARENT\_IS\_005288543-pri\\
005201115-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_005288543-pri\\
005201593-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005201619-pri\\
005201596-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005201619-pri\\
005201676-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005201619-pri\\
005201695-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_005201619-pri\\
005201756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
005201756-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005201872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005202905-01 & 1932.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005202905-02 & 1932.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005202905-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005202905-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005206128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005206128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005206233-01 & 3779.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
005206233-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005206767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005206767-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005207238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005207238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
005207710-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005207966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005207966-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005208962-01 & 4912.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005209234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005209234-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005209234-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005209669-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005209712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005209712-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005209845-01 & 2883.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005209910-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005209910-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005209910-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005210475-01 & 1568.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005211199-01 & 2158.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005211199-02 & 2158.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005211470-01 & 6541.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005211470-02 & 6541.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005211922-01 & 3273.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005212220-01 & 2495.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005212696-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005212696-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005212696-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005212696-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005212962-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005212962-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005212962-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005212962-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005213157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005213157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005213157-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005213221-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005213221-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005213230-01 & 3474.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005213404-01 & 3468.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005213902-01 & 1941.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005214214-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005215251-01 & 3903.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005215465-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005215508-01 & 6542.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005215632-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005215669-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
005215672-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005215672-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005215700-01 & 3740.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005215980-01 & 3866.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005215999-pri\\
005216727-01 & 6543.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
005217288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005217574-01 & 4151.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005217586-01 & 1592.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005217688-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
005217733-01 & 3155.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005217733-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005217791-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005217891-01 & 3036.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_005217733-pri\\
005217891-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005217910-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005217910-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005218014-01 & 6544.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005218014-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
005218441-01 & 0407.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005218441-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005218486-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005218618-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005218835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005219207-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005219207-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005219234-01 & 1563.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005219234-02 & 1563.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005219234-03 & 1563.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005219234-04 & 1563.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005219530-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005219533-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005219533-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005219533-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005219708-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005219708-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005219708-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
005219774-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005219874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005220201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005220201-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005220762-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
005220979-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005220979-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005252423-01 & 0825.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005252423-02 & 0825.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005253014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005253740-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005253740-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005253740-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005253802-01 & 4713.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005254230-01 & 5999.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005254230-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005254896-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005255552-01 & 6545.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
005255552-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005255939-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005257082-01 & 3368.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005262539-01 & 5144.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
005262664-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005262724-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005263167-01 & 6546.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005263732-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005263749-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005263749-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005263749-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005263802-01 & 5145.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005264304-01 & 3563.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005264304-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005264764-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_005264818-pri\\
005264764-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_005264818-sec\\
005264888-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005264818-sec\\
005265212-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005265699-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005265699-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005266937-01 & 6547.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
005267721-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005267721-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005267867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005267867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
005268955-01 & 7557.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005269407-01 & 6548.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005269411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005269467-01 & 1672.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005269603-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005270698-01 & 1543.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005270698-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005271090-01 & 7558.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005271224-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005271224-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005271224-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005271224-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005271608-01 & 1673.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005271803-01 & 6549.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF\\
005271803-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005272233-01 & 2711.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005272233-02 & 2711.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005272524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005272571-01 & 6550.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005097446-pri\\
005272590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005272673-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005272673-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005272673-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005272878-01 & 0826.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005273195-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005273625-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005273973-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005280587-01 & 3274.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005280983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005281113-01 & 4411.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005281249-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005281281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005281619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005281619-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005281619-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005282049-01 & 1545.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005282049-02 & 1545.02 & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_502.01\\
005282051-01 & 0502.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1545.01\\
005282345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005282477-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005282656-01 & 6551.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005283458-01 & 1547.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005283542-01 & 0827.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005283728-01 & 5149.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005284133-01 & 6552.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
005284217-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005284283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005284779-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005284779-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005285359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
005285607-01 & 6553.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
005286045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005286045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005286548-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005286780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005286780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005286786-01 & 6554.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005286786-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
005287619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005287983-01 & 0828.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005287983-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005288019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005288071-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005288071-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005288543-01 & 6555.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005288570-01 & 2136.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005288543-pri\\
005288577-01 & 4010.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005288543-pri\\
005288937-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005288937-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005289854-01 & 1593.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005289854-02 & 1593.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005289857-01 & 5150.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005289959-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
005294571-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005294571-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005294571-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005294739-01 & 6556.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
005294945-01 & 3463.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005295206-01 & 6557.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005295670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005296455-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005296647-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005296692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005296692-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005296692-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005296943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005297298-01 & 0130.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005297343-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005297343-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005297681-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005297681-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005297681-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005298310-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005298466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005298466-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005298620-01 & 6558.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_V380-Cyg-pri\\
005299459-01 & 1576.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005299459-02 & 1576.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005299596-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005299904-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005299904-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005300878-01 & 6559.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005301091-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005301091-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005301101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005301101-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005301101-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005301101-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005301474-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005301750-01 & 1589.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005301750-02 & 1589.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005301750-03 & 1589.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005301750-04 & 1589.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
005301750-05 & 1589.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005301952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005301955-01 & 6560.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005302006-01 & 1755.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005302167-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005302556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005302556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005302643-01 & 2746.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005302643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005302643-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
005302643-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005302881-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005303322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005303346-01 & 3275.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
005303346-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005303551-01 & 0553.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3982.01\\
005303557-01 & 3982.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005304184-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005304184-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005304184-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005304456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005304548-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005304634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005304634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005304819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005304819-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005304893-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005305128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005305128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005305148-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
005305237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005305240-01 & 3239.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005305404-01 & 3820.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_005217733-pri\\
005305404-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_005217733-sec\\
005305451-01 & 3843.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_005217733-pri\\
005305471-01 & 3806.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005217733-pri\\
005305553-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005305553-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005305709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005305709-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005306368-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
005306383-01 & 4158.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005306383-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005306368-01\\
005306631-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005306720-01 & 1991.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005306862-01 & 6561.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005306862-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005307271-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005307568-01 & 2804.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
005307574-01 & 6562.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005307858-01 & 2558.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005307990-01 & 3228.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005308052-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005308052-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005308052-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005308296-01 & 4750.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
005308387-01 & 2724.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---CLEAR\_APO---PARENT\_IS\_3887.01\\
005308419-01 & 3887.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---CLEAR\_APO---PARENT\_IS\_2724.01\\
005308537-01 & 4409.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005308663-01 & 1562.01 & FP & 0 & 0 & 0 & 1 & TOO\_FEW\_CENTROIDS---PARENT\_IS\_2718.01\\
005308663-02 & 1562.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005308666-01 & 2718.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1562.01\\
005308666-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
005308777-01 & 5152.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005308778-01 & 6563.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005308780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005308780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005308851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005308886-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005309078-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005309353-01 & 0643.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005309353-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005309547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005309796-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005309796-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005309849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005309849-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005310172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005310172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005310435-01 & 6564.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005310857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005310857-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005339567-01 & 2440.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005340644-01 & 0503.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005340878-01 & 4199.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005342061-01 & 2666.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005342473-01 & 2297.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005343976-01 & 6565.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005343997-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005343997-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005347537-01 & 6566.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
005347784-01 & 6567.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005350244-01 & 2555.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005350447-01 & 4008.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005350447-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005350598-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005350598-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005351250-01 & 0408.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005351250-02 & 0408.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005351250-03 & 0408.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005351250-04 & 0408.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005351540-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005352640-01 & 4467.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005353938-01 & 6568.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005354183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005354490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
005355850-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005355882-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
005356349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005356349-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005356349-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005356593-01 & 0644.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005356593-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
005356665-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005357470-01 & 1674.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005357470-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005357545-01 & 2219.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005357901-01 & 0188.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005358212-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005358241-01 & 0829.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005358241-02 & 0829.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005358241-03 & 0829.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005358323-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005358624-01 & 0830.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005359678-01 & 6569.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005360082-01 & 3768.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005360082-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
005360920-01 & 1675.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005360974-01 & 3289.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005360974-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005361145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005364071-01 & 0248.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005364071-02 & 0248.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005364071-03 & 0248.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005364071-04 & 0248.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005369827-01 & 2690.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005370023-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005370023-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005370023-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005370302-01 & 0831.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005370302-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005370646-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005370646-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005371013-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005371090-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_005371109-pri\\
005371492-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005371492-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005371676-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005371776-01 & 1557.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005371776-02 & 1557.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005371776-03 & 1557.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005371776-04 & 1557.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005371777-01 & 4327.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005371796-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005372141-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005372141-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005372310-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005372348-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005372348-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005372966-01 & 0832.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005372966-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005373377-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_003973002-sec\\
005373377-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005374279-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005374279-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005374403-01 & 2556.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005374551-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005374838-01 & 5155.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005374854-01 & 0645.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005374854-02 & 0645.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005375003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005375194-01 & 1825.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005376067-01 & 0833.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005376106-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005376614-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005376624-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005376552-sec\\
005376624-02 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM---PARENT\_IS\_005376552-pri\\
005376642-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005376552-sec\\
005376836-01 & 0182.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005376836-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005376893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005380812-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005380812-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005380812-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005380812-04 & 6570.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005381448-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005381448-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005381448-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005383248-01 & 0261.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005383476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005383615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005384079-01 & 2011.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005384079-02 & 2011.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005384183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005384194-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005384194-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
005384653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005384653-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005384713-01 & 3444.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005384713-02 & 3444.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005384713-03 & 3444.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005384802-01 & 0646.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005384802-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005385139-01 & 6000.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385139-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005385141-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005385141-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005385141-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005385150-01 & 6001.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005385150-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_V380-Cyg-sec\\
005385187-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-sec\\
005385187-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_V380-Cyg-pri\\
005385269-01 & 6002.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-pri\\
005385269-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385304-01 & 2370.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005385410-01 & 4323.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005385410-02 & 4323.02 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385410-03 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005385439-01 & 2478.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385439-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005385469-01 & 6571.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005385471-01 & 3502.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005385471-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005385491-01 & 3988.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385491-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005385509-01 & 6003.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385509-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385548-01 & 6128.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005385548-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005385548-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005385566-01 & 6004.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385566-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385575-01 & 3965.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385575-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005385647-01 & 6572.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_V380-Cyg-pri\\
005385667-01 & 6573.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-pri\\
005385667-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005385697-01 & 3967.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005385697-02 & 3967.02 & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005385750-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V380-Cyg-pri\\
005385750-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385750-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005385754-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005385754-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005385773-01 & 6005.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005385773-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005385778-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_V380-Cyg-pri\\
005385778-02 & \nodata & FP & 1 & 0 & 1 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_V380-Cyg-pri\\
005385778-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385778-04 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005385778-05 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385778-06 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005385792-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_V380-Cyg-pri\\
005385838-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V380-Cyg-pri\\
005385838-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005385838-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005385838-04 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V380-Cyg-pri\\
005385838-05 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005385838-06 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005385838-07 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-pri\\
005385838-08 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005386163-01 & 6006.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET---PARENT\_IS\_V380-Cyg-pri\\
005386163-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_CENTROIDS---PARENT\_IS\_V380-Cyg-sec\\
005386264-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_V380-Cyg-sec\\
005386264-02 & 4135.01 & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_V380-Cyg-pri\\
005386271-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005386403-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005386872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005386872-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005386872-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005386904-01 & 3813.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005387183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005387211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005387843-01 & 1762.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005388229-01 & 6574.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005388891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005389066-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005389110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005389184-01 & 6575.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005389234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005389234-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005389540-01 & 1836.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005389540-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005389856-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005389956-01 & 4591.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005390069-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005390069-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005390657-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005390672-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005390672-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005390694-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005390694-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005390694-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005390733-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005390913-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005391059-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005391059-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005391059-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005391338-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005391338-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005391416-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005391416-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005391416-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005391911-01 & 5157.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005392089-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005392089-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005392089-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005392089-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005392402-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005392413-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005392413-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005392451-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005392451-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005392514-01 & \nodata & FP & 1 & 0 & 1 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005392702-01 & 2510.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005392871-01 & 3292.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3342.01\\
005392871-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005392897-02\\
005392897-01 & 3342.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005392897-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005393558-01 & 6576.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005393558-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005393558-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005393589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005393589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005393589-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005393984-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005393984-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005393984-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005393984-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005394574-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005394574-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005395323-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
005395490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
005396122-01 & 1935.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005396122-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
005396265-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
005396265-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005396936-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005396936-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005396936-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005396950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005396950-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005397160-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005397166-01 & 3856.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005397516-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005397905-01 & 6577.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005398002-01 & 3213.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005427524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005428254-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005428254-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005428254-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005428254-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005428254-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005428471-01 & 4671.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_005513861-pri\\
005428657-01 & 6130.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005428668-01 & 2794.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
005429100-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005429100-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005429151-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
005430471-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005430471-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005430471-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005431027-01 & 4558.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
005435597-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005435597-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005435620-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005435620-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005435620-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005435620-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005435816-01 & 3696.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436013-01 & 2471.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436338-01 & 2835.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436502-01 & 0834.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436502-02 & 0834.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436502-03 & 0834.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436502-04 & 0834.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005436502-05 & 0834.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
005437206-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005437206-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005437206-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005437243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005437348-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005437348-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005437762-01 & 4907.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005437787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005437945-01 & 3791.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005437945-02 & 3791.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005438099-01 & 1567.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005438099-02 & 1567.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005438099-03 & 1567.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005438099-04 & 1567.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005438757-01 & 1601.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005438757-02 & 1601.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005440317-01 & 3141.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005440651-01 & 5168.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005440852-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005440852-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005440852-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005441980-01 & 0607.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005442047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005442451-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005442451-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005442481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005443410-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005443410-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005443410-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005443604-01 & 2713.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005443604-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005443775-01 & 1676.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005443837-01 & 0554.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005443837-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443980-01\\
005443980-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005444276-01 & 7559.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005444276-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005444334-01 & 4064.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005444392-pri\\
005444384-01 & 1778.01 & FP & 0 & 1 & 1 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005444392-01\\
005444384-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
005444392-01 & 6578.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005444491-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_005444392-01\\
005444548-01 & 0409.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005444549-01 & 1551.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
005444549-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005445681-01 & 3039.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005446009-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005446068-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005446068-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005446285-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005446285-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005446372-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005449777-01 & 0410.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005450428-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005450428-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005450503-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005450814-01 & 1780.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005450814-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005450881-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005450881-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005450881-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005450881-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005450893-01 & 2970.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005455407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005455434-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005456023-01 & 3521.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005456023-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005456359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005456359-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005456359-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
005456651-01 & 0835.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005456651-02 & 0835.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005456979-01 & 6579.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005457326-01 & 4508.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005458428-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005458779-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005458880-pri\\
005458795-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_005458880-pri\\
005458845-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_005458880-pri\\
005458845-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_005458880-sec\\
005458882-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005458882-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005458953-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_005458880-pri\\
005459805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005459805-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005459805-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005460434-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005460434-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005460835-01 & 6580.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005460835-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005460900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005460900-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005460900-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005461440-01 & 0504.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005461501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005461501-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005461501-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005461501-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005462649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005462692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005462692-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005462901-01 & 6581.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005462901-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005462901-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---KIC\_OFFSET\\
005466109-01 & 6582.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005466537-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005466537-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005466537-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005466537-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005466732-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005467102-01 & 3840.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3825.01\\
005467102-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005467113-sec\\
005467113-01 & 3825.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
005467124-01 & 2161.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3825.01\\
005467126-01 & 5171.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3825.01\\
005467531-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005467531-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005467531-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005467531-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005470739-01 & 1585.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005470851-01 & 5172.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005470960-01 & 6007.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-pri\\
005470960-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471010-01 & 6583.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471010-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005471059-01 & 3956.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005471059-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005471059-03 & 3956.02 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET---PARENT\_IS\_V380-Cyg-pri\\
005471059-04 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471068-01 & 6008.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471068-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471108-01 & 5173.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-pri\\
005471108-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471108-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005471141-01 & 6584.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005471141-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471158-01 & 3504.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471158-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471192-01 & 6009.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471192-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005471202-01 & 2911.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471202-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005471217-01 & 6010.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005471217-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471271-01 & 4155.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005471271-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471289-01 & 3485.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_V380-Cyg-pri\\
005471289-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005471328-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V380-Cyg-pri\\
005471328-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471328-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005471328-04 & 6585.01 & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V380-Cyg-sec\\
005471328-05 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471328-06 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_V380-Cyg-pri\\
005471415-01 & 6586.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_V380-Cyg-pri\\
005471415-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005471415-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005471415-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005471480-01 & 6587.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-pri\\
005471480-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM---PARENT\_IS\_V380-Cyg-sec\\
005471489-01 & 4368.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_V380-Cyg-pri\\
005471489-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471489-03 & 4368.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005471496-01 & 3914.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-pri\\
005471496-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471566-01 & 4863.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_005471619-pri\\
005471574-01 & 2505.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_005471619-pri\\
005471574-02 & 2505.02 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471574-03 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471606-01 & 3723.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---SATURATED---PARENT\_IS\_005471619-pri\\
005471619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005471619-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005471623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005471675-01 & 4000.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_005471619-pri\\
005471675-02 & 4000.02 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005471688-01 & 3499.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-pri\\
005471688-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471688-03 & 3499.02 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005471619-pri\\
005471690-01 & 4006.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_V380-Cyg-pri\\
005471690-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471690-03 & 4006.02 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_005471619-pri\\
005471769-01 & 6011.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471769-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-sec\\
005471770-01 & 6012.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V380-Cyg-pri\\
005471770-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_V380-Cyg-sec\\
005471792-01 & 4110.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V380-Cyg-pri\\
005471792-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_V380-Cyg-sec\\
005472644-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
005472644-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005472950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005472950-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005473087-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005473171-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
005473171-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005473171-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005473171-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005473535-01 & 3894.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005473535-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005473556-01 & 2939.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005473556-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005473584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005473584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005473584-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005473584-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005473611-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005474424-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005474424-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005474427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005474427-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005474427-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005474613-01 & 1599.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005474613-02 & 1599.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005474733-01 & 1610.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005475042-01 & 3050.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005475187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005475187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005475431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005475431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005475494-01 & 3969.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005475668-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005475668-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005475712-01 & 6588.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005475735-01 & 4167.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_005475712-pri\\
005475736-01 & 3798.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005475712-pri\\
005475736-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005475712-sec\\
005475736-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_005475712-sec\\
005476002-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005476273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005476273-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005476273-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005476473-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
005476473-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
005476495-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005476671-01 & 4598.02 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005476671-02 & 4598.01 & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005476864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005476864-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005476864-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005476864-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005477744-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005477805-01 & 1607.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005478055-01 & 0411.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005478083-01\\
005478083-01 & 3738.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
005478337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005478766-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005478766-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005478766-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005478788-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005479106-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005479106-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005479605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005479717-01 & 3962.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
005479800-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005479871-01\\
005479802-01 & 2251.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005479821-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005479821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005479821-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_005479800-01\\
005479871-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_005479800-01\\
005479932-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005479950-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_005479800-01\\
005479973-01 & 6589.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005480040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005480040-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005480040-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005480040-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005480114-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005480273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005480640-01 & 2707.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005480640-02 & 2707.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005480640-03 & 2707.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005480714-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005480730-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005480730-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005480736-01 & 3904.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005480736-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005480766-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005480766-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005480884-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005480884-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005481148-01 & 2701.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005481285-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005481416-01 & 0836.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3772.01\\
005481426-01 & 3772.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
005481482-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005481781-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005481781-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005481781-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005481980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005482030-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005482030-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005482030-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005482415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005482494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005482494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005482603-01 & 3199.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005511081-01 & 1930.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005511081-02 & 1930.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005511081-03 & 1930.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005511081-04 & 1930.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005511363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005511363-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005511659-01 & 4541.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005511659-02 & 4541.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005512309-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005512513-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005513012-01 & 2668.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005513648-01 & 1962.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005513822-01 & 6590.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_005513861-pri\\
005513833-01 & 6591.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005513861-pri\\
005513857-01 & 4119.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005513861-pri\\
005513866-01 & 2854.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005513861-pri\\
005513893-01 & 2741.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005513861-pri\\
005513897-01 & 2591.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_005513861-pri\\
005514283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005514283-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005514383-01 & 0257.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005517340-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005520547-01 & 2990.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005521300-01 & 2456.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005521300-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005521686-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005521686-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005522154-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005522154-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005522154-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005524229-01 & 5174.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005524881-01 & 3030.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005525210-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005525655-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005526527-01 & 1838.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005526545-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
005526545-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005526717-01 & 1677.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005527172-01 & 1678.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005527172-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005528773-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005528773-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005528773-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005529084-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005529501-01 & 6592.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_005444392-pri\\
005529552-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005444392-01\\
005529560-01 & 6593.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_005444392-pri\\
005529643-01 & 1679.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005444392-pri\\
005529738-01 & 2518.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005444392-pri\\
005530112-01 & 4067.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005530441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005530689-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005530714-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005530714-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005530714-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005530806-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005530816-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005530881-01 & 6594.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005530881-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005530882-01 & 1680.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005530881-01\\
005530935-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005530963-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005531576-01 & 0837.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531576-02 & 0837.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531657-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005531657-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005531657-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005531694-01 & 0647.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531694-02 & 0647.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531953-01 & 1681.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531953-02 & 1681.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531953-03 & 1681.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005531953-04 & 1681.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005534476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005534476-02 & 6595.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_005534702-pri\\
005534702-01 & 6596.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005534814-01 & 0838.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005534941-01 & 2332.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005534965-01 & 3557.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005535280-01 & 6597.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005535280-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005535792-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005535792-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005535792-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005535890-01 & 3865.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005536008-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005536038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005536038-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005536715-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005536715-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005536715-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005537236-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005541836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005541836-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005542211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005542211-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005542224-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005542466-01 & 1590.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005542466-02 & 1590.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005542466-03 & 1590.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005542983-01 & 2501.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005544356-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005544903-01 & 2499.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005545321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005545566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005545566-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005545815-01 & 2452.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005546277-01 & 3797.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
005546277-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005546691-01 & 2587.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005546761-01 & 2160.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005546767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005547480-01 & 0224.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005547480-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005551220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005551220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005551220-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005551220-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005551228-01 & 4154.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005551240-01 & 5178.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005551417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005551417-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
005551504-01 & 3989.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005551625-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005551625-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005551672-01 & 3119.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005551779-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005551920-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005552485-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005552562-01 & 4495.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005552761-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005552808-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005552808-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005552808-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
005552808-04 & 6598.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005553624-01 & 6599.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005553624-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005553624-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005553652-01 & 1575.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005553652-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005553959-01 & 3377.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005554685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005554685-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005556726-01 & 3223.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM---PARENT\_IS\_005471619-pri\\
005556769-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005556804-01 & 6013.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005556804-02 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_V380-Cyg-sec\\
005556830-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V380-Cyg-pri\\
005557072-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005557072-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005557072-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005557810-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005557821-01 & 1571.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005558085-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005558379-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005558379-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005558379-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005558458-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_006543496-02\\
005558458-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005558894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005558894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005559631-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005559651-01 & 4660.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005559850-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005559903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005560556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005560556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005560556-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005560556-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005560691-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005560691-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005560691-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005560731-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
005560731-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005560731-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005561278-01 & 1621.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005561316-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005561316-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005561905-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005561905-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005562090-01 & 2664.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005562784-01 & 0608.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005563024-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005563024-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005563057-01 & 5179.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005563080-01 & 4220.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005563289-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005563289-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005563300-01 & 3309.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005563507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005563507-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005563937-01 & 4406.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005563937-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
005564082-01 & 6600.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005564247-01 & 1566.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005564325-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005564325-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005564597-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005564600-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005564600-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005564600-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005565247-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005565261-01 & 5180.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005565393-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005565486-01 & 3742.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005565497-01 & 1789.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3742.01\\
005565497-02 & \nodata & FP & 1 & 0 & 1 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005565497-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005565700-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005565700-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005565700-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
005565707-01 & 4161.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005566206-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005566536-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005566536-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005566536-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005566636-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005566645-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---KIC\_OFFSET\\
005566645-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005566775-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005566775-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005566778-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005567499-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005567499-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005567711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005596440-01 & 0648.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005596440-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005597361-01 & 6601.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005597644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
005597970-01 & 6014.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005597970-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005598595-01 & 3949.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005598639-sec\\
005598639-01 & 6602.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005598645-01 & 7560.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_005598639-sec\\
005599579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005599579-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005599774-01 & 2337.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005600162-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005601258-01 & 2191.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005602405-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
005602588-01 & 2369.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005602588-02 & 2369.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005603049-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005603049-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005603049-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005607631-01 & 2254.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005607784-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005607784-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005608334-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005608334-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005608334-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005608566-01 & 0609.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005608566-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005609593-01 & 2834.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005609986-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005610698-01 & 6603.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005611160-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005611160-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005611966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005612697-01 & 3206.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005613330-01 & 0649.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005613821-01 & 2915.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005614247-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
005614247-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005614247-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005614247-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005615282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005616197-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005616250-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005616489-01 & 6604.01 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT\\
005616896-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005617102-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005617102-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005617102-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
005617110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
005617259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005617259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005617342-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005617510-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005617510-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005617510-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005617510-04 & 6605.01 & PC & 0 & 0 & 0 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---SATURATED\\
005617535-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005617535-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005617535-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005617854-01 & 1588.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005618126-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005618126-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005620305-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005620305-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005620305-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005620305-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005620395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005620654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005620654-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005620711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005621125-01 & 1814.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005621294-01 & 6606.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
005621299-01 & 6607.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005621294-pri\\
005621333-01 & 3341.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005621333-02 & 3341.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005621586-01 & 2415.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005622250-01 & 6608.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005622250-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005622396-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005622707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005622707-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005622759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005622759-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005622812-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005623833-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
005623852-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005629353-01 & 6132.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005629353-02 & 6132.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005629353-03 & 6132.03 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005629449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005629449-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005629449-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005629449-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
005629538-01 & 2345.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005629985-01 & 1578.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005630212-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005630212-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005630362-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005630362-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005630362-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005631630-01 & 2010.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005631648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005631655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005632093-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005632701-01 & 4213.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_005632781-pri\\
005632781-01 & 6609.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
005632912-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005632912-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005632912-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005633259-01 & 6610.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005636642-01 & 3817.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005636642-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005636648-01 & 1565.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3817.01\\
005636882-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005636882-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005636882-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005636937-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005637237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005637237-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005638409-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005638409-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005638429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005640085-01 & 0448.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005640085-02 & 0448.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005640438-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005640438-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005640438-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005641294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005641294-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005641294-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005641294-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005641294-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005641490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005641490-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005641711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005641711-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005641711-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005642620-01 & 2882.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005642620-02 & 2882.02 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005642620-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005642688-01 & 4705.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005643103-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005643103-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005643103-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005643201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005643201-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005643492-01 & 6015.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005643492-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005644412-01 & 4194.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005644602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005644758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005645170-01 & 4837.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005645258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005645694-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005645694-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005645788-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005645788-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005645788-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005645883-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005645883-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005645888-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005646170-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005646170-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005646170-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005646176-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005647010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005647514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005647514-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005647514-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005647638-01 & 6611.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005647974-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005648096-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005648096-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005648096-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005648096-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005648425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005648449-01 & 0979.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005648449-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005648562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005648562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005648688-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005648823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005648823-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005649177-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005649177-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005649206-01 & 3636.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005649215-01 & 0839.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3636.01\\
005649301-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005649325-01 & 2676.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---LARGE\_RM\\
005649833-01 & 2799.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3831.01\\
005649836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005649837-01 & 4078.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_3831.01\\
005649956-01 & 1540.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005649964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005649964-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005649964-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005650062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005650062-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005650062-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005650314-01 & 3731.01 & FP & 0 & 0 & 1 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
005650341-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005650341-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005650341-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005650341-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005650341-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005650420-01 & 5187.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---CLEAR\_APO\\
005650583-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005650583-02 & \nodata & FP & 1 & 0 & 1 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005650699-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005650699-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005650699-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005650699-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005651104-01 & 0840.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005651181-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005651181-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005651181-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005651327-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005651327-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005651829-01 & 4778.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
005651846-01 & 4827.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005652071-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
005652188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005652237-01 & 0164.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3703.01\\
005652260-01 & 3703.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
005652303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005652893-01 & 2790.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005652983-01 & 0371.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005652983-02 & 0371.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005653072-01 & 3252.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005653126-01 & 6612.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF\\
005653152-01 & 5189.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005653163-01 & 5190.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_6134.01\\
005653693-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005653795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005653849-01 & 3711.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---LARGE\_RM\\
005653849-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005653921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005682974-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005683743-01 & 0412.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005685699-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005685704-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005686174-01 & 0610.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005686974-01 & 6613.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_5206.01\\
005687700-01 & 4587.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005687986-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005688669-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005688683-01 & 4097.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005688683-02 & 4097.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005688790-01 & 3144.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005688910-01 & 2856.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005688997-01 & 3784.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005689351-01 & 0505.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005689351-02 & 0505.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
005689351-03 & 0505.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005689351-04 & 0505.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005689351-05 & 0505.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005693165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005693926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005695396-01 & 0283.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005695396-02 & 0283.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005695396-03 & 0283.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005695524-01 & 1897.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005695615-01 & 4756.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005695904-01 & 2983.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005695904-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005696518-01 & 7561.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005696909-01 & 6614.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
005696918-01 & 4594.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_005696909-pri\\
005696918-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005696909-sec\\
005697628-01 & 6615.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005698883-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
005700330-01 & 6616.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005700330-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005702111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005702180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005702637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005702637-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005702637-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005702770-01 & 6617.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
005702939-01 & 3000.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005703256-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_005703230-pri\\
005705411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005705411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005705575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005705575-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005705613-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005705819-01 & 2091.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005705927-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005705927-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005705927-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005706592-01 & 6618.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005706595-01 & 2183.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005706595-02 & 2183.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005706866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005706866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005706866-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005706966-01 & 1908.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005706966-02 & 1908.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005707205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
005707308-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005707308-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005707308-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005707985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005707985-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005707999-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005709664-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005709664-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005709725-01 & 0555.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005709725-02 & 0555.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005709889-01 & 2783.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005709906-01 & 4744.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
005710069-01 & 3396.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005716101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005716101-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005716244-01 & 6619.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
005716330-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005716330-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005716472-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005716763-01 & 0272.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005716932-01 & 2358.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005717140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005717140-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005717567-01 & 2752.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005718385-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005718628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
005721628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005721628-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005721632-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005721632-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005722346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005722346-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005722346-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005722737-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005722737-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005722737-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005722895-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005722895-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005722895-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005723310-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005723310-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005723310-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005724440-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005724440-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005724523-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005724523-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005724523-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005724810-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_005724811-01\\
005724810-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005724811-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005724811-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005725087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005725202-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005725312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005725312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005725312-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005725443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005725846-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005725851-01 & 6620.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_005725846-01\\
005726667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005726667-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005726667-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005726910-01 & 4124.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CROWDED\_DIFF\\
005727773-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005727773-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005727773-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005727964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005727964-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005728139-01 & 0206.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005728217-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005728217-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
005728217-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005728283-01 & 1011.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005728283-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
005728283-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
005728283-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
005728843-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005728843-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005728843-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005730389-01 & 1956.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3603.01\\
005730394-01 & 3603.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
005730445-01 & 2189.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005730714-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005730714-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005730854-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005730854-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005730867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005730867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005730867-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005730867-04 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
005731312-01 & 6621.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005731312-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005731421-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005731421-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005731451-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005731623-01 & 1793.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005731646-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005732026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005732155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005732553-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005732862-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005734003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
005734003-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005735248-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005735248-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005735762-01 & 0148.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005735762-02 & 0148.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005735762-03 & 0148.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005735878-01 & 6622.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005735878-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005736461-01 & 6623.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005736461-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005736537-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005737104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005737104-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005737166-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005737166-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005737166-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
005737687-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005737687-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005737687-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005737687-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005737869-01 & 6624.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005737902-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
005737902-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005737902-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005738127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005738127-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005738346-01 & 1006.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005738346-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005738431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005738431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005738431-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005738496-01 & 0556.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_005738506-01\\
005738496-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3676.01\\
005738506-01 & 3676.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005738506-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005738634-01 & 3951.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_6134.01\\
005738698-01 & 6134.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
005739204-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005739204-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005739204-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005739204-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005768816-01 & 3288.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005768927-01 & 6135.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005768927-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005769810-01 & 4913.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005769810-02 & 4913.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005769943-01 & 3810.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005770074-01 & 1928.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005771589-01 & 6625.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005771589-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
005771719-01 & 0190.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005771719-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005772411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005772452-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005772911-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005773121-01 & 4002.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005774349-01 & 0557.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005774375-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005774375-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005774442-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
005774557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005774557-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005774557-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005774557-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005774743-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005774743-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005774743-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005774743-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005775128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005775128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005775129-01 & 2802.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005775232-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005775232-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005775232-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005775232-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005779724-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005779852-01 & 0449.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005780269-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005780269-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005780269-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005780460-01 & 1005.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005780715-01 & 0506.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005780855-01 & 4443.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005780885-01 & 0097.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005780885-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005780930-01 & 3412.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005781192-01 & 6626.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005781774-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005781774-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005781841-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005781841-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005781841-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005781862-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005783203-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005783203-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005784777-01 & 3916.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005785279-01 & 4259.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005785707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005785707-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
005786376-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005786376-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005786676-01 & 0650.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005787131-01 & 2927.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005787972-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005787972-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005788363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005788363-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005788363-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005788363-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005790807-01 & 0259.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
005790807-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005790837-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005791720-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005791786-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005791786-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005791986-01 & 0413.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005791986-02 & 0413.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005792102-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005792093-pri\\
005792202-01 & 0841.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005792202-02 & 0841.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005792202-03 & 0841.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005792202-04 & 0841.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005792558-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005792656-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005792900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005792900-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005793275-01 & 5202.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
005793552-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005794038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005794197-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005794197-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005794197-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005794240-01 & 0254.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005794339-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED---PARENT\_IS\_005443837-02\\
005794379-01 & 0842.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005794379-02 & 0842.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005794570-01 & 2675.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005794570-02 & 2675.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005794619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005794722-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
005795522-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005795648-01 & 6016.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005795648-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005796185-01 & 3369.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005796185-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005796186-01 & 0651.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3369.01\\
005796675-01 & 0652.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005801452-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005801452-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005801452-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005801452-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005801571-01 & 0225.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005802115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
005802246-01 & 1044.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005802246-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005802285-01 & 6627.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
005802398-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005802398-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005802470-01 & 6628.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005802478-01 & 1834.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005802470-01\\
005802478-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005802470-01\\
005802479-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005802479-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005802486-01 & 1039.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005802486-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005802637-01 & 4398.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005806860-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005806860-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005806877-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005806877-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005807415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005807415-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005807415-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005807579-01 & 6629.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005807579-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005807769-01 & 2614.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005808231-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005808231-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005809372-01 & 6630.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005809890-01 & 1050.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005809890-02 & 1050.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005809954-01 & 1902.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005810113-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005810113-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005810113-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005810197-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005810806-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005811454-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005811454-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005812648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005812648-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005812701-01 & 0012.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005812960-01 & 0507.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005812973-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005812973-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005812973-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005812973-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005814013-01 & 4865.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005814635-01 & 6136.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005814635-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005814635-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005814635-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED\\
005816165-01 & 1043.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005816288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005816806-01 & 3645.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
005816811-01 & 1042.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3645.01\\
005817023-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005817023-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005817210-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005817243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005817533-01 & 4293.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_005817566-sec\\
005817533-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
005817553-01 & 1040.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_005817566-sec\\
005817566-01 & 6138.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005817613-01 & 4256.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005817566-sec\\
005817712-01 & 5204.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005817566-sec\\
005817986-01 & 2897.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005818068-01 & 3332.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
005818068-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005818165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005819013-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005819157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005819157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005819178-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005819178-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005819178-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005819801-01 & 4686.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005819807-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005819807-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005819807-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005820218-01 & 1048.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005821056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005821056-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005821056-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005821165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005821165-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005821557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
005822171-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005822286-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005823159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005823159-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005823170-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005823170-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005823587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005823587-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005823587-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
005853692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005856372-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005856571-01 & 1839.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005857540-01 & 2448.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005857714-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005857714-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005857714-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005857836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005858519-01 & 5206.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
005859725-01 & 5207.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005860347-01 & 6631.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005860848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005860968-01 & 4384.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005864975-01 & 1787.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005865654-01 & 3071.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005865766-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005865766-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005865766-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005866001-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005866001-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005866001-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005866001-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005866001-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005866098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005866098-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005866099-01 & 1055.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005866104-01\\
005866099-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_005866104-02\\
005866104-01 & 3651.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005866104-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005866555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005866555-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005866724-01 & 0085.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005866724-02 & 0085.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005866724-03 & 0085.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005868059-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005868793-01 & 4290.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005870047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005870686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005871918-01 & 6632.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005871918-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005871985-01 & 2703.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005872150-01 & 0414.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005872150-02 & 0414.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005872150-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005872552-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005872972-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005872972-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005873209-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
005873209-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005876187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005876187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005876187-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005876360-01 & 4279.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005876368-01 & 1049.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_4279.01\\
005876368-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
005876805-01 & 3331.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
005876805-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
005878307-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005878506-01 & 7562.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005879187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005879187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005879641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005880320-01 & 1060.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005880320-02 & 1060.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005880320-03 & 1060.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005880320-04 & 1060.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005880537-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005880661-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005880770-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
005881108-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005881108-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005881108-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
005881120-01 & 4156.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005881688-01 & 0843.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005881704-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005881813-01 & 2744.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005881813-02 & 2744.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005882306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005887393-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005888009-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
005888069-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005888069-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005891196-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005891196-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005891196-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005891708-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005891708-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005891975-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005891975-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005891975-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005892660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
005892660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
005892916-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005892969-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005892969-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005893123-01 & 0653.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005893839-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005893839-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005893839-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
005893839-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005894044-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005894044-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005894073-01 & 2187.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005894449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005894449-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005894549-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005894549-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005894825-01 & 6633.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
005894825-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005894972-01 & 6634.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005894972-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
005895158-01 & 3935.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005895238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
005895238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005895238-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005895588-01 & 3981.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
005896353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005896353-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005896353-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005896353-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005896439-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005896439-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005896439-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005896585-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
005897396-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005897645-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005897645-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
005897826-01 & 0126.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005897826-02 & 0126.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005898780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005898780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005898983-01 & 3422.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005899544-01 & 1034.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005899544-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
005899971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005899971-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005900235-01 & 3426.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005900260-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005900260-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005900390-01 & 4063.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005900574-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005900574-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005900574-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005902653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005903301-01 & 3692.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005903312-01 & 0008.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3692.01\\
005903453-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
005903749-01 & 3029.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005903749-02 & 3029.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005904622-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
005904699-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
005904699-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005904699-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005904928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005904928-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005905234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005905234-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005905234-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005905822-01 & 2801.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005905878-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005905878-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005906426-01 & 2377.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005906502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005906502-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005906694-01 & 4069.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005908086-01 & 7563.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005908086-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005938266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005938970-01 & 4016.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005940165-01 & 2031.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005940165-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
005940273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005940273-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005940273-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005940273-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005940490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005940490-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005940490-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005941160-01 & 0654.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005941160-02 & 0654.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005941759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005941836-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
005941836-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
005941928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005942093-01 & 1995.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005942300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005942808-01 & 2250.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005942808-02 & 2250.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005942949-01 & 2525.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005946568-01 & 5211.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005949911-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005949911-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005950759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005950759-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005951140-01 & 6635.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005952309-01 & 6636.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_6139.01\\
005952366-01 & 3947.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_6139.01\\
005952366-02 & 3947.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005952403-01 & 6139.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED---PARENT\_IS\_3947.01\\
005952403-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005952457-01 & 6637.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_6139.01\\
005953297-01 & 2733.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005953849-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
005954001-01 & 4633.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005954264-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005954795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005955321-01 & 6140.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005955321-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
005955621-01 & 4624.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
005956342-01 & 1052.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005956342-02 & 1052.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005956342-03 & 1052.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005956342-04 & 1052.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
005956354-01 & 4726.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005956656-01 & 1053.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005956656-02 & 1053.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005956776-01 & 3821.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005957093-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005957093-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005959719-01 & 2498.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005959719-02 & 2498.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005959753-01 & 0226.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005959837-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005959837-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005959837-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005959837-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005960484-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005960484-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005960899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005960899-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005960899-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005960899-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005961350-01 & 6017.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005961350-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005961350-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
005962262-01 & 4661.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005962509-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_005962514-pri\\
005962514-01 & 6639.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
005962716-01 & 6640.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
005963222-01 & 1035.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
005963222-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
005963556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005963582-01 & 2479.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005963591-01 & 5215.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005963732-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005964024-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005964069-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005964069-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005964173-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005964173-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005964173-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005964350-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005964350-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005964483-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005964483-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005965819-01 & 3319.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005965819-02 & 3319.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005965819-03 & 3319.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005965837-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005965860-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005965860-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005966154-01 & 0655.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005966154-02 & 0655.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005966212-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
005966212-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS\\
005966212-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS\\
005966322-01 & 0303.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005966660-01 & 0656.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005966732-01 & 6641.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005966810-01 & 3909.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005972334-01 & 0191.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005972334-02 & 0191.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005972334-03 & 0191.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
005972334-04 & 0191.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
005976413-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005976681-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005976681-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005977470-01 & 4550.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005977541-01 & 6642.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005977804-01 & 6643.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005977984-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005977984-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005978154-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005978170-01 & 3140.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005978295-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_006389755-01\\
005978295-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005978361-01 & 0558.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
005978436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005978559-01 & 2321.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005978559-02 & 2321.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
005978862-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
005978913-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005978913-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005979800-01 & \nodata & FP & 1 & 0 & 1 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005979863-01 & 6018.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
005979863-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005979866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005979866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005979866-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005980061-01 & 4817.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
005980061-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
005980208-01 & 2742.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005980354-01 & 5218.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
005980555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
005980783-01 & 2967.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005981039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005981039-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005981039-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005981058-01 & 5219.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
005981819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
005982073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005982353-01 & 1036.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005982353-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005982368-01 & 1041.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_005982353-pri\\
005982378-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005983348-01 & 6644.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
005983348-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005983348-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005983532-01 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
005984278-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005984278-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005984615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
005984615-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005984615-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
005984619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005985441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005985441-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005985441-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
005985713-01 & 3190.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
005986209-01 & 3476.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
005986209-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
005986209-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
005986270-01 & 5220.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
005987529-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
005988031-01 & 1047.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005988140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
005988140-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005988140-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005988140-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005988140-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005988387-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005989391-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
005989391-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
005989391-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
005990753-01 & 6645.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
005990753-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
005990915-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
005990915-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
005991070-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
005991591-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
005991591-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
005991765-01 & 4538.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005991936-01 & 2606.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005991936-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
005992210-01 & 4271.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
005992270-01 & 1855.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006019416-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006019416-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006019416-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006019416-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006019872-01 & 3942.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006019971-01 & 6646.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
006020753-01 & 0657.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006020753-02 & 0657.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006020898-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_006020929-01\\
006020929-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_006020898-01\\
006021111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006021111-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006021193-01 & 2148.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006021193-02 & 2148.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006021193-03 & 2148.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006021275-01 & 0284.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006021275-02 & 0284.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006021275-03 & 0284.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006021275-04 & 0284.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006022419-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006022556-01 & 0844.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006022792-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006022792-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006023835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006023835-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006023859-01 & 3414.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006024477-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006024477-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006025124-01 & 3411.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006025174-01 & 5224.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006025466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006026059-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006026438-01 & 2045.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006026438-02 & 2045.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006026438-03 & 2045.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006026737-01 & 2949.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006026737-02 & 2949.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006026924-01 & 4276.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006028860-01 & 2950.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006029130-01 & 6647.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006029130-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006029214-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006029239-01 & 0304.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006029239-02 & 0304.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006032172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006032172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006032172-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006032448-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006032497-01 & 0845.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006032517-01 & 2070.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006032730-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006032730-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006033602-01 & 5225.01 & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
006033640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006034945-01 & 1683.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006035124-01 & 2071.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006035335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006035335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006035335-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006035335-04 & 6648.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
006035535-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006037187-01 & 1061.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006037581-01 & 1916.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006037581-02 & 1916.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006037581-03 & 1916.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006037612-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006037612-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006037624-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006037987-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006037990-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006037990-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006038805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006039039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006041511-01 & 6649.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006041680-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006041680-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006041734-01 & 2167.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006041734-02 & 2167.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006041803-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006042031-01 & 4165.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006042116-01 & 6650.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
006042214-01 & 0450.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006042663-01 & 6651.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006042663-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006042663-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006043562-01 & 4764.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006044064-01 & 6652.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006044064-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006044188-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
006044553-01 & 2646.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006044543-pri\\
006044999-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
006045093-01 & 6653.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006045250-01 & 3948.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_006045264-pri\\
006045784-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
006046299-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006046311-01 & 6654.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006046311-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006046540-01 & 0200.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006047059-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006047059-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006047072-01 & 2100.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006047498-01 & 1013.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006048024-01 & 1684.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006048106-01 & 6655.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
006048255-01 & 6656.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006048345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
006048345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006048411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006049108-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006049190-01 & 1685.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006049886-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006050594-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
006050594-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006056992-01 & 0051.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006057080-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006057080-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006057233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006057233-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006057401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006057401-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006057401-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006057684-01 & 3972.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006057750-01 & 6657.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006058006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006058006-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006058544-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006058544-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
006058614-01 & 1799.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006058614-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006058816-01 & 3500.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006058816-02 & 3500.02 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006058830-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006058875-01 & 3616.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006058896-01 & 5233.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3616.01\\
006059860-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006060203-01 & 1059.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006060277-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006060277-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006060355-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006060355-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006060490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006060580-01 & 6658.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006060580-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006060845-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006061119-01 & 0846.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006061584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006061584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006061584-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006061773-01 & 2001.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006062088-01 & 0658.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006062088-02 & 0658.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006062088-03 & 0658.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006062766-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006062766-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006062929-01 & 2315.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006063190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006063220-01 & 0305.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006063322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006063322-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
006063322-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006063448-01 & 6659.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006063448-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006063448-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006063448-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006064237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006064237-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006065351-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006065351-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006065351-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006065651-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006065651-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006065678-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_006065699-04\\
006065699-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006065699-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006065699-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006065699-04 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_006065678-01\\
006065699-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006065823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006065823-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006065934-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006065934-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006066107-01 & 6660.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006066379-01 & 3649.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
006066403-01 & 1045.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_3649.01\\
006066416-01 & 1057.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3649.01\\
006066675-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006067545-01 & 5236.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006067707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006067707-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006067817-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006067817-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006067817-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006067942-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006068038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006068038-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
006068170-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006068502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006068947-01 & 6661.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF\\
006069985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006069985-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006070312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006070312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006070312-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006070337-01 & 4632.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006070392-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006070714-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006070714-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006071684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006071684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006071684-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006071903-01 & 0306.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006072593-01 & 3070.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006073006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006100062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006100469-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006103049-01 & 6662.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006103377-01 & 3004.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006103377-02 & 3004.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006105113-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006105113-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006105462-01 & 2098.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006105462-02 & 2098.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006106282-01 & 4087.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006109688-01 & 6663.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006109688-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006109688-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006109688-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006110119-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006111011-01 & 6664.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006113656-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006113656-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006113806-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
006113864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006113864-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006113864-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006113871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006113871-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006113871-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006114387-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006114387-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
006114387-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006114403-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006114539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006115025-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006115025-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006115466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006115466-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006115516-01 & 3134.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006115603-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006115603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006116172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006116172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006116172-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006116612-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006117415-01 & 6019.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006117832-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006118370-01 & 3458.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006118616-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006119141-01 & 2343.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CROWDED\_DIFF\\
006119407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006119407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006119788-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006119788-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006122790-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006122790-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006123324-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006123324-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006123324-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006123324-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006124426-01 & \nodata & FP & 1 & 0 & 0 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005878081-pri\\
006124512-01 & 2627.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006124836-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006124941-01 & 1058.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006125282-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_006044543-pri\\
006125481-01 & 0659.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006126012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006126076-01 & 4553.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_006045264-pri\\
006126076-02 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM---PARENT\_IS\_006045264-sec\\
006126562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006126562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006127239-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006127239-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
006127822-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006128027-01 & 6020.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006128027-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006128141-01 & 6665.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006128245-01 & 6666.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006128579-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006128830-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006128830-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006128995-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006128995-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006129524-01 & 2886.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006129694-01 & 4131.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006130500-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006130500-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006130500-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
006131130-01 & 3307.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006131236-01 & 1051.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006131659-01 & 6667.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006131659-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006132064-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006132064-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
006132064-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006132088-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006137681-01 & 3932.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3605.01\\
006137704-01 & 3605.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006137779-01 & 4728.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006138109-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006138109-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006138109-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006139220-01 & 5241.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006139591-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006139591-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006139982-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006139982-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006139982-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006140015-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
006140059-01 & 4123.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006140084-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006140581-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006141372-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006141503-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006141503-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006141725-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006142862-01 & 2336.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006142919-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006142919-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006142919-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006143315-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006143316-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006143929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006143929-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006144039-01 & 4602.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006145201-01 & 3475.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006145201-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006145471-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006145614-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006145614-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006145939-01 & 5243.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006146418-01 & 6021.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006146418-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006146838-01 & 6668.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006147122-01 & 1062.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006147122-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006147122-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006147573-01 & 6669.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006147573-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006148271-01 & 3812.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006148498-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006148498-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006149910-01 & 2469.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006150518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006150977-01 & 6022.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
006150977-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
006152521-01 & 6670.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006152521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
006152974-01 & 0216.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006152974-02 & 0216.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006153201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006153201-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006153233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006153233-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006153407-01 & 3179.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006153672-01 & 1794.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
006153673-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006153673-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006153673-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006154326-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006181674-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006181674-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006182019-01 & 6023.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006182019-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006182019-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006182093-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006182093-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006182093-03 & 6143.02 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
006182846-01 & 3591.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3512.01\\
006182846-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006182849-02\\
006182849-01 & 3512.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006182849-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
006183128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006183478-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006183478-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006183511-01 & 2542.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006184298-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006184894-01 & 5245.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006185331-01 & 1727.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006185416-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006185476-01 & 0227.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006185496-01 & 2858.01 & FP & 0 & 0 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
006185496-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
006185711-01 & 0169.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006185717-01\\
006185717-01 & 6671.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006185717-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006186029-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006186029-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006186964-01 & 2839.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006187341-01 & 4216.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006187341-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006187508-01 & 6672.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006187665-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006187665-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006187665-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006187893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006191521-01 & 0847.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006191945-01 & 6024.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006195556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006195556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006195556-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006196457-01 & 0285.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006196457-02 & 0285.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006196457-03 & 0285.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006197038-01 & 6144.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006197215-01 & 2829.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006197344-01 & 4463.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006197810-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006197810-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006198182-01 & 2636.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006198182-02 & 2636.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006198999-01 & 1687.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006199043-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_CENTROIDS\\
006199056-01 & 2398.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006199702-01 & 2211.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_1812.01\\
006199731-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006199731-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006199731-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006200235-01 & 2350.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006200709-01 & 3694.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006200709-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006200715-01 & 0451.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3694.01\\
006200810-01 & 3397.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006205228-01 & 1882.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006205384-01 & 5250.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_006205460-pri\\
006205405-01 & 5251.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_006205460-pri\\
006205460-01 & 6673.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006205460-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006205468-01 & 1037.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_006205460-pri\\
006205481-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_006205460-pri\\
006205483-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_006205460-pri\\
006205507-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_006205460-pri\\
006205852-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006205852-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006205897-01 & 1967.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006206125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006206125-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006206125-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006206143-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006206214-01 & 2252.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006206470-01 & 5252.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005962716-pri\\
006206559-01 & 3240.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_006206751-pri\\
006206627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006206627-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006206627-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006206665-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006206751-01 & 6674.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006207053-01 & 6675.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006207535-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
006208741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006209225-01 & 6676.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006209293-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006209293-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006209347-01 & 6025.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006209347-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006209637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006209677-01 & 1750.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006209677-02 & 1750.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006209798-01 & 2196.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006210148-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006210480-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006211370-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006211547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006211547-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006211812-01 & 2638.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006213774-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
006219684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006219684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006220010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006220010-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006220312-01 & 4793.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006220470-01 & 6677.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006220470-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006221385-01 & 6145.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006221385-02 & 6145.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006221385-03 & 6145.03 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006221411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006222079-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006222079-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006222381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006222381-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006222529-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006222529-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006222627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
006222884-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006222884-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006222884-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006222884-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
006222898-01 & 3896.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006222898-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006223324-01 & 4274.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006223877-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
006224148-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006224148-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006224312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006224312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006224785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006225475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006226290-01 & 2019.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006226293-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006226293-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006226293-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006226908-01 & 4068.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006227118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
006227118-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
006227118-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006227199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006227560-01 & 3650.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
006228201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006228201-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006228201-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006228201-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006228306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006228306-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006228306-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006228306-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006228371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006228703-01 & 6678.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
006229130-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006229130-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006229130-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006229502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006229502-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006229502-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006230532-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006230532-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006230921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006230921-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
006231401-01 & 6679.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006231401-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006231451-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006231451-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006231451-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006231538-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006231538-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006231538-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006231813-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006231813-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006233466-01 & 3552.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006233466-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006233483-01 & 3291.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006233466-01\\
006233483-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006233466-02\\
006233573-01 & 2725.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006233748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006233748-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006233748-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006233890-01 & 1624.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006233903-01\\
006233890-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
006233890-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006233899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006233899-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006233903-01 & 3609.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
006234144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006235301-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006263470-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006263593-01 & 3049.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006263593-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006264750-01 & 4715.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006264768-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006265665-01 & 3436.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006265792-01 & 2753.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006265961-01 & 6680.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006266219-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006266741-01 & 0508.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006266741-02 & 0508.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006266750-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006267414-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006267425-01 & 0848.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006267425-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006267535-01 & 0660.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006268017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006268531-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006268648-01 & 1613.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006268648-02 & 1613.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006268722-01 & 6026.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006268722-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006268890-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006268890-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006268890-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006269070-01 & 2608.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006272413-01 & 1129.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006273239-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006273239-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006276477-01 & 0849.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006276791-01 & 4477.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006276791-02 & 4477.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006276994-01 & 4095.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
006277167-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006277594-01 & 5255.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006278127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006278403-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006278762-01 & 3158.05 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006278762-02 & 3158.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006278762-03 & 3158.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006278762-04 & 3158.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006279388-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006279388-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006279388-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006279696-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006279823-01 & 6681.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006279974-01 & 1812.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006280952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006280952-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006280952-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006283224-01 & 6682.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006283224-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006284209-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006284363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006285094-01 & 6683.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_TT-Lyr-pri\\
006285396-01 & 6684.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006285397-01 & 6685.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006285545-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_TT-Lyr-pri\\
006285985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006285985-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006286155-01 & 3803.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_006286161-01\\
006286155-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3501.01\\
006286161-01 & 3501.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006286161-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006287169-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006287313-01 & 2221.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006287517-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006287517-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006288034-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006288034-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CENTROID\_SIGNIF\_UNCERTAIN\\
006288034-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
006288896-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006289081-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006289257-01 & 0307.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006289257-02 & 0307.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006289344-01 & 4319.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006289468-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006289468-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006289468-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006289468-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006289650-01 & 0415.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006289739-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006289897-01 & 5260.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_006048106-pri\\
006290382-01 & 3869.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
006290382-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
006290382-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006290411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006290411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006290648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006290648-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006290935-01 & 4302.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006291033-01 & 0452.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006291110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006291473-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006291653-01 & 0850.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006291837-01 & 0308.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006292162-01 & 1125.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006292162-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006292398-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006292452-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006292452-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006292732-01 & 6686.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006293266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006294556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006294556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006294556-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006294819-01 & 2852.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006294889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006294889-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
006300348-01 & 0212.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006301030-01 & 6027.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006301030-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006301030-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006301030-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
006301035-01 & 1124.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006301030-02\\
006301035-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_6027.01\\
006301132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006301428-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006301428-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006301745-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006301745-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006301745-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006301745-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006301749-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006302589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006302589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006302589-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006302655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006302655-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006302655-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006302655-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006302655-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
006302903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006302903-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006303436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
006303679-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006305192-01 & 0219.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006305572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006305572-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006305572-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006305938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006306896-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006306896-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006307000-01 & 6687.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006307062-01 & 3153.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006307062-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006307062-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
006307063-01 & 2702.01 & FP & 0 & 1 & 0 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_5:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_006307062-01\\
006307063-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006307062-01\\
006307063-03 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_006307062-02\\
006307083-01 & 2050.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006307062-01\\
006307083-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006307062-01\\
006307083-03 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_006307062-02\\
006307083-04 & 2050.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006307243-01 & 7564.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---EYEBALL---SATURATED\\
006307521-01 & 1126.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_006307537-pri\\
006307521-02 & 1126.02 & PC & 0 & 0 & 0 & 0 & PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_8:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006307537-01 & 1120.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006307537-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006308416-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006308416-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006308416-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006309129-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006309129-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006309264-01 & 3387.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006309763-01 & 0611.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006310397-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006310397-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006310397-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006310414-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006310636-01 & 1688.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006310929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
006310979-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006311382-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006311520-01 & 4115.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006311520-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006311520-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006311564-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006311637-01 & 6688.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006311681-01 & 1122.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
006311891-01 & 4627.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006312314-01 & 1625.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006312521-01 & 3656.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
006312534-01 & 1689.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_3656.01\\
006312643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006314173-01 & 3708.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006314185-01 & 3752.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3708.01\\
006314185-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED---PARENT\_IS\_006314173-sec\\
006314475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006314475-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006341932-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006342333-01 & 2065.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006342398-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006342566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006343170-01 & 2419.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006343576-01 & 4438.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_3512.01\\
006344431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006344431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006345732-01 & 2857.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006345732-02 & 2857.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006345758-01 & 6689.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006346698-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006346698-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006346698-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006346721-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006346809-01 & 2775.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006346894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006347258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006347299-01 & 0661.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006347299-02 & 0661.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006349881-01 & 4121.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006350031-01 & 5267.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006350476-01 & 2710.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006350522-01 & 7565.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
006350882-01 & 4410.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006351097-01 & 2618.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006352349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CENTROID\_SIGNIF\_UNCERTAIN\\
006356207-01 & 2021.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006356627-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_005007640-01\\
006356627-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006356627-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006356627-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006356692-01 & 2948.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006356928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006356928-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006356928-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006357290-01 & 3040.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006357667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006357702-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006357702-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
006357702-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006357702-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006357795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006357795-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006357958-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006358937-01 & 4794.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006359228-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006359320-01 & 1127.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006359320-02 & 1127.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006359320-03 & 1127.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006359798-01 & 1121.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
006359798-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
006359802-01 & 3399.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_1121.01\\
006359802-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_006359798-02\\
006359802-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006359802-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006359926-01 & 4391.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006362386-01 & 6146.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006362386-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006362386-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006362874-01 & 1128.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006363494-01 & 3634.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
006363560-01 & 5270.02 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_006363494-pri\\
006363900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006363900-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006364064-01 & 5271.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_TT-Lyr-pri\\
006364067-01 & 4221.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006364126-01 & 6690.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_TT-Lyr-pri\\
006364143-01 & 5272.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006364162-01 & 2889.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006364195-01 & 6691.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_TT-Lyr-pri\\
006364200-01 & 6692.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_TT-Lyr-pri\\
006364215-01 & 2404.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006364215-02 & 2404.02 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006364247-01 & 6693.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006364276-01 & 2873.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_TT-Lyr-pri\\
006364294-01 & 6694.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_TT-Lyr-pri\\
006364307-01 & 5273.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_TT-Lyr-pri\\
006364327-01 & 1744.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_TT-Lyr-pri\\
006364582-01 & 3456.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006365076-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006365156-01 & 0662.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006365321-01 & 1123.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006366501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006366501-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006366501-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006366501-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006366501-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006366512-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006366512-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006366512-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006366617-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006366617-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006366617-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006367260-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006367365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006367439-01 & 6695.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_006367628-pri\\
006367628-01 & 6696.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006368175-01 & 3503.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006368175-02 & 3503.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006368222-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006368222-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006368222-03 & 6697.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006368230-01 & 3356.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006368414-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006368414-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006368414-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006368905-01 & 5276.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006369131-01 & 4554.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006369222-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006369539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006370120-01 & 2811.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_CENTROIDS\\
006371322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006371322-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006371322-03 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---KIC\_OFFSET\\
006372135-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006372194-01 & 5278.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006372268-01 & 6698.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
006372268-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED\\
006372268-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
006372320-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006372320-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006372633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006372633-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006372942-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006373680-01 & 2127.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006374004-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006374004-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006374063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006374063-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006380217-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006380533-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
006380544-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006380544-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006380593-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006380631-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006380750-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006381128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006381128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006381128-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006381128-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006381306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006381306-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006381309-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006381517-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006381517-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006381846-01 & 0509.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006381846-02 & 0509.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006381846-03 & 0509.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006382217-01 & 2036.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006382217-02 & 2036.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006382916-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006382916-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006382943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006383595-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006383595-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006383785-01 & 0239.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006383785-02 & 0239.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006383821-01 & 1238.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006383932-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006383932-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006383932-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006384840-01 & 6699.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006385010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006385010-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006385302-01 & 7566.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
006385943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006386598-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006386784-01 & 6700.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_006545018-pri\\
006386823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006387185-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006387185-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006387257-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006387257-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006387257-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006387450-01 & 1228.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
006387450-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
006387542-01 & 1626.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006387557-01 & 5279.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006387591-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
006387591-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
006387819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006387819-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006387819-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
006387887-01 & 5280.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006387887-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006387895-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006387895-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006387895-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006388333-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006388333-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006388333-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006388443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006388443-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006388443-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006388466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006388466-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006388770-01 & 3035.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006388994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006388994-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006389098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006389098-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006389098-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006389396-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
006389755-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006390013-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006390080-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006390080-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006390080-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006390236-01 & 6701.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED---PARENT\_IS\_006390205-pri\\
006390236-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED---PARENT\_IS\_006390205-pri\\
006390243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
006390243-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006390824-01 & 1234.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006391733-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
006392244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006392581-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006392581-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006392601-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006392601-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006392727-01 & 0851.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006421137-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006421188-01 & 6702.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006421188-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006421483-01 & 6703.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006421503-01 & 3990.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006421483-pri\\
006421759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006421759-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006421759-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006421759-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006421937-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006421937-02 & 6704.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_3:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_3:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006421937-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006422070-01 & 0852.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006422155-01 & 0510.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006422155-02 & 0510.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006422155-03 & 0510.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006422155-04 & 0510.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006422367-01 & 0559.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_005343976-pri\\
006423922-01 & 6705.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006424561-01 & 4900.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006425135-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006425597-01 & 4861.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006425957-01 & 0663.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006425957-02 & 0663.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006426158-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006426158-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006426158-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006426158-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006426158-05 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006426158-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006426592-01 & 3554.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
006426592-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006428700-01 & 0853.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006428700-02 & 0853.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006428794-01 & 4054.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006428850-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006428850-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006428850-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006428850-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006428850-05 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
006428942-01 & 6706.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
006429742-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006429742-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006429742-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006429812-01 & 2408.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006430330-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006430330-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006431624-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006431670-01 & 3534.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006431670-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006432054-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006432054-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006432054-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006432054-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006432059-01 & 1229.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006432345-01 & 2757.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006435936-01 & 0854.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006436029-01 & 2828.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006436029-02 & 2828.02 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
006436505-01 & 6707.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
006437719-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006437993-01 & 6708.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---KIC\_OFFSET\\
006438099-01 & 2976.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006438216-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006440528-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
006440685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006441258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006441258-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006441436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006441436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006441729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006441729-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006441729-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006441729-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006441738-01 & 1246.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006441836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006441836-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006442060-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006442060-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006442193-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006442246-01 & 6709.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_006521542-pri\\
006442340-01 & 0664.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006442340-02 & 0664.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006442340-03 & 0664.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006442377-01 & 0176.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006442735-01 & 5283.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006443093-01 & 5284.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006443122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006443122-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006443122-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006443274-01 & 7567.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006443392-01 & 6710.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006443392-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006444896-01 & 3138.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006445116-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006445601-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006445969-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006446130-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006446951-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006446951-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006447258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006447258-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006447258-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006447258-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006447326-01 & 6711.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
006448173-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006448173-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006448173-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006448362-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006448362-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006448362-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006448666-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006448768-01 & 6712.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
006448768-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006448768-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
006448768-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006448890-01 & 1241.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006448890-02 & 1241.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006449291-01 & 6713.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_006449358-pri\\
006449358-01 & 6147.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006449552-01 & 6714.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006449552-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006449552-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
006449552-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
006450067-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006450067-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
006450067-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006450067-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---KIC\_OFFSET\\
006450934-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006450934-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006451125-01 & \nodata & FP & 1 & 0 & 1 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
006451160-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006451160-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006451160-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
006451160-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006451294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006451294-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006451605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006451605-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006451605-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006451876-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006451876-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006451936-01 & 0511.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006451936-02 & 0511.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006452607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006452607-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
006452607-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006452742-01 & 6715.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
006452742-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
006452742-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006460857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006460857-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006461219-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006461219-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006461601-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006461601-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006461850-01 & 3054.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006462033-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006462033-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006462033-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006462033-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006462863-01 & 0094.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006462863-02 & 0094.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006462863-03 & 0094.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006462863-04 & 0094.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006462874-01 & \nodata & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_17:1---CLEAR\_APO---PARENT\_IS\_94.01\\
006462874-02 & \nodata & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_94.01\\
006462901-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006462901-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006462901-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006463047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006463047-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006463436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006463436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006463436-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006463499-01 & 4163.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006463772-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006463772-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006464285-01 & 6716.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006464285-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006464938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006464938-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006464938-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006465159-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_006629588-pri\\
006465159-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006466443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006466583-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006466583-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006466939-01 & 6717.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
006467349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
006467363-01 & 2840.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006467363-02 & 2840.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006467826-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006468089-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006468138-01 & 1826.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006468337-01 & 1620.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006468848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006468904-01 & 4743.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006468938-01 & 6718.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006468938-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006468987-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006468987-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006468987-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006468987-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006469599-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006469599-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006469690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006469690-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006469690-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006470149-01 & 1230.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006470232-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006470232-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006470232-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006470516-01 & 3705.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006470516-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
006470521-01 & 3701.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3705.01\\
006470917-01 & 1690.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006470973-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006470973-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
006470973-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CENTROID\_SIGNIF\_UNCERTAIN\\
006470998-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006470998-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006471021-01 & 0372.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006471229-01 & 6719.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_5335.01\\
006471230-01 & 6720.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5335.01\\
006471244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006471490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006497146-01 & 3284.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006500206-01 & 2451.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006500206-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006500714-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006501635-01 & 0560.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006503434-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006504534-01 & 3152.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006504534-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006504954-01 & 1790.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006507427-01 & 2455.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_3815.01\\
006507433-01 & 3815.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006508221-01 & 0416.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006508221-02 & 0416.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006508221-03 & 0416.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006508221-04 & 0416.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006508478-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006508478-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006508478-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006508478-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006508734-01 & 7568.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
006508943-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
006509175-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006509175-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006509175-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006509175-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006509282-01 & 5287.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006509328-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
006509713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006509713-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006510059-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006510174-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006510174-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006511019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006511019-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006511019-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006511019-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006511182-01 & 5288.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006511354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006511354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006511354-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006511799-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
006511799-02 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED---PARENT\_IS\_005443837-02\\
006515246-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006515488-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006515722-01 & 3818.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006515722-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006515722-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006515722-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006515722-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006516185-01 & 2445.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006516825-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006516874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006516874-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006517512-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006519892-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006520011-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006520011-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006520259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
006520519-01 & 4749.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
006520533-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006520658-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006520753-01 & 4504.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
006520753-02 & 4504.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006520923-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006520969-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006521045-01 & 0041.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006521045-02 & 0041.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006521045-03 & 0041.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006521110-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
006521110-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006521136-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006521136-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006521174-01 & 6721.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006521542-01 & 6722.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006522144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006522144-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006522179-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006522179-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
006522242-01 & 0855.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006522353-01 & 6723.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006522735-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006522735-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006522735-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006522745-01 & 4574.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_006522750-01\\
006522750-01 & 6724.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
006522750-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
006522750-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006522823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006522823-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006522823-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006522824-01 & 4882.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_006522750-01\\
006523058-01 & 4549.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006523216-01 & 6725.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006523216-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006523259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006523351-01 & 3117.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006523440-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006523440-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006523587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
006525106-01 & 4483.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_5293.01\\
006525185-01 & 2568.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5293.01\\
006525193-01 & 2653.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5293.01\\
006525196-01 & 5293.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
006525209-01 & 3479.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006525209-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006525209-03 & 3479.02 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_5293.01\\
006525249-01 & 2197.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_5293.01\\
006525280-01 & 4277.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_5293.01\\
006525462-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_006367628-pri\\
006525946-01 & 2093.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006525946-02 & 2093.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006525946-03 & 2093.03 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006525946-04 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006526377-01 & 5295.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006526568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006526568-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006526710-01 & 0856.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006526875-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006526875-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006527050-01 & 7569.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006527078-01 & 4657.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006527078-02 & 4657.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006527090-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006527229-01 & 5296.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006527363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006527363-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006527579-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
006528048-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006528141-01 & 4340.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006528464-01 & 0270.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006528464-02 & 0270.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006528720-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006528744-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006529378-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006529483-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006529483-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006530137-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006531485-01 & 6726.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006531485-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006531491-01 & 1237.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3646.01\\
006531491-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006531496-02\\
006531491-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
006531496-01 & 3646.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
006531496-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
006531496-03 & \nodata & FP & 1 & 0 & 1 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_006531491-03\\
006531801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006531801-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
006531801-03 & 6727.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006535143-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006535143-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006535143-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006535166-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006541920-01 & 0157.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006541920-02 & 0157.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006541920-03 & 0157.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006541920-04 & 0157.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
006541920-05 & 0157.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006541920-06 & 0157.06 & PC & 0 & 0 & 0 & 0 & \nodata\\
006542001-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006542001-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
006542751-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006542751-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006542751-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006542790-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006542790-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006543192-01 & 5297.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006543441-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---TOO\_FEW\_QUARTERS\\
006543496-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006543496-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006543645-01 & 4679.01 & FP & 0 & 0 & 0 & 1 & CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_006543682-01\\
006543674-01 & 5298.01 & FP & 0 & 0 & 0 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED---PARENT\_IS\_006543682-01\\
006543682-01 & 6728.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
006543683-01 & 3769.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006543682-01\\
006543893-01 & 1627.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006543893-02 & 1627.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006543893-03 & 1627.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006544977-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006544977-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006544977-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006545018-01 & 6729.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006545051-01 & 2777.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006545018-pri\\
006545358-01 & 1233.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
006545358-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006545358-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006545358-04 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
006545986-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006545986-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006546327-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006546327-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006546456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006546508-01 & 3613.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
006546528-01 & 1235.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006546508-01\\
006546582-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006546582-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006546614-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
006548447-01 & 6730.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006548447-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006548709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006548709-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006549466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006549623-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_005033298-01\\
006550607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006551106-01 & 6731.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006551110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
006551110-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006579643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
006579643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006579643-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006579806-01 & 0967.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006579806-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006584042-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006584042-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006584167-01 & 6732.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_006669809-pri\\
006584273-01 & 3287.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006584278-01 & 6733.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006586052-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006586052-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006586333-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006586333-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006586333-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006586746-01 & 2747.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587002-01 & 0612.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587002-02 & 0612.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587002-03 & 0612.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587105-01 & 2721.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587280-01 & 0857.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587280-02 & 0857.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587458-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006587458-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006587551-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006587551-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006587796-01 & 3237.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006587796-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006590362-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
006590362-02 & 7570.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
006590403-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
006590403-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006590403-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006590403-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006590726-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006590726-02 & 6734.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006591789-01 & 6735.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006591789-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006592335-01 & 4777.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006592832-01 & 4082.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
006593140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006593140-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
006593150-01 & 3037.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006593353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006593353-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006593363-01 & 6736.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006593363-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006593488-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006593734-01 & 4722.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006594972-01 & 6737.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006594972-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006595315-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006595315-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006595406-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006595406-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006595662-01 & 6738.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006595662-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006599881-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006599919-01 & 0858.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006599975-01 & 3438.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006603026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006603043-01 & 0368.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---SATURATED\\
006603087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
006603113-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
006603756-01 & 1729.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006603756-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006603765-01 & 6739.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006604303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006604303-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006604303-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006604303-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006604328-01 & 1736.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006605493-01 & 2559.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006606229-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006606229-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006606229-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006606229-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006606282-01 & 6740.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
006606438-01 & 2860.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006606481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006606653-01 & 1224.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006606653-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006606653-03 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
006606669-01 & 6741.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006606756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006606934-01 & 6028.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006606934-02 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
006607150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006607150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006607191-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006607286-01 & 1239.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006607286-02 & 1239.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006607357-01 & 2838.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006607357-02 & 2838.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006607447-01 & 1242.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006607610-01 & 6742.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006607610-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006607644-01 & 4159.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006609270-01 & 3090.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006609270-02 & 3090.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006610064-01 & 4529.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006610219-01 & 6743.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
006610433-01 & 6744.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006611330-01 & 1691.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006611476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006612284-01 & 2908.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF---PARENT\_IS\_006206751-pri\\
006612327-01 & 3270.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006612327-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006612353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006612411-01 & 5305.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006612411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006612411-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006612411-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006612589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006612589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006613006-01 & 1223.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006613006-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006613627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006614168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006614168-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006614168-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006614492-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006614492-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006614629-01 & 2737.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006614630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006614748-01 & 6745.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006614892-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006614892-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006614892-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006614926-01 & 6029.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006614926-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006615511-01 & 3306.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006615600-01 & 5307.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006616211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006616211-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006616211-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006616218-01 & 1692.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006616218-02 & 1692.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006619815-01 & 3361.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006619830-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006619854-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006619942-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006620003-01 & 1225.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006620691-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006621116-01 & 1226.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006621280-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006621643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006627507-01 & 2697.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006627684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006627684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006628008-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006628237-01 & 6030.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
006628237-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006628740-01 & 7571.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006628926-01 & 6746.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006629106-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006629106-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006629156-01 & 6747.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006629156-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006629156-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
006629332-01 & 1227.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006629588-01 & 6748.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006629993-01 & 4392.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006630507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006630943-01 & 2738.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006631188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006631188-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006631188-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006631721-01 & 0160.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006632383-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006632435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006632945-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006632945-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006632945-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006633452-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
006633452-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006633452-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006633952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006634112-01 & 5308.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006634133-01 & 2262.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5308.01\\
006635026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006635026-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006635493-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006635493-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006635493-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006636020-01 & 6749.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006636041-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006636067-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006636320-01 & 2989.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006664842-01 & 6750.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006665064-01 & 6751.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006665064-02 & 6751.02 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006665223-01 & 1232.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006665512-01 & 2005.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006665695-01 & 0561.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006665860-01 & 4840.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006666233-01 & 2306.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006668712-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006668729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006668729-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006670075-01 & 2382.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006670373-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006670373-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006670610-01 & 6752.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006670742-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006670742-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006670742-03 & 6753.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006670894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006670894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006670894-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006670894-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006672229-01 & 6754.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED\\
006672229-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006672229-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
006674908-01 & 6149.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006675056-01 & 0859.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3611.01\\
006675060-01 & 3611.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006675318-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006675944-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006675944-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006675944-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006676174-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006676174-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006676516-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006676725-01 & 6755.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006677256-01 & 1243.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006677267-01\\
006677256-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006677267-02\\
006677267-01 & 3622.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
006677267-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006677841-01 & 1236.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006677841-02 & 1236.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006677841-03 & 1236.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006678383-01 & 0111.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006678383-02 & 0111.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006678383-03 & 0111.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006678614-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006679295-01 & 2862.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006681473-01 & 5312.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006685526-01 & 0861.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006685609-01 & 0665.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006685609-02 & 0665.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006685609-03 & 0665.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006690082-01 & 1240.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006690082-02 & 1240.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006690171-01 & 3320.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006690343-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006690836-01 & 2699.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006690940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006690940-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006691169-01 & 4890.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006691244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006691244-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
006691244-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006691244-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006691244-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006691244-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006692833-01 & 1244.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006693640-01 & 1245.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006694186-01 & 6031.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006694649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006694649-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006695329-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006695622-01 & 6756.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006695801-01 & 5316.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_006695889-pri\\
006695889-01 & 6757.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006696381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006696381-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006696462-01 & 1693.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006696580-01 & 2092.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006696580-02 & 2092.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006696580-03 & 2092.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006696713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006697128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006697128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006697518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006697605-01 & 2851.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006697605-02 & 2851.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006697609-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006697609-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006697609-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006697609-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006697716-01 & 6758.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
006697756-01 & 2798.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006697817-01 & 3508.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006697976-01 & 6759.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006698670-01 & 6760.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006698670-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006699023-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006699368-01 & 1694.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006699562-01 & 5317.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006699984-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006700200-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006700200-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006700870-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006700870-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006701115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006701115-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006701459-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006701459-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
006705026-01 & 3374.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006705026-02 & 3374.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006705137-01 & 2609.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_1758.01\\
006705142-01 & 1758.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006706000-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006706038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006706199-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006706287-01 & 6761.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
006706982-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006707691-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006707691-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006707691-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006707833-01 & 0563.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006707835-01 & 0666.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006707908-01 & 2014.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006707942-01 & 3569.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
006707942-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006708053-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006715221-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006715331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006715434-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006715434-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006715434-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006715577-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006715577-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006715809-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006715809-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006715809-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006715809-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006715997-01 & 6762.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006716021-01 & 2679.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006716161-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
006716161-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
006716545-01 & 2906.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006716670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006716670-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006717252-01 & 4651.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006717417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006717417-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006717417-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006718300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006719086-01 & 1357.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006719266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006719266-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006720188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006720363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006720363-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006720720-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006720720-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006720720-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006720889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006720889-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006720889-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006721089-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006721089-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006721089-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006721123-01 & 0114.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006721123-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006721380-01 & 4488.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006721523-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006721523-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006721523-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006721523-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006721526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006721526-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006721727-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006750902-01 & 3980.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006750902-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006751874-01 & 2282.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006752002-01 & 4184.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006752043-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006752502-01 & 0667.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006752876-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006752876-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006752876-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006755676-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006755944-01 & 4072.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006756202-01 & 3547.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
006756386-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006756386-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006756386-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006756481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006756481-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006756669-01 & 0862.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006756669-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006757075-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006757160-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006757160-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006757160-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006757160-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006758917-01 & 0453.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006758917-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006761498-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006761539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006761539-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006761539-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006761539-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006761777-01 & 4571.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006762188-01 & 5323.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006762829-01 & 1740.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006762829-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006762829-03 & \nodata & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006762829-04 & \nodata & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
006762992-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006762992-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006762992-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006763132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006763633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
006763633-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006763884-01 & 6763.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006765135-01 & 2592.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006765518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006765518-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006765575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
006765575-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006765575-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
006766634-01 & 1375.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006766748-01 & 6764.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006766990-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006767227-01 & 4871.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006767227-02 & 4871.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006767337-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006767840-01 & 2506.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006768394-01 & 2086.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006768394-02 & 2086.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006768394-03 & 2086.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006768616-01 & 6765.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006773862-01 & 1868.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006774408-01 & 6766.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006774408-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
006774537-01 & 2146.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006774826-01 & 1376.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006774880-01 & 2062.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006775985-01 & 3780.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006776331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006776331-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006776331-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006776401-01 & 1847.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006776555-01 & 5327.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006776957-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006777016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006777360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006777538-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006777538-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006777538-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006778008-01 & 4373.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006778050-pri\\
006778008-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006778050-sec\\
006778019-01 & 2953.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006778050-pri\\
006778019-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006778050-sec\\
006778050-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006778063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006778063-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006778063-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006778274-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006778289-01 & 6767.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006778289-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006779260-01 & 2678.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006779726-01 & 3375.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006780052-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006780158-01 & 2231.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006781047-01 & 6768.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS\\
006781047-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
006781535-01 & 6769.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006781535-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006781548-01 & 2944.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006781535-01\\
006781548-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006781535-02\\
006782960-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006783365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006783562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006783879-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006783879-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006783879-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006784155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006784155-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006784155-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006784235-01 & 0863.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006784887-01 & 5328.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006785401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006785401-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006785401-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006785967-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006786037-01 & 0564.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006786037-02 & 0564.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006786037-03 & 0564.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006786224-01 & 4850.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006786348-01 & 1749.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006789950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
006790335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006790335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006790346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006790346-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006790451-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006790451-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006791090-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006791090-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006792124-01 & 6770.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_006791604-pri\\
006792908-01 & 4341.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006792983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006793409-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006793409-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006793409-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006794857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006801692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006801692-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006802081-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006802081-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006802602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006803202-01 & 0177.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006803855-01 & 1695.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006803964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006803964-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006804592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006804592-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006804648-01 & 6771.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
006804821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006804821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006804957-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006804957-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006804957-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006805146-01 & 0668.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006805146-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006805146-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006805146-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006805146-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006805414-01 & 5329.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006806122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006806122-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
006806632-01 & 6772.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006806632-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006806695-01 & 4061.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
006806695-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
006806724-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006836589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006836589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006836658-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006836658-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006836871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006837146-01 & 1362.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006837283-01 & 2914.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006838050-01 & 0512.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006838565-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006838565-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006838565-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006838565-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
006839010-01 & 4674.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006841577-01 & 6773.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006842139-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006842139-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006842139-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006842345-01 & 6774.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006842682-01 & 2649.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006842807-01 & 2921.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006843454-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006844024-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006846911-01 & 2477.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006847018-01 & 1349.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006847018-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006848584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006849046-01 & 0201.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006849310-01 & 0864.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006849310-02 & 0864.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006849310-03 & 0864.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006850504-01 & 0070.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006850504-02 & 0070.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006850504-03 & 0070.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006850504-04 & 0070.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006850504-05 & 0070.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
006850665-01 & 3244.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006851425-01 & 0163.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006851827-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006852488-01 & 6775.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006853172-01 & 6776.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
006853248-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006854461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006854623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006854623-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006854623-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006859437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006859437-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006859546-01 & 6777.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006859619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006859801-01 & 3321.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_006859813-01\\
006859801-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006859813-02\\
006859813-01 & 6778.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006859813-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006860836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006860836-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006860968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
006860968-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006860968-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006861403-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
006861403-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_RR-Lyr-pri\\
006862114-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006862328-01 & 0865.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006862332-01 & 4023.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_865.01\\
006862333-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006862333-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006862333-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006862603-01 & 0866.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
006862603-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
006862721-01 & 1982.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006862920-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006862920-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006862920-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006862920-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006863161-01 & 3757.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---TOO\_FEW\_QUARTERS\\
006863161-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
006863839-01 & 1373.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_006863840-01\\
006863840-01 & 6779.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006863998-01 & 0867.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006864276-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006864276-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006864276-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006864536-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
006864569-01 & 6780.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
006864569-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
006864569-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006864706-01 & 6781.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
006864859-01 & 6782.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006864859-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006864859-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006864885-01 & 2434.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006864859-02\\
006864885-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006864859-01\\
006864891-01 & 5330.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_006864859-01\\
006864891-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_006864859-02\\
006864893-01 & 2375.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006864859-01\\
006864893-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006864859-02\\
006865077-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006865077-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006865077-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006865966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006866122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
006866228-01 & 1348.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006866228-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006866346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006867155-01 & 0868.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006867219-01 & 6783.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006867555-01 & 2439.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006867555-02 & 2439.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006867588-01 & 2571.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006867766-01 & 1798.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006868952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006869184-01 & 1732.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006869292-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_006869313-01\\
006869313-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_006869292-01\\
006869345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006869373-01 & 5331.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006870432-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
006870438-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006871071-01 & 2220.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006871071-02 & 2220.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006871071-03 & 2220.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006871071-04 & 2220.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006871350-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006871390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006871462-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006871672-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006871672-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006871866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006871866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CENTROID\_SIGNIF\_UNCERTAIN\\
006875337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006875342-01 & 5332.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006876575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006876575-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006876575-03 & 7572.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006876878-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006876878-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006877258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006877311-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006877609-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006877609-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006877673-01 & 6784.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
006877673-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006877871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006877871-02 & 6785.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006877871-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006878167-01 & 1371.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006878173-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006878240-01 & 2681.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006878240-02 & 2681.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006878288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006878288-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006878408-01 & 6786.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
006878641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006879171-01 & 4188.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006879183-01 & 5333.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006879594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006879594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006879594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006879787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006879865-01 & 0417.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006880517-01 & 3305.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006881829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006887746-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006887746-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006887746-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006887983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006889190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006889190-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006889190-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006889235-01 & 0074.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
006889235-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
006889235-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006890618-01 & 6787.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED\\
006891366-01 & 1696.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CROWDED\_DIFF---PARENT\_IS\_5335.01\\
006891512-01 & 5335.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
006891513-01 & 4413.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006891543-01 & 1354.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5335.01\\
006891543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
006891543-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
006891637-01 & 1697.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5335.01\\
006891998-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006891998-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006891998-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006921944-01 & 2114.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006922203-01 & 2578.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006922244-01 & 0010.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006922690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006922690-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006922710-01 & 2087.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006922834-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006922995-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006922995-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006922995-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006923424-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006923424-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006923424-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006924203-01 & 1370.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006924968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006924968-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006925263-01 & 6788.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
006927556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006927556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006927629-01 & 6789.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006928906-01 & 3242.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
006929016-01 & 6790.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_006669809-pri\\
006929285-01 & 4572.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006929583-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006929841-01 & 3026.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006929841-02 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006932987-01 & 1366.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006932987-02 & 1366.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006933567-01 & 2643.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006933781-01 & 3737.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
006933781-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
006934045-01 & 5336.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006934291-01 & 1367.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006934306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006934587-01 & 6032.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006934587-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
006934986-01 & 2294.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006935020-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006935020-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006935020-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006935062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
006935062-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
006935101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006935101-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006935850-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006936025-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006936038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006936075-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
006936075-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM---PARENT\_IS\_FN-Lyr-pri\\
006936075-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_FN-Lyr-pri\\
006936115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006936178-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
006936261-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006936909-01 & 1363.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006936909-02 & 1363.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006936977-01 & 6791.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
006937131-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
006937131-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006937199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006937402-01 & 2894.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006937529-01 & 4382.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006937692-01 & 0513.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006937758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006937758-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006937758-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006938584-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006939203-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006939291-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006939291-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006939670-01 & 6792.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
006939670-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
006940255-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006941084-01 & 2348.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006945362-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006945362-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006945500-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006945500-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006945500-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006945786-01 & 3136.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006946158-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006946199-01 & 1359.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006946199-02 & 1359.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006946465-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
006946681-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006946681-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006946700-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
006946819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006946871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006946871-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006946871-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006947064-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
006947064-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006947064-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006947095-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
006947099-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
006947164-01 & 3531.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006947300-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
006947591-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
006947623-01 & 6793.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006947668-01 & 3455.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
006947837-01 & 6794.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
006948006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006948006-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
006948054-01 & 0869.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006948054-02 & 0869.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006948054-03 & 0869.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006948054-04 & 0869.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006948480-01 & 2975.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006948815-01 & 5339.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
006949061-01 & 1960.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006949061-02 & 1960.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006949204-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006949204-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006949204-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006949204-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
006949326-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006949550-01 & 6795.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006949607-01 & 0870.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006949607-02 & 0870.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006949898-01 & 3031.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006950275-01 & 6796.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_006864859-02\\
006950275-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006864859-01\\
006950556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006951231-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006951231-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006951231-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
006951365-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006951642-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006951642-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006951642-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006951642-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
006951851-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006951851-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
006952259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006952259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006952259-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006952966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006952966-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006952966-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006953047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006953047-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006953047-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006953219-01 & 6797.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
006953281-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
006953692-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
006954721-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006954748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006955671-01 & 3329.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006955713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
006956014-01 & 0031.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
006956176-01 & 6798.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006956216-01 & 3604.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
006956233-01 & 1352.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_006956216-pri\\
006956233-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_006956216-sec\\
006957044-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006960377-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006960445-01 & 0669.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3654.01\\
006960446-01 & 3654.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006960456-01 & 0613.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3654.01\\
006960487-01 & 3386.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006960592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006960592-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006960913-01 & 1361.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006961285-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006961285-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006962018-01 & 6799.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
006962109-01 & 2182.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006962329-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
006962380-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006962380-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006962668-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
006962668-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006962752-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006962752-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006962752-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006962977-01 & 1364.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006962977-02 & 1364.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
006962977-03 & 1364.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006962977-04 & 1364.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
006962977-05 & 1364.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
006963153-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006963285-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
006963285-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
006963490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
006963490-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006964043-01 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_2:1---TOO\_FEW\_QUARTERS\\
006964043-02 & 1351.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006964159-01 & 3129.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
006964804-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006964804-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006964929-01 & 2756.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
006964929-02 & 2756.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006965293-01 & 6800.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006965758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006965758-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
006965789-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006965789-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006965789-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
006966132-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
006967278-01 & 6152.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
006967360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006967360-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
006967430-01 & 6801.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008504570-pri\\
006973796-01 & 3726.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
006974111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006974111-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006974111-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
006974658-01 & 2925.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006974867-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
006974867-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
006975129-01 & 1628.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
006975129-02 & 1628.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
006975129-03 & 1628.03 & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006975466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
006975466-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
006975615-01 & 1698.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
006976420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
006976465-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
006976754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
006976754-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007007099-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007007099-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007007099-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007007169-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
007007169-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007008149-01 & 2918.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007008149-02 & 2918.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007008200-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007008211-01 & 2102.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007008221-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007009041-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007009828-01 & 6802.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007013649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007017274-01 & 3209.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007017372-01 & 3689.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007018210-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007018210-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007019489-01 & 2128.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007019489-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007019524-01 & 2877.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007020234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007020707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007020707-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007020707-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007021124-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007021124-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007021131-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007021177-01 & 3452.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007021177-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007021177-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
007021534-01 & 2267.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007021681-01 & 0255.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
007021681-02 & 0255.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007021689-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007021689-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007021993-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007021993-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007022432-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007022573-01 & 3112.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007022603-01 & 5346.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007022603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007023060-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007023060-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007023110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007023110-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007023872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007023872-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_007023917-sec\\
007023960-01 & 0187.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007023960-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007023973-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_007023917-pri\\
007024222-01 & 0309.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007024511-01 & \nodata & FP & 0 & 0 & 0 & 1 & PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_6:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_6:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_007024530-01\\
007024530-01 & 3922.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT\\
007024530-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007024928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007024928-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007024928-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007024928-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007025526-01 & 1380.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3550.01\\
007025540-01 & 3550.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
007025846-01 & 0565.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007025851-pri\\
007025851-01 & 6803.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
007030610-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007030676-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007030715-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007030996-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007031066-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031126-01 & 7573.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031132-01 & 6804.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007031175-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007031192-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031195-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031208-01 & 7574.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031293-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031316-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007031340-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031352-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031399-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007031421-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031430-01 & 4472.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007031477-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007031504-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031515-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031517-01 & 0871.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007031520-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007031565-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007031573-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007031638-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031656-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007031659-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007031716-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007031716-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031726-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007031732-01 & 6805.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007031742-01 & 7575.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_RR-Lyr-pri\\
007031753-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031767-01 & 6806.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007031781-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031824-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007031853-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031872-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007031880-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031898-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031904-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007031914-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007031942-01 & 4420.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007031948-01 & 6807.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007031956-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007031992-01 & 6808.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007032001-01 & 4518.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032116-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007032116-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_RR-Lyr-pri\\
007032117-01 & 6809.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007032132-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007032136-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007032174-01 & 6810.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007032180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007032274-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032365-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007032369-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007032383-01 & 6811.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032388-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007032388-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007032421-01 & 1747.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007032421-02 & 1747.02 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032429-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007032438-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032456-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007032481-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032524-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007032568-01 & 7576.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032687-01 & 7577.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007032807-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007032833-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007032891-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007032923-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007032938-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007032968-01 & 6812.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007032999-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007033044-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007033067-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007033233-01 & 2339.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007033421-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007033671-01 & 0670.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007033713-01 & 6813.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007033748-pri\\
007033748-01 & 6814.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
007033846-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007035099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007035099-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007035179-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007035179-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007035179-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007035179-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007035274-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007035274-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007035274-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007035394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007037540-01 & 1347.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007037540-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007037540-03 & 1347.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007038096-01 & 4020.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007038372-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007038372-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007039007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007040629-01 & 0671.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007040629-02 & 0671.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007040629-03 & 0671.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007040629-04 & 0671.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
007040897-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
007041634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007041634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007041856-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007041856-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007041882-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007042019-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007045280-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007045280-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007045435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007045496-01 & 1939.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007045605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007045605-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007045685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007046035-01 & 4424.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007046148-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
007046804-01 & 0205.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007047151-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007047207-01 & 2494.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007047299-01 & 5351.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007047356-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007047356-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007047356-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007047356-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007047363-01 & 2432.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007047496-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007047824-01 & 2806.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007047922-01 & 1899.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
007047922-02 & 1899.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007047963-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007047963-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007047963-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007048016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007048016-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007049486-01 & 6815.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007049486-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007049849-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007049860-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007049860-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007050060-01 & 2215.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007050100-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007050100-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007050754-01 & 6816.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF\\
007050989-01 & 0312.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007050989-02 & 0312.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007051180-01 & 0064.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007051180-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007051690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007051984-01 & 2879.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007051984-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007052048-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007052048-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007052511-01 & 4824.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007053328-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007053456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007060001-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007060001-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007060736-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007060736-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007060736-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007061062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007061062-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007061062-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
007090524-01 & 2920.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007090801-01 & 6817.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007091432-01 & 3353.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007091594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007091594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007091610-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007092048-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007093284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007093401-01 & 3433.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007094486-01 & 1907.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007094944-01 & 4859.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007095218-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007097201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007097534-01 & 3126.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET---PARENT\_IS\_007097571-pri\\
007097571-01 & 6818.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
007097965-01 & 2083.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007098255-01 & 4762.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007098355-01 & 0454.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007100673-01 & 4032.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007100673-02 & 4032.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007100673-03 & 4032.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007100673-04 & 4032.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
007100673-05 & 4032.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
007100673-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007101676-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007101828-01 & 0455.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007102227-01 & 1360.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007102227-02 & 1360.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007102227-03 & 1360.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007102316-01 & 2028.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007102316-02 & 2028.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007102316-03 & 2028.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007102507-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007102615-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007103006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007103277-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007103300-01 & 6819.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007103919-01 & 4310.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007104854-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007105574-01 & 6820.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007105574-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007106173-01 & 3083.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007106205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007106205-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007106648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007106648-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007106648-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007106877-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007106877-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007106877-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007107547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007107561-01 & 3100.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_5353.01\\
007107567-01 & 5353.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007107762-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007107802-01 & 2420.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007107802-02 & 2420.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007108433-01 & 6153.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007108433-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007109598-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007109598-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007109598-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007109675-01 & 0872.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007109675-02 & 0872.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007109851-01 & 3012.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007110077-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007115085-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115200-01 & 6821.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007115237-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115249-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115291-01 & 3357.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007115291-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115308-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007115323-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115323-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115323-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115332-01 & 6822.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115366-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007115384-01 & 7578.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007115390-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115427-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115450-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007115463-01 & 6823.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115499-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007115530-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115550-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115597-01 & 6824.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007115661-01 & 3174.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007115671-01 & 5355.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007115733-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115785-01 & 0672.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007115785-02 & 0672.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007115785-03 & 0672.03 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115816-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007115842-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115869-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115878-01 & 6825.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007115879-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007115923-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007115925-01 & 4258.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007116043-01 & 6826.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007116046-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007116072-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007116117-01 & 3163.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007116166-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007116217-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007116226-01 & 6827.01 & FP & 0 & 0 & 0 & 1 & FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007116236-01 & 6828.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007116282-01 & 7579.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007116382-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007116466-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007116519-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007116561-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007116632-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007116670-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007116766-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007116842-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007116849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
007116851-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007116859-01 & 7580.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007117003-01 & 3514.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---FIT\_FAILED\\
007117003-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007117003-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007117020-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007117126-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007117147-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007117178-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007117226-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007117270-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007117284-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007117348-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007117355-01 & 4866.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007117413-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007117436-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007117457-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007117485-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007117491-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007117492-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007117513-01 & 6829.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007117541-01 & 6830.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007117541-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007117549-01 & 4874.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007117561-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007117568-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007117585-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007117610-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007117710-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007117723-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007118167-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007118167-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007118167-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007118364-01 & 0873.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
007118545-01 & 6831.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007118545-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007119080-01 & 6154.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007119080-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007119080-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007119481-01 & 0566.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007119481-02 & 0566.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007119522-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007119530-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007119530-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007120108-01 & 2325.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007121016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007121016-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007121885-01 & 3467.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007121885-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007122259-01 & 3454.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007122259-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007122746-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007122746-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007122746-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007122746-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007124026-01 & 2275.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007124145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007124613-01 & 0673.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007124680-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007125636-01 & 6832.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007125636-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007128918-01 & 6833.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007129465-01 & 6155.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
007129537-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007130418-01 & 3317.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007130612-01 & 5359.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007131760-01 & 3407.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007132015-01 & 6834.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
007132542-01 & 3517.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007132798-01 & 0220.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007132798-02 & 0220.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007133286-01 & 7581.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007133286-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007133294-01 & 4473.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007134502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007134502-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007134976-01 & 0874.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007134976-02 & 0874.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007135042-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007135042-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007135042-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007135045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007135045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007135545-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007135545-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007135549-01 & 6835.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007135852-01 & 0875.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007136729-01 & 2872.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007136958-01 & 3350.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007136958-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007137213-01 & 3907.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007137725-01 & 1699.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM---PARENT\_IS\_007137798-pri\\
007137798-01 & 6836.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007137798-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007137952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007137952-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007137952-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007137952-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007138415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007138415-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007138415-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007138841-01 & 5361.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007173839-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007173839-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007173839-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007174349-01 & 3844.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007174349-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007174351-01 & 1365.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3844.01\\
007174372-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007174372-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007174617-01 & 6156.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007174617-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007174617-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007175184-01 & 0369.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007175184-02 & 0369.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007175896-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007175943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007175943-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007175943-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007176080-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007176268-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007176268-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007177105-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007177105-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007177553-01 & 6837.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007177553-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007177555-01 & 3299.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_007177553-01\\
007177555-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007177553-02\\
007177766-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007177766-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_007259917-pri\\
007177892-01 & 6838.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007177892-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
007177892-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007177892-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007183123-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007183123-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007183123-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007183745-01 & 2521.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007183745-02 & 2521.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007185134-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007185487-01 & 6839.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
007185924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007186259-01 & 7582.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007186665-01 & 3033.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007186665-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007187135-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007191646-01 & 4358.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007198648-01 & 6840.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007198734-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007198769-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007198791-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007198817-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007198834-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007198846-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007198881-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007198881-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007198906-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007198906-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_007198959-01\\
007198925-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007198941-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007198941-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007198959-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007199010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007199013-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_007198959-01\\
007199013-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007199036-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007199037-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007199058-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007199060-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007199168-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007199203-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007199203-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_RR-Lyr-pri\\
007199225-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007199235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007199235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007199272-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007199343-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007199343-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007199351-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007199397-01 & 0075.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007199418-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007199724-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007199756-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007199774-01 & 1346.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007199774-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007199814-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007199883-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007199884-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007199906-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007199917-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007199935-01 & 6841.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007199989-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007200001-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007200012-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007200013-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007200050-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007200092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007200102-01 & 6842.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007200102-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007200102-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
007200111-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007200148-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007200156-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007200225-01 & 6843.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007200299-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007200301-01 & 6844.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007200303-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007200359-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007200463-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007201831-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007202395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007202395-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007202592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007202957-01 & 2687.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007202957-02 & 2687.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007203179-01 & 6845.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
007203194-01 & 6846.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_007203179-pri\\
007204073-01 & 6847.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007204233-01 & 5371.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007204237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007204237-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007204237-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007204981-01 & 2164.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007205499-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007205868-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007206837-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007207061-01 & 2113.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007207061-02 & 2113.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007207391-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007207520-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007207672-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007207672-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007210948-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
007210959-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007211141-01 & 1355.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007211157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007211221-01 & 1379.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007211469-01 & 1377.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007211635-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007211743-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007211743-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007211759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007211759-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007211759-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007211759-04 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007211879-01 & 4342.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007212040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007212040-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007212066-01 & 3610.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
007212066-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
007212184-01 & 2487.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007212722-01 & 6848.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007214055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007214055-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007214055-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007214090-01 & 7583.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007214090-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007214475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007214475-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007214475-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007215603-01 & 1618.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007215607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007215678-01 & 2354.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007215678-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007215678-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007216003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007216284-01 & 3056.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007216690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007216690-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007216979-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007216979-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007217088-01 & 6849.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007217303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007217483-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007217483-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007219251-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007219251-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007219502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007219502-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007219502-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007219825-01 & 0238.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007219825-02 & 0238.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007219906-01 & 6033.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
007219906-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007220320-01 & 3775.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
007220322-01 & 1350.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_3775.01\\
007220338-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007220338-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007220429-01 & 1700.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007220508-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007221108-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007221584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007221584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007222086-01 & 1701.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007222086-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007222086-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007222362-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007222939-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007222939-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007255336-01 & 0019.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007256442-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007256914-01 & 4136.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007256914-02 & 4136.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007257008-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007257008-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007257363-01 & 2292.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007257373-01\\
007257373-01 & 6034.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
007257966-01 & 4185.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007258902-01 & 5378.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_007258889-pri\\
007259249-01 & 4237.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007259249-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
007259298-01 & 2561.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007264671-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007265298-01 & 2051.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007265298-02 & 2051.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007265427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007265427-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007265427-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007266212-01 & 4737.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007266266-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007267370-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007268500-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007268500-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
007268500-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
007269493-01 & 1961.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007269623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007269623-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007269623-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007269623-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007269881-01 & 2916.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007269881-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007269974-01 & 0456.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007269974-02 & 0456.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007270159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007270230-01 & 0876.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007270230-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007271007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007271007-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007271007-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007271221-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007271892-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007271892-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007271892-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007272132-01 & 4466.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007273277-01 & 1979.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
007277317-01 & 0674.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007280785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007280944-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_RR-Lyr-pri\\
007280953-01 & 6850.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007281217-01 & 6851.01 & FP & 0 & 0 & 0 & 1 & FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007281229-01 & 6852.01 & FP & 0 & 0 & 0 & 1 & FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007281301-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007281311-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281356-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281356-02 & 6853.01 & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007281357-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281372-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007281399-01 & 6854.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007281410-01 & 6855.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007281411-01 & 4339.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007281454-01 & 3055.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007281468-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281484-01 & 4536.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007281503-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007281615-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007281616-01 & 6856.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007281644-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281664-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281668-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281694-01 & 7584.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007281699-01 & 6857.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007281825-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281838-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281856-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007281864-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_RR-Lyr-pri\\
007281947-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007281951-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007281979-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007281980-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007282008-01 & 6858.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007282028-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007282042-01 & 4718.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007282078-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007282154-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007282158-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007282162-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007282168-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007282209-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007282209-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007282209-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007282209-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007283507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007283604-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007283604-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007284688-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007284688-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007284688-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007284775-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007285602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007285616-01 & 6859.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007285673-01 & 4559.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007285757-01 & 3271.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007285757-02 & 3271.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
007286137-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007286137-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007286173-01 & 1862.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007286276-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007286276-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007286343-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007286410-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007286531-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007286739-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007286911-01 & 2180.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007287118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007287118-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007287162-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007287162-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007287165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007287165-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007287328-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007287328-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007287391-01 & 3546.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007287391-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007287415-01 & 1369.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007287592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007287677-01 & 4815.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007287683-01 & 1622.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007287683-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007287683-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007287786-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007287786-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007287995-01 & 0877.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007287995-02 & 0877.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007287995-03 & 0877.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007288306-01 & 3443.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007288444-01 & 3482.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007289068-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007289068-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007289068-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007289124-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
007289157-01 & 0399.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007289157-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007289157-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007289157-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
007289158-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
007289162-01 & 2539.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_399.01\\
007289165-01 & 3847.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_399.01\\
007289165-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007289157-03\\
007289317-01 & 2450.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007289317-02 & 2450.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007289338-01 & 3420.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007289338-02 & 3420.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007289577-01 & 1974.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007292380-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007292469-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007292469-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007292935-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007292935-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007292935-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007293769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007293769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007293937-01 & 3211.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007374746-01\\
007294135-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007294135-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007294135-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007294598-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007294598-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007294598-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007294743-01 & 2516.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007295235-01 & 0987.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007295520-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
007295520-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS\\
007295570-01 & 6035.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
007295570-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007296086-01 & 1374.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007296094-01\\
007296094-01 & 3790.01 & PC & 0 & 0 & 0 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED\\
007296877-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007296877-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007296877-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007296877-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007297189-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007299869-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007299869-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007299869-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007299905-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007300184-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007300184-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007300387-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007300387-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007300387-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007300623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007300623-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007301014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007301014-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007301014-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007301202-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007301202-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007301640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007301640-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007302940-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007303253-01 & 0878.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007303287-01 & 1353.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007303287-02 & 1353.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007303287-03 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007304121-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007304393-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007304449-01 & 1702.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007335514-01 & 6860.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007335713-01 & 3250.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
007335713-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
007335972-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007335972-02 & 4599.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007336640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007336754-01 & 6861.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007336754-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007337049-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007337049-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007338125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007344999-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007344999-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007345248-01 & 4864.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007345335-01 & 6862.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
007346691-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007346811-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007347246-01 & 3014.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007350067-01 & 6863.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007351433-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007351433-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007351518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007352016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
007352016-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007352425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007352425-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007352425-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007352727-01 & 5382.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007352776-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007352776-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007352776-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007352995-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007353970-01 & 3574.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007353970-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007354213-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007357531-01 & 1368.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007362073-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007362301-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007362355-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007362364-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_RR-Lyr-pri\\
007362391-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007362420-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007362434-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007362450-01 & 7585.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_RR-Lyr-pri\\
007362501-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007362534-01 & 6864.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_RR-Lyr-pri\\
007362573-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_RR-Lyr-pri\\
007362579-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007362579-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_RR-Lyr-pri\\
007362587-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007362592-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007362631-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007362632-01 & 6865.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007362695-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007362696-01 & 3937.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007362696-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007362696-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_RR-Lyr-pri\\
007362852-01 & 6036.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
007362865-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_RR-Lyr-pri\\
007363405-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007363405-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007363962-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007364176-01 & 0373.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007364845-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007364845-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007365447-01 & 6866.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
007365528-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007365528-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007365537-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007365557-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_007365569-01\\
007365569-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED---PARENT\_IS\_007365557-01\\
007366036-01 & 6867.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_RR-Lyr-pri\\
007366065-01 & 6868.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007366258-01 & 0880.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007366258-02 & 0880.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007366258-03 & 0880.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007366258-04 & 0880.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
007367431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
007367431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007368103-01 & 6869.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007368137-01 & 4265.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007368103-pri\\
007368295-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007368590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007368590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007368664-01 & 0614.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007368898-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007368960-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007368960-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007369523-01 & 6870.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007369865-01 & 1918.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
007373451-01 & 0881.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007373451-02 & 0881.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007374160-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007374160-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007374160-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007374160-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007374160-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007374746-01 & 3537.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
007375348-01 & 0266.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007375348-02 & 0266.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007375795-01 & 1378.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
007375795-02 & 1378.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007375997-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007376490-01 & 3586.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3535.01\\
007376490-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007376500-sec\\
007376500-01 & 3535.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
007376500-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
007376500-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
007376500-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
007376500-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
007376982-01 & 6871.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_007212722-01\\
007376983-01 & 1358.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007376983-02 & 1358.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007376983-03 & 1358.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007376983-04 & 1358.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007377033-01 & 0882.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007377343-01 & 5384.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007377422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007377466-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007377660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007378020-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007378020-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007378020-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007378049-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007378067-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007379385-01 & 2207.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007379646-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007379646-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007380537-01 & 0883.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007380829-01 & 1703.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007381580-01 & 6872.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007381616-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
007381695-01 & 6873.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007381977-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007382099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007382313-01 & 2392.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007383227-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007383764-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007383764-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007383764-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007384711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007385073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007385387-01 & 6874.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_007385478-pri\\
007385478-01 & 6875.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
007385500-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007385500-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007385500-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007385509-01 & 0675.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007385478-pri\\
007385783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007385783-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007386431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007386431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007386827-01 & 1704.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007387226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007387226-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007387226-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
007387226-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007387226-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007387593-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007416306-01 & 5388.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
007418173-01 & 3995.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007418359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007418507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
007418507-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007418507-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007419085-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007419318-01 & 0313.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007419318-02 & 0313.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007421876-01 & 6876.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007421876-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
007421876-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007422883-01 & 6159.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
007422883-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
007427283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
007427764-01 & 4364.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007427780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007427780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007428316-01 & 2809.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007428489-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007428489-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007428489-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007428736-01 & 2827.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007429237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007429240-01 & 4450.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
007429256-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007430034-01 & 1848.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007430876-01 & 3193.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007431665-01 & 6877.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007431709-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_007431703-pri\\
007431838-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007431838-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007431838-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007431838-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007431838-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007431838-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007431887-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007432548-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007433279-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007433585-01 & 2999.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
007434470-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007434875-01 & 0884.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007434875-02 & 0884.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
007434875-03 & 0884.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007435286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007435780-01 & 4757.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_007518816-pri\\
007435780-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_007518816-pri\\
007436177-01 & 6038.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
007436177-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
007439060-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007439240-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007439316-01 & 1501.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007440748-01 & 0457.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007440748-02 & 0457.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007445098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007445445-01 & 0567.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007445445-02 & 0567.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007445445-03 & 0567.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007445732-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007445885-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
007446184-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007446631-01 & 2598.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007446835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007447200-01 & 0676.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007447200-02 & 0676.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007447200-03 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007447895-01 & 6878.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
007448023-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_RR-Lyr-pri\\
007448023-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007449136-01 & 1890.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007449541-01 & 2063.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007449554-01 & 2357.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007449554-02 & 2357.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007449695-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
007449844-01 & 1452.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
007450284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007450284-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007450284-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007450284-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007450360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007450360-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007450747-01 & 4267.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007454979-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007454979-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007454990-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007454990-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007455287-01 & 0886.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007455287-02 & 0886.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007455287-03 & 0886.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007455553-01 & 6879.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007455624-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007455624-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007455624-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007455733-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007455914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007455914-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
007455981-01 & 3096.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007456001-01 & 1517.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007456441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007456441-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007456521-01 & 6880.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
007457278-01 & 3188.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007457296-01 & 2213.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007457355-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007457355-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007458050-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007458309-01 & 3957.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007458285-pri\\
007458433-01 & 5392.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_007458285-pri\\
007458697-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007458697-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007458697-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007458762-01 & 0887.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007459411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007459411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007460399-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007460436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
007461022-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007461307-01 & 2909.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
007461314-01 & 6881.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_2909.01\\
007461354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007461354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007461382-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007461382-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007461436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007461436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007461521-01 & 6882.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007461607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007461963-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007461963-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007463044-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007463044-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007463623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007463623-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007463685-01 & 2890.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007463737-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007463737-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007463903-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
007464205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007464205-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007464361-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007464386-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007464417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007465661-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007465661-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007465661-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007466270-01 & 2959.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007466828-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007466828-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
007466863-01 & 0677.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007467185-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007467185-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007467518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007467518-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007467518-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007467518-04 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007467539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007470159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007470491-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007499398-01 & 1473.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007499407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007499407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007499407-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007499571-01 & 6883.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
007500268-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007501194-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_007501230-pri\\
007501194-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_007501230-sec\\
007501405-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007501405-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007501646-01 & 2572.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007502559-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007502559-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007502559-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007502559-04 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007503885-01 & 3417.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007504328-01 & 0458.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007504778-01 & 2316.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007505674-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007505674-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007506881-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007509572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007509886-01 & 0678.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007509886-02 & 0678.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007510049-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007510820-01 & 3303.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007511994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007512130-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007512130-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
007512982-01 & 1480.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007512982-02 & 1480.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007513405-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007514582-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_007431703-pri\\
007515212-01 & 0679.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007515212-02 & 0679.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007515336-01 & 4663.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007515468-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007515670-01 & 2360.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007515679-01 & 3728.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007515679-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007515679-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007515762-01 & 2524.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007515964-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007516379-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_007516345-pri\\
007516781-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007516781-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007516809-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007516809-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007517261-01 & 3496.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007517261-02 & 3496.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007518797-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007522019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007522572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007522572-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007522911-01 & 1705.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007523115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007523340-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007523340-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007523340-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007523733-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007523733-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007529180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007529266-01 & 0680.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007530196-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007530366-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007531677-01 & 2601.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007532891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007532891-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007532973-01 & 1450.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007532973-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007533425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
007533425-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007533694-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007533694-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007533694-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007533694-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007534037-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007534267-01 & 3147.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007537660-01 & 6884.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007537945-01 & 6039.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
007538176-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007538176-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007538450-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007538622-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007538711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007538839-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007538839-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007538950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007538950-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007538950-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007539108-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
007539174-01 & 5397.02 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT\\
007540755-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007540965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007541502-01 & 6885.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007541502-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007541659-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007541659-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007541659-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007541746-01 & 6886.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
007541746-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007542369-01 & 2465.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007542813-01 & 2302.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007543167-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007543649-01 & 1469.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007545719-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
007547306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007547306-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007547306-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007547573-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007547573-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007547573-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007547573-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007547925-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007547969-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007548035-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007548259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007548259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007548259-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007548479-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007548479-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007548479-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007549209-01 & 1518.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007549389-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007549389-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007549852-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007549852-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007549852-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007551589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007551993-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007551993-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007552119-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007552265-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007552265-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007552341-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007552344-01 & 0888.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
007552344-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007552701-01 & 3994.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007553235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007553235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007553237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007553237-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007553237-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007582608-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007582608-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007582608-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007582608-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007582608-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007582608-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007582608-07 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007582689-01 & 3097.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007582689-02 & 3097.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007582689-03 & 3097.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007582691-01 & 4419.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
007582691-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007583208-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007583208-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007583208-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007583299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007583299-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007583437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007583437-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007583437-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007583650-01 & 4614.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007583650-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007583939-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007583939-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007583939-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007584650-01 & 2631.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007584755-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007584778-01 & 6887.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_007584826-pri\\
007585445-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007585445-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007585445-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007585481-01 & 0890.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007587506-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007588292-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007588436-01 & 6888.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
007591772-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007592529-01 & 6889.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007592922-01 & 6890.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
007593110-01 & 1748.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007593110-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007595157-01 & 0568.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007595157-02 & 0568.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007595579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007595579-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007595579-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007595579-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007595579-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007595928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007596224-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007596240-01 & 4295.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007596250-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007597005-01 & 3961.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007597703-01 & 6891.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007597771-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007597771-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007597771-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007598111-01 & 4507.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007598128-pri\\
007598128-01 & 0681.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007598128-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007598492-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007598492-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007598492-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007599004-01 & 5403.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
007599132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007599171-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007601633-01 & 0136.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007601917-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007601917-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007601918-01 & 4133.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007602070-01 & 0514.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
007602070-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
007602351-01 & 6892.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007603200-01 & 0314.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007603200-02 & 0314.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007603200-03 & 0314.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007604266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007604328-01 & 2458.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007604328-02 & 2458.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007605093-01 & 2817.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007605527-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007605527-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007605600-01 & 6893.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007605600-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007609553-01 & 2924.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007609674-01 & 3128.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007610663-01 & 4160.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007612691-01 & 3836.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
007613246-01 & 3062.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007617977-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007618364-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
007618364-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007618364-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007620413-01 & 2103.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007620413-02 & 2103.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
007620537-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007620654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007620654-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007620660-01 & 3832.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007620660-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_007620664-pri\\
007620801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007620844-01 & 3551.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT\\
007620844-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007621172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007621172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007621172-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007621172-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007621759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007621759-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007621759-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007622059-01 & 6161.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007622059-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_007622072-01\\
007622059-03 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
007622072-01 & 6894.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
007622208-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007622473-01 & \nodata & FP & 1 & 0 & 0 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_1447.01\\
007622486-01 & 1447.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007622486-02 & 1447.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007622486-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007623120-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
007624297-01 & 6040.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007624297-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007624741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007624741-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
007624753-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007624753-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007625221-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007626370-01 & 1706.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007626425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007626506-01 & 0150.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007626506-02 & 0150.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007626595-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007626595-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007626595-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007627570-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007627570-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007627746-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007628336-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007628336-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007628336-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007629287-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007629518-01 & 1495.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007630229-01 & 0683.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007630232-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007630232-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007630232-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007630232-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007630417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007630417-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007630417-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007630658-01 & 6895.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
007630733-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007631194-01 & 6896.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007631194-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007658229-01 & 5409.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007658578-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007658578-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007658578-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007658578-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007658578-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007658796-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007658796-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007658882-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007658925-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007658925-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007658925-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007659389-01 & 2734.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007659782-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007660542-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
007660542-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007660607-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007660607-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007661065-01 & 2307.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007661409-01 & 0957.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007661500-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007661500-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007661500-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007661500-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007661893-01 & 4296.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007662076-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007662209-01 & 6897.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
007662502-01 & 5410.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007662697-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007663405-01 & 1519.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007663405-02 & 1519.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007663691-01 & 0891.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007663804-01 & 6898.01 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT\\
007663830-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
007667142-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007667560-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007667560-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007667971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007668385-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007668416-01 & 3089.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007668648-01 & 6899.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007668648-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007668663-01 & 1898.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007668791-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007668791-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007668791-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007668911-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007668911-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007670485-01 & 6900.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
007670617-01 & 6901.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007670617-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007670943-01 & 0269.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007671081-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007671594-01 & 6902.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007671833-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007671833-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007671974-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007672097-01 & 2255.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007672215-01 & 5411.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007672453-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007672453-02 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007673192-01 & 2722.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007673192-02 & 2722.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007673192-03 & 2722.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007673192-04 & 2722.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
007673192-05 & 2722.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
007673841-01 & 2585.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007673841-02 & 2585.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007673841-03 & 2585.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007674050-01 & 5412.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007674265-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007676423-01 & 3113.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007677005-01 & 6903.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007677005-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007677005-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
007678099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007678385-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007678385-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007678434-01 & 0892.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007678434-02 & 0892.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007679812-01 & 3943.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007680114-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007681230-01 & 4294.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007681230-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_CENTROIDS\\
007684873-01 & 0014.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
007684873-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
007685010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007685010-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007685307-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007685307-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007685307-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007685408-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007685408-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007685408-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007685981-01 & 0893.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007687365-01 & 6904.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007687705-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
007687705-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007690844-01 & 1508.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007691260-01 & 1528.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007691527-01 & 6905.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007691527-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007692093-01 & 3337.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007692248-01 & 4886.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
007692619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007692619-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007694191-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007694191-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007694615-01 & 4489.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007695087-01 & 3693.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_6041.01\\
007695087-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_6041.01\\
007695093-01 & 6041.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
007695093-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007695445-01 & 6906.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007697103-01 & 3430.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007697568-01 & 1829.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007697568-02 & 1829.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
007697795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007697795-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007698258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007698937-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007698937-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007699056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007699056-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007699056-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007699056-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007699298-01 & 4534.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_3706.01\\
007699478-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007699478-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007700033-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007700033-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007700500-01 & 6907.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007700561-01 & 5414.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_007700578-pri\\
007700578-01 & 6908.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007700578-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007700590-01 & 3750.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_007700578-pri\\
007700622-01 & 0315.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007700871-01 & 0088.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007700871-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
007700871-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
007700880-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007700880-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007700880-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
007700963-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007702705-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007702705-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007702705-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007703305-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007703305-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007703305-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007703530-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007703785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007703785-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007703882-01 & 4403.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
007703910-01 & 4379.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007703955-01 & 1707.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007703955-02 & 1707.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007704028-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007704028-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007707736-01 & 6909.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_007707742-pri\\
007707742-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007707742-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007707742-03 & 3998.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
007708193-01 & 3666.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007708193-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007708215-01 & 0894.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3666.01\\
007708215-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007708193-02\\
007708315-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007708315-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007708315-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007708418-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007708984-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007730747-01 & 0684.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007731281-01 & 5416.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007732285-01 & 3023.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007732458-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007732458-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007732458-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007732458-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007732461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007732461-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007732461-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007732791-01 & 3623.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007732791-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
007732964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007733540-01 & 6910.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007733685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007733685-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007733685-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007733731-01 & 4022.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
007738436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007739152-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007739172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007739172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
007741048-01 & 6911.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007741837-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007741837-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007741837-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007742408-01 & 3478.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007743124-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007743464-01 & 5417.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007744087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007744634-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
007746958-01 & 2324.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007747091-01 & 5418.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007747425-01 & 1952.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007747425-02 & 1952.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007747425-03 & 1952.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
007747425-04 & 1952.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007747457-01 & 4561.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007748238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007748238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007748238-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007748238-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007748487-01 & 3394.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007749002-01 & 4325.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007749318-01 & 6042.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007749552-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007749552-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007749552-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007749552-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007749773-01 & 2848.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007750294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007750330-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---LARGE\_RM\\
007750419-01 & 1708.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007750740-01 & 6162.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007751542-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007751562-01 & 6912.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
007751562-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007751571-01 & 1460.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_007751562-01\\
007751571-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007751562-sec\\
007755636-01 & 1921.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007755741-01 & 6913.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007755741-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007755741-03 & 6913.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
007755741-04 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007755932-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007755932-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007755932-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007756853-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007761545-01 & 1472.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007761855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007761855-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007761855-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007761918-01 & 1808.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007762723-01 & 2663.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007763269-01 & 3721.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007764367-01 & 0685.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007765006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007765006-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007765236-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007765374-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007765374-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007765528-01 & 1840.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007765528-02 & 1840.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007765585-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007765585-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007765585-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007765684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007765762-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007766113-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_007766185-pri\\
007766113-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM---PARENT\_IS\_007766185-sec\\
007766199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007766199-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007766209-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_007766185-pri\\
007767162-01 & 2869.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007767367-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007767367-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007767367-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007767367-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007767559-01 & 0895.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007767559-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007767733-01 & 3322.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007767733-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007767774-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007768451-01 & 1527.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007768952-01 & 1709.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007768952-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007769072-01 & 6914.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007769815-01 & 6915.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007769819-01 & 2778.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007770256-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007770256-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007770256-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007770450-01 & 1467.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3706.01\\
007770471-01 & 3706.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007770471-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007770901-01 & 5426.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007771970-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007771991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007771991-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007772914-01 & 3339.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007772919-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007772919-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007773041-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007773133-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007773133-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007773179-01 & 4038.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007773209-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007777365-01 & 6916.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_007777443-pri\\
007777372-01 & 3958.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_007777443-pri\\
007777397-01 & 6043.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_007777416-02\\
007777397-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_007777416-02\\
007777416-01 & 3960.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007777416-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007777435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007777435-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007777435-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007777471-01 & 4075.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_007777443-pri\\
007777522-01 & 4415.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_007777443-pri\\
007777818-01 & 4380.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CROWDED\_DIFF\\
007778108-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007778108-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007778108-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007778427-01 & 4482.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007778437-01 & 0131.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007778621-01 & 4725.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007778767-01 & 2523.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007778767-02 & 2523.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
007778826-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007778826-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007778826-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007778838-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007778838-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007778838-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007778980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007778980-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007778980-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007779077-01 & 1842.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007779411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007779411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007779942-01 & 6163.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007779942-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007779942-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007779942-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007779942-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007797715-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007798259-01 & 6917.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007798259-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007798339-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007798339-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007798339-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007798339-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007798924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007798924-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007799575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007800087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007800087-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007800285-01 & 5427.01 & FP & 0 & 0 & 1 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
007800750-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_007938870-pri\\
007801070-01 & 4361.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007802136-01 & 1449.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007802136-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007802719-01 & 2247.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007808587-01 & 1533.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007808747-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
007810483-01 & 1943.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007811211-01 & 6918.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
007811397-01 & 1477.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007812167-01 & 1482.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3665.01\\
007812167-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007812175-sec\\
007812175-01 & 3665.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007812179-01 & 0515.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3665.01\\
007812179-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007812175-sec\\
007812455-01 & 2881.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007812455-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
007812594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007812594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007812594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007812594-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007812893-01 & 6919.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
007812990-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
007812990-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007813039-01 & 3787.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007813370-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007815744-01 & 1710.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007815931-01 & 2861.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007816137-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_007816201-sec\\
007816137-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_007816201-pri\\
007816665-01 & 4227.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_007816680-01\\
007816680-01 & 6920.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007816935-01 & 6921.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007816992-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007816992-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007818762-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007819024-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007819024-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007819024-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007819833-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007819833-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007820985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007820985-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007821010-01 & 2938.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
007821010-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
007821689-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007821926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---TOO\_FEW\_QUARTERS\\
007825680-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007825680-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007825899-01 & 0896.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007825899-02 & 0896.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007825899-03 & 0896.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007826620-01 & 4268.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007826659-01 & 2686.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007826705-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007827152-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007827152-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007829836-01 & 5433.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007830321-01 & 6044.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007830321-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007830341-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
007830351-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007830637-01 & 1454.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007830637-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007830684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007830684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007831264-01 & 0171.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007831264-02 & 0171.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007831302-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007831302-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007831302-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007831363-01 & 3804.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
007832356-01 & 1456.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007832829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007833144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007833305-01 & 4528.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007834045-01 & 4630.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007834063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
007834063-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007834441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007834612-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007834612-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007835312-01 & 6164.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007836096-01 & 5435.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007836330-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007836863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007836863-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007837129-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007837214-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
007837214-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007837302-01 & 0048.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007837526-01 & 5436.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007837733-01 & 4628.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007837767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007838213-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007838214-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_007838213-01\\
007838214-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007838639-01 & 6922.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007838655-01 & 1464.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_007838639-pri\\
007838675-01 & 4169.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007838889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007838889-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007838906-01 & 6165.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007838906-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007838906-03 & 6165.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
007838908-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
007838908-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007839003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007839003-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007839003-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007839007-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007839814-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007840035-01 & 3758.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
007840035-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007840044-01 & 0516.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_3758.01\\
007840145-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007840358-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007840502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007840642-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007840642-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007841514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007841514-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007841640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007841640-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007841925-01 & 1499.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007841925-02 & 1499.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007841925-03 & 1499.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007841986-01 & 6045.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
007841986-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007842286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007842286-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007842286-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007842328-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007842328-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007842610-01 & 1453.01 & FP & 0 & 1 & 1 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
007842610-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007842610-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
007842621-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007842621-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007846404-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007846730-01 & 6923.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007846730-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007847104-01 & 4412.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007847927-01 & 6924.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007847927-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007848033-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007848288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007848288-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007848303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007848303-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007848303-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007848324-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007849854-01 & 0897.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007849879-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007866921-01 & 3360.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---KIC\_OFFSET\\
007866921-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
007867348-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007867348-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007867348-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007867348-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007868889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007868899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007868899-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007868967-01 & 6925.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007869917-01 & 1525.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007870032-01 & 1818.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007870250-01 & 6926.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_007938870-pri\\
007870282-01 & 4732.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007870306-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_007938870-pri\\
007870350-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
007870390-01 & 0898.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007870390-02 & 0898.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007870390-03 & 0898.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
007870958-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007870980-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
007871395-01 & 6927.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
007871954-01 & 1515.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007871954-02 & 1515.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007872212-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007872212-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007872212-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007877496-01 & 0202.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007877496-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007877818-01 & 3816.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3530.01\\
007877818-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007877824-02\\
007877820-01 & 6046.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3530.01\\
007877820-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_007877824-02\\
007877824-01 & 3530.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
007877824-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007877824-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
007877978-01 & 2760.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007878396-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
007878396-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007878396-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007879404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007879404-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007879433-01 & 2527.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007879433-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007879648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
007881228-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007881722-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007881722-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007884866-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_007884842-pri\\
007885518-01 & 6928.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_007885570-pri\\
007885518-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_007885570-sec\\
007885558-01 & 5439.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_007885570-pri\\
007885570-01 & 6929.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
007885570-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
007886102-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007886102-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007886329-01 & 6930.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
007887791-01 & 1964.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
007888863-01 & 5440.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
007889486-01 & 3300.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_007821010-01\\
007889486-02 & 3300.02 & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_007821010-02\\
007889617-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007890526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007890526-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007891294-01 & 4699.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007897915-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
007898352-01 & 1486.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007898352-02 & 1486.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007898445-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007898445-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007898576-01 & 3566.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
007899070-01 & 2683.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007899980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007900137-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007900367-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007900367-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007900450-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007901016-01 & 4257.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007901718-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007901718-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007901718-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007901948-01 & 1511.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007902001-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007902003-01 & 3236.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007902035-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007902035-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007902035-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007902204-01 & 6931.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007902286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007902287-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007903086-01 & 2761.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007904375-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007905106-01 & 4582.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007905191-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007905683-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007905683-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007905683-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007906671-01 & 3018.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
007906739-01 & 2165.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
007906865-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007906882-01 & 0686.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007906892-01 & 4773.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007907423-01 & 0899.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007907423-02 & 0899.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007907423-03 & 0899.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007907476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007907808-01 & 4109.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007907983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007908367-01 & 6166.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007908367-02 & 6166.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007908633-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_008111622-03\\
007908633-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007908633-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
007908633-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007908893-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
007909044-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007909392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007909392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007910148-01 & 3661.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
007910148-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
007914464-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007914906-01 & 6047.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007914906-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
007914906-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007914906-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007915386-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007915386-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007915458-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007915458-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
007915515-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007915824-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007916058-01 & 5445.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007916872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007916872-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007917014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007917014-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007917485-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007917485-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007917485-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007918172-01 & \nodata & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_6:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_6:1---CLEAR\_APO\\
007918172-02 & \nodata & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_3:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_3:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_007918217-01\\
007918172-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007918217-01 & 1770.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---SATURATED---PARENT\_IS\_007918172-02\\
007918401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
007918478-01 & 4209.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007918652-01 & 2984.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007918688-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
007918688-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007918688-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007918737-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007918737-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007918992-01 & 2095.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007919653-01 & 6932.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007919763-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007935997-01 & 5447.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007936033-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
007937391-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
007938179-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007938179-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007938180-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_007938179-02\\
007938468-01 & 6933.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
007938496-01 & 0900.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007938499-01 & 5448.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_V481-Lyr-pri\\
007939330-01 & 1581.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007939330-02 & 1581.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007939761-01 & 6934.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007939835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007940533-01 & 6167.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007940533-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007940533-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
007941200-01 & 0092.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007941635-01 & 5449.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
007943535-01 & 6935.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007943535-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007943602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007943602-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
007943602-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007943929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007943929-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007947631-01 & 6936.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007948108-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007948108-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007948108-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007948779-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007948784-01 & 1968.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007949593-01 & 4759.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007950644-01 & 0192.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007950775-01 & 6937.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007950775-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007950994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
007951015-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007951018-01 & 1553.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007953247-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007953880-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007953880-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007954107-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007954107-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007954278-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007954278-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007954705-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007955301-01 & 6938.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007955301-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007955545-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007955580-01 & 1711.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007955898-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007955898-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007955898-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007956132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007956461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007956461-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007956520-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007956547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007957709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007957881-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007957881-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007959579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007959867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
007959867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
007959867-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
007960295-01 & 6939.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007960410-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007960410-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007960547-01 & 6940.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007960980-01 & 2274.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007966705-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007967100-01 & 6941.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
007967100-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
007967293-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007967293-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007969047-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
007969754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007970283-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007970629-01 & 6942.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007970760-01 & 6943.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
007971389-01 & 6944.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007972785-01 & 0184.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007972785-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007973199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007973404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007973706-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
007973867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007973867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007974032-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007974032-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007974032-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
007974626-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007974634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007974634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007974634-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007974853-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007974853-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007974853-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007974877-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007975727-01 & 0418.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007975727-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007976136-01 & 6945.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
007976435-01 & 6946.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007976435-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007976520-01 & 0687.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007976845-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
007977197-01 & 0459.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007977197-02 & 0459.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
007977198-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007977198-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007977198-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007977198-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007977956-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
007977956-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007977996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007977996-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007978202-01 & 5454.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
007978226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007978226-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007978458-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
007979504-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007983108-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007983108-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007983117-01 & 3214.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007983117-02 & 3214.02 & PC & 0 & 0 & 0 & 0 & CENTROID\_SIGNIF\_UNCERTAIN\\
007983274-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
007983299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007983299-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
007983320-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007983320-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
007983756-01 & 3846.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
007983756-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
007984047-01 & 1552.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
007984574-01 & 2400.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007984890-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007984890-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007985134-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
007985167-01 & 6947.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
007985733-01 & 3219.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
007986162-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
007986166-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007986166-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007987086-01 & 3536.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007987749-01 & 6948.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
007987749-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
007987866-01 & 2363.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
007988039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007988343-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
007988343-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
007988962-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
007988962-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007988994-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007988994-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007988994-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007988994-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007988994-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007988994-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007988994-07 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007989079-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
007989079-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007989187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
007989187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
007989348-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
007989348-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
007989422-01 & 2151.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008004558-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008004558-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008004903-01 & 2594.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008006773-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008007174-01 & 5458.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008007262-01 & 7586.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008007644-01 & 2328.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008007675-01 & 6949.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008008067-01 & 0316.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008008067-02 & 0316.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008008067-03 & 0316.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008008128-01 & 6950.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008008128-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008008206-01 & 0569.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008008206-02 & 0569.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008009350-01 & 1569.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008009496-01 & \nodata & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_9:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_9:1---CLEAR\_APO---PARENT\_IS\_008009500-01\\
008009500-01 & 6951.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008012437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008012437-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008012437-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008013289-01 & 6952.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008013419-01 & 0901.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008013439-01 & 2352.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008013439-02 & 2352.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008013439-03 & 2352.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008015907-01 & 0517.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008016211-01 & 5460.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008016214-01 & 6953.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008016691-01 & 3286.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008016692-01 & 6954.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008017379-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008017703-01 & 0518.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008017703-02 & 0518.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008017703-03 & 0518.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008018340-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008018404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008018404-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008018547-01 & 0902.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008018769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008018769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008018769-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008019250-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008019250-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008022144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008022144-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008022244-01 & 0519.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008022244-02 & 0519.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008022489-01 & 2674.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
008022489-02 & 2674.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008022489-03 & 2674.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008023317-01 & 6049.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008023668-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008023848-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED---PARENT\_IS\_005443837-02\\
008024918-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008024918-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008025357-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008025357-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008025596-01 & 2615.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008026371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008026752-01 & 0240.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008026752-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
008026752-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
008026887-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008026887-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008027456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008027456-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008027456-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008027902-01 & 6955.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008028063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008029197-01 & 4147.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008098300-pri\\
008029546-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008029546-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008029848-01 & 5463.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008030148-01 & 0155.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008030339-01 & 3954.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008030339-02 & 3954.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008035262-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008035802-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008036287-01 & 3984.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008036315-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008036315-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008036426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008037038-01 & 5466.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008037145-01 & 0520.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008037145-02 & 0520.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008037145-03 & 0520.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008037145-04 & 0520.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008038388-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
008038609-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008038609-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008038609-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008038679-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008038679-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008038679-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008039892-01 & 0903.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008039925-01 & 6956.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
008041216-01 & 0237.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008042004-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008042044-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008042044-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008042044-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008042057-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008042057-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008042057-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008042453-01 & 2304.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008042644-01 & 6957.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008042789-01 & 3838.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008042789-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008042835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008043052-01 & 3695.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008043052-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008043299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008043299-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008043299-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008043436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008043436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008043436-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008043638-01 & 0460.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008043638-02 & 0460.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
008043714-01 & 1765.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008043714-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008043721-01 & 4812.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_008043961-pri\\
008043882-01 & 6169.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008043961-pri\\
008043968-01 & 5469.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008043961-pri\\
008044008-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_008043961-pri\\
008044016-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_008043961-pri\\
008044075-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008044075-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008044600-01 & 4612.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008044608-01 & 3523.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008044608-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008044889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008044889-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008045482-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008046010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008046010-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008046010-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008046223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008046659-01 & 1560.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008046689-01 & 3092.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008046934-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008046934-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008047283-01 & 3760.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008047283-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008047428-01 & 4747.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008051946-01 & 3038.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008052016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008052016-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008052016-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008052474-01 & 3640.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008052474-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008053021-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008053552-01 & 1549.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008054146-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008054719-01 & 4776.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008056286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008056286-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008056313-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008056319-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008056337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008056337-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008056337-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008056651-01 & 4869.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008056665-01 & 0089.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008056665-02 & 0089.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008056665-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008056861-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
008057693-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CROWDED\_DIFF\\
008058082-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008058082-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008058082-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008058127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008058127-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008058127-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
008058135-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_008058127-01\\
008058211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008058241-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008058507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008058507-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008059291-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008073705-01 & 3245.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008073806-01 & 2411.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008073821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
008073821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
008074328-01 & 2486.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008074805-01 & 2670.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008074805-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008075618-01 & 5471.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008075991-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008076630-01 & 2235.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008077137-01 & 0274.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008077137-02 & 0274.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008078502-01 & 3383.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008081187-01 & 1951.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008081239-01 & 3352.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008081389-01 & 6958.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008081389-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008081482-01 & 1539.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008081482-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008081566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008081899-01 & 2426.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008081905-01 & 2619.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008082001-01 & 1570.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008082478-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008085273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008085273-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008086490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008086490-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008086490-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008086600-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008087018-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008087018-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008087018-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008087018-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008087269-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008087812-01 & 4343.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008087887-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008088354-01 & 6959.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008091197-01 & 6960.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008092865-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008094120-01 & 4881.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008094120-02 & 4881.02 & FP & 0 & 0 & 0 & 1 & FIT\_FAILED---PARENT\_IS\_008094140-pri\\
008094140-01 & 6961.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008094140-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008094221-01 & 6962.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008095099-01 & 6171.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008095110-01 & 3619.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_6171.01\\
008095321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008095321-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008095441-01 & 2743.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008096395-01 & 7587.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008096395-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008097825-01 & 6963.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008098120-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008098120-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008098212-01 & 4487.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008098300-01 & 6964.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008098515-01 & 6965.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008098515-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008098728-01 & 2008.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008098728-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008098728-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008098728-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008098960-01 & 6966.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008099138-01 & 2338.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008103917-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008103917-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008103917-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008103917-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008104030-01 & 3269.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
008104030-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
008104065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008104065-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008104436-01 & 6967.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_006706287-pri\\
008104598-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008104598-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008105398-01 & 5475.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008105398-02 & 5475.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008106592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008106610-01 & 0570.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008106610-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008106973-01 & 7588.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
008106973-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008107225-01 & 0235.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008107380-01 & 0162.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008107611-01 & 4656.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008107903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
008108099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008108437-01 & 5478.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008108997-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008109107-01 & 4501.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008109934-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008110733-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008110733-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008110733-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008110757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008110767-01 & 2504.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008111381-01 & 1550.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008111381-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008111437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008111622-01 & 6968.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008111622-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008111622-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008111716-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008111919-01 & 2030.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008112013-01 & 6969.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008112039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008112039-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008112515-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008112584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008112584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008113154-01 & 1542.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008113154-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008113154-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008113154-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
008113255-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008114532-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008114532-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008114532-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008114921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008114921-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008114921-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
008115647-01 & 6970.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008120184-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008120608-01 & 0571.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008120608-02 & 0571.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008120608-03 & 0571.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008120608-04 & 0571.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008120608-05 & 0571.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
008120820-01 & 6971.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008121067-01 & 6050.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008121280-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008121310-01 & 0317.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008121328-01 & 3486.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008121586-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008122232-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008122232-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008122232-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008123127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008123127-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008123170-01 & 6972.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
008123197-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008123197-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008123197-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008123377-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008123377-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008123377-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008123377-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008123628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008123628-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM---PARENT\_IS\_009304367-02\\
008123645-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008123645-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008123645-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008123937-01 & 6973.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008124735-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008124735-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008124751-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008124751-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008124751-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008124788-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008124788-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008125219-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008125219-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008125219-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008125580-01 & 1014.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008125652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008125652-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008125652-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008125652-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008126371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008126422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008126422-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008126486-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008126486-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008126558-01 & 2259.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008127448-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008127586-01 & 1752.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008127607-pri\\
008127607-01 & 1919.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008127639-01 & 1012.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3713.01\\
008127648-01 & 3713.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008127684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008127684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008128067-01 & 4314.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008128067-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008128247-01 & 4094.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_008128965-pri\\
008128965-01 & 6974.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008129005-01 & 4741.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008128965-pri\\
008129189-01 & 6975.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008129189-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008129588-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008129619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008129631-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008129631-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008142547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008142547-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008142787-01 & 4005.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008142942-01 & 1985.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008143170-01 & 6976.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008143170-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008143646-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008143783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008144096-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008145462-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008145789-01 & 6977.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008145958-01 & 6978.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008149341-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008149341-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008149350-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008149484-01 & 4306.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM---PARENT\_IS\_008081389-pri\\
008150320-01 & 0904.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008150320-02 & 0904.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008150320-03 & 0904.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008150320-04 & 0904.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008150320-05 & 0904.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
008151055-01 & 3298.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008153568-01 & 6051.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008153568-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008153747-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008153747-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008153747-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008154223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008154223-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008154223-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008155291-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008155368-01 & 5481.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008155584-01 & 6979.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
008155654-01 & 6980.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008156120-01 & 0318.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008158127-01 & 1015.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008158127-02 & 1015.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008158127-03 & 1015.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008158324-01 & 6981.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008158429-01 & 5482.01 & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008160953-01 & 1858.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008161561-01 & 0688.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008161715-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008161715-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_008161816-01\\
008161808-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008161816-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_008161830-01\\
008161816-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_008161830-02\\
008161825-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET---PARENT\_IS\_008161830-02\\
008161830-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_008161816-01\\
008161830-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_008161816-02\\
008162376-01 & 6982.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_008094140-pri\\
008162789-01 & 0521.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008162789-02 & 0521.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008162790-01 & 1712.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_521.01\\
008164012-01 & 2116.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008164257-01 & 2073.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008164257-02 & 2073.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008164257-03 & 2073.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008164262-01 & 1810.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008164262-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008164262-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008164262-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE\\
008164812-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
008165617-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008165617-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008165946-01 & 2105.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008166299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008166299-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008166912-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008167504-01 & 6983.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008167922-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008167922-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008167922-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008167938-01 & 6052.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008167938-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008167978-01 & 6053.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008167978-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008167996-01 & 1867.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008167996-02 & 1867.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008167996-03 & 1867.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008168187-01 & 2209.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008168187-02 & 2209.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008168509-01 & 7589.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008168581-01 & 6054.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008168581-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008172936-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008173017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008173017-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008174072-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008174306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008174306-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008174306-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008174625-01 & 1017.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008175131-01 & 2139.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008175177-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008175399-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008175399-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008176564-01 & 2720.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008176634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008176650-01 & 0960.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008176650-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008176653-01 & 1016.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008176783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008177179-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008177179-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008177179-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008177179-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008177748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008177748-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008177748-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008177748-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008177798-01 & 3624.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008178616-01 & 6984.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008380743-pri\\
008178778-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008178778-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008178778-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008178825-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008179190-01 & 4196.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008179190-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008179325-01 & 2359.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008179747-01 & 5483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008180020-01 & 1741.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008180020-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008180063-01 & 0905.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008180063-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008180290-01 & 6985.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008181016-01 & 6174.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
008181415-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008181880-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008181880-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008182427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008182427-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008182857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008182857-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008183288-01 & 3255.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008183389-01 & 6986.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008183389-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008183389-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
008183404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008183805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008183911-01 & 1018.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008184075-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008184075-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008187917-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
008188157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008188157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008188360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008189641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008189641-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008189801-01 & 2480.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008190354-01 & 2781.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
008190627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008190627-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
008190872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008190872-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008191020-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008191020-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008191589-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008191589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008191589-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008191602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008191602-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008191602-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008191611-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008191611-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008191611-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008191672-01 & 0018.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
008192427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008192427-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008192427-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008192637-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008192637-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008192861-01 & 6987.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008192911-01 & 3058.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008193178-01 & 0572.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008193178-02 & 0572.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008193315-01 & 6988.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008193315-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008193441-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008193441-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008193441-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008193712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008194874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008194969-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008195877-01 & 6989.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008196180-01 & 6990.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
008196180-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
008196226-01 & 4634.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008196840-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008196903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008196903-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008197019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008197019-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008197176-01 & 5485.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008197220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008197220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008197343-01 & 1746.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008197355-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008197355-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008197355-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008197406-01 & 5486.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008197544-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
008197544-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008197560-01 & 3074.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008197653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008197761-01 & 6175.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008197788-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008197788-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008197788-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008197793-01 & 3123.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008198031-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008198031-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008198031-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008210018-01 & 2762.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008210721-01 & 6991.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008211521-01 & 6992.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008212002-01 & 2593.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008212251-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008212251-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008213326-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008213326-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008216763-01 & 4838.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008216763-02 & 4838.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008216910-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008217331-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008218274-01 & 1064.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008218379-01 & 1920.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008218379-02 & 1920.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008218649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008218803-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008219268-01 & 2133.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
008219673-01 & 0419.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008222156-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008222627-01 & 4098.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008222690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008222690-02 & \nodata & FP & 1 & 0 & 1 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008222813-01 & 1069.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008222813-02 & 1069.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008223328-01 & 1767.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
008223328-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008223568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008223568-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008223655-01 & 5488.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008223931-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008226050-01 & 1910.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008226994-01 & 0906.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008226994-02 & 0906.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008226994-03 & 0906.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008227086-01 & 6993.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008227464-01 & 6994.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008227661-01 & 2826.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008227661-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008229048-01 & 6995.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008229074-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008229458-01 & 2238.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008229696-01 & 1072.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008230616-01 & 1713.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008230616-02 & 1713.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008230809-01 & 6055.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008230809-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008231370-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008231370-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008231370-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008231370-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
008231667-01 & 3494.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008231830-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008231877-01 & 6996.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008233072-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008233072-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008233326-01 & 4834.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008233504-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008233702-01 & 2140.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008233802-01 & 3302.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008233804-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008233804-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008234477-01 & 6997.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008234889-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008235853-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008235853-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008235924-01 & 2347.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008236479-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008236479-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008240109-01 & 6998.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008240109-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008240123-01 & 3826.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008240109-pri\\
008240797-01 & 1809.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008240797-02 & 1809.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008240861-01 & 6999.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008240904-01 & 1070.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008240904-02 & 1070.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008241079-01 & 3020.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008242350-01 & 5493.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008242434-01 & 1726.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008242681-01 & 1065.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008242681-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008242709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008243263-01 & 7000.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008243283-01 & 2952.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008243263-pri\\
008243804-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008243804-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008244173-01 & 3545.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
008244190-01 & 1071.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3545.01\\
008244295-01 & 7001.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_3545.01\\
008244755-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008244755-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008244755-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008244757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008244757-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008244757-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008244758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008244758-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008245118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008245132-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
008245192-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008245192-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008245197-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008245197-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008245366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008245366-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008246781-01 & 1067.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008246833-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008246833-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008247116-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008247116-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008247543-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008247543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008247638-01 & 0907.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008247638-02 & 0907.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008247638-03 & 0907.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008247638-04 & 0907.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008247770-01 & 2569.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008247771-01 & 2344.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008248103-01 & 7002.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008248415-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
008248630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008248630-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008248939-01 & 0061.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008250687-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008250824-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008250824-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008251079-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008254882-01 & 4164.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008254901-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008255058-01 & 5495.01 & FP & 0 & 0 & 1 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
008255272-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008255272-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008255272-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008255799-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008255799-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008255887-01 & 0908.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008256044-01 & 3652.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008256049-01 & 0909.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3652.01\\
008256453-01 & 2573.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008256478-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008256478-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008256643-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_008456151-01\\
008256643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008256643-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008256882-01 & 7003.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008257115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008257205-01 & 1986.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008257205-02 & 1986.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008257407-01 & 1063.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008257407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008257407-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008258103-01 & 7590.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF\\
008258160-01 & 3870.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008258160-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008258171-01 & 0286.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_008258160-01\\
008258171-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008258160-02\\
008258171-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008258171-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
008259061-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008259061-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008259061-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008259177-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
008259177-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008259183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008259709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008259713-01 & 2935.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008259713-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008259713-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008259713-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008259835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008260198-01 & 3888.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
008260218-01 & 1066.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008260234-01 & 2085.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1066.01\\
008260818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008260818-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008260885-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008260902-01 & 2144.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008261157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008261157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008261920-01 & 2174.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008261920-02 & 2174.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008261920-03 & 2174.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008262210-01 & 1073.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_008262223-pri\\
008262223-01 & 7004.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008262223-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008262409-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008262409-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008262436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008262436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008262490-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008263545-01 & 2822.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008263746-01 & 3581.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008263746-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008263746-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---KIC\_OFFSET\\
008263746-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008263752-01 & 3338.02 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3581.01\\
008263752-02 & 3338.01 & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008263746-02\\
008263882-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008263970-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008263970-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008264037-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008264037-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264061-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008264070-01 & 1068.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3655.01\\
008264097-01 & 3655.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
008264097-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008264287-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
008264304-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008264402-01 & 4037.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008264404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264404-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008264492-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008264492-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008264494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008264494-03 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008264494-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008264526-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008264543-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_008264588-01\\
008264543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008264543-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264543-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008264546-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008264546-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008264546-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
008264550-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008264550-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264565-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264581-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008264583-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264583-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264588-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_008264543-01\\
008264588-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264588-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264588-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008264623-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008264623-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008264635-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008264667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008264667-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008264667-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008264674-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264674-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264674-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008264674-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008264674-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008264698-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008264698-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008264706-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264706-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008264708-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
008264708-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008264720-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008264767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
008264949-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008264949-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008265022-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008265022-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008265068-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008265068-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008265068-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008265126-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008265126-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008265156-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CROWDED\_DIFF\\
008265156-02 & 6177.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008265204-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008265218-01 & 0522.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008265244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008265244-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF\\
008265269-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008265481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008265520-01 & 7005.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008265528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008265876-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008265876-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008265921-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_008265951-pri\\
008265921-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_008265951-sec\\
008265953-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_008265951-pri\\
008265953-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_008265951-sec\\
008265990-01 & 7006.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_008265951-pri\\
008265993-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_008265951-pri\\
008265993-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_008265951-sec\\
008266004-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_008265951-pri\\
008266276-01 & 1731.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008266276-02 & 1731.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008277004-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008277797-01 & 1820.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008277797-02 & 1820.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008278073-01 & 4799.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008278371-01 & 1150.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008278685-01 & 4435.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008279765-01 & 1130.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008279765-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008280511-01 & 1151.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008280511-02 & 1151.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008280511-03 & 1151.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008280511-04 & 1151.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
008280511-05 & 1151.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008280615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008282651-01 & 2193.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008282730-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008282730-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008282730-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008282846-01 & 4015.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008283875-01 & 7007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008284676-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008285254-01 & 7008.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
008285254-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008285787-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008285970-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008285970-02 & 7009.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008288248-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008288404-01 & 5498.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
008288553-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008288719-01 & 7010.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008288947-01 & 1142.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008289804-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008292150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008292150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008292840-01 & 0260.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008292840-02 & 0260.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008292840-03 & 0260.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008293692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008293692-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008294484-01 & 7011.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
008294484-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
008295531-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008295671-01 & 4593.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---LARGE\_RM\\
008295671-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008296467-01 & 7012.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008296467-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008296467-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008296467-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008296467-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008296467-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008297017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008297017-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008297017-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008297319-01 & 7591.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008299332-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008299332-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008299332-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008299947-01 & 3631.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008299955-01 & 1147.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3631.01\\
008301013-01 & 7013.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008301878-01 & 3301.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008302223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008302302-01 & 3732.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
008302450-01 & 1144.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_008302455-01\\
008302455-01 & 7014.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008302473-01 & 7015.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_008302455-01\\
008307165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008308260-01 & 4436.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008308347-01 & 3761.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
008308347-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
008308526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008310243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008310243-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008310243-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008311110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008311110-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008311110-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008311180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008311180-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008311304-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008311304-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008311304-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008311534-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008311864-01 & 7016.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
008312222-01 & 7017.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008312222-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008312852-01 & 1143.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008313144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008313144-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008313667-01 & 1145.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008314392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008314392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008314392-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008314487-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008314525-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008314525-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008314525-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008314525-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008314525-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008314801-01 & 7018.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT\\
008314801-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008315394-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
008316195-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008316195-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008316195-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008316503-01 & 7019.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008316526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008320630-01 & 4846.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008320954-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008321252-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008321270-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
008321270-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008321314-01 & 2293.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008321604-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008321604-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
008322177-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008322177-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008322243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008322243-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008322243-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008322263-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008322861-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008322861-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008322973-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008322973-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
008323096-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008323096-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008323096-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008323104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008323753-01 & 0175.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3767.01\\
008323764-01 & 3767.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
008324032-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008324268-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008324292-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008324292-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008324305-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008324305-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008324490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008324490-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008324490-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008324518-01 & 4393.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008326342-01 & 2680.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008326356-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008326356-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008326936-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008327660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008327675-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008328005-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008328005-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008328005-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008329014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008329014-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008329014-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008329062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008329062-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008329506-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008329629-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008329629-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008329728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008329728-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008329728-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008329790-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008330056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008330102-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008330102-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008330102-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008330207-01 & 4390.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008330312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008330312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008330548-01 & 1132.01 & FP & 0 & 1 & 1 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008330575-01\\
008330548-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008330575-01 & 7020.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008330712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008330790-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008330790-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008330790-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008330895-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008330895-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008330895-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008330910-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008331612-01 & 3318.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008331612-02 & 3318.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008331919-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008331919-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008331919-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008332279-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008332279-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008332383-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008332383-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008332426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008332521-01 & 4567.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008332521-02 & 4567.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008332986-01 & 1137.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008344004-01 & 0573.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008344004-02 & 0573.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008344042-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008344381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008344381-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008345172-01 & 2385.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008345358-01 & 7021.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
008345358-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
008345384-01 & 4399.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CROWDED\_DIFF\\
008346392-01 & 1141.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008346686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008346686-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008349399-01 & 4763.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008349582-01 & 0122.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008351704-01 & 1146.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008351778-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008351778-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008351778-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008351916-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008352420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008352420-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008352420-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008352439-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008352439-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008352537-01 & 0420.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008355131-01 & 4711.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008355178-01 & 6178.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008355207-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008355239-01 & 0574.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008355239-02 & 0574.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008356054-01 & 3424.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008356054-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008356054-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008356054-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008357961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008357961-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008358008-01 & 7022.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008358008-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008358012-01 & 2929.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_008358008-01\\
008358253-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008358253-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008359498-01 & 0127.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008359671-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008359671-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008359671-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
008359848-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008359848-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008359848-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008360041-01 & 4854.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008360640-01 & 2982.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008361905-01 & 0689.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008362204-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008362880-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008362880-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008362899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008362899-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
008362899-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008362974-01 & 7023.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008364115-01 & 6056.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_008364119-01\\
008364115-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008364119-02\\
008364119-01 & 7024.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008364119-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008364249-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008364969-01 & 5508.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008365739-01 & 3722.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008365739-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008367113-01 & 0575.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008367298-01 & 7025.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008367410-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008367644-01 & 1879.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008374077-01 & 6179.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008374396-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008374396-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008374494-01 & 1133.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008374499-01\\
008374494-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008374499-02\\
008374499-01 & 7026.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008374499-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008374580-01 & 0615.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008375132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008375665-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008375665-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008376471-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008376471-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008376471-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008376848-01 & 4007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008377197-01 & 4727.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008377201-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008377201-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008377511-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008377511-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008377511-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008378590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008378634-01 & 1139.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008378656-pri\\
008378634-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008378656-pri\\
008378656-01 & 7027.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008378779-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
008378922-01 & 7028.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008378922-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008379021-01 & 3268.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008379547-01 & 7029.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008379547-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008379705-01 & 2507.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008379705-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008379833-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008379833-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008379833-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008379965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008379965-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
008379965-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008380088-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008380088-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008380088-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008380242-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008380389-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008380389-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008380389-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008380389-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008380709-01 & 2468.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008380743-01 & 5510.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008381204-01 & 2145.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008381234-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008381592-01 & 7030.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008381693-01 & 4017.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008382075-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_008382182-pri\\
008382114-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_008382182-pri\\
008382207-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008382207-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008382223-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_008382182-pri\\
008382253-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008382339-01 & 7031.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008385813-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008386122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008386122-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008386122-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008386158-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008388318-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008388399-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008388610-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008388610-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008388610-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008389052-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008389518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008389518-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008389948-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008389948-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008390631-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008390631-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008390631-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008390667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008391086-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008391086-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
008391983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008392519-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008394475-01 & 7032.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008394721-01 & 0152.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008394721-02 & 0152.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008394721-03 & 0152.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008394721-04 & 0152.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008394753-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008394753-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008394756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008394756-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008395203-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008395660-01 & 0116.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008395660-02 & 0116.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008395660-03 & 0116.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008395660-04 & 0116.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008395860-01 & 4724.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008396062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008396062-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008396062-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008396184-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008396259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008396259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008396288-01 & 5512.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008396309-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008396405-01 & 1733.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008396660-01 & 4407.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008396791-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008396901-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008396901-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008396901-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008397017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008397138-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008397138-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008397426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008397426-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008397426-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008397446-01 & 1135.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
008397675-01 & 1140.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
008397947-01 & 4772.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008398221-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008398290-01 & 7033.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
008398290-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008398303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008409295-01 & 3404.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008409588-01 & 0690.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
008410415-01 & 2291.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008410490-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
008410637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008410727-01 & 1148.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008410727-02 & 1148.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008411693-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008411693-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008411947-01 & 7034.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008413996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008414116-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008414159-01 & 7035.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008414159-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008414159-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
008414216-01 & 7036.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_008414159-01\\
008414492-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008414716-01 & 0910.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008414845-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008414907-01 & \nodata & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_5513.01\\
008414907-02 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008414907-03 & 1134.02 & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_008414914-02\\
008414907-04 & 1134.01 & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_5513.01\\
008414907-05 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_008414914-02\\
008414914-01 & 5513.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008414914-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008415109-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008415200-01 & 2730.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008415745-01 & 1138.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008415752-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008415752-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008415863-01 & 7037.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008415863-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008415928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008416152-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008416523-01 & 4441.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008416523-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008416925-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008417078-01 & 4693.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008420490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008420644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008420644-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008420752-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008420752-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
008423344-01 & 7592.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008423903-01 & 7038.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008424002-01 & 3497.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008424446-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008424446-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008424446-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008424446-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008426007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008426567-01 & 1914.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008427895-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008429314-01 & 2624.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008429314-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008429415-01 & 2965.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008429450-pri\\
008429450-01 & 7039.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008429528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008429528-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008429528-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
008429528-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008429566-01 & 2511.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008429634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008429634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008429668-01 & 4449.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008429756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008429756-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008429817-01 & 5515.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008430053-01 & 4603.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008430105-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008430105-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008430105-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008430119-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008430119-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008430119-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008430954-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008430964-01 & 3078.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
008431006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008431006-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008431006-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008431372-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008432040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008432040-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008432040-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008432959-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008432962-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008432962-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008435232-01 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008435232-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008435232-03 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008435232-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008439323-01 & 4153.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008439566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008439566-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008439566-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008442040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008442040-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008442437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
008442437-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008442795-01 & 7040.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008443132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008443311-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008443311-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008443311-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008443527-01 & 3197.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008443812-01 & 7041.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
008444552-01 & 1769.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008444802-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008444802-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008444802-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008444868-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008444868-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008444868-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008444868-04 & 7593.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008445775-01 & 7042.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008445775-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
008446738-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008446738-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008446738-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008450600-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008450600-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008450600-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008450600-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
008451143-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008451777-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008451868-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008452639-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008452639-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008453191-01 & 7043.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008453211-01 & 0236.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008453191-01\\
008453214-01 & 1776.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008453191-01\\
008453324-01 & 7044.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008453431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008453431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008453527-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008453722-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008453722-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008453851-01 & 4565.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008454250-01 & 1254.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008454250-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008454553-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008454553-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008454553-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008454553-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008455627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008455848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008455848-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008455998-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008456151-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008456679-01 & 0102.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008456679-02 & 0102.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008456728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008457330-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008457330-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008458207-01 & 6057.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008458207-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008458662-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008458662-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008458690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008458690-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008459354-01 & 3863.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008459354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008459354-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008459663-01 & 4356.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008460081-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008460126-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008460126-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008460126-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008460600-01 & 1730.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
008460600-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
008460993-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008460993-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008461529-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008461529-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008461529-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008461529-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008461967-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008461967-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008462258-01 & 1253.01 & FP & 0 & 0 & 1 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
008463118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---CROWDED\_DIFF\\
008463118-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
008463118-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008463272-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008463346-01 & 2529.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008463346-02 & 2529.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008474365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008474365-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008474898-01 & 0576.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5520.01\\
008474900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008478994-01 & 0245.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008478994-02 & 0245.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008479107-01 & 7045.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008479386-01 & 7046.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008480235-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008480263-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008480263-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008480263-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008480285-01 & 0691.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008480285-02 & 0691.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008480582-01 & 4386.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008480642-01 & 5521.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008481000-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008481000-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008481006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008481006-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008481129-01 & 2402.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008487242-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008487645-01 & 4254.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008487748-01 & 3905.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2277-Cyg-pri\\
008487805-01 & 4206.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2277-Cyg-pri\\
008487838-01 & 4596.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V2277-Cyg-pri\\
008488717-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008488717-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008488876-01 & 7047.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_1248.01\\
008488876-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008488876-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
008488876-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
008488878-01 & 1248.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008490255-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008490255-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008490255-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008490993-01 & 0911.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008490993-02 & 0911.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008491152-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008491152-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008491277-01 & 0234.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008491447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008491745-01 & 3555.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008491745-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008491816-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008491816-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008491816-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008492026-01 & 2016.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008492101-01 & 4437.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_008621026-pri\\
008493159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008493159-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008493159-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008493354-01 & 4505.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494142-01 & 0370.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494142-02 & 0370.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494263-01 & 1255.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008494280-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008494410-01 & 3685.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494410-02 & 3685.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494542-01 & 2204.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494617-01 & 2389.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008494769-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008494783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008494783-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008494783-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008494783-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008495232-01 & 5524.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008495415-01 & 2362.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008495415-02 & 2362.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008495616-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008495616-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008496367-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008496367-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008496367-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008496883-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
008499639-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008499639-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008499639-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008499900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008500899-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008500899-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008500899-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008504544-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008504570-01 & 7048.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008505554-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
008505554-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008505670-01 & 0912.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008505670-02 & 0912.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008505920-01 & 2094.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008505920-02 & 2094.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008505928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008506388-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008506388-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008506388-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008506766-01 & 0138.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008506766-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008507040-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
008507073-01 & 5527.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
008507325-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008507325-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008507325-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008507475-01 & 4300.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008508126-01 & 4299.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008508126-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008508981-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008508981-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008509346-01 & 7049.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008509346-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
008509361-01 & 1280.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008509346-01\\
008509442-01 & 2992.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008509469-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008509469-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008509694-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008509694-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_008509703-01\\
008509694-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008509703-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008509781-01 & 5529.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008510314-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008510534-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008510534-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008510534-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008516008-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008516008-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008516008-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008516041-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008516686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008516686-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008517303-01 & 6181.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008517361-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008517378-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008517433-01 & 7050.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008517859-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008517859-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008518426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008518426-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008519253-01 & 1267.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008519253-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008520426-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008520426-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008520433-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008520433-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008520436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008520436-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008520436-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
008520456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008521059-01 & 4093.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008521098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008521128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008521128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008522919-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008523427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008523595-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008523595-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008523595-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008523871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008523871-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008523871-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
008524110-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_6060.01\\
008524346-01 & 4083.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_3518.01\\
008524464-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008524464-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008524464-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008524481-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
008524481-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008524712-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
008524712-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008524728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
008525024-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008525214-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008525214-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
008525286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
008525286-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
008526241-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008526387-01 & 7051.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008526451-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008526451-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008526451-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008527297-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008539939-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008539939-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008539939-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008542993-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008542993-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008543100-01 & 1975.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008543102-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008543278-01 & 7052.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
008543278-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
008543279-01 & 3759.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_008543278-01\\
008543279-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008543278-01\\
008544992-01 & 2466.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008544992-02 & 2466.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008544996-01 & 0913.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008546542-01 & 3073.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008546937-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008546937-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008547140-01 & 1266.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008547366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008547429-01 & 2658.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008552202-01 & 0914.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008552365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008552498-01 & 1272.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_V2277-Cyg-pri\\
008552498-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
008552500-01 & 7053.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2277-Cyg-pri\\
008552540-01 & 7054.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
008552540-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008552540-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008552565-01 & 1277.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET---PARENT\_IS\_V2277-Cyg-pri\\
008552583-01 & 1265.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2277-Cyg-pri\\
008552587-01 & 3941.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_V2277-Cyg-pri\\
008552607-01 & 5542.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_V2277-Cyg-pri\\
008552719-01 & 1792.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008552719-02 & 1792.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008552719-03 & 1792.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008552907-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008552907-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008552947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008553462-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008553462-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008553788-01 & 7055.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008553907-01 & 7056.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008553907-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008554446-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008554498-01 & 0005.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008554701-01 & 3315.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008555360-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008556061-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008556077-01 & 2027.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008556233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008556233-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008556233-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008557374-01 & 0692.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008557374-02 & 0692.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008557474-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008557474-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008558011-01 & 0577.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008558011-02 & 0577.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008559125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008559146-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008559146-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008559152-01 & 2488.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008559208-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008559589-01 & 3697.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008559589-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008559644-01 & 0139.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008559644-02 & 0139.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008559796-01 & 7057.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008559863-01 & 7058.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008559863-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008559962-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008560194-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
008560285-01 & 1249.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
008560285-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
008560475-01 & 5543.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008560804-01 & 2969.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_008560861-01\\
008560804-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_008560861-02\\
008560840-01 & 1263.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_008560861-01\\
008560840-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_008560861-02\\
008560861-01 & 7059.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008560861-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008560867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008560867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008560867-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
008560921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008560940-01 & 3450.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_008560861-01\\
008560996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008560996-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008561063-01 & 0961.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008561063-02 & 0961.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008561192-01 & 5544.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
008561231-01 & 2346.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008564587-01 & 1270.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008564587-02 & 1270.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008564674-01 & 2022.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008564674-02 & 2022.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008564695-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008564976-01 & 3890.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008565229-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008565229-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008565229-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008565266-01 & 0578.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008565900-01 & 7060.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008565912-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008566113-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008566113-02 & 7061.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008566353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008569819-01 & 7062.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008569819-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008569819-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008569986-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008569986-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008569986-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008570117-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008570117-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008570117-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008570333-01 & 2436.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008571022-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008571022-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008571125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008571795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008571795-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008571822-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008572168-01 & 4263.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008572324-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008572324-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008572936-01 & 2459.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED\\
008572936-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008572936-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008572936-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
008572936-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008573168-01 & 4610.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008573193-01 & 4337.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008573459-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008573459-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008573774-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008573774-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008573774-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008573774-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008574270-01 & 7063.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008574270-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008574652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008574840-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008574840-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008578742-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008578742-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008578780-01 & 2023.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008579615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008579615-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008579615-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008579615-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008579684-01 & 7594.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008579684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008580028-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008580028-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008580028-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008580028-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008580228-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008580228-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008580228-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008580228-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008580438-01 & 6058.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008580438-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008581232-01 & 6059.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
008581232-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008581240-01 & 3111.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008581240-02 & 3111.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008581658-01 & 7064.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008581658-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008582121-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008582291-01 & 2330.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008582533-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008582533-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008583696-01 & 1275.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008583770-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008583770-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008584222-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008585472-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008585472-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008585472-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008586745-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008586745-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008586745-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008586760-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008588031-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008588031-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008588031-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008588377-01 & 3861.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008589526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008589526-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008589731-01 & 3668.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3518.01\\
008589754-01 & 3518.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008590149-01 & 6182.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008590527-01 & 7065.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
008590553-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008590553-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008590780-01 & 6183.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
008590780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008591109-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
008591109-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008591109-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
008591173-01 & 2181.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008591404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008591498-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008591693-01 & 2123.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008604575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008604993-01 & 7066.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008604993-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008605074-01 & 0915.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008605074-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008605096-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008608260-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008608260-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008608260-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008608490-01 & 7067.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008609193-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008609193-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008609450-01 & 1278.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008609450-02 & 1278.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008609450-03 & 1278.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008609450-04 & 1278.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008610168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008610483-01 & 7068.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008610483-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008610483-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008611257-01 & 2931.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008611781-01 & 2185.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008611832-01 & 2414.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008611832-02 & 2414.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008612275-01 & 2111.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008612275-02 & 2111.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008612847-01 & 1264.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008613236-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
008613446-01 & 7069.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008613535-01 & 2263.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008613535-02 & 2263.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008613594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008613594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008613594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008616637-01 & 0579.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008616637-02 & 0579.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008616873-01 & 1251.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
008617363-01 & 2945.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008618226-01 & 7070.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008618728-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_008554005-pri\\
008619436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008619448-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_008619436-01\\
008619448-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008620402-01 & 3267.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008620561-01 & 3753.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
008620565-01 & 1250.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_008620561-01\\
008620684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008621026-01 & 7071.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008621348-01 & 0461.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3682.01\\
008621348-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008621353-02\\
008621353-01 & 3682.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008621353-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008622268-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008622268-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008622268-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008623953-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008623953-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008624143-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008624520-01 & 1816.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008624860-01 & 7072.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008625408-01 & 7073.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008625632-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
008625632-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008625732-01 & 4701.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008560861-01\\
008625813-01 & 3285.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1859.01\\
008625821-01 & 1859.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008625821-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008625925-01 & 0580.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008626219-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008626219-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008626219-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008626219-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008626325-01 & 4775.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008628665-01 & 3434.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008628758-01 & 1279.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008628758-02 & 1279.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008628761-01 & 4580.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008628973-01 & 0916.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008630254-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008630254-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008630254-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008630788-01 & 1258.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008630788-02 & 1258.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008630788-03 & 1258.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008631160-01 & 1271.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008631504-01 & 2503.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008631751-01 & 2453.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008635938-01 & 3498.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM---PARENT\_IS\_008700506-01\\
008636333-01 & 3349.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008636434-01 & 3946.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008636539-01 & 2656.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008636600-01 & 4478.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008638036-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008638728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008639063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008639063-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008639063-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008639063-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008639063-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008639155-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
008639908-01 & 2700.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008640132-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008640132-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008643851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008643851-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008643851-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008643880-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008643880-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
008644288-01 & 0137.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008644288-02 & 0137.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008644288-03 & 0137.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008644365-01 & 3384.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008644365-02 & 3384.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008644545-01 & 5552.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008644911-01 & 5553.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008644943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008645191-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---LARGE\_RM\\
008645191-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008645191-03 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008645806-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008645806-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008645874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008645874-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008645874-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008645874-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008646141-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008646213-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008646235-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008646235-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008646235-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008646425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008646425-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008646702-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
008646702-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
008647299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008647299-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008647299-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008647753-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008647753-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008647777-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008647777-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008648866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008648866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008649198-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008649876-01 & 7595.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008650155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008650155-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008650155-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008650819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008650819-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008650819-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008650819-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008651389-01 & 1754.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008651452-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008651452-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008651452-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008651551-01 & 3841.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
008652213-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008652213-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008652360-01 & 4562.02 & FP & 0 & 0 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008652360-02 & 4562.01 & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008652577-01 & 4458.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008652939-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008652939-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008652999-01 & 1953.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008653100-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008653100-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008653134-01 & 6186.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008653183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008653563-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008653563-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008653675-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008653675-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008654122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008654122-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008654122-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
008654122-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008654540-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008654540-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008654790-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008654790-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008654790-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008655354-01 & 0917.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008655354-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
008655458-01 & 6060.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
008655712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008655712-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008656375-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008656375-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008656391-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008668810-01 & 3538.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008668810-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
008669092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008669092-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008672910-01 & 0918.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008676148-01 & 2544.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008677034-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008677034-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008677952-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008678594-01 & 1261.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008678594-02 & 1261.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008678664-01 & 1782.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008680979-01 & 1891.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008680979-02 & 1891.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008681734-01 & 2340.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008681833-01 & 2865.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008682015-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008682094-01 & 7596.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008682555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008682555-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008684359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008684730-01 & 0319.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008685497-01 & 1629.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008686097-01 & 0374.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008686150-01 & 0919.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008686150-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008686373-01 & 4066.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008686442-01 & 7074.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
008686975-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008686975-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008686975-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008687088-01 & 2749.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008687088-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008689031-01 & 0920.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008689373-01 & 0921.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008689373-02 & 0921.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008689373-03 & 0921.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008689793-01 & 1893.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008690001-01 & 7075.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
008690471-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008692861-01 & 0172.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008692861-02 & 0172.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008692983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008693536-01 & 7076.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008693545-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008693545-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008693545-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008694197-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008694309-01 & 4027.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008694481-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008695156-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008695156-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008695156-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008695311-01 & 3042.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008695628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008695628-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008695779-01 & 6061.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008695779-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008700506-01 & 7077.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008700506-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008700506-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008700529-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008700537-01 & 4170.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_008700506-02\\
008700537-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_008700506-01\\
008700558-01 & 0320.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008700558-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008700771-01 & 1283.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008700895-01 & 4523.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008701099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008701099-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008701099-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008701124-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008701124-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008701276-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008701327-01 & 7078.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008701662-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008701662-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008702381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008702424-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008702874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008702921-01 & 6187.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008702921-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008703129-01 & 2758.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008703413-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008703413-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008703884-01 & 1262.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008703887-pri\\
008703887-01 & 0287.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008703887-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008703887-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED---PARENT\_IS\_1262.01\\
008703887-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008703887-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---SATURATED\\
008707354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008707639-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008707670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008707670-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008709688-01 & 3019.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008709688-02 & 3019.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
008710207-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008710207-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008711527-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008711548-01 & 7079.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008711548-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008711555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008711794-01 & 0105.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008711908-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008712155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008712760-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008712760-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008713594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008713594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008713594-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008713828-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008713828-02 & 7080.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008714856-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008714886-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008715392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008715392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008715589-01 & 5563.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008716028-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008716028-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008716028-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008717065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008717065-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008717065-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008717374-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008717374-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008718273-01 & 5564.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008718465-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008718678-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008718678-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008719324-01 & 3716.02 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008719324-02 & 3716.01 & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008719324-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008719419-01 & 3506.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008719675-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008719897-01 & 7081.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008733497-01 & 3527.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008733898-01 & 2842.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008733898-02 & 2842.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008733898-03 & 2842.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008736245-01 & 7082.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008737501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008738115-01 & 7083.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008738115-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008738244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008738244-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008738591-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008738735-01 & 0693.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008738735-02 & 0693.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008738775-01 & 3432.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008739209-01 & 7084.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008739366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008739952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008740378-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008740898-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
008740898-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008740898-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008740898-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008741367-01 & 5566.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008741470-01 & 4251.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008742270-01 & 5567.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008742590-01 & 1281.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008745553-01 & 5568.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008745924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008745924-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008746295-01 & 2475.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008746310-01\\
008746310-01 & 7085.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008746310-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008747222-01 & 5569.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008747222-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008747357-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008747735-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008747865-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008747865-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008747865-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008747904-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V2277-Cyg-pri\\
008748251-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008748251-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008748251-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008748251-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008748670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008748670-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008749284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008750043-01 & 2017.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008750094-01 & 7086.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008750094-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008750446-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008750446-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008751056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008751056-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008751056-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008751770-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008751796-01 & 3125.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008751933-01 & 1257.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008752359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008752359-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008752359-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008752493-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008752493-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008752817-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_008817929-01\\
008752817-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008752914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008752940-01 & 4730.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008753023-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008753657-01 & 0321.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008753657-02 & 0321.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008753657-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008753896-01 & 2473.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008753896-02 & 2473.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008754603-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008754603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008754603-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008754603-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008756819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008757649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008757824-01 & 2552.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008757910-01 & 1269.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008758136-01 & 3006.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_008758161-01\\
008758161-01 & 7087.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008758204-01 & 2841.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008758366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008758366-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008758366-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008759145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008759145-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008760040-01 & 2963.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008760040-02 & 2963.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008760135-01 & 3524.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008760135-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008760760-01 & 7088.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008760767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008760767-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008765560-01 & 3891.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008766222-01 & 1260.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008766285-01 & 5571.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---SATURATED---PARENT\_IS\_1260.01\\
008766405-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008766619-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008766619-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008766619-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008766650-01 & 1904.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008766808-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008767034-01 & 7089.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
008771498-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008771498-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008771498-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008772391-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008773015-01 & 4301.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008773015-02 & 4301.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008773445-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008773445-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008773869-01 & 0462.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008773948-01 & 7090.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
008773948-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
008773948-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
008773961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008773961-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008776920-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008776920-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008777524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008777609-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008777609-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008777609-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008777843-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008777843-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008777843-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008779047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008779047-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008779891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008779891-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008779891-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008780099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
008780959-01 & 3741.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008780968-01\\
008780959-02 & 3741.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008780959-03 & 3741.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008780959-04 & 3741.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008780959-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008780959-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008780968-01 & 3653.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008782002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008782002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008782561-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008782561-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008782805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008782805-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008782805-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008782821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008782821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008783270-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008783270-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008783270-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008784288-01 & 7091.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008801316-01 & 2956.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008801343-01 & 1247.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008801343-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008801343-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008802165-01 & 0694.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008802693-01 & 2000.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008803757-01 & 4904.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008803940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008804261-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008804283-01 & 1276.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008804283-02 & 1276.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008804358-01 & 7092.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
008804397-01 & 1853.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008804455-01 & 2159.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
008804455-02 & 2159.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008804845-01 & 2039.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008804845-02 & 2039.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008805348-01 & 0695.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008805736-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008806072-01 & 1273.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008806123-01 & 0523.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008806123-02 & 0523.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008806985-01 & 4588.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008807057-01 & 7093.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008811490-01 & 4811.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008811811-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008812045-01 & 3481.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008812627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008812627-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008812627-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008813491-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT\\
008813698-01 & 1268.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008815279-01 & 7094.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008815923-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008816310-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008816310-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008816310-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008816832-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
008816881-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008816959-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008817159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008817759-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS---PARENT\_IS\_008817929-01\\
008817926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008817929-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_008817759-01\\
008818050-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_008752817-02\\
008818095-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS---PARENT\_IS\_008817929-01\\
008818497-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008818497-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008818497-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008819528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008819528-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008819528-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008822216-01 & 0581.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008822216-02 & 0581.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008822366-01 & 1282.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008822421-01 & 6188.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
008822585-01 & 7095.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008822585-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008822585-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008823397-01 & 7096.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
008823397-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008823426-01 & 1259.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_008823397-pri\\
008823833-01 & 3968.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_008823397-pri\\
008823868-01 & 0081.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008823868-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008823868-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008823893-01 & 5575.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---LARGE\_RM---PARENT\_IS\_008823397-pri\\
008823893-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008824737-01 & 3347.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008825320-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008826007-01 & 3266.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008826102-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008826168-01 & 1850.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008826317-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008826317-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008826718-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
008826718-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008826878-01 & 0922.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008827407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008827407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008827505-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008827572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008827572-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008827572-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008827575-01 & 3052.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008827575-02 & 3052.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008827821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008827821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008827821-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008827930-01 & 3801.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008827961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008831932-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008832417-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008832512-01 & 1821.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008836888-01 & 2508.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008837530-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008837839-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008838950-01 & 2421.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008838950-02 & 2421.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008839947-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008840004-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008840083-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008840083-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008840083-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008840083-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008840117-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008840117-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008840117-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008840117-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008840117-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008841616-01 & 7097.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008841616-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
008841813-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008841813-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008841813-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008841894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008841894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008842025-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008842025-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008842494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008842494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008842494-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008842494-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008843082-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008843268-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008843313-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008843313-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008843687-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008845026-01 & 0044.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008845026-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008845205-01 & 0463.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008845221-01 & 7098.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008845312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008845312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008845552-01 & 7099.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008845574-01 & 1734.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008845574-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008846809-01 & 7597.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008846823-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008846848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008846900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008847111-01 & 2985.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008847349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008847349-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008847759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008848104-01 & 7100.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
008848104-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
008848115-01 & 7101.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_008454553-04\\
008848271-01 & 1256.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008848271-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008848288-01 & 3886.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008848916-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008848942-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008849165-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008849165-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008866102-01 & 0042.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
008866137-01 & 2074.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008866467-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
008868364-01 & 3541.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008868649-01 & 3927.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_008868650-pri\\
008868657-01 & 7102.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_008868650-pri\\
008868686-01 & 7598.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_008868650-pri\\
008868907-01 & 3539.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008868907-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008869680-01 & 0696.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008869855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
008869892-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008869892-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008869892-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008870545-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008871494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008871494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008873090-01 & 2968.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008874090-01 & 1404.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008874090-02 & 1404.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008878187-01 & 0697.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008878681-01 & 7103.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
008878681-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
008878681-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008879427-01 & 7104.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008879427-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008879681-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
008879915-01 & 7105.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008880123-01 & 3493.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008880153-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008880157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008880157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008880162-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008880162-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008880162-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008881169-01 & 7106.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008881697-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008881697-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008881883-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008881883-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008881883-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008882561-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008882561-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008882847-01 & 3490.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008883075-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008883329-01 & 2595.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008883329-02 & 2595.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008883593-01 & 0923.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
008883727-01 & 3822.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
008883727-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
008884274-01 & 2868.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008885638-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008885643-01 & 2789.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008885673-01 & 2611.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008885841-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
008888719-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008890150-01 & 2650.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008890150-02 & 2650.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008890783-01 & 0464.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008890783-02 & 0464.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008890924-01 & 4269.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008890924-02 & 4269.02 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008890996-01 & 7107.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_008823397-pri\\
008891278-01 & 0698.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008891278-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---KIC\_OFFSET\\
008891395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008891684-01 & 5581.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
008892157-01 & 2224.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008892303-01 & 2688.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008892720-01 & 3336.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
008892720-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
008892721-01 & 1844.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3336.01\\
008892910-01 & 0132.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008892910-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008893443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008893443-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008894646-01 & 2641.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008894646-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_008894630-pri\\
008895336-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008895758-01 & 3106.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008896357-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008896357-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008903643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008903643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008903917-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
008904714-01 & 5582.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008905010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008905010-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008905010-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008905010-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008905246-01 & 3473.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008905246-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008906045-01 & 3789.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_008906039-pri\\
008906045-02 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_008906039-pri\\
008906045-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008906089-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008906294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008906294-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008906676-01 & 7108.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008906676-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008907191-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008907597-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008907597-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008907618-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008907618-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008907769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008908102-01 & 0699.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008908102-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008908544-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008908767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008908767-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008908977-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008908977-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008912730-01 & 3850.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008912730-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008912730-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008912730-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008912730-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008913111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
008913894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008913894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008914322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008914322-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008914779-01 & 2230.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008914866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008914866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008914866-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008915238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008915335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008915335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008915335-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008916266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008916266-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008916266-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
008916356-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008916492-01 & 1414.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
008934103-01 & 4009.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008934103-02 & 4009.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008934495-01 & 0524.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008935140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008935352-01 & 5584.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
008935810-01 & 1395.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008937019-01 & 3754.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008937019-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
008937021-01 & 1394.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_008937019-01\\
008937021-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_008937019-02\\
008937762-01 & 4668.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008938257-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008938257-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008938628-01 & 7109.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008938801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008938937-01 & 4758.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008939211-01 & 5586.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008939650-01 & 5587.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008940640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008940640-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008940640-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008940642-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
008940918-01 & 4784.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008940961-01 & 7110.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
008947520-01 & 2517.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008948424-01 & 0322.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
008948424-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
008949247-01 & 1387.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008949316-01 & 3849.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
008949316-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008949925-01 & 2972.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008949925-02 & 2972.02 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
008950568-01 & 2038.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008950568-02 & 2038.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008950568-03 & 2038.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008950853-01 & 1412.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008951096-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
008951205-01 & 4099.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008951215-01 & 0924.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008951965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008951965-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008953059-01 & 6062.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008953059-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008953257-01 & 1383.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008953257-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008953278-01 & 7111.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008953281-01 & 7112.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_008953296-pri\\
008953296-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008953414-01 & 4332.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_008953426-pri\\
008953426-01 & 7113.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
008953475-01 & 7114.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_008953426-pri\\
008955709-01 & 4471.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
008955709-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
008955867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008955867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008955889-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
008956206-01 & 2048.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008956206-02 & 2048.02 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008956850-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---LARGE\_RM\\
008956850-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008957572-01 & 7115.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008957572-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008957572-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008957954-01 & 6189.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008958035-01 & 1391.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008958811-01 & 7116.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008958939-01 & 7117.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008958939-02 & 7117.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008959062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
008959062-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008959745-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008959769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008959769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008959769-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008959839-01 & 2253.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008960985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008960985-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008961823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008962094-01 & 0700.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008962094-02 & 0700.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008962094-03 & 0700.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
008962094-04 & 0700.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
008963002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008963002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
008963002-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008963721-01 & 2233.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_5614.01\\
008964050-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008964935-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
008964935-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008964935-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008971294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008971294-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008971294-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008971432-01 & 1384.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008971432-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008971879-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008972058-01 & 0159.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008972058-02 & 0159.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008972489-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008972489-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008972908-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
008972966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008972966-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008972966-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
008973000-01 & 7118.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008973000-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
008973067-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008973129-01 & 2286.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
008973285-01 & 4782.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
008973529-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008973529-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008973811-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008973811-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008973811-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008974140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008974140-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008975368-01 & 3227.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
008975485-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008975644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008975644-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008975644-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008975644-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
008976187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008976187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008976195-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008976195-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008976589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008976589-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
008977176-01 & 7119.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008977223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008977223-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008978528-01 & 1874.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008978528-02 & 1874.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
008978630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008978630-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
008978630-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008979190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008979190-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008979238-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
008979238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008979238-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
008979487-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
008979487-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008979487-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008979487-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
008981233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008981446-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
008982583-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
008982583-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008982583-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
008982857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
008984131-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
008984131-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
008984706-01 & 6190.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
008984706-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
008984755-01 & 4664.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
008984831-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
008984831-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008984831-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
008985157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
008985157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
008985157-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009001468-01 & 7120.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009001558-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
009001558-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
009001926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009002237-01 & 1389.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009002237-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009002278-01 & 0701.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009002278-02 & 0701.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009002278-03 & 0701.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009002278-04 & 0701.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009002278-05 & 0701.05 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009002538-01 & 3196.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009002538-02 & 3196.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009003401-01 & 2319.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009005042-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_009005043-pri\\
009005042-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009005047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009005854-01 & 7121.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009006186-01 & 2169.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009006186-02 & 2169.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009006186-03 & 2169.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009006186-04 & 2169.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009006449-01 & 1413.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009006449-02 & 1413.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009006449-03 & 1413.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009006474-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009007332-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009007332-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009007609-01 & 4795.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009007918-01 & 7122.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009007953-01 & 7123.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009007918-pri\\
009008103-01 & 3283.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009008220-01 & 0466.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009008220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009008427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009008427-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009008737-01 & 2768.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009009036-01 & 4585.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009009211-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009009514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009009953-01 & 4014.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009011825-01 & 2530.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009011877-01 & 5597.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009015437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
009015738-01 & 1616.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009016295-01 & 0925.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009016295-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009016344-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009017682-01 & 1630.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009017929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009017929-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009017929-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009018021-01 & 5600.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009018502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009019191-01 & 2604.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009020114-01 & 3088.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009020160-01 & 0582.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009020160-02 & 0582.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009020160-03 & 0582.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009020199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009020199-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009020199-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009020426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
009020774-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009020774-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009020774-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009020774-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009021052-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009021052-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
009021052-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
009021075-01 & 4733.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009021291-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009022166-01 & 2175.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009022166-02 & 2175.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009024857-01 & 7124.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009025029-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009025557-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009025600-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009025600-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009025600-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009025600-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009025662-01 & 7599.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009025739-01 & 7125.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009025914-01 & 3596.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009025914-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009025914-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009025922-01 & 0043.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3596.01\\
009025922-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009025914-02\\
009025971-01 & 3680.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009026611-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009026611-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009026611-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009026749-01 & 2564.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009026749-02 & 2564.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009027841-01 & 4266.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
009027876-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009027876-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009027876-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009027909-01 & 3428.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009028104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009028104-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009028104-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
009028134-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009028134-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009028154-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009028154-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009028474-01 & 3510.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009028474-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009029486-01 & 7126.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009030447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009030447-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009030537-01 & 1892.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009031086-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009031209-01 & 3316.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009031507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009031703-01 & 4520.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009031731-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009032551-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009032551-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009032551-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009032900-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL\\
009032900-02 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
009032900-03 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009033798-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009034103-01 & 1402.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009040422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009040422-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009040849-01 & 1392.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009040983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009040983-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009042357-01 & 1993.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
009042357-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009044063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009044063-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009044228-01 & 1988.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009044831-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009045002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009045002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009045401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009045401-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009045521-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009045521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009045521-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009045611-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009047103-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009047103-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009047103-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009047284-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_008977390-pri\\
009047416-01 & 5605.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009048145-01 & 6063.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009048145-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009048161-01 & 0146.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_6063.01\\
009048161-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009048145-sec\\
009049010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
009049010-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009049010-03 & 7127.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009049010-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009049550-01 & 5606.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009049673-01 & 3799.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
009049697-01 & 5607.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3799.01\\
009050337-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009050337-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009050785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009050785-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009050785-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009051487-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009051487-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009051487-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009051487-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009051650-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
009051650-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009051650-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009051902-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009051902-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009051902-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009051991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009051991-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009051991-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009052363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009052849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009052849-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009052849-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009052883-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009052883-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009052883-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009053086-01 & 3751.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM---PARENT\_IS\_702.01\\
009053086-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009053086-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009053112-01 & 0702.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3751.01\\
009054553-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009054553-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009070666-01 & 3008.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009071343-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_009071373-pri\\
009071343-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_009071373-pri\\
009071386-01 & 0023.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009071386-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009071593-01 & 2257.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009071593-02 & 2257.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009071682-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009072011-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009072011-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009072190-01 & 1933.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009072639-01 & 4198.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009072693-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009072693-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009073007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009073007-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009073007-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009074955-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009076513-01 & 0583.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009076902-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009076971-01 & 2981.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009077124-01 & 0926.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009077483-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009077633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009083470-01 & 4731.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_009083523-pri\\
009083503-01 & 7128.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009083564-01 & 3249.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_009083523-pri\\
009084512-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009084778-01 & 1631.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009084778-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009084820-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009084820-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009085039-01 & 7129.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009085563-01 & 3393.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009086154-01 & 4060.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009086251-01 & 2367.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009087580-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
009091730-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009091755-01 & 4052.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009092496-01 & 4193.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009092496-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009092496-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009092504-01 & 2716.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009092504-02 & 2716.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009092529-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009092529-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009092897-01 & 7600.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009092897-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009092897-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
009092940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009092940-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009092940-03 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009092940-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009093033-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009093086-01 & 6191.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009093266-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009093266-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009093349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009093566-01 & 7130.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009093566-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009094600-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009094694-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009094694-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009094763-01 & 4779.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009095152-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009095152-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009095245-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009095292-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009095849-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009097120-01 & 0927.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009097419-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009097423-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009097423-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009097423-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009097892-01 & 3809.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
009098590-01 & 7131.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009098810-01 & 7132.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009099427-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
009099773-01 & 7133.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009099927-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009099927-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009099927-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009099927-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009099927-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009099950-01 & 4125.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_009164694-pri\\
009100325-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009100484-01 & 1399.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009100869-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
009100953-01 & 4500.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009100953-02 & 4500.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009100953-03 & 4500.03 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009101208-01 & 7134.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_5614.01\\
009101279-01 & 5614.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
009101400-01 & 6192.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009101496-01 & 1915.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009101496-02 & 1915.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009108058-01 & 5615.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009108058-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009108085-01 & 2470.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_5615.01\\
009108615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009108615-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009108715-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009108715-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009109743-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009109743-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009109857-01 & 2833.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009110346-01 & 3607.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
009110357-01 & 0016.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3607.01\\
009111056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009111056-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009111056-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009111056-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009111056-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009111056-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009111849-01 & 2042.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009111849-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009111849-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009111849-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009112301-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009112931-01 & 2256.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009113058-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009113058-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009114182-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009114182-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009115029-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
009115039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009115039-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
009115681-01 & 1865.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009115800-01 & 0421.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009116075-01 & 5617.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
009116568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009117123-01 & 5619.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF\\
009117390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009117390-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009117390-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009117390-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009117416-01 & 3425.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009117416-02 & 3425.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009117416-03 & 3425.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009117875-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009117875-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009118695-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009118716-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009119402-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009119402-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009119405-01 & 7135.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009119405-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009119458-01 & 0525.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009119536-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009119536-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009119536-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
009119568-01 & 3087.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009119652-01 & 6193.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
009119893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009120066-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009137447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009137447-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009137728-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009138411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009138872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009138872-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009138872-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009139084-01 & 0323.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009139163-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009140402-01 & 0928.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009141355-01 & 5622.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009141746-01 & 0929.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009142773-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009142974-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009143254-01 & 1386.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009143785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009143785-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009145369-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009145369-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009145369-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009145762-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009145861-01 & 6194.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009146018-01 & 0584.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009146018-02 & 0584.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009146018-03 & 0584.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009147004-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009147012-01 & 5625.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009149789-01 & 2874.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009149789-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009149959-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009149959-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009149986-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009150012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009150012-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009150012-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009150012-04 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009150827-01 & 1408.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009150870-01 & 7136.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009152634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009152999-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009153554-01 & 3044.01 & FP & 0 & 0 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
009153554-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009153570-01 & 2625.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009153823-01 & 6195.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009156461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009156585-01 & 2054.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009156808-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009156808-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009156957-01 & 7137.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009157001-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009157030-01 & 5628.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009157634-01 & 0526.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009157634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
009157908-01 & 1400.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
009157908-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
009158038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009159242-01 & 2566.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_009159301-pri\\
009159265-01 & 3877.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_009159301-pri\\
009159275-01 & 0930.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_009159301-pri\\
009159275-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009159275-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009159301-01 & 7138.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009159301-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009161118-01 & 3898.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
009161894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009161894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009161894-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009161894-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009161945-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009161945-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009162224-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009162503-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009162741-01 & 0703.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009163180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009163180-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009163180-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009163221-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
009163221-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009163221-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009163458-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
009163458-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009163674-01 & 7139.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009163769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009164788-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009164788-02 & 7140.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009164788-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009164836-01 & 0213.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009164836-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009164938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009164938-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009164938-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009164938-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009164952-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009165393-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009165393-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009166386-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009166700-01 & 5632.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009166826-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009166826-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009166826-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009166862-01 & 0931.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009166870-01 & 0932.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_931.01\\
009171801-01 & 0933.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
009171801-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009171954-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009171954-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009171954-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009172506-01 & 7141.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009172506-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009172506-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009172981-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009172981-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009172981-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009173014-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009173055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009174121-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009174121-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009174536-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009174919-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009174919-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009175104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009175346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009177629-01 & 2522.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009178185-01 & 3868.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
009178185-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009178425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009178501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009178502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009178502-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009178502-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009178548-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009178894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009178894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009178929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009178929-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009179044-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009179044-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009179531-01 & 7142.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
009179771-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009179771-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009179771-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009180282-01 & 5636.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
009180282-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009180566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009180566-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009180566-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009180821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009180821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009180906-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009180906-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009180906-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009180906-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009181012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009181012-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009181340-01 & 7143.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009182355-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009182484-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
009182617-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009182617-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009182617-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
009183378-01 & 4222.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009201644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009201644-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009201644-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009202046-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009202151-01 & 1393.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009202434-01 & 4253.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009203154-01 & 7144.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009203405-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009204103-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009204103-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009204718-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009204718-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009205633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009205855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009205907-01 & 2528.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009205938-01 & 2162.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009205938-02 & 2162.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009205993-01 & 7145.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009205993-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
009206046-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009207344-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009207508-01 & 7146.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009207508-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009209247-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009209247-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009209624-01 & 2443.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009209624-02 & 2443.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009210037-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009210037-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009210387-01 & 2416.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009210823-01 & 0090.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---CLEAR\_APO---PARENT\_IS\_009210828-pri\\
009210828-01 & 7147.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009210943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009210943-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009210943-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009210943-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009214712-01 & 6064.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009214712-02 & 6064.02 & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_6065.01\\
009214715-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
009214715-02 & 6065.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_6064.01\\
009214715-03 & 6065.02 & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_6064.01\\
009214942-01 & 1403.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009215655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009215655-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009215655-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009215655-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009216775-01 & 4513.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009216810-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009220002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009220002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009220612-01 & 4059.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009220600-pri\\
009221398-01 & 6066.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009221398-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009221517-01 & 2281.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009221528-01 & 3355.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009221627-01 & 7148.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009222516-01 & 4492.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
009222516-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
009222942-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009222942-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009224836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009224836-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009225395-01 & 2107.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009226081-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009226081-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009226081-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009226339-01 & 3477.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009226439-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
009226540-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009228115-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009228115-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009229318-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009229318-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009229342-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009229342-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009229342-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009229571-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009229571-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009229657-01 & 2491.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009230007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009230007-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009230007-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009230021-01 & 3429.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009230021-02 & 3429.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
009230478-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009236858-01 & 7149.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009236858-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009237149-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009239124-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009239124-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009239124-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009239211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009239211-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009239211-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009239681-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009239681-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009239681-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009240664-01 & 4338.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009240664-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009241509-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009241509-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009241509-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009242059-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009242059-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009242127-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009242127-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009242383-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009242383-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009242383-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009243421-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009243421-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009243464-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009243464-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009243562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009243562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009243562-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009243671-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009243795-01 & 7150.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009243826-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009244508-01 & 2830.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009244508-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009244756-01 & 1969.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009245848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009245855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009246481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009246481-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009246481-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009246481-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009246715-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009246715-02 & 7601.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_7:1---EYEBALL---SATURATED\\
009246715-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009264949-01 & 1405.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009265050-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009265050-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009265306-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009266285-01 & 7151.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009266285-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009266431-01 & 0704.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009267042-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009267042-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009267042-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009267305-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009267996-01 & 3431.01 & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009268205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009268205-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009268481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009269042-01 & 2397.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009269063-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009269281-01 & 1398.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009269884-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009271752-01 & 1406.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009272070-01 & 4126.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009272938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009273647-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009273730-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
009273824-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
009277896-01 & 1632.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009278021-01 & 7152.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009278021-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009278216-01 & 4710.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009278553-01 & 1385.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009278696-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009278696-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009278696-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009278696-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009278725-01 & 2223.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009279354-01 & 2060.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009279669-01 & 0585.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009279763-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009279865-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009279865-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009280239-01 & 3975.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009282687-01 & 6196.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
009282687-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009282762-01 & 4113.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_BR-Cyg-pri\\
009282769-01 & 3959.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_BR-Cyg-pri\\
009282853-01 & 5651.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009283002-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009283002-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009283002-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009283128-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009283128-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009283128-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009283156-01 & 2657.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009284487-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009284487-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009284560-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009284741-01 & 7153.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009284741-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009284741-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009284741-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009285265-01 & 3410.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009285265-02 & 3410.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009285568-01 & 4241.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009285587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009285587-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009285587-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009286728-01 & 7154.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_009159301-pri\\
009287502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009287646-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009288237-01 & 3114.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009288444-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---LARGE\_RM\\
009288444-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009288444-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
009288786-01 & 1390.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009288786-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009289704-01 & 2222.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009289704-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009289704-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009289960-01 & 6197.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009289960-02 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009289960-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009291039-01 & 3230.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009291039-02 & 3230.02 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_009291368-pri\\
009291275-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009291275-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009291368-01 & 7155.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
009291368-02 & 7155.02 & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---TOO\_FEW\_QUARTERS\\
009291378-01 & 3776.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_009291368-pri\\
009291618-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009291618-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009291629-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009291629-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009291748-01 & 7156.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009291748-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009292130-01 & 7602.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---EYEBALL---SATURATED\\
009299986-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009300285-01 & 0705.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
009300295-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009300295-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009300295-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009300946-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009300946-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009300946-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009301183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009301183-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009301183-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009301183-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009301183-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009301183-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009301506-01 & 3047.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009301506-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009301564-01 & 7157.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009302543-01 & 4272.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009302543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009302543-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009303041-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009303041-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009303041-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009304101-01 & 2067.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009304367-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009304367-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009304367-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009304409-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009304409-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009304561-01 & 7158.01 & FP & 0 & 0 & 0 & 1 & CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_3597.01\\
009304698-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009304821-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009304842-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009304842-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009304857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009304907-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_009304976-03\\
009304913-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009304913-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009304923-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009304923-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009304923-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009304955-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_009305157-01\\
009304976-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009304976-02 & 5654.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009304976-03 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF---PARENT\_IS\_009304907-01\\
009304997-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009305012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009305012-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009305012-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009305012-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009305136-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009305136-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET---PARENT\_IS\_009304976-01\\
009305157-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_009304907-01\\
009305540-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009305574-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009305574-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009305831-01 & 0204.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009305952-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009305952-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009306095-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009306095-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009306893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009306893-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009306900-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009306900-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009306998-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009306998-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009306998-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009306998-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
009307105-01 & 3304.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM\\
009307105-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
009307509-01 & 2096.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009307966-01 & 4910.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009308289-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009308289-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009324334-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009324334-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009328641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009328641-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009328852-01 & 7159.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009328864-01 & 7160.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009328852-pri\\
009331207-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009333652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009333652-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009334289-01 & 0934.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009334289-02 & 0934.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009334289-03 & 0934.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009334490-01 & 7161.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009334490-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009334893-01 & 2298.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009334893-02 & 2298.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009335664-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009336200-01 & 2242.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009340411-01 & 7162.01 & PC & 0 & 0 & 0 & 0 & CENTROID\_SIGNIF\_UNCERTAIN\\
009340980-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2281-Cyg-pri\\
009341241-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009341241-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009341241-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
009341241-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009341243-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009343862-01 & 6201.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009343862-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
009343888-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009343888-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009344493-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009344493-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009344493-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
009344572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009344572-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009344623-01 & 7163.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009344623-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009345771-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_009345819-01\\
009345819-01 & 4615.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_009345771-01\\
009345933-01 & 3264.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009346253-01 & 1388.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009346253-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009346655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009347009-01 & 1971.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009347095-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009347095-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009347095-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009347339-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009347494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009347494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009347494-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009347494-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009347899-01 & 0935.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009347899-02 & 0935.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009347899-03 & 0935.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009347899-04 & 0935.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009349226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009349226-02 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009349226-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
009349482-01 & 2020.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009349690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009349757-01 & 3348.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009349757-02 & 3348.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009350552-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009350686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
009350686-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009350690-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009351205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009351205-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009351205-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009351316-01 & 2078.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009351316-02 & 2078.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009351622-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009351622-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009351622-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009351622-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009351622-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009351920-01 & 2129.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009353182-01 & 7164.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009353182-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009353314-01 & 1900.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009353742-01 & 3867.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009353949-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009357275-01 & 7165.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009357375-01 & 7166.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_009357275-pri\\
009362445-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009362445-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009364192-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009364192-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009364290-01 & 2374.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009364290-02 & 2374.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009364543-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009364543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009364609-01 & 2137.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009366617-01 & 4215.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009366886-01 & 2901.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009366988-01 & 3597.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009366988-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009366988-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009366989-01 & 1785.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3597.01\\
009366989-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED---PARENT\_IS\_3597.01\\
009366994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009366994-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009366994-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009367382-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009367382-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009367382-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009367382-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009367382-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009367926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009368220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009368220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009368220-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009368360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
009368360-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009368360-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009368424-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009368524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009368524-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009369047-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009369047-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009369366-01 & 2905.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009369547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009369547-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009369547-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009369756-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009388435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009388435-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009388479-01 & 0936.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009388479-02 & 0936.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009389206-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009389245-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
009390653-01 & 0249.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009390655-01 & 5662.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_249.01\\
009391208-01 & 1409.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009391395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009391395-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009391506-01 & 1410.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009391817-01 & 5663.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009392668-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009392668-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_009392682-sec\\
009392702-01 & 7167.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
009393006-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009394601-01 & 3684.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009394605-01 & 6203.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_009394601-pri\\
009394920-01 & 7168.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
009394920-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
009394920-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009395024-01 & 2383.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009395222-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009395222-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009395222-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009395246-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009395246-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009395246-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009395719-01 & 2472.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009396760-01 & 4788.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_FL-Lyr-pri\\
009397064-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009397900-01 & 7169.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009398382-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009398382-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009401997-01 & 1633.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009402195-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009402479-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009402583-01 & 4168.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V2281-Cyg-pri\\
009402649-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_V2281-Cyg-pri\\
009402670-01 & 5667.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2281-Cyg-pri\\
009402693-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009402709-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V2281-Cyg-pri\\
009405541-01 & 3788.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---SATURATED\\
009405541-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009405595-01 & 2125.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009405865-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009405865-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009406892-01 & 4186.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009406990-01 & 0937.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009407225-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009407225-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009407225-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009407261-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009408373-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009408694-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009408694-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009408917-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009409216-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009409238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009409239-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009409239-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009410527-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009410527-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009410930-01 & 0196.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009410930-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009411166-01 & 1922.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009411166-02 & 1922.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009411317-01 & 6067.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
009411317-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
009411412-01 & 2101.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009411943-01 & 7170.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
009412445-01 & 3970.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009412462-01\\
009412462-01 & 7171.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009412462-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009412623-01 & 4640.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009412760-01 & 1977.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009412760-02 & 1977.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009413057-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009413057-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009413057-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009413156-01 & 4700.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009413335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009413335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009413816-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009414417-01 & 0974.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009414857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009415108-01 & 2121.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009415172-01 & 0938.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009415172-02 & 0938.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009415172-03 & 0938.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009415300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009418205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009418205-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009418508-01 & 5672.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009418619-01 & 6068.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
009418619-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009418619-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009418619-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009418994-01 & 7172.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009418994-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009419020-01 & 4808.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009425139-01 & 1411.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009426071-01 & 0706.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009426473-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009426473-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009426817-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009426817-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009426817-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009427067-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
009427220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009427220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009427402-01 & 1397.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009428078-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009428078-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009428817-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009429060-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009429060-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009429060-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009429998-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009430371-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009430843-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009446824-01 & 1382.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009446824-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009447166-01 & 3296.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009449455-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009449455-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009450392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009450392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009450647-01 & 0110.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009450940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009451096-01 & 7173.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009451096-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009451127-01 & 1381.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009451127-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009451299-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009451706-01 & 0271.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009451706-02 & 0271.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009451706-03 & 0271.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009452897-01 & 3391.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009453075-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009453075-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009453075-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009453452-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009453452-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009455325-01 & 1813.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009455556-01 & 1396.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009455556-02 & 1396.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009455677-01 & 4076.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009456165-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009456281-01 & 4207.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009456389-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009456389-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009456595-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009456595-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009456651-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009456651-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009456932-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009456985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009456996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009456996-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009457145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009457541-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009457728-01 & 4637.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009457948-01 & 4694.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458266-01 & 7174.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009458343-01 & 2246.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458613-01 & 0707.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458613-02 & 0707.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458613-03 & 0707.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458613-04 & 0707.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458613-05 & 0707.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
009458754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009459087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009462914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009463288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009466030-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009466030-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009466030-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009466042-01 & 7175.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009466058-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009466429-01 & 2786.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009466668-01 & 0939.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009466668-02 & 0939.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009466668-03 & 0939.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009466668-04 & 0939.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009467345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009467345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009467345-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009467404-01 & 2717.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009468126-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009468126-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009468126-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009468296-01 & 7176.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009468296-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009468382-01 & 3409.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3466.01\\
009468382-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009468384-02\\
009468384-01 & 3466.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009468384-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009468551-01 & 2980.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009468717-01 & 1954.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009468717-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009469010-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009469775-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009469775-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009469775-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009469775-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009471268-01 & 1835.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009471268-02 & 1835.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009471268-03 & 1835.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009471284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009471360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009471360-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009471360-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009471419-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009471419-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009471539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
009471539-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009471539-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
009471539-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009471755-01 & 6204.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
009471755-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
009471755-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
009471846-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009471846-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009471974-01 & 0119.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009471974-02 & 0119.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009472000-01 & 2082.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009472074-01 & 2735.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009472363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009473078-01 & 2079.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
009473570-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
009474222-01 & 7177.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009474222-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009474225-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
009474225-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009474232-01 & 4760.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009474232-pri\\
009474239-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009474483-01 & 4697.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED---PARENT\_IS\_5683.01\\
009474485-01 & 5683.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
009474493-01 & 2574.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009474493-02 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_5683.01\\
009474717-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009474717-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009474756-01 & 3495.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
009474756-02 & 3495.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009474969-01 & 7178.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009474995-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009475552-01 & 2694.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009475552-02 & 2694.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009478990-01 & 0423.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009479273-01 & 0940.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009479306-01 & 4906.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009479460-01 & 6205.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009479460-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009479537-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009479539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009479661-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009479661-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009480189-01 & 0941.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009480189-02 & 0941.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009480189-03 & 0941.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009480237-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009480310-01 & 1470.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009480398-01 & 7179.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009480535-01 & 3901.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009481724-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009486646-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009487546-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009487871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
009488426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009488426-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009488426-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009488445-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009488445-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009488445-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009488454-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009489348-01 & 5686.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_009489411-pri\\
009489348-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
009489524-01 & 2029.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009489524-02 & 2029.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009489524-03 & 2029.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009489524-04 & 2029.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009489590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009489590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009489590-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009489626-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009489626-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009489626-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009489947-01 & 3385.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009489953-01 & 3238.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009490067-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009490067-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009490067-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009490067-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009490342-01 & 7180.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009490506-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009490506-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009490653-01 & 4173.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009491205-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009491205-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009491205-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009491303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009491303-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009491303-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009491339-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009491339-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009491339-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009491800-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009491832-01 & 4226.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009491961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009508655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009509207-01 & 7181.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
009509223-01 & 4867.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_009509207-sec\\
009509223-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_009509207-pri\\
009509296-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009509296-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009509296-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009509343-01 & 4346.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009512687-01 & 0942.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009512981-01 & 1466.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009513168-01 & 7182.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
009513865-01 & 0943.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009513921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009513921-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009514372-01 & 4242.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009517393-01 & 2076.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009517393-02 & 2076.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009517991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
009518318-01 & 1978.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009518318-02 & 1978.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009518651-01 & 4433.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_FL-Lyr-pri\\
009518710-01 & 3207.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009518710-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009518710-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009519210-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009520019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009520019-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009520226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009520226-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009520443-01 & 2893.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
009520443-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009520668-01 & 1514.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009520700-01 & 7183.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009520700-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009520838-01 & 1866.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009526946-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009526946-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009526946-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009527052-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009527334-01 & 0049.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009527915-01 & 0165.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009528212-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009528212-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009528420-01 & 1742.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009528420-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009528430-01 & 3489.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009528430-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009529073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009529073-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009529073-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009529294-01 & 7184.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009529652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009529733-01 & 3600.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009529744-01 & 1806.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3600.01\\
009529744-02 & 1806.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009529744-03 & 1806.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009529856-01 & 7185.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009529856-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009530945-01 & 0708.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009530945-02 & 0708.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009531823-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009531823-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009531850-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009531971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009531971-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
009531971-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009531991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009532052-01 & 2115.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009532117-01 & 3241.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_6069.01\\
009532117-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009532123-02\\
009532123-01 & 6069.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_CENTROIDS\\
009532123-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_CENTROIDS\\
009532321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009532421-01 & 3710.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009532421-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009532424-01 & 2941.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3710.01\\
009532445-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009532594-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009532594-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009532603-01 & 5688.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009532637-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009532637-02 & 3842.01 & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009532644-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009532644-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009532710-01 & 2364.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009533354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009533354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009533354-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009533449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009533449-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009533449-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009533489-01 & 3783.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009533489-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009533489-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
009533751-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009533751-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009533751-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009535080-01 & 1509.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009535876-01 & 4225.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_4228.01\\
009535876-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009536048-01 & 7186.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009536108-01 & 3472.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009536515-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009536515-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009536692-01 & 1948.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009536870-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009537008-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009537008-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009540226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
009540295-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009540295-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009540450-01 & 7187.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
009540675-01 & 7188.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V995-Cyg-pri\\
009541089-01 & 4182.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009541127-pri\\
009541094-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_009541127-pri\\
009541144-01 & 7603.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_009541127-pri\\
009541163-01 & 7189.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009541127-pri\\
009541223-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_009541127-pri\\
009541295-01 & 3132.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_009541127-pri\\
009541322-01 & 2089.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009541567-01 & 7190.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
009541567-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009541567-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
009542697-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009543302-01 & 5691.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009548991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009549471-01 & 6070.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_6206.01\\
009549471-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009549472-02\\
009549472-01 & 6206.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009549472-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009549472-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009549513-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009549648-01 & 1886.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009550035-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009550886-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009550886-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009550886-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009551200-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009551281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009551281-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009551430-01 & 4030.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009552411-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009552411-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009552574-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009552574-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009552608-01 & 0080.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
009552608-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009552758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009552758-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009569479-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009569479-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009569711-01 & 3232.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009569838-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009569838-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
009569866-01 & 7191.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009569866-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009570073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009570741-01 & 0586.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009571186-01 & 3313.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009573539-01 & 0180.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009573685-01 & 2057.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009574158-01 & 2512.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009574179-01 & 2637.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009574614-01 & 1745.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009575728-01 & 5692.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009576197-01 & 6207.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009576197-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009577855-01 & 4522.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009578461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009578461-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009578461-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009578461-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009578686-01 & 0709.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009578833-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009578833-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009579192-01 & 7192.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009579208-01 & 3165.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009579266-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009579266-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009579499-01 & 1461.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009579499-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009579584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009579584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009579641-01 & 0115.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009579641-02 & 0115.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009579789-01 & 7193.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_FL-Lyr-pri\\
009579818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009579818-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009579818-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009579860-01 & 6208.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009580167-01 & 2548.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009580794-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009580794-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009580794-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009580992-01 & 2217.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009581498-01 & 7194.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009581589-01 & 4877.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009582692-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009583881-01 & 0467.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009588514-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009588822-01 & 4388.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009588822-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009588822-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009588862-01 & 7195.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009588946-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009588953-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009588953-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009588953-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009589323-01 & 1488.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009589524-01 & 0468.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009590976-01 & 0710.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009590976-02 & 0710.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009590976-03 & 0710.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009591070-01 & 2825.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009591480-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
009591503-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009591503-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009591519-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009591519-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009591519-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009591728-01 & 5695.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009592575-01 & 3565.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009592579-01 & 0243.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3565.01\\
009592705-01 & 0288.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---SATURATED\\
009592818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009592831-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_009592855-01\\
009592850-01 & 3883.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_009592855-pri\\
009592855-01 & 7196.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009592855-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009592859-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009592918-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_009592855-pri\\
009593528-01 & 3939.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
009593757-01 & 2774.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_009593759-01\\
009593757-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3800.01\\
009593759-01 & 3800.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009593759-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009593773-01 & 4240.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
009594007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009594022-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009594022-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009594022-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009594022-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009594184-01 & 5696.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009594437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009594857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009594857-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009595686-01 & 0944.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009595827-01 & 0217.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009595956-01 & 7604.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
009596064-01 & 7197.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009596089-01 & 3675.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009596093-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009596093-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009596187-01 & 7198.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009596187-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009596300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009596355-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009596355-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009596469-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009596469-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009596469-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009596892-01 & 7199.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009597042-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009597058-01 & 1819.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009597095-01 & 7200.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009597095-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009597214-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009597218-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009597218-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
009597345-01 & 0711.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009597345-02 & 0711.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009597345-03 & 0711.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009597411-01 & 0424.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009597729-01 & 4417.02 & FP & 0 & 0 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
009597729-02 & 4417.01 & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009597806-01 & 1481.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009597854-01 & 7201.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009597882-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
009598448-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009598448-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009601232-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
009602421-01 & 4631.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V995-Cyg-pri\\
009602431-01 & 7202.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V995-Cyg-pri\\
009602514-01 & 1490.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V995-Cyg-pri\\
009602514-02 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
009602538-01 & 7203.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V995-Cyg-pri\\
009602562-01 & 3985.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_V995-Cyg-pri\\
009602595-01 & 5700.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
009602613-01 & 2612.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009602613-02 & 2612.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009602775-01 & 4684.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_V995-Cyg-pri\\
009605514-01 & 0945.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009605514-02 & 0945.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009605514-03 & 0945.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009606739-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009606739-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009606739-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009606739-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009607164-01 & 0587.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009612084-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009612084-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009612084-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009612178-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009612225-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009612225-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009612825-01 & 2685.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
009612825-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009613070-01 & 3601.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
009613302-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
009614124-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009614124-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009614124-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009630640-01 & 7204.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009630640-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009630640-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009631498-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009631498-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009631762-01 & 0588.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009631995-01 & 0022.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009632007-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009632895-01 & 1451.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009632895-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009634821-01 & 2037.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009634821-02 & 2037.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009634821-03 & 2037.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009635510-01 & 2234.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_009635529-pri\\
009635520-01 & 7205.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009635529-01 & 7206.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009635606-01 & 2535.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009636135-01 & 1498.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009636135-02 & 1498.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009636283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009636283-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009636283-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---FIT\_FAILED\\
009636283-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009636559-01 & 3618.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
009636563-01 & 2892.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3618.01\\
009636569-01 & 0527.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3618.01\\
009636569-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009637299-01 & 7207.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009637299-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009639106-01 & 7208.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009640123-01 & 7209.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009640285-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009640439-01 & 2912.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009640891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009640891-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009640907-01 & 4172.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_FL-Lyr-pri\\
009640921-01 & 7210.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009640921-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009640921-03 & 7210.02 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_FL-Lyr-pri\\
009640924-01 & 4239.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_FL-Lyr-pri\\
009640931-01 & 4175.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_FL-Lyr-pri\\
009640946-01 & 4542.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_FL-Lyr-pri\\
009640962-01 & 4177.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_FL-Lyr-pri\\
009640976-01 & 0712.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_FL-Lyr-pri\\
009640976-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_009641031-01\\
009640985-01 & 0713.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_FL-Lyr-pri\\
009641008-01 & 3860.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_FL-Lyr-pri\\
009641018-01 & 1504.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_FL-Lyr-pri\\
009641031-01 & 7211.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
009641041-01 & 0324.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_FL-Lyr-pri\\
009641076-01 & 4250.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_FL-Lyr-pri\\
009641103-01 & 7212.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_FL-Lyr-pri\\
009641144-01 & 4262.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_FL-Lyr-pri\\
009641481-01 & 2152.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009641484-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009642018-01 & 4430.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009642018-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009642292-01 & 2946.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009642894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009642894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009643043-01 & 3297.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
009643043-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009643705-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009643813-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009643874-01 & 1457.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009644411-01 & 7213.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009644411-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009644683-01 & 7214.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009644680-pri\\
009645188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009645298-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_CENTROIDS\\
009649222-01 & 6071.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009649222-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009649300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009649324-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
009649706-01 & 2049.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009649801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009650390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009650390-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009650501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009650501-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009650501-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009650808-01 & 1970.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009650808-02 & 1970.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009650957-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009650957-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009650957-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009650989-01 & 3095.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
009651065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009651065-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009651065-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009651169-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009651234-01 & 1938.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009651374-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009651374-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009651374-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009651602-01 & 7215.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009651668-01 & 0183.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009652166-01 & 7216.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009652632-01 & 7217.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009652649-01 & 2884.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009652632-01\\
009652655-01 & 4578.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009652632-01\\
009653622-01 & 2513.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009654468-01 & 2417.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009654875-01 & 2272.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009655005-01 & 4047.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009655055-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009655055-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009655114-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655114-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655114-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655129-01 & 1714.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
009655151-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655151-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009655155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009655169-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
009655169-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
009655177-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009655177-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009655177-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009655288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655288-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009655312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009655312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009655393-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655393-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009655402-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---LARGE\_RM\\
009655402-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009655402-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
009655404-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009655407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655419-01 & 3934.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
009655419-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009655419-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009655422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009655422-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009655422-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009655424-01 & 7218.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
009655433-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CROWDED\_DIFF\\
009655433-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF\\
009655437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655444-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009655444-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009655444-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009655461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009655470-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655470-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655471-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009655471-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009655501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009655501-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009655514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009655514-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009655711-01 & 6209.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009655711-02 & 6209.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009655718-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
009655769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009655792-01 & 7605.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
009655858-01 & 3733.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009655858-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009655909-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655909-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009655978-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009656252-01 & 2044.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009656397-01 & 3543.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009656397-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009656543-01 & 3588.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009656543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009656741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009656741-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009656994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009657636-01 & 7219.01 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009658012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009658012-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009658089-01 & 7220.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009658118-01 & 3516.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009658118-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009659036-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009661869-01 & 3647.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
009661869-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
009661877-01 & 0946.01 & FP & 0 & 0 & 1 & 1 & SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3647.01\\
009661979-01 & 2132.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009662811-01 & 1854.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009663113-01 & 0179.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009663224-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009663677-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009664142-01 & 2654.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009664215-01 & 6072.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009664215-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009664276-01 & 3460.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009665170-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009665503-01 & 7221.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009665503-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009665503-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009665503-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009665503-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009665503-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009665922-01 & 2815.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009666465-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009666465-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009666465-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009667584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009667584-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009673009-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
009673173-01 & 7222.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009673173-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009673173-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009673173-04 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009673338-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009673338-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009673483-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009673483-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009673785-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009674320-01 & 7223.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009674346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009674346-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009674346-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009674564-01 & 4096.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_009674592-01\\
009674564-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3729.01\\
009674568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009674568-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009674592-01 & 3729.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
009674592-02 & 3729.01 & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
009674608-01 & 1795.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009674608-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009691284-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_009691311-01\\
009691311-01 & \nodata & FP & 1 & 0 & 1 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_009691284-01\\
009692128-01 & 2769.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_009569866-pri\\
009692345-01 & 1485.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3859.01\\
009692557-01 & 2831.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009693006-01 & 2913.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009693116-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009693282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009693282-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009693282-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009693803-01 & 7224.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009696358-01 & 2545.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009696853-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009696853-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009696853-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009697131-01 & 2706.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009697825-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009699950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009699950-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009700145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009700145-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009700145-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009700322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009700322-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009700322-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009700449-01 & 4120.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009701962-01 & 4617.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009702006-01 & 4372.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009702072-01 & 0714.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009702945-01 & 4822.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009703198-01 & 0469.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009704050-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009704050-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009704377-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009704384-01 & 1913.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009705459-01 & 1448.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009705459-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009710326-01 & 0947.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009710475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009710475-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009710475-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009710475-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009711751-01 & 7225.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009711941-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009711941-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009712350-01 & 2613.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009712799-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009712799-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009712799-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009713213-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
009713213-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
009713244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009713244-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009713632-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009713632-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009714123-01 & 3392.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009714123-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009714209-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009714209-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009714358-01 & 6073.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009714550-01 & 3048.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009714572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009714633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009714633-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009714696-01 & 0616.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009715359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009715359-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009715488-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009715631-01 & 5706.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009715923-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009715923-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009715925-01 & 3599.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009715939-01 & 3690.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009716028-01 & 4273.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009716107-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009716107-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009716107-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009716220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009716220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009716256-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009716256-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009716262-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009716262-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009716301-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009716302-01 & 4142.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF---PARENT\_IS\_BR-Cyg-pri\\
009716358-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009716358-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009716385-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009716385-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009716385-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009716391-01 & 3025.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009716431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009716523-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009716523-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009716563-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009716563-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009716628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009716667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
009716667-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009716667-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009716947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009716947-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009716955-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009717032-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009717032-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009717861-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009717861-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009717861-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009717943-01 & 2273.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009717958-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009717958-02 & 4313.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
009718066-01 & 2287.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009718066-02 & 2287.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009718378-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009718378-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009718379-01 & 2379.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
009718379-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009719634-01 & 1500.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3686.01\\
009719636-01 & 3686.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009719636-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009723838-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009724220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009724220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009724984-01 & 0325.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009724993-01\\
009724993-01 & 5708.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009725543-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009725543-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009725543-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009726020-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009726045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009726045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009726452-01 & 7226.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009726659-01 & 1491.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009726982-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009726982-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009726982-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009727765-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009728465-01 & 2270.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009729691-01 & 1751.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009729691-02 & 1751.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009730163-01 & 2704.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009730163-02 & 2704.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009730163-03 & 2704.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009735426-01 & 1849.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009752973-01 & 3162.01 & FP & 0 & 1 & 0 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED---PARENT\_IS\_3871.01\\
009752973-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009752973-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009752982-01 & 3871.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009752982-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009753154-01 & 2457.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009754625-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009757613-01 & 0250.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009757613-02 & 0250.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009757613-03 & 0250.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009757613-04 & 0250.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009758032-01 & 3137.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009758089-01 & 1871.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009758089-02 & 1871.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009758615-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009758615-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009760994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009760994-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009761199-01 & 1459.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
009761573-01 & 3837.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009761615-01 & 3911.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009761882-01 & 0948.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009762514-01 & 7227.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009762519-01\\
009762519-01 & 7228.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009762519-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009762713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009762713-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009762713-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009762866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009762866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009762866-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
009763348-01 & 1852.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009763612-01 & 3465.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009763640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009764489-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009764506-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009764506-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009764506-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009764506-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
009764544-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
009764544-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009764544-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009764868-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
009764965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009764965-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009764965-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009765489-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009765489-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009765975-01 & 1520.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009766218-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009766437-01 & 0949.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009767322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009767392-01 & 6211.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
009767486-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009767486-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009772075-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009772075-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009772087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009772087-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009772087-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009772531-01 & 0950.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009772586-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009773094-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009773094-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009773099-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---CLEAR\_APO\\
009773099-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
009773270-01 & 4636.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009773512-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009773512-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009773512-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009773869-01 & 3568.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---FIT\_FAILED\\
009773869-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009773869-03 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_3457.01\\
009773869-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009773869-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009773869-06 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009773980-01 & 4691.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009773980-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009774286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009774286-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009774314-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009774314-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009774314-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009774357-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009774357-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009774357-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009774400-01 & 6212.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009774400-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009775253-01 & 3621.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---TOO\_FEW\_QUARTERS\\
009775385-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009775385-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009775385-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009775385-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009775475-01 & 5711.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009775938-01 & 0951.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009775938-02 & 0951.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009776186-01 & 4543.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009776474-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CROWDED\_DIFF\\
009776474-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009776474-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009776692-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED---PARENT\_IS\_009776718-sec\\
009776794-01 & 4363.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
009776816-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009776816-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009776816-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009777062-01 & 7229.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009777062-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009777062-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
009777062-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009777062-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009777087-01 & 3747.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS---PARENT\_IS\_009777090-01\\
009777087-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS---PARENT\_IS\_009777090-02\\
009777087-03 & 3747.02 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_009777062-01\\
009777090-01 & 3672.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009777090-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
009777200-01 & 4455.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_BR-Cyg-pri\\
009777246-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009777246-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009777246-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009777251-01 & 2600.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009777256-01 & 2997.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009777290-01 & 4316.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009777453-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009777556-01 & 4814.01 & FP & 0 & 0 & 0 & 1 & TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009777724-01 & 4197.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_BR-Cyg-pri\\
009777757-01 & 4243.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009777864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009777864-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009777864-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
009777988-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
009778156-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009778156-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009778742-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009780149-01 & 5713.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009782691-01 & 0590.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009782691-02 & 0590.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009782748-01 & 4856.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
009783760-01 & 3487.01 & PC & 0 & 0 & 0 & 0 & SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
009784230-01 & 3851.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
009784590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009784590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009785454-01 & 3577.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV\\
009785454-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009785921-01 & 3372.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009786017-01 & 5714.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009786062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009786335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009786821-01 & 7230.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009786821-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009786859-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009786859-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009787065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009787239-01 & 0952.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009787239-02 & 0952.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009787239-03 & 0952.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009787239-04 & 0952.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009787239-05 & 0952.05 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009788457-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009788457-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009788457-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009788612-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009788612-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009790034-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009790034-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009790144-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009790144-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009790144-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009790785-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
009790785-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009790806-01 & 2035.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009790965-01 & 7231.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009790965-02 & 7231.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009791112-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009791112-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009791381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009791381-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009791381-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009791509-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009791509-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
009791509-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009811915-01 & 7232.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
009812351-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009812351-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009812716-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009813078-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009813078-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009813078-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009813078-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
009813092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009813499-01 & 1505.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009813603-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009813678-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
009814809-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009815053-01 & 2923.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009818269-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009818269-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009818269-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009818381-01 & 0135.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009818462-01 & 1521.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009818732-01 & 7233.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009818732-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009818983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009820483-01 & 0953.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009821078-01 & 7234.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009821078-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009821078-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009821151-01 & 3243.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_009821078-01\\
009821428-01 & 7235.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009821454-01 & 1529.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009821454-02 & 1529.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009822284-01 & 4807.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
009822284-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009822703-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009822703-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009823457-01 & 0954.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009823457-02 & 0954.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009823487-01 & 1489.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009823519-01 & 2793.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009823519-02 & 2793.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009823602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
009823602-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009823652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009823652-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009824673-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009824711-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009824805-01 & 1526.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009824928-01 & 4650.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009825174-01 & 2880.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
009825625-01 & 0955.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009826171-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009826562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009826562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009826562-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009827149-01 & 2586.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009827596-01 & 4855.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_6211.01\\
009828127-01 & 4192.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009828127-02 & 4192.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009828226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009832208-01 & 2553.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009832655-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009832655-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009832655-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009832655-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009832678-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009832678-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009832727-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009832727-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009832727-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009832727-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009833599-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_009833618-pri\\
009834040-01 & 1998.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009834257-01 & 3457.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_009773869-01\\
009834257-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3568.01\\
009834719-01 & 0715.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009834731-01 & 3043.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009835366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009835505-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009835697-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009835697-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009836020-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009836020-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009836020-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009836073-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009836073-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009836073-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009836073-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009836149-01 & 1958.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009836563-01 & 4421.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009836563-02 & 4421.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009836959-01 & 1715.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009837013-01 & 7236.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009837083-01 & 3719.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009837083-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009837267-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009837267-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009837544-01 & 3529.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009837544-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009837544-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009837544-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
009837544-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009837573-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
009837578-01 & 2937.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009837578-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009837586-01 & 3442.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009837578-01\\
009837659-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009837659-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009837661-01 & 2715.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009837661-02 & 2715.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009837661-03 & 2715.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009837685-01 & 2461.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009837828-01 & 4670.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009838060-01 & 3314.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009838060-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009838168-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
009838168-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
009838311-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009838414-01 & 5717.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009838468-01 & 2943.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009838537-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009838557-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009838608-01 & 4677.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009838804-01 & 3028.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009838949-01 & 1716.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009838975-01 & 0218.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
009838975-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
009839062-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009839081-01 & 6213.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009839081-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009839184-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009839184-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009839547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009839547-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009839701-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009839821-01 & 2012.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009839824-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009842890-01 & 1479.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
009842906-01 & 1493.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_009842890-pri\\
009842937-01 & 2567.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009842890-pri\\
009843435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009843435-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
009843517-01 & 3480.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009844088-01 & 0470.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009844514-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009844791-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009844791-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009845573-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009845573-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009845898-01 & 2423.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009845907-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009845907-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009845907-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009845909-01 & 3354.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009845931-01 & 5721.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009846086-01 & 0617.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009846258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009846348-01 & 0716.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009846419-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009846419-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009847239-01 & 5722.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009848420-01 & 7237.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009848460-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009849107-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009849107-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009849107-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009849884-01 & 4516.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_009971475-01\\
009850387-01 & 7238.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009850393-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009850393-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009850393-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009850409-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009850843-01 & 5724.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_009851142-pri\\
009850893-01 & 1523.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009851142-pri\\
009850912-01 & 7239.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009851142-pri\\
009850957-01 & 2446.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_009851142-pri\\
009850966-01 & 4879.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_009851142-pri\\
009851021-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED---PARENT\_IS\_009851142-pri\\
009851123-01 & 6074.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM---PARENT\_IS\_009851142-pri\\
009851123-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_009851142-02\\
009851126-01 & 3592.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_009851142-pri\\
009851126-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009851142-02\\
009851126-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
009851126-04 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
009851142-01 & 3513.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
009851142-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009851226-01 & 1468.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_009851142-pri\\
009851226-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_009851142-02\\
009851271-01 & 2003.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_009851142-pri\\
009851360-01 & 4381.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009851142-pri\\
009851662-01 & 2483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009851822-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009851845-01 & 4696.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_009851944-pri\\
009851943-01 & 4001.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_009851944-pri\\
009851970-01 & 4122.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_009851944-pri\\
009851983-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009852050-01 & 7240.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
009872283-01 & 1815.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009872292-01 & 1537.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009872831-01 & 4230.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009873254-01 & 0717.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009873254-02 & 0717.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009873759-01 & 4635.01 & FP & 0 & 0 & 0 & 1 & TOO\_FEW\_CENTROIDS---PARENT\_IS\_009873869-01\\
009873847-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009873869-01 & 7241.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
009874181-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009874181-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009874181-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009875566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009875566-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009875711-01 & 0956.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009880190-01 & 2509.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009880467-01 & 0326.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009880467-02 & 0326.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009881077-01 & 2751.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009881258-01 & 7242.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009881660-01 & 5727.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009881662-01 & 0327.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009881662-02 & 0327.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009883311-01 & 1872.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009883606-01 & 4383.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009883606-02 & 4383.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009884104-01 & 0718.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009884104-02 & 0718.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009884104-03 & 0718.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009884818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
009885417-01 & 3246.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009886221-01 & 0591.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3614.01\\
009886224-01 & 3614.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009886224-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009886255-01 & 1846.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009886361-01 & 2732.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009886361-02 & 2732.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009886361-03 & 2732.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009886361-04 & 2732.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009886661-01 & 1606.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009887224-01 & 2464.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009892471-01 & 3584.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009892471-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009892624-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009892624-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009892624-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009892749-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009892749-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009892816-01 & 1955.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009892816-02 & 1955.02 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009892816-03 & 1955.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009892816-04 & 1955.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009892822-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
009892822-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009892856-01 & 3906.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009893318-01 & 2660.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009893365-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_009953894-sec\\
009893463-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_009953894-sec\\
009895004-01 & 0328.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009895006-01 & 1717.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009895269-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009895269-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009895709-01 & 1594.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009895857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009896018-01 & 2579.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009896018-02 & 2579.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009896018-03 & 2579.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009896435-01 & 3755.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009896435-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009896438-01 & 5728.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3755.01\\
009896558-01 & 1718.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009896558-02 & 1718.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009896606-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
009896606-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009897089-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009897089-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009897089-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009897364-01 & 4189.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009898017-01 & 4484.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009898181-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009898364-01 & 1579.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009898447-01 & 2803.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009899065-01 & 4108.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899141-01 & 3254.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_BR-Cyg-pri\\
009899153-01 & 7243.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---KIC\_OFFSET---PARENT\_IS\_BR-Cyg-pri\\
009899181-01 & 2867.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_BR-Cyg-pri\\
009899193-01 & 7244.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_BR-Cyg-pri\\
009899217-01 & 3979.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_BR-Cyg-pri\\
009899233-01 & 4090.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899256-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_BR-Cyg-pri\\
009899280-01 & 1559.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899315-01 & 4181.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_BR-Cyg-pri\\
009899352-01 & 3135.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_BR-Cyg-pri\\
009899355-01 & 1554.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_BR-Cyg-pri\\
009899410-01 & 7245.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_BR-Cyg-pri\\
009899414-01 & 3955.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_BR-Cyg-pri\\
009899416-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009899416-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009899421-01 & 7246.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899449-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899483-01 & 1719.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_BR-Cyg-pri\\
009899505-01 & 3064.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899514-01 & 5729.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_BR-Cyg-pri\\
009899538-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_BR-Cyg-pri\\
009899577-01 & 7247.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_BR-Cyg-pri\\
009899583-01 & 7248.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---INVERT\_DIFF---PARENT\_IS\_BR-Cyg-pri\\
009899607-01 & 5730.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_BR-Cyg-pri\\
009899630-01 & 4439.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_BR-Cyg-pri\\
009902856-01 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_3:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_3:1---TOO\_FEW\_QUARTERS\\
009904006-01 & 2135.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009904006-02 & 2135.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009904006-03 & 2135.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009904059-01 & 0145.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009904420-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009906489-01 & 7249.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009906802-01 & 7250.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
009906841-01 & 7251.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
009907129-01 & 3127.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009907505-01 & 3427.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009907505-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009908486-01 & 5731.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009908496-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009908496-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009908496-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009909735-01 & 1779.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009909735-02 & 1779.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009909965-01 & 7252.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009910043-01 & 5732.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009910533-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009910533-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009910828-01 & 4897.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_009851142-pri\\
009910942-01 & 4324.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_009851142-pri\\
009911112-01 & 5733.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009911882-01 & 2429.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009913481-01 & 7253.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
009913798-01 & 7254.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009913798-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009932197-01 & 7255.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
009932970-01 & 1587.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009933043-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009934208-01 & 7256.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009934208-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009934274-01 & 5735.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_009873869-01\\
009935422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009935642-01 & 4885.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009936080-01 & 4431.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009936518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009936518-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009936518-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
009936698-01 & 7257.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009940565-01 & 1548.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
009941066-01 & 1584.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009941387-01 & 5738.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009941387-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
009941387-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009941662-01 & 0013.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
009941662-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
009941859-01 & 0528.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009941859-02 & 0528.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009941859-03 & 0528.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009942881-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009943009-01 & 7258.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009943435-01 & 2788.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009944201-01 & 7259.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
009944201-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009944356-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
009944421-01 & 7260.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009944421-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009945280-01 & 7261.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
009945370-01 & 2285.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009945390-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009945805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009946525-01 & 0398.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009946525-02 & 0398.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009946525-03 & 0398.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009946569-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
009946597-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009947026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009947389-01 & 4460.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009947653-01 & 4647.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009947653-02 & 4647.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009948002-01 & 3562.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009948002-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009950612-01 & 0719.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009950612-02 & 0719.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009950612-03 & 0719.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009950612-04 & 0719.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009953508-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009953617-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009953617-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
009953617-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009953736-01 & 7262.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
009953851-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_009953894-sec\\
009954225-01 & 5742.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
009954225-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
009955262-01 & 0076.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009955598-01 & 1925.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
009955807-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009955807-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009956082-01 & 4139.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009957627-01 & 0592.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009957659-01 & \nodata & FP & 0 & 0 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_5744.01\\
009957668-01 & 5744.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009958053-01 & 7263.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
009958053-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
009958053-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009958053-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE\\
009958055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009958055-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009958071-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
009958387-01 & 2677.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009958962-01 & 0593.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009958962-02 & 0593.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009958962-03 & 0593.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009958962-04 & 0593.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
009959093-01 & 7264.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009959279-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009959279-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009959492-01 & 3051.02 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_BR-Cyg-pri\\
009959492-02 & 3051.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
009959494-01 & 3205.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET---PARENT\_IS\_BR-Cyg-pri\\
009959545-01 & 4195.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_BR-Cyg-pri\\
009959589-01 & 3098.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_BR-Cyg-pri\\
009959855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
009962455-01 & 2748.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009962455-02 & 2748.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009962595-01 & 5745.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009963009-01 & 7265.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009963009-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009963265-01 & 2299.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009963461-01 & 1538.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009963461-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009963524-01 & 0720.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009963524-02 & 0720.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009963524-03 & 0720.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
009963524-04 & 0720.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
009963609-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009963609-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009963639-01 & 7266.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009963667-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
009963667-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009963667-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009964670-01 & 2192.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009964748-01 & 2496.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
009964801-01 & 0721.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009965121-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009965165-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
009965184-01 & 2428.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_009965206-02\\
009965184-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_3558.01\\
009965206-01 & 3558.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009965206-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009965439-01 & 0722.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009965470-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
009965691-01 & 7267.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009965957-01 & 1911.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009966115-01 & 6075.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009966115-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
009966219-01 & 3401.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009966915-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009967009-01 & 3462.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009967009-02 & 3462.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009967129-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009967771-01 & 1875.02 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
009967771-02 & 1875.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009967884-01 & 0425.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
009969287-01 & 4820.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009970139-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009970396-01 & 7606.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
009970568-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009970568-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009970568-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009971475-01 & 7268.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
009971475-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
009971786-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
009971786-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
009971786-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
009972385-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009972385-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009972385-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009972385-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009972385-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
009973109-01 & 2018.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009973109-02 & 2018.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009973187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
009973633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009973633-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
009973855-01 & 1966.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009974087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009974087-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
009974142-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
009974142-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009974142-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
009991621-01 & 3382.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
009992325-01 & 2205.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009993529-01 & 2644.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
009993683-01 & 5748.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009995402-01 & 2832.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009995753-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009995771-01 & 3470.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
009995771-02 & 3470.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
009995942-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
009996632-01 & 2621.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010000135-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010000490-01 & 7269.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
010000490-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
010000941-01 & 4146.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010001145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010001145-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010001154-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010001368-01 & 2785.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010002049-01 & 7270.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010002261-01 & 0959.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010002266-01 & 5750.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010002261-pri\\
010002866-01 & 0723.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010002866-02 & 0723.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010002866-03 & 0723.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010002897-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
010002897-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010002897-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010003593-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010004519-01 & 1572.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010004660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010004660-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
010004660-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010004738-01 & 1598.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010004738-02 & 1598.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010004738-03 & 1598.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010004772-01 & 5752.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010004975-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010005020-01 & 0724.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010005758-01 & 1783.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010005758-02 & 1783.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010005788-01 & 1940.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010006096-01 & 5753.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
010006096-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
010006581-01 & 1595.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010006641-01 & 4469.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010006641-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010007492-01 & 5754.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
010007492-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
010008394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010010440-01 & 2309.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010010595-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010014548-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010014702-01 & 7271.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---PARENT\_IS\_5742.01\\
010015516-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010015516-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010015937-01 & 1720.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010016317-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010016874-01 & 0426.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010018233-01 & 2655.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010019065-01 & 1721.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010019065-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010019399-01 & 1796.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010019643-01 & 0471.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010019643-02 & 0471.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010019708-01 & 0199.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010019708-02 & 0199.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010019763-01 & 1558.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010019854-01 & 7272.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010019950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010020423-01 & 7273.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010020423-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010022908-01 & 1586.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010023469-01 & 5757.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010024051-01 & 2409.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010024701-01 & 2002.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010025929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010026136-01 & 7274.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010026136-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010026457-01 & 7275.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010026457-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010026458-01 & 6076.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_010026457-01\\
010026458-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010026457-02\\
010026502-01 & 4706.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010026614-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010026779-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010027247-01 & 2418.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010027323-01 & 1596.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010027323-02 & 1596.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010028140-01 & 1591.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010028352-01 & 1957.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010028352-02 & 1957.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010028524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010028535-01 & 2493.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010028792-01 & 1574.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010028792-02 & 1574.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
010028792-03 & 1574.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010028792-04 & 1574.04 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010029999-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010029999-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
010030092-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010030778-01 & 3265.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
010030778-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
010031409-01 & 7276.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010031500-01 & 3107.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_010031808-01\\
010031526-01 & 7277.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_010031808-01\\
010031634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010031634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010031656-01 & 2629.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010031808-01\\
010031707-01 & 1827.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PARENT\_IS\_010031808-01\\
010031707-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_010031808-02\\
010031808-01 & 7278.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
010031808-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
010031885-01 & 0329.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_010031808-01\\
010031885-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010031808-02\\
010031907-01 & 3828.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_010031808-01\\
010031907-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_010031808-01\\
010031918-01 & 4894.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_010031808-01\\
010032795-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010032819-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010033279-01 & 1604.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010033959-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010034425-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010034643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010035150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010035155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010035155-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010035155-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010035363-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010035363-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010035772-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010035772-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010035772-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010035772-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010053138-01 & 7279.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010053675-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010055126-01 & 1608.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010055126-02 & 1608.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010055126-03 & 1608.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
010056297-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
010056297-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010056297-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010056931-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010056931-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010057494-01 & 3234.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010059645-01 & 2520.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010063044-01 & 7280.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010063208-01 & 4292.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010063802-01 & 1888.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010064256-01 & 2849.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010064921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010065244-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010065244-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010065244-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010065244-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010066755-01 & 7281.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010066755-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
010068024-01 & 2891.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_529.01\\
010068024-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
010068024-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
010068030-01 & 0529.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
010068030-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
010068030-03 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010068383-01 & 0725.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
010068383-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010068659-01 & 2602.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010068797-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
010068919-01 & 3573.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010070331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010070468-01 & 2628.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010070479-01 & 7282.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010071056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010071339-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CROWDED\_DIFF\\
010071339-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010073654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
010073672-01 & 2764.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010074067-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010074466-01 & 1917.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010074700-01 & 5760.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
010074737-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010074841-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
010079420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010079420-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010079420-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010079420-04 & 7607.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010080248-01 & 1722.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010080943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010080943-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010080943-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010080943-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
010081256-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010081748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010081748-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010081748-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010082556-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010082844-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010082844-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010083134-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
010083134-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010083325-01 & 5761.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010083510-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010083510-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010083623-01 & 3921.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
010083623-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
010087801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010087801-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
010087973-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010088162-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010088162-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010089123-01 & 7283.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010089911-01 & 4034.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010089911-02 & 4034.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010090219-01 & 3978.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010090246-pri\\
010090257-01 & 2476.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010090246-pri\\
010090345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010090345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010090854-01 & 5762.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010091110-01 & 3627.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010091110-02 & 3627.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010091110-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010091175-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010091257-01 & 7284.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010091703-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010091792-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010091829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010092003-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
010092003-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
010092312-01 & 1823.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010092312-02 & 1823.02 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_1080.01\\
010093664-01 & 7285.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
010094670-01 & 1984.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010095484-01 & 3839.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010095496-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010095496-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010095512-01 & 7286.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010096641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010096641-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010096653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010097149-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010098322-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010098322-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010098534-01 & 7287.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
010098844-01 & 2964.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010118750-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010118750-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010118750-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
010118816-01 & 1085.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010119471-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010120548-01 & 4451.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010120971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010122012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010122012-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010122255-01 & 1086.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010122538-01 & 2926.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010122538-02 & 2926.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010122538-03 & 2926.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010122538-04 & 2926.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010122937-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010123064-01 & 0472.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010125352-01 & 0021.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
010125352-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
010128033-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010128033-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010128033-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010128713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010129349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010129349-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010129482-01 & 7288.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010130039-01 & 1909.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010130039-02 & 1909.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010130039-03 & 1909.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010130057-01 & 4675.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_FL-Lyr-pri\\
010130777-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010130777-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010132618-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010132832-01 & 2313.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010132867-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010132867-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010134152-01 & 2056.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010134709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010134709-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010134800-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010134800-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010134800-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010134800-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010135362-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010135362-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010135362-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010135493-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010136240-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010136549-01 & 1929.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010136549-02 & 1929.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010139305-01 & 6077.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
010139305-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
010139691-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010139691-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010139691-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010140122-01 & 4545.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010140274-01 & 4334.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010140665-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010140665-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
010141439-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010141900-01 & 1082.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010141900-02 & 1082.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010141900-03 & 1082.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010141900-04 & 1082.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010146103-01 & 5769.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010147217-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010147217-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
010147217-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010147854-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010148521-01 & 1084.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
010148787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010149023-01 & 1081.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010152836-01 & 3952.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010152836-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010153011-01 & 1773.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010153555-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010153855-01 & 1981.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010154094-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010154094-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010154094-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010154388-01 & 0991.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010154592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010154966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010154966-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010154994-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010154994-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010154994-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010155026-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---KIC\_OFFSET\\
010155029-01 & 3208.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010155080-01 & 7289.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
010155321-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010155321-02 & 4422.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010155434-01 & 0473.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010155816-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010155816-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010155816-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010156055-01 & 4284.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010156064-pri\\
010156064-01 & 7290.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
010156332-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010157458-01 & 1083.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010157458-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010157573-01 & 0726.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010158223-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010158223-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010158418-01 & 1784.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010158729-01 & 2097.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010158990-01 & 1080.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_1823.02\\
010161923-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
010161923-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010162509-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010162509-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010163067-01 & 7291.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010163067-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010163885-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
010164018-01 & 7292.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010164569-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010164569-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010164895-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010165660-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010166274-01 & 1078.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010166274-02 & 1078.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010166274-03 & 1078.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010166297-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010186945-01 & 4070.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010186945-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010187017-01 & 0082.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010187017-02 & 0082.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010187017-03 & 0082.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010187017-04 & 0082.04 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010187017-05 & 0082.05 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010187159-01 & 1870.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010188940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010189523-01 & 7293.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010189542-01 & 5773.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_427.01\\
010189546-01 & 0427.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010189546-02 & 0427.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010189546-03 & 0427.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010189557-01 & 2427.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010190075-01 & 3007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010190777-01 & 1937.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010191036-01 & 3218.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_T-Lyr1-00687-sec\\
010191056-01 & 5774.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010191070-01 & 0727.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_T-Lyr1-00687-sec\\
010191070-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010191142-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
010195926-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_010195933-02\\
010195926-02 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_010195933-02\\
010195926-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010195926-04 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED---PARENT\_IS\_010195933-01\\
010195926-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010195933-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_010195926-04\\
010195933-02 & \nodata & FP & 1 & 0 & 1 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_010195926-02\\
010196750-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010196863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010196863-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010197293-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010198109-01 & 7294.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010198109-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010198662-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010198662-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010198662-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010198872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010199055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
010199055-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
010200627-01 & 6217.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010201143-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010201143-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS---PARENT\_IS\_1783.01\\
010202759-01 & 2405.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010202859-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010203349-01 & 2212.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010206049-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010206643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010206643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010206675-01 & 2283.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010208140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010208303-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010208303-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010208345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010208345-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010208759-01 & 7295.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
010212441-01 & 2342.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010212441-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010212620-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010213902-01 & 1723.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010213964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010213964-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
010214039-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010214162-01 & 1724.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010214328-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010214328-02 & 7296.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010215422-01 & 7297.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010215422-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010215584-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
010215869-01 & 3548.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
010215869-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
010216016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010219475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010219475-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010220150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010220150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010220150-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010220150-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010220707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010220707-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010220707-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010220837-01 & 4613.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010220950-01 & 4544.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010221013-01 & 0728.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010221505-01 & 4768.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010222702-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010223616-01 & \nodata & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010224550-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010224550-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010224920-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010224920-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010224920-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010225800-01 & 0729.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010226083-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010226083-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010226083-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010226343-01 & \nodata & FP & 1 & 0 & 1 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_010226388-pri\\
010226420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010226448-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010226388-pri\\
010226451-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_010226388-pri\\
010226451-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_010226388-sec\\
010226487-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_010226388-pri\\
010226488-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010226388-pri\\
010226498-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_010226388-pri\\
010227020-01 & 0730.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010227020-02 & 0730.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010227020-03 & 0730.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010227020-04 & 0730.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010227501-01 & 0985.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010227501-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
010227863-01 & 3983.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_5780.01\\
010227881-01 & 5780.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010228942-01 & 6219.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010228942-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
010228991-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010229903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010230120-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010231017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010231119-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010231171-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010231171-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
010232091-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010232123-01 & 1075.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010232123-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010232693-01 & 2341.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010252131-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010252275-01 & 3130.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010252275-02 & 3130.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010253547-01 & 2153.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010253547-02 & 2153.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010253638-01 & 7608.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010253943-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010253943-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010253943-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010253943-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010256023-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010256787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010256787-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010257229-01 & 4557.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010257713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010257903-01 & 7298.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010257903-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010258260-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010258558-01 & 7299.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010258558-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010259029-01 & 3630.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010259029-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010259031-01 & 0731.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_3630.01\\
010259031-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010259029-02\\
010259301-01 & 3608.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010262272-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010262574-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010263705-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010263800-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010264202-01 & 7300.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010264293-01 & 7301.01 & PC & 0 & 0 & 0 & 0 & CENTROID\_SIGNIF\_UNCERTAIN\\
010264660-01 & 0098.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010264728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010264728-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010264728-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010264728-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010265524-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010265524-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010265524-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010265602-01 & 2689.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010265898-01 & 0732.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010265898-02 & 0732.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010265898-03 & 0732.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010266615-01 & 0530.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010267121-01 & 7609.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
010268809-01 & 7302.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010268809-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010268835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010268903-01 & 3773.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010268907-01 & 1077.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_CENTROIDS---PARENT\_IS\_3773.01\\
010268907-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_CENTROIDS---PARENT\_IS\_3773.01\\
010271806-01 & 0733.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010271806-02 & 0733.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010271806-03 & 0733.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010271806-04 & 0733.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010272389-01 & 4048.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---LARGE\_RM---PARENT\_IS\_V850-Cyg-pri\\
010272442-01 & 0734.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010272442-02 & 0734.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010272640-01 & 1074.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
010272747-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010272747-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
010272747-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010273384-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010273384-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
010273384-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010274244-01 & 7303.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010274244-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010275074-01 & 3606.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
010275284-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010275420-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010275766-01 & 2810.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010275747-pri\\
010275805-01 & 2782.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010275880-01 & 3734.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_010275887-pri\\
010275880-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010275887-sec\\
010275887-01 & 7304.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010275887-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010279745-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010279745-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010281118-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010281221-01 & 3913.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010281311-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010281311-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010281360-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010281360-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010281360-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010281639-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010281639-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010281639-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010281890-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010281890-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010284603-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
010284603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
010284901-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010284967-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
010285114-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010285525-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010285631-01 & 0331.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010287242-01 & 0735.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010287248-01 & 1152.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
010287248-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
010287874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010287874-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010288443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010288922-01 & 6078.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
010288922-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
010289119-01 & 2390.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010289211-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010289211-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010289432-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010290021-01 & 7305.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010290447-01 & 7306.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010290666-01 & 0332.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010290666-02 & 0332.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010291589-01 & 4754.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010292238-01 & 3526.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010292238-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010292465-01 & 7307.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
010292465-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
010292540-01 & 4689.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010293818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
010293818-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010293818-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010294509-01 & 4143.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_010294608-pri\\
010294608-01 & 7308.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
010294613-01 & 1896.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_010294608-pri\\
010294613-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010294608-01\\
010295951-01 & 1154.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
010296029-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010296163-01 & 7309.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010296163-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010296428-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010297233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010318874-01 & 0104.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010319341-01 & 5784.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010319385-01 & 1169.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010319590-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010320341-01 & 5786.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010321305-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010322290-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010322473-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010322797-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_T-Lyr1-00687-sec\\
010324412-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010324439-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010328393-01 & 1905.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010328393-02 & 1905.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010328393-03 & 1905.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010328458-01 & 2214.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010328476-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010329196-01 & 4446.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010329469-01 & 2271.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010329835-01 & 2058.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010330115-01 & 1160.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010330435-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010330435-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010330435-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010330495-01 & 7310.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010330495-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010330536-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010332213-01 & 2919.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010332320-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010332320-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010332789-01 & 7311.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010332789-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010332883-01 & 1880.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010333254-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010333254-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010334122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010336951-01 & 2401.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010337035-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010337258-01 & 0333.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010337323-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010337323-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
010337441-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010337517-01 & 1165.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010337517-02 & 1165.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010338279-01 & 3216.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010338279-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010338624-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010338624-02 & 3222.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010338624-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010339590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010340212-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010340228-01 & 7312.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010340423-01 & 0736.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010340423-02 & 0736.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010341072-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010341072-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010341072-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010341704-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010341755-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2083-Cyg-pri\\
010341777-01 & 7610.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_V2083-Cyg-pri\\
010341781-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_V2083-Cyg-pri\\
010341787-01 & 7313.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010341831-01 & 1164.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010341878-01 & 6220.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010341878-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010341878-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
010341905-01 & 2391.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2083-Cyg-pri\\
010341913-01 & 1172.01 & FP & 0 & 1 & 1 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010341913-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
010341913-03 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010341917-01 & 2823.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010342097-01 & 7314.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010342248-01 & 4315.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2083-Cyg-pri\\
010342316-01 & 4547.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2083-Cyg-pri\\
010345478-01 & 0737.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010345478-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010345862-01 & 7315.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010345862-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010346286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010346424-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010346424-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010346522-01 & 7316.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
010347481-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010347481-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010347481-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010347630-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010350571-01 & 1175.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010350571-02 & 1175.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010351231-01 & 1166.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010351735-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010351767-01 & 1153.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
010351834-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010352333-01 & 3991.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010352603-01 & 7317.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010352603-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010352938-01 & 3756.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010352945-01 & 1158.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3756.01\\
010353924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010353968-01 & 0618.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010354039-01 & 1159.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010355055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010357831-01 & 6221.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
010357831-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---TOO\_FEW\_QUARTERS\\
010357965-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
010357965-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
010358759-01 & 0738.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010358759-02 & 0738.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010358909-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010359526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010360294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010360722-01 & 4051.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010360907-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
010361364-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010362031-01 & 2118.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010362577-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010362577-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010363115-01 & 3908.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010363281-01 & 2726.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010363300-pri\\
010363300-01 & 7318.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
010363300-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010383429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CROWDED\_DIFF\\
010383429-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CROWDED\_DIFF\\
010383687-01 & 0334.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3671.01\\
010383687-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010383696-02\\
010383696-01 & 3671.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
010383696-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
010383729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010384298-01 & 3224.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010384798-01 & 1997.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010384962-01 & 0619.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010384962-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010385438-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010385438-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
010385682-01 & 6223.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
010386922-01 & 0289.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010386922-02 & 0289.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010386984-01 & 0739.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010387742-01 & 2583.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010388033-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010388286-01 & 0596.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010388451-01 & 7319.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010389724-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010394172-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010394172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010394802-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010394802-02 & 5790.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010395381-01 & 0740.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010395543-01 & 0531.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010395652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010396708-01 & 7320.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
010397751-01 & 2859.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010397751-02 & 2859.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010397751-03 & 2859.05 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010397751-04 & 2859.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010398088-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010398659-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010399321-01 & 4556.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010403036-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010404582-01 & 2147.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010404582-02 & 2147.02 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010405019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010405019-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010405019-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010405266-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010405470-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010407020-01 & 3987.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010407047-01 & 7321.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V2083-Cyg-pri\\
010407054-01 & 2500.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---PARENT\_IS\_V2083-Cyg-pri\\
010407086-01 & 4568.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010407210-01 & 4662.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_V2083-Cyg-pri\\
010407221-01 & 2605.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010407271-01 & 7611.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010407430-01 & 7322.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---PARENT\_IS\_V2083-Cyg-pri\\
010407464-01 & 7323.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V2083-Cyg-pri\\
010407482-01 & 4255.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010407522-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
010414727-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010415087-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010415087-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010415087-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010415087-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010415160-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010415227-01 & 2562.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010415502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
010415502-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010416390-01 & 5792.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
010416779-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010416779-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010416779-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010417704-01 & 7324.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
010417704-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010417704-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
010418224-01 & 0428.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010418470-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010418797-01 & 0741.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010418797-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010419211-01 & 0742.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010419211-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010419312-01 & 2412.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010419797-01 & 4073.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010420279-01 & 7325.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010420279-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010420279-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010420279-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010420279-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010422241-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010422241-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
010422241-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010422241-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
010422852-01 & 7326.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010422852-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010422852-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
010424228-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010424228-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010424228-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010424977-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010425482-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
010426656-01 & 1161.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010426656-02 & 1161.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010426656-03 & 1161.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010427700-01 & 4394.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010427996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010448626-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010448764-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010448764-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010448764-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010449486-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010449827-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010450504-01 & 7327.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010451090-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010451090-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010451090-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010453588-01 & 2484.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010454313-01 & 0532.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010454401-01 & 7328.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010454401-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010454401-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
010454589-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010454632-01 & 1877.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010460984-01 & 0474.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010460984-02 & 0474.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010460984-03 & 0474.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010460984-04 & 0474.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010462826-01 & 7329.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010462826-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010462980-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010462980-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010462980-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010464050-01 & 1851.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010464078-01 & 0743.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010464078-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010464199-01 & 7330.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010464666-01 & 3578.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010464666-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010464666-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010467714-01 & 4480.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010468404-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
010468514-01 & 7331.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
010468514-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010468883-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
010468883-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010468883-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010468883-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010468885-01 & 2589.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010468940-01 & 1163.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010468940-02 & 1163.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010469984-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010469984-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010469984-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010470099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010470206-01 & 0335.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010470294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010470294-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010470294-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010470294-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010470309-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010470309-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
010470616-01 & 2112.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010470882-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010470968-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010471055-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010471113-01 & 7332.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V2083-Cyg-pri\\
010471167-01 & 7612.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_V2083-Cyg-pri\\
010471174-01 & 7613.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2083-Cyg-pri\\
010471204-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010471345-01 & 7614.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_V2083-Cyg-pri\\
010471515-01 & 2961.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010471601-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010471621-01 & 2554.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010471780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010471780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010471914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010471914-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010471914-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010472431-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010472431-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010473272-01 & 4648.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010473929-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010480915-01 & 2040.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010480921-01 & 1173.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5797.01\\
010480952-01 & 5797.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
010480982-01 & 0744.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010480982-02 & 0744.02 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_5797.01\\
010481045-01 & 2320.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_5797.01\\
010481054-01 & 7333.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_5797.01\\
010481462-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010482160-01 & 1170.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010482774-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010482774-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010483436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010483436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010483436-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010483436-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010483644-01 & 6225.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010483644-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010484409-01 & 3366.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010484808-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010484808-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010484808-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010484808-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010484817-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010484817-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010484817-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010485035-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_010485137-pri\\
010485035-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010485047-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010485137-pri\\
010485069-01 & 1171.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_010485137-pri\\
010485165-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_010485137-pri\\
010485179-01 & 1167.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010485137-pri\\
010485179-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_010485137-pri\\
010485250-01 & 0745.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010485250-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010485961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010486425-01 & 7334.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010486425-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010487119-01 & 1635.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010487532-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
010488450-01 & 0290.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
010488715-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010489019-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010489019-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010489206-01 & 0251.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010489206-02 & 0251.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010489265-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010489265-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010489265-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010489345-01 & 2266.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010489373-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010489521-01 & 3625.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
010489525-01 & 0106.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3625.01\\
010489525-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010489521-01\\
010489539-01 & 3231.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010489783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010489783-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010490282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010490558-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010490558-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010490561-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010490561-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010490960-01 & 7335.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
010491031-01 & 7336.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
010491044-01 & 1763.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010491031-sec\\
010491062-01 & 3910.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010491031-sec\\
010491525-01 & 4589.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010491544-01 & 3639.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---LARGE\_RM---PARENT\_IS\_010491554-01\\
010491544-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_010491554-sec\\
010491554-01 & 3576.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---KIC\_OFFSET\\
010491554-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010513530-01 & 0533.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010513530-02 & 0533.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010514429-01 & 1614.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010514430-01 & 0263.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---SATURATED---PARENT\_IS\_010514429-01\\
010514770-01 & 1156.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
010516986-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010517437-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010518399-01 & 2800.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_010583181-pri\\
010518424-01 & 2188.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_010583181-pri\\
010518424-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_010583181-sec\\
010518725-01 & 0336.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3612.01\\
010518725-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010518735-02\\
010518735-01 & 3612.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
010518735-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
010521496-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010521496-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010524994-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010525027-01 & 2006.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010525049-01 & 4252.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010525077-01 & 5800.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010525592-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010525592-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010525592-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010525592-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010525662-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010526549-01 & 0746.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010526887-01 & 4261.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010527135-01 & 2622.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010527135-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010528068-01 & 1162.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010528093-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010528093-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010528286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010528564-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010528873-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010528873-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010529091-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010531955-01 & 2208.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010532030-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010532461-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010532771-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010532771-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010532771-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010533233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010533491-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010533616-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010533906-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010534150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010534155-01 & 4345.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010535424-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010535708-01 & 5801.02 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010535807-01 & 7337.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010535807-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
010535858-01 & 7338.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_V2083-Cyg-pri\\
010535867-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010535897-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_V2083-Cyg-pri\\
010536147-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
010536593-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010536593-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010537110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010537528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010537528-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010537528-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010537528-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010537907-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010537907-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010537907-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010538176-01 & 1301.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010538176-02 & 1301.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010538299-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010538299-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010544677-01 & 2244.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010545066-01 & 0337.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010546063-01 & 7339.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
010546563-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010547352-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010547685-01 & 7340.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010548114-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
010548195-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010548640-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010549023-01 & 2131.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010549292-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010549292-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010549292-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010549371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010549415-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---CLEAR\_APO\\
010549422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010549422-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010549562-01 & 1294.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_010549576-pri\\
010549562-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010549576-sec\\
010549576-01 & 7341.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010549576-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010549643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010549643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010549902-01 & 4826.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010549924-01 & 4214.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010550397-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010550660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
010551346-01 & 5804.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010551707-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010552016-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
010552016-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
010552151-01 & 5805.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
010552611-01 & 0338.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010552611-02 & 0338.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010552700-01 & 7342.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010552700-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
010553627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
010553884-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010553884-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010553884-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010554967-01 & 3059.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010554999-01 & 0534.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010554999-02 & 0534.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010555365-01 & 3771.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
010555375-01 & 0158.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_3771.01\\
010556064-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010556064-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
010556180-01 & 4828.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010556578-01 & 7343.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010577994-01 & 0475.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010577994-02 & 0475.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010580834-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010580834-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010581918-01 & 3807.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010581918-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010582569-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010583066-01 & 0747.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010583180-01 & 0748.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_010583181-pri\\
010583180-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_010583181-sec\\
010583181-01 & 7344.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
010583225-01 & 3902.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_010583181-pri\\
010583225-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_010583181-sec\\
010583761-01 & 2300.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010584140-01 & 4833.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010585738-01 & 3032.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010585749-01 & 4563.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010585852-01 & 1314.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010586004-01 & 0275.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010586004-02 & 0275.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010586045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010586045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010586045-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010586208-01 & 1308.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010586619-01 & 7345.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010586744-01 & 4892.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010587105-01 & 0339.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010587105-02 & 0339.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010587105-03 & 0339.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010590285-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010590857-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010590857-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010590857-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010590887-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010590887-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010590887-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010591855-01 & 2845.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010592106-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010592163-01 & 7346.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010592163-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010592258-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010592818-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010592860-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010593535-01 & 4204.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010593626-01 & 0087.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010593759-01 & 0025.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010593761-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010594394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
010594394-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
010596359-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010597164-01 & 7347.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_V850-Cyg-pri\\
010597693-01 & 2958.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010598279-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010599206-01 & 0476.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010599397-01 & 1285.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
010600261-01 & 0597.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010600261-02 & 0597.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010600261-03 & 0597.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010600540-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010600540-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010600540-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010600540-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010600955-01 & 2227.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010601284-01 & 0749.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010601284-02 & 0749.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010601284-03 & 0749.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010601538-01 & 7348.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010601549-pri\\
010601549-01 & 6226.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010601549-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
010601579-01 & 7349.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010602088-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010602291-01 & 0210.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010602324-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010602324-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010604335-01 & 1298.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010604335-02 & 1298.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010604335-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010604429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
010604429-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010604521-01 & 2797.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010604592-01 & 4447.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010604747-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010604747-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010609602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010609641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010609641-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010609641-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010610039-01 & 4577.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010611049-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010611049-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
010611420-01 & 3148.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010612865-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010613718-01 & 7350.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010613718-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
010614012-01 & 1807.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010614094-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010614158-01 & 6227.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010614845-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010615125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010615440-01 & 4765.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010616415-01 & 1999.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010616571-01 & 0340.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010616571-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010616571-03 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010616656-01 & 5814.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010616679-01 & 0429.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010616829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010617017-01 & 2149.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010617638-01 & 3016.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---CLEAR\_APO\\
010618078-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010618236-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_010618253-pri\\
010618475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010618543-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010619109-01 & 7351.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
010619142-01 & 3082.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_010619109-pri\\
010619192-01 & 0203.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010619192-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010619192-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010621643-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010621643-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010621666-01 & 1636.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_010686876-01\\
010621666-02 & 1636.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010621791-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010645230-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010646620-01 & 7352.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010647452-01 & 4366.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010647493-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010647493-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010647493-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010647611-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010647611-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010647611-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010649230-01 & 7353.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010651816-01 & 3953.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
010651945-01 & 3441.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010651945-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010651961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010652379-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010652379-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010652379-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010653179-01 & 3280.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010656508-01 & 0211.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010656823-01 & 0598.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010656823-02 & 0598.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010657150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010657150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010657406-01 & 1837.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010657406-02 & 1837.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010657634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010657634-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010657634-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010657664-01 & 0964.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010657664-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010657664-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
010658122-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010658122-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010658177-01 & 5817.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010658802-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010658802-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010658802-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010659313-01 & 6079.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010659313-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
010659624-01 & 7354.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010659654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010659654-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010661679-01 & 5818.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010661718-01 & 3931.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010661783-pri\\
010661721-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010661721-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010661771-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010661771-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010661778-01 & 4118.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_010661783-pri\\
010661913-01 & 7355.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_010661783-pri\\
010661917-01 & 4901.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_010661783-pri\\
010661976-01 & 7356.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---TOO\_FEW\_QUARTERS\\
010662021-01 & 7357.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_010661783-pri\\
010662202-01 & 0750.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010662202-02 & 0750.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010662202-03 & 0750.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010663294-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010663294-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010663294-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010663396-01 & 2046.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010663738-01 & 4698.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010664416-01 & 2599.01 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010664703-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010664703-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010664703-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010664703-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010665228-01 & 7358.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010665749-01 & 7359.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010666230-01 & 1295.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010666242-01 & 0198.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010666592-01 & 0002.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
010666592-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
010667698-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010668233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010668233-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010668665-01 & 3986.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010669199-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010669199-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010669515-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010669994-01 & 4360.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010670112-01 & 7360.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010670119-01 & 2179.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010670119-02 & 2179.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010670412-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010670412-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010674871-01 & 2068.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010675762-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010675762-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010675762-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010676014-01 & 1797.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010676395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010676750-01 & 4804.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010676824-01 & 0599.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010676923-01 & 1297.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3830.01\\
010676927-01 & 3830.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010677186-01 & 3595.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010677186-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010677193-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010677193-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010678547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010678547-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010678817-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010678817-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010678963-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010679246-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010679429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010679429-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010679583-01 & 2549.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010680424-01 & 7361.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
010681475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010681550-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010682541-01 & 0751.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010684587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010684587-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010684587-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010684670-01 & 2317.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010685175-01 & 7362.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010685175-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
010685653-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010685653-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010685897-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010685897-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
010686752-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010686814-01 & 2978.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_010686876-01\\
010686864-01 & 1637.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010686876-01 & 7363.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
010686876-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010686930-01 & 7364.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_010686876-01\\
010709622-01 & 2108.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010710755-01 & 6080.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010710755-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010711551-01 & 3359.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010711551-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010711551-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
010711913-01 & 7365.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010711913-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010713398-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010713398-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010713616-01 & 1311.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010714072-01 & 4024.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010717220-01 & 6228.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010717241-01 & 0430.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010717241-02 & 0430.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010717721-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010717871-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010717871-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010718726-01 & 0600.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010721830-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
010722485-01 & 4312.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010722668-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
010723367-01 & 2236.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010723367-02 & 2236.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010723618-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010723618-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010723618-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
010723750-01 & 0209.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010723750-02 & 0209.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010724369-01 & 1302.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010724372-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_010724533-pri\\
010724379-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010724533-pri\\
010724429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010724450-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_010724533-pri\\
010724544-01 & \nodata & FP & 1 & 0 & 0 & 1 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS---PARENT\_IS\_010724533-pri\\
010724551-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_010724533-pri\\
010724569-01 & 5823.01 & FP & 1 & 0 & 1 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010724533-pri\\
010724619-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_010724533-pri\\
010724621-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010724533-pri\\
010724635-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010724533-pri\\
010727668-01 & 6081.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010727668-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010728219-01 & 6229.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010728219-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010728219-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
010729645-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010729645-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010730034-01 & 1305.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010730034-02 & 1305.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010730070-01 & 4335.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010730571-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010730571-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010730703-01 & 2327.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010730703-02 & 2327.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010730838-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
010730838-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010730838-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010730838-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010732401-01 & 7366.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---INVERT\_DIFF---PARENT\_IS\_V2083-Cyg-pri\\
010732407-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_V2083-Cyg-pri\\
010732638-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
010732638-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010732638-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010733174-01 & 3889.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010733174-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010733174-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
010733208-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
010734935-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010734935-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010734935-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
010734935-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
010735331-01 & 3720.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010735519-01 & 6082.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010735519-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010735564-01 & 3617.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010735575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010735575-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
010735757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010735757-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010735757-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010735988-01 & 6230.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010735988-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010736179-01 & 4408.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_V2290-Cyg-pri\\
010736223-01 & 7367.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
010736489-01 & 7368.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010736591-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010741920-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010741920-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010741920-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010741920-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010743597-01 & 0989.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010743597-02 & 0989.04 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010743597-03 & 0989.02 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010743600-01\\
010743597-04 & \nodata & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
010743600-01 & 7369.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010744335-01 & 1304.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010744342-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010744342-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010744575-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010745159-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010745159-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010745365-01 & 4405.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010747037-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010747439-01 & 1638.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_2673.01\\
010747445-01 & 2673.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
010747445-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
010747501-01 & 4891.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010748390-01 & 0003.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010748393-01 & 1289.01 & FP & 0 & 0 & 0 & 1 & KIC\_OFFSET---CENTROID\_SIGNIF\_UNCERTAIN---PARENT\_IS\_010748390-01\\
010748621-01 & 3532.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010748621-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010749059-01 & 3086.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
010749745-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_010815379-pri\\
010749766-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_010815379-pri\\
010749775-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010749775-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010749793-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010749793-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010749793-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010750903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010750903-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010750903-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
010751515-01 & 3589.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV\\
010751638-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010751908-01 & 7370.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010753210-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010753210-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
010753734-01 & 7371.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010753734-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010753734-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
010753734-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010753734-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010775748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010775968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010777060-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010777591-01 & 5827.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010777903-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010777903-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010777903-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010777903-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010779233-01 & 1989.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010779585-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010779585-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010783150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010783150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
010783150-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010783150-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010784473-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010784473-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010785538-01 & 1313.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010788451-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010788451-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010788461-01 & 3925.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
010788461-02 & 3925.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
010788461-03 & 3925.03 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
010788617-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010788617-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010789361-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010789361-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010789864-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010789864-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010790387-01 & 1288.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010790660-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010790706-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010790706-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010793114-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010793172-01 & 2871.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010793172-02 & 2871.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010793172-03 & 2871.03 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
010793576-01 & 3451.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010794087-01 & 1316.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010794242-01 & 7372.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
010794405-01 & 7373.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010858720-pri\\
010794509-01 & 4673.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_010858720-pri\\
010794509-02 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---PARENT\_IS\_010858720-sec\\
010794974-01 & 4235.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010795103-01 & 3683.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010796473-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010796477-pri\\
010796473-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_010796477-pri\\
010797123-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010797460-01 & 0752.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010797460-02 & 0752.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010797891-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010798331-01 & 2373.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010798605-01 & 3390.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010798605-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010798838-01 & 3449.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010799291-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010799291-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010799735-01 & 0193.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010799735-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010801100-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010801249-01 & 4611.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM---PARENT\_IS\_3617.01\\
010801738-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010801951-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---PARENT\_IS\_V2290-Cyg-pri\\
010802820-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
010803371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010803371-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010809677-01 & 7374.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
010810140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
010810838-01 & 0174.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010810859-01 & 4801.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010811496-01 & 0753.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010811720-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
010811753-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010811753-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010812504-01 & 2570.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010812541-01 & 7375.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010812657-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010812657-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010813078-01 & 5831.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010813132-01 & 2378.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010813172-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
010813172-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010813841-01 & 1640.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010813970-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010813970-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010813970-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010814711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010814711-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010814863-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010814863-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010814863-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010815466-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010815677-01 & 7376.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010815916-01 & 4470.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010815932-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010815932-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010815932-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010816107-01 & 7377.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010816107-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010816278-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010816278-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010817600-01 & 5832.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010817620-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010842192-01 & 2736.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010843203-01 & 1287.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010843431-01 & 7378.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010843590-01 & 0431.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010843590-02 & 0431.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010844890-01 & 1946.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010845188-01 & 3602.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010847907-01 & 7379.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET---PARENT\_IS\_010586874-pri\\
010847907-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET---PARENT\_IS\_010586874-sec\\
010848097-01 & 7380.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010848459-01 & 0754.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
010849244-01 & 7381.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010850327-01 & 5833.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010851035-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010853783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
010853908-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010853908-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010854166-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010854166-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010854546-01 & 2104.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010854555-01 & 0755.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010854768-01 & 1309.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010854977-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
010854977-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
010855545-01 & 5834.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010857342-01 & 3739.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
010857519-01 & 2075.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010857589-01 & 7382.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010857589-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010857698-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010857698-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010858117-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
010858117-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
010858691-01 & 1306.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010858691-02 & 1306.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010858691-03 & 1306.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010858691-04 & 1306.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010858737-01 & 4183.01 & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_010858720-sec\\
010858737-02 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CROWDED\_DIFF---PARENT\_IS\_010858720-pri\\
010858785-01 & 4171.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_010858720-pri\\
010858785-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_010858720-sec\\
010858803-01 & 4130.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_010858720-pri\\
010858803-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_010858720-sec\\
010858832-01 & 0432.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010859386-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010859386-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010859386-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010859386-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
010860098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010862354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010862354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010862354-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010862759-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010862889-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010863608-01 & 2368.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010864531-01 & 2080.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010864531-02 & 2080.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010864656-01 & 1299.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010864709-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010865397-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010865801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
010866969-01 & 7383.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010867017-01 & 7384.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
010867017-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
010867062-01 & 1303.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010872983-01 & 0756.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010872983-02 & 0756.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010872983-03 & 0756.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010873178-01 & 4597.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010873260-01 & 0535.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010873344-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010873947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010874215-01 & 2305.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010874226-01 & 1290.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010874226-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010874614-01 & 0017.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010874822-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010874926-01 & 1293.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010874926-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
010875007-01 & 4149.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010875007-02 & 4149.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010875245-01 & 0117.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010875245-02 & 0117.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010875245-03 & 0117.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---CROWDED\_DIFF\\
010875245-04 & 0117.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
010876237-01 & 2960.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
010876944-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
010877024-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_010934755-pri\\
010877182-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010877182-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010877367-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010877669-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_010877703-pri\\
010877999-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010877999-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010877999-03 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
010878263-01 & 0341.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010878263-02 & 0341.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010879038-01 & 1641.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010879208-01 & 1286.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010879213-01\\
010879213-01 & 3730.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
010879656-01 & 1642.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
010879656-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
010879833-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
010880041-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010880041-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010880041-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010880507-01 & 2936.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010880895-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010881457-01 & 3484.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010881855-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010881855-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010903251-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010903251-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010904004-01 & 2957.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010904343-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010904343-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010904343-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010904343-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010904857-01 & 0194.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010904857-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010905239-01 & 0046.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010905239-02 & 0046.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010905746-01 & 1725.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010905911-01 & 2754.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010907132-01 & 4503.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010908248-01 & 3146.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010909127-01 & 2200.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010909274-01 & 7385.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010909274-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010909274-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010910878-01 & 0757.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010910878-02 & 0757.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010910878-03 & 0757.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010913758-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010916600-01 & 2623.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010916600-02 & 2623.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010916978-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010917043-01 & 2770.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010917433-01 & 3248.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010917681-01 & 1963.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010918393-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010918393-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010919230-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010920086-01 & 5841.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010920086-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010920086-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010920447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010920447-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010920813-01 & 7386.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010920813-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
010921238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010921757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010921757-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010921894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010921894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010921894-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010922093-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010922506-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010922610-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010922659-01 & 3335.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010923260-01 & 7387.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010923260-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010923282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010923282-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010923282-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010923648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
010923648-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010923649-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
010924282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010924282-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010924282-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010924340-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM---PARENT\_IS\_010924400-01\\
010924340-02 & 4326.01 & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
010924400-01 & 7388.01 & FP & 0 & 1 & 1 & 1 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM---PARENT\_IS\_010924340-01\\
010924400-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_4326.01\\
010924562-01 & 3063.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010924853-01 & 1292.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010925104-01 & 0156.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010925104-02 & 0156.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010925104-03 & 0156.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010925113-01 & 2557.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_010925104-01\\
010925227-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010925227-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010928043-01 & 1315.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010931507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010931805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010931805-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010932270-01 & 7389.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010933306-01 & 5842.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010933561-01 & 0291.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010933561-02 & 0291.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010934313-01 & 3121.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010934556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010934556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010934674-01 & 0477.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010935310-01 & 6083.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010935310-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010935383-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010935383-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010935993-01 & 3367.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010936427-01 & 7390.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010936786-01 & 4179.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010937029-01 & 0433.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010937029-02 & 0433.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
010937527-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010937527-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010937527-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010937609-01 & 7391.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
010937628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010937628-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010937749-01 & 4499.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010938094-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010959320-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010959320-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010959320-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010959320-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010960993-01 & 1284.01 & FP & 0 & 1 & 0 & 1 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED---PARENT\_IS\_3564.01\\
010960995-01 & 3564.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---KIC\_OFFSET\\
010963065-01 & 1612.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
010963242-01 & 1312.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010963497-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
010964265-01 & 2934.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010964265-02 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
010964422-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010964440-01 & 1310.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010965008-01 & 0536.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010965588-01 & 2177.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010965740-01 & 1887.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
010965963-01 & 7392.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010969616-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
010971633-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010971674-01 & 1296.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010971674-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010971944-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010972902-01 & 4692.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS---PARENT\_IS\_4673.01\\
010972902-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
010973583-01 & 6232.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
010973583-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010973664-01 & 0601.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010973664-02 & 0601.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010973664-03 & 0601.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010973814-01 & 1307.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010973814-02 & 1307.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010975126-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
010975146-01 & 1300.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010976412-01 & 7393.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
010977671-01 & 5846.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
010977859-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010978763-01 & 1931.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010978763-02 & 1931.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010978763-03 & 1931.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010979139-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010979716-01 & 7394.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
010982373-01 & 7395.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010982872-01 & 0343.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010982872-02 & 0343.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010982872-03 & 0343.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
010982884-01 & \nodata & FP & 1 & 0 & 0 & 1 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
010983528-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010983635-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
010984090-01 & 0112.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010984090-02 & 0112.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
010987439-01 & 7396.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
010987439-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
010987985-01 & 0758.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010988009-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
010988009-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010988009-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
010988009-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
010989032-01 & 7397.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
010989032-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
010989032-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010989032-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010989032-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
010989166-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_009851142-pri\\
010989274-01 & 6233.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
010989345-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010989859-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010989859-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010990083-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010990083-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
010990092-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010990452-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
010990452-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010990452-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
010990885-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
010990886-01 & 0478.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
010990917-01 & 1643.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010990961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
010990961-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
010991114-01 & 4374.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010991360-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
010991389-01 & 5850.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
010991989-01 & 7398.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
010991989-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
010992011-01 & 4025.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_010991989-pri\\
010992733-01 & 7399.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
010992733-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
010992733-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
011013201-01 & 0972.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011013201-02 & 0972.02 & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011013201-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011014282-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011014282-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011014932-01 & 1432.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011014932-02 & 1432.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011014932-03 & 1432.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011014932-04 & 1432.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
011015108-01 & 0344.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011015323-01 & 0479.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011017070-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_011017077-pri\\
011017094-01 & 4106.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF---PARENT\_IS\_011017077-pri\\
011017401-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011017901-01 & 1800.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011018648-01 & 0759.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011018648-02 & 0759.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011019739-01 & 7400.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011019987-01 & 3060.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011019987-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011020521-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011020521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011020521-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011021188-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011021188-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011021188-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011021188-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011021252-01 & 6084.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011021252-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011025754-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011026045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011026045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011026304-01 & 1420.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011026582-01 & 5854.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011027270-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011027270-02 & 7401.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011027624-01 & 1439.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011027708-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011027722-01 & 7402.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011027729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011027729-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011027806-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011029626-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011029877-01 & 7403.01 & FP & 0 & 1 & 1 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---LARGE\_RM\\
011030475-01 & 2248.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011030475-02 & 2248.03 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011030711-01 & 1429.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011031512-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011031512-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011031728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011031728-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011032227-01 & 1440.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011032402-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---CENTROID\_SIGNIF\_UNCERTAIN\\
011032573-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011033504-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011036168-01 & 5855.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011036440-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011036440-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011036440-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011036972-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011037105-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011037105-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011037105-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011037105-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011037128-01 & 4309.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011037335-01 & 1435.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011037335-02 & 1435.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011037511-01 & 2580.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011037818-01 & 5856.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011043136-01 & 1644.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011043136-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011043167-01 & 1444.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011044196-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011044372-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011044372-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011044372-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011044372-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011044384-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011044384-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011044394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011044394-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011044547-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011044547-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011044547-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011044770-01 & 0170.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_3327.01\\
011044770-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_011044779-02\\
011044779-01 & 3327.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
011044779-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
011045383-01 & 1645.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011046025-01 & 1646.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011046028-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011046028-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011046458-01 & 0214.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011046569-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011046870-01 & 5858.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_1418.01\\
011068630-01 & 7404.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011069176-01 & 2007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011069176-02 & 2007.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011071200-01 & 2696.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011071200-02 & 2696.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011071207-01 & 7405.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011071207-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011071207-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011072016-01 & 4852.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011073223-01 & 7406.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011073223-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011073223-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
011073351-01 & 0537.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011073656-01 & 2206.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011074178-01 & 1889.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011074178-02 & 1889.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011074514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
011074541-01 & 0345.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011074835-01 & 2533.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011075124-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011075279-01 & 1431.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011075429-01 & 2198.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011075737-01 & 0292.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011076176-01 & 5862.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011076276-01 & 4645.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_011076279-pri\\
011076279-01 & 7407.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011076400-01 & 2759.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011080405-01 & 2442.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011080405-02 & 2442.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011080702-01 & 5863.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011080711-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
011080961-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
011081490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011081490-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011081490-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011081504-01 & 4287.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011081504-02 & 4287.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011081512-01 & 3364.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011081512-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011081512-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
011081971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011084474-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011086270-01 & 0124.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011086270-02 & 0124.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011086712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011086712-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011087914-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011090405-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011090405-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011090405-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011090556-01 & 2977.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011090556-02 & 2977.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011090561-01 & 5865.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011090765-01 & 0538.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011091029-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011092783-01 & 7408.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011093203-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011093203-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011093335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011093335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011093335-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011093538-01 & 3326.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
011093538-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
011098013-01 & 2712.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011098069-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011099031-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011099031-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011099351-01 & 6234.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011099351-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011100331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011100383-01 & 0346.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011100522-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011100522-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011100522-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011100532-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011100532-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011100657-01 & 1418.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
011100657-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011100670-01 & 2885.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
011100670-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
011121752-01 & 2333.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011121752-02 & 2333.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011122894-01 & 1426.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011122894-02 & 1426.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011122894-03 & 1426.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011124436-01 & 4442.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011124509-01 & 7409.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011124904-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011124904-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011125613-01 & 2485.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011125613-02 & 2485.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011125613-03 & 2485.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011125666-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM\\
011125706-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011125706-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011125706-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011125756-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
011125764-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011125764-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011125764-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011125797-01 & 3371.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011125936-01 & 1419.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
011125936-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011126381-01 & 1863.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011127000-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011127190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011127479-01 & 2792.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011127641-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011127641-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011129258-01 & 2898.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011129738-01 & 1427.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011129738-02 & 1427.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011133190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011133190-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011133306-01 & 0276.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011134079-01 & 7410.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011134079-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011134456-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011134682-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
011134879-01 & 0480.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011135308-01 & 2805.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011137061-01 & 7411.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011137065-01 & 4620.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_V2083-Cyg-pri\\
011137180-01 & 3027.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011137913-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
011138155-01 & 0760.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011139567-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
011140501-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011140501-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011140501-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011144439-01 & 7412.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011144554-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011145138-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011145138-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
011145408-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011145831-01 & 4039.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
011145831-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
011147276-01 & 7413.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011147460-01 & 6235.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011147460-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011147814-01 & 3334.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011152054-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011152159-01 & 0761.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
011152159-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
011152428-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
011152428-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
011152463-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011152511-01 & 5874.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011152625-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011152625-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011152649-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011152649-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011152649-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011153121-01 & 1647.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011153121-02 & 1647.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011153121-03 & 1647.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011153259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011153259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011153476-01 & 4601.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011153539-01 & 0762.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011154043-01 & 7414.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011154043-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011154043-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
011154043-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011154043-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011175316-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011176127-01 & 1430.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011176127-02 & 1430.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011176127-03 & 1430.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011176166-01 & 5875.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
011176166-02 & 5875.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
011177543-01 & 1648.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011177676-01 & 3281.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011177707-01 & 1423.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011177741-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011177941-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011179076-01 & 2497.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011179734-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011181260-01 & 4653.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011182260-01 & 7415.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
011182260-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
011182608-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011182608-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011182608-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011182840-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011183259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011183259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011183539-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011183539-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011186590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011186590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011186929-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
011187436-01 & 1804.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011187716-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
011187716-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011187837-01 & 0252.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---KIC\_OFFSET\\
011187972-01 & 7416.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011188249-01 & 2765.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011189127-01 & 0347.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011189284-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011189284-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011189284-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011189284-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011189311-01 & 3220.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011191328-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011192141-01 & 0977.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011192235-01 & 2329.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011192998-01 & 0481.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011192998-02 & 0481.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011192998-03 & 0481.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011193046-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011193046-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011193263-01 & 1438.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011193447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011193457-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011193457-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011194032-01 & 0348.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011194055-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011194055-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011196937-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011196937-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011196937-03 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011197126-01 & 1443.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
011197126-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
011197654-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011197654-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011197853-01 & 2813.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011197934-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011197934-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011197934-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011198723-01 & 7417.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011198723-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011199228-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011199228-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011199228-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011199725-01 & 7418.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011199736-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011199801-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011200405-01 & 3724.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_CENTROIDS\\
011200405-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---TOO\_FEW\_QUARTERS\\
011200415-01 & 0293.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3724.01\\
011200767-01 & 3667.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_011200773-01\\
011200773-01 & 7419.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
011201483-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011206038-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011206038-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011206038-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011206101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011228612-01 & 7420.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011228612-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011229003-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011229102-01 & \nodata & FP & 1 & 0 & 1 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011231162-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011231334-01 & 0258.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
011231334-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
011232111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011232111-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011232745-01 & 7421.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011233743-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011233743-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011233911-01 & 7422.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011234677-01 & 7423.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011234677-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011235323-01 & 7424.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011235323-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011235536-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
011235536-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---TOO\_FEW\_CENTROIDS\\
011236035-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011236244-01 & 2460.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011236745-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011237410-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011240948-01 & 7425.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011240948-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011240948-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011240948-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011241560-01 & 7426.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011241814-01 & 3717.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011241912-01 & 3346.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011242721-01 & 0763.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011243547-01 & 4517.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_011401845-pri\\
011244137-01 & 2994.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011244571-01 & 7427.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011244682-01 & 3933.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011244787-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011246161-01 & 2796.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011249624-01 & 3553.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011249624-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011249624-03 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE\\
011250587-01 & 0107.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011250867-01 & 7428.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011250867-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011251058-01 & 7429.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_011250867-01\\
011252617-01 & 6236.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011252617-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011252617-03 & 6236.02 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
011253711-01 & 1972.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011253711-02 & 1972.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011253827-01 & 2672.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011253827-02 & 2672.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011254382-01 & 1425.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011255231-01 & 3003.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011255761-01 & 0482.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011259686-01 & 0294.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011259967-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011259967-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011260307-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011260307-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011260307-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
011260307-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011282568-01 & 7430.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011283615-01 & 2816.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011284505-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011284505-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011284505-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011284772-01 & 4622.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011285136-01 & 1774.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011285136-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011285625-01 & 7431.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
011285767-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011285767-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011285767-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011285870-01 & 3110.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011286311-01 & 7432.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011287726-01 & 7433.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011288051-01 & 0241.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011288051-02 & 0241.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011288051-03 & 0241.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011288072-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011288072-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011288492-01 & 7434.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011288505-01 & 1433.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011288686-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
011288686-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
011288686-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011288772-01 & 7435.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011289905-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011289905-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011290515-01 & 4716.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011290515-02 & 4716.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011293898-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011293898-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011294394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011294394-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011294394-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011294453-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011294931-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011294931-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011294931-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011295085-01 & 7436.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
011295085-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011295085-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011295349-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011295349-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011295426-01 & 0246.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011295426-02 & 0246.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011295582-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011295729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011295729-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011295729-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011295805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011295805-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011295805-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011295805-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011296045-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011296045-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011296045-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011296437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011296724-01 & 7437.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011296798-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011296798-02 & 7615.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011297236-01 & 1857.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011297440-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011298020-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011298220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011298298-01 & 1802.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011298815-01 & 2015.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011302565-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011302627-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011302627-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011302627-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011303065-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011303090-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011303322-01 & 3345.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011303811-01 & 3744.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
011303811-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011303815-01 & 2645.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3744.01\\
011304344-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011304344-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011304436-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011304436-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011304436-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011304436-04 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
011304958-01 & 0764.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011304987-01 & 2993.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
011305366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011305996-01 & 3256.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
011306840-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011307947-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011308499-01 & 2168.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011308499-02 & 2168.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011309335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011309335-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011336614-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011336614-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011336883-01 & 1445.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011337012-01 & 4666.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011337141-01 & 1649.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011337372-01 & 1650.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011337372-02 & 1650.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011337566-01 & 2632.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011337833-01 & 1651.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011338056-01 & 4735.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011338250-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
011338940-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011340713-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011340713-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011341164-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011341164-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011341314-01 & 5887.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_011235323-pri\\
011342032-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011342416-01 & 2366.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011342573-01 & 1771.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011342880-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011342880-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011348997-01 & 2090.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011350118-01 & 4509.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011350238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011350238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011350238-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011350238-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011350389-01 & 7438.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---LARGE\_RM\\
011351454-01 & 5889.01 & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
011356260-01 & 1441.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011356602-01 & 7439.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
011357192-01 & 3782.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011357302-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
011357664-01 & 4464.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011358389-01 & 2163.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011358389-02 & 2163.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011358389-03 & 2163.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011358392-01 & 7440.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011358392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011358392-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011359305-01 & 7441.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011359305-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011359657-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011359657-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011359657-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011359786-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011359879-01 & 0128.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011360571-01 & 2069.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011360704-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011360805-01 & 2422.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011360805-02 & 2422.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011361283-01 & 2551.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011361646-01 & 0330.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011361646-02 & 0330.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011362162-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011389737-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011389737-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011389737-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011389771-01 & 1436.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011389771-02 & 1436.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011389771-03 & 1436.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011390595-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011390595-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011390941-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011390941-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011390941-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011391018-01 & 0189.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011391181-01 & 7442.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011391181-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011391636-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011391667-01 & 1652.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011391755-01 & 2639.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011391957-01 & 0765.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011392017-01 & 1653.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011392618-01 & 1623.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011393217-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011393634-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011394027-01 & 0349.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011395310-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
011395392-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011395392-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011395392-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011395587-01 & 0350.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011395936-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011395936-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011395936-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011400413-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011400413-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011400842-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011400961-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011401182-01 & 1428.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401253-01 & 4823.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401755-01 & 0277.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401755-02 & 0277.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401767-01 & 2195.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401767-02 & 2195.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401767-03 & 2195.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011401822-01 & 2454.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_011401845-pri\\
011401845-01 & 5894.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011401845-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
011401869-01 & 7443.01 & FP & 1 & 0 & 0 & 1 & LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET---PARENT\_IS\_011401845-pri\\
011402817-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011402951-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011402951-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011402951-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011402995-01 & 0173.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011403044-01 & 0766.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011403216-01 & 3561.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011403216-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011403339-01 & 2143.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011403389-01 & 2482.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011403530-01 & 3015.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011404033-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011404644-01 & 6085.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011404644-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011404698-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011404698-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011407569-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011407569-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011407811-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011407847-01 & 5895.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011408237-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011408935-01 & 6086.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011408935-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011409698-01 & 7444.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011409698-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011409748-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011409748-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011409748-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011410904-01 & 2171.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011410915-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
011411639-01 & 7445.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011411670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011411670-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011412250-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
011413125-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011413125-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011413125-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011413125-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011413812-01 & 1885.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011414465-01 & 2836.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011414511-01 & 0767.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011414527-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011414527-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011414527-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011414527-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011414684-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
011414684-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011415243-01 & 4036.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011415556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011415556-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011416104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011416104-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011416506-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011416506-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011416506-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011442175-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011442353-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011442353-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011442353-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011442465-01 & 0768.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
011442465-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
011442793-01 & 0351.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
011444434-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011444514-01 & 4371.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011444952-01 & 4040.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
011445111-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011445913-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011445913-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011445913-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011445913-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011446254-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_011904038-pri\\
011446443-01 & 0001.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011446961-01 & 5899.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011449844-01 & 0125.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011450414-01 & 1992.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011450414-02 & 1992.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011450414-03 & 1992.03 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011453592-01 & 2705.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011453930-01 & 5900.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
011454304-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011454341-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
011454487-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
011454487-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
011454487-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011454525-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
011455181-01 & 3131.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011455428-01 & 3365.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011455484-01 & 3673.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011455491-01 & 0178.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_011455484-01\\
011455491-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_011455484-sec\\
011455507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011455507-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011455795-01 & 7446.01 & FP & 0 & 1 & 0 & 0 & OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
011455795-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
011455795-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
011456154-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011456154-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011456279-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011456279-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011456279-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011456382-01 & 2771.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_4845.01\\
011456405-01 & 4845.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF---PARENT\_IS\_2771.01\\
011457191-01 & 7447.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011457191-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011457198-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011457198-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011457726-01 & 2047.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011459949-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011460018-01 & 0769.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011460462-01 & 2110.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011461433-01 & 2399.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011461821-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011461821-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011461844-01 & 2356.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011462151-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011462151-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011462151-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011462341-01 & 2124.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011462556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011462556-02 & 7448.01 & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011463211-01 & 0770.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011463950-01 & 7616.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011463950-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011464245-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011464245-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011464245-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
011465134-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011465134-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011465651-01 & 4150.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011465678-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011465950-01 & 2620.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011465959-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---LARGE\_RM\\
011466960-01 & 3917.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011467509-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011468301-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011469049-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
011493431-01 & 1434.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011493732-01 & 0772.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011494130-01 & 0978.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011495305-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011495305-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011495458-01 & 2318.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011495989-01 & 7449.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011495989-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011496366-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011496490-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---LARGE\_RM\\
011496490-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
011496490-03 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
011497012-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011497648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011497958-01 & 1422.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011497958-02 & 1422.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011497958-03 & 1422.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011497958-04 & 1422.05 & PC & 0 & 0 & 0 & 0 & \nodata\\
011497958-05 & 1422.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
011497977-01 & 0483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011498128-01 & 2296.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011498764-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011499192-01 & 3120.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011499228-01 & 2109.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011499263-01 & 3620.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011499757-01 & 7450.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011499757-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011501774-01 & 7451.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT\\
011502172-01 & 7452.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011502172-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011502179-01 & 7453.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_970.01\\
011502218-01 & 0970.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
011502218-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
011502867-01 & 0195.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011506235-01 & 7454.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011506235-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011506508-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011506654-01 & 4586.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011506768-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011506938-01 & 5906.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011507101-01 & 0773.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011508233-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011508397-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011508397-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011508397-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011508587-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011508587-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011508644-01 & 3101.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011508874-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011509051-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011509504-01 & 4232.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011509728-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011512246-01 & 0168.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011512246-02 & 0168.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011512246-03 & 0168.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011512815-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011513155-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011513155-02 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011513441-01 & \nodata & PC & 0 & 0 & 0 & 0 & PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_5:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_5:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011513486-01 & 4748.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011514977-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011515221-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011515221-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011515221-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011516242-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED---PARENT\_IS\_005443837-02\\
011516930-01 & 6240.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011517719-01 & 1416.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011517719-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011517934-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011517934-02 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
011518142-01 & 3762.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011518193-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011518201-01 & 3104.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011519134-01 & 3419.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011519180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011519180-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011519180-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011519187-01 & 4625.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011519226-01 & 6087.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011519226-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011519466-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011520114-01 & 5909.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011520150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011520274-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011520459-01 & 2226.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011520787-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
011520787-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
011520793-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED---PARENT\_IS\_011520787-01\\
011520793-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011520793-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011521048-01 & 0540.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
011521048-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
011521678-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011521793-01 & 0352.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011521793-02 & 0352.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011546211-01 & 1654.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011546920-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011546920-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011547271-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011547505-01 & 1655.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011547513-01 & 0295.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011547513-02 & 0295.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011547869-01 & 3749.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
011548140-01 & 0256.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011548888-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011548888-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
011551652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011551652-02 & 7455.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011551692-01 & 1781.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011551692-02 & 1781.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011551692-03 & 1781.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011553706-01 & 0009.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
011553706-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
011554435-01 & 0063.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011558882-01 & 6241.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011559263-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011559304-01 & 7617.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011560037-01 & 3874.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011560037-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011560037-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011560273-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011560273-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011560382-01 & 7456.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_011560447-pri\\
011560397-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011560431-01 & 7457.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_011560447-pri\\
011560447-01 & 7458.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
011560447-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011560897-01 & 2365.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011560897-02 & 2365.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011564013-01 & 3714.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011564882-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011564882-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011565544-01 & 3013.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011565924-01 & 2837.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011566064-01 & 0353.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011566064-02 & 0353.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011566256-01 & 2361.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011567149-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_011618883-sec\\
011567375-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011568224-01 & 3973.01 & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---LARGE\_RM\\
011568224-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011568331-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011568331-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011568624-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011568624-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
011568987-01 & 0354.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011568987-02 & 0354.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011569443-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011569475-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011569475-02 & 4029.01 & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
011569628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011569628-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011569628-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011569782-01 & 2225.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011570749-01 & 1856.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011571757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011571757-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011571757-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011571757-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011572029-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011572046-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011572046-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011572193-01 & 3109.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011572263-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011572490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011572666-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011572666-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011599038-01 & 1437.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011599264-01 & 1417.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
011599264-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011599937-01 & 5915.01 & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011600889-01 & 1442.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011601357-01 & 7459.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
011601425-01 & 5917.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011601584-01 & 1831.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011601584-02 & 1831.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011601584-03 & 1831.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
011601584-04 & 1831.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011601597-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LARGE\_RM\\
011602449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
011602449-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011602449-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011602794-01 & 7460.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011605209-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011605209-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011605209-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011606351-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011606351-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011607008-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011607017-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011607017-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011607176-01 & 3930.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
011607176-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011607193-01 & 0983.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
011607193-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM\\
011611275-01 & 4234.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011611600-01 & 1424.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011611727-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011612274-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011612274-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011612280-01 & 4304.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011612611-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011612611-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011614502-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011614528-01 & 3885.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
011614617-01 & 1990.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011615481-01 & 7461.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
011616200-01 & 7462.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011616596-01 & 4229.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_011616594-pri\\
011616631-01 & 7463.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_011616594-pri\\
011616663-01 & 7464.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_011616594-pri\\
011617030-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
011617670-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011618043-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011618569-01 & 4792.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011618601-01 & 3022.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011618601-02 & 3022.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011618798-01 & 7465.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011618998-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011618998-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011619202-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011619861-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011619861-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011619861-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011619868-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011619868-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011619868-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011619964-01 & 7466.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011619964-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011620101-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011621223-01 & 0355.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011621897-01 & 7618.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
011622535-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011622535-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011622600-01 & 1876.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011622985-01 & 2550.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011623629-01 & 0365.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011623878-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011623878-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011624191-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011624191-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011624191-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011624249-01 & 0356.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011624521-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011624521-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011649459-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011650401-01 & 4566.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011650543-01 & 7467.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011651105-01 & 7468.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011651712-01 & 3363.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011652870-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011653381-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011653381-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011654113-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011654267-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011655826-01 & 4643.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
011656246-01 & 1532.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011656302-01 & 0434.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
011656302-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
011656492-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011656492-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011656492-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011656721-01 & 0541.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011656840-01 & 0774.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011656840-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011656840-03 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---EYEBALL---INVERT\_DIFF\\
011656918-01 & 1945.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011656928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011656928-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011656928-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011657371-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011657371-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011657371-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011657371-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011657614-01 & 3370.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011657614-02 & 3370.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011657891-01 & 1965.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011658996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011658996-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011658996-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011661993-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011661993-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011662184-01 & 2791.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011662370-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011662440-01 & 7469.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
011662440-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
011662513-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011662513-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011662513-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011665531-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011665531-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011665531-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011665852-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
011666104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011666104-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011666104-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011666141-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011666141-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011666141-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011666429-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011666429-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011666429-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011666429-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011666503-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011666503-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011666503-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011666881-01 & 0167.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011667548-01 & 3926.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011668602-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011668602-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011668783-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011668950-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011668950-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011669125-01 & 1535.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011669239-01 & 0542.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011669239-02 & 0542.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011670125-01 & 2355.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011670599-01 & 4282.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011670605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---CENTROID\_SIGNIF\_UNCERTAIN\\
011671226-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011671226-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011671226-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011671226-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011671226-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011671429-01 & 3567.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
011671429-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
011671429-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011671579-01 & 4510.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011671646-01 & 7470.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011672354-01 & 7471.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011673674-01 & 0133.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_011673686-pri\\
011673674-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_011673686-pri\\
011673686-01 & 6243.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011673686-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---PARENT\_IS\_133.01\\
011673802-01 & 1894.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011700185-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011700370-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011700370-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011700604-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011701407-01 & 2376.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011701911-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
011702835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011702948-01 & 1465.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011704044-01 & 7472.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011704044-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011704044-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
011704336-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011705004-01 & 2199.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011705004-02 & 2199.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
011706449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011706518-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011706518-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011706518-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011706658-01 & 7473.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011706658-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
011706658-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011708170-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011708170-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011708170-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011708170-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011708238-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011708238-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011708238-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011709022-01 & 7474.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
011709059-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011709124-01 & 0435.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011709124-02 & 0435.05 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011709124-03 & 0435.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011709124-04 & 0435.03 & PC & 0 & 0 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
011709124-05 & 0435.06 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011709124-06 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
011709244-01 & 1832.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011709244-02 & 1832.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011709244-03 & 1832.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011709423-01 & 3001.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011710462-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011710462-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011713245-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011713924-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011713981-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011714150-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011714150-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011714150-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011714231-01 & 3115.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011716643-01 & 5929.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011717240-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011717240-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
011718053-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
011718144-01 & 2310.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011718389-01 & 4444.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011718839-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011718839-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011718839-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011720424-01 & 3116.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011721444-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011721834-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011722906-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011723564-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011723564-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011723564-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011723926-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011724091-01 & 7475.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011724091-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011724094-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011724210-01 & 6244.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011724210-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011725829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011725829-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011751338-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011751652-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011751939-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET---CENTROID\_SIGNIF\_UNCERTAIN\\
011751939-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
011752358-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011752632-01 & 2492.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011752906-01 & 0253.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011752906-02 & 0253.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011752908-01 & 2651.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_253.01\\
011754430-01 & 3403.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011754430-02 & 3403.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011754553-01 & 0775.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011754553-02 & 0775.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011754553-03 & 0775.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011754974-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011754974-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011756821-01 & 6088.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011756821-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011757334-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011757422-01 & 7476.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011757451-01 & 4745.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011757490-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011758544-01 & 1883.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011759297-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011759297-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011759297-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011759685-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011760231-01 & 1841.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011760312-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011760312-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011760312-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011760312-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011760860-01 & 3892.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011760959-01 & 1484.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011761199-01 & 2669.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011761199-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011763910-01 & 7477.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---CLEAR\_APO\\
011764462-01 & 1531.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011766996-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011766996-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011766996-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011768142-01 & 2626.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011768756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011768763-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
011768970-01 & 7478.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
011768970-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011769146-01 & 6089.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011769146-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011769689-01 & 4551.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011769890-01 & 1980.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011769929-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011769929-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011769929-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011770258-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
011770258-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011771430-01 & 2582.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011771931-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011771931-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011772510-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011772971-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011772971-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011773022-01 & 0620.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011773022-02 & 0620.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011773022-03 & 0620.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011773245-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO\\
011773328-01 & 1906.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011773460-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011773460-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011773625-01 & 7479.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011773909-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011773909-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011773909-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011773909-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
011774303-01 & 2269.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011774387-01 & 1497.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011774387-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
011774991-01 & 2173.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011774991-02 & 2173.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011775354-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011775354-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011775507-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011775507-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011775511-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
011775530-01 & 7480.01 & FP & 1 & 0 & 1 & 0 & LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
011802615-01 & 0296.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011802766-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011802766-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011802860-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011802860-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011802875-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011804465-01 & 0020.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET\\
011805075-01 & 0436.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011807274-01 & 0262.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011807274-02 & 0262.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011807603-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011807603-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011807603-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011808036-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011809145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011809179-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011809179-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011809346-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011810124-01 & 3344.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011810124-02 & 3344.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011810124-03 & 3344.03 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
011810798-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011811140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011811193-01 & 2260.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011811382-01 & 5934.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011811454-01 & 7481.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
011811856-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011812062-01 & 0776.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011812199-01 & 6090.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---SEASONAL\_DEPTH\_DIFFS\_IN\_DV---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO\\
011812199-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
011815158-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---KIC\_OFFSET\\
011815158-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
011816957-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011817750-01 & 7482.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011818166-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011818581-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011818607-01 & 2467.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011818800-01 & 0777.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011818872-01 & 2581.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011819135-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
011819135-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011820820-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011820820-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011820820-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011820830-01 & 1728.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011820830-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---RESID\_OF\_PREV\_TCE\\
011820830-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---FIT\_FAILED\\
011821140-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011821140-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011821363-01 & 1494.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011822666-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011822666-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011822666-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011822789-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011822789-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011822789-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011823054-01 & 0543.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011823054-02 & 0543.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011823661-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011823836-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011823836-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011824218-01 & 3845.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_437.01\\
011824222-01 & 0437.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011824578-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011824786-01 & 2371.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011824964-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011824964-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011824964-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011825955-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011825955-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011825955-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011825996-01 & 7483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011826400-01 & 6091.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011826400-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011826440-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011826440-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011852982-01 & 0247.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011853130-01 & 3263.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011853255-01 & 0778.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011853301-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011853878-01 & 1833.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011853878-02 & 1833.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011853878-03 & 1833.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011853905-01 & 0007.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011854636-01 & 7484.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
011855538-01 & 7485.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_012004679-pri\\
011856076-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011856178-01 & 6246.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
011858541-01 & 7486.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011858541-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011858741-01 & 3633.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011858741-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011858748-01 & 1471.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_011858741-01\\
011858979-01 & 4062.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---TOO\_FEW\_QUARTERS\\
011859333-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011860395-01 & 3445.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011861572-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011867071-01 & 6247.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---TOO\_FEW\_QUARTERS\\
011867071-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011868514-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011868514-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011868514-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011869052-01 & 0120.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011869257-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
011870545-01 & 1510.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
011872139-01 & 4350.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_011922782-pri\\
011872512-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011872512-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011872534-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
011872848-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011872848-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011873143-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
011873166-01 & 7487.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011873171-01 & 7488.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_011873166-pri\\
011874338-01 & 3464.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011874338-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011874577-01 & 2779.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011874676-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011874676-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011874676-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011875511-01 & 3471.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
011875511-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
011875734-01 & 1828.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011876098-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011876098-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011876098-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---CENTROID\_SIGNIF\_UNCERTAIN\\
011904151-01 & 0072.02 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011904151-02 & 0072.01 & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
011904704-01 & 7489.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011904734-01 & 1764.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011905011-01 & 0297.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011905398-01 & 5940.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011905409-01 & 3312.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---TOO\_FEW\_QUARTERS\\
011905562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011905562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011905761-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011905761-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011906217-01 & 7490.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
011908559-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011908559-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011909375-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011909375-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011909375-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011909497-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011909497-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011909686-01 & 1483.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011909839-01 & 0779.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011909839-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011910220-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011910220-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011910642-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
011910896-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011911561-01 & 3875.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011911580-01 & 3900.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_003644542-01\\
011911580-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_3511.01\\
011912764-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011912911-01 & 4607.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_011913071-pri\\
011912916-01 & 4475.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_011913071-pri\\
011912932-01 & 3085.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_011913071-pri\\
011912941-01 & 4481.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_011913071-pri\\
011912987-01 & 4461.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_011913071-pri\\
011913012-01 & 0544.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_011913071-pri\\
011913012-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---LARGE\_RM---PARENT\_IS\_011913071-sec\\
011913013-01 & 1462.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO---PARENT\_IS\_011913071-pri\\
011913013-02 & \nodata & FP & 1 & 1 & 1 & 1 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO---PARENT\_IS\_011913071-sec\\
011913052-01 & 7491.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_011913071-pri\\
011913071-01 & 7492.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED\\
011913072-01 & 4729.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_011913071-pri\\
011913073-01 & 0011.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_011913071-pri\\
011913835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011918099-01 & 0780.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011918099-02 & 0780.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011918482-01 & 7493.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
011919145-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
011919658-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED\\
011919829-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011919829-02 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011919968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011919968-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011920497-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011920497-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
011920541-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011920541-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011920541-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011920542-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011921886-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011922283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011922283-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011922648-01 & 7494.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_011922782-pri\\
011922678-01 & 2425.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_011922782-pri\\
011922722-01 & 2301.01 & FP & 0 & 0 & 1 & 1 & LARGE\_RM---PARENT\_IS\_011922782-pri\\
011922778-01 & 3408.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011922782-01 & 7495.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---SATURATED\\
011923213-01 & 5943.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011923255-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011923270-01 & 0781.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011923284-01 & 2026.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011923562-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011923562-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011923819-01 & 7496.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011923819-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011924025-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011924025-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011924366-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
011924366-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011924426-01 & 5944.01 & PC & 0 & 0 & 0 & 0 & FIT\_FAILED\\
011925068-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
011925968-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011953224-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011953224-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011953224-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011954651-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011954651-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011954842-01 & 1530.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011955499-01 & 1512.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011957183-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011957183-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011957286-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011958062-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011959569-01 & 7497.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
011959569-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
011959893-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011959893-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011960862-01 & 0782.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011961072-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
011961695-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011961695-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011962284-01 & 2647.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011963206-01 & 2820.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011966253-01 & 2772.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011966557-01 & 7498.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
011967004-01 & 7499.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
011967004-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
011967356-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011967356-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011967758-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011967758-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011967788-01 & 4021.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011967788-02 & 4021.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011968439-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011968439-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011968439-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011968463-01 & 2433.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
011968463-02 & 2433.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011968463-03 & 2433.05 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
011968463-04 & 2433.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
011968463-05 & 2433.04 & PC & 0 & 0 & 0 & 0 & \nodata\\
011968463-06 & 2433.06 & PC & 0 & 0 & 0 & 0 & \nodata\\
011968490-01 & 7500.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
011968513-01 & 3587.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
011968513-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011968514-01 & 5947.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---SATURATED---PARENT\_IS\_3587.01\\
011969092-01 & 4375.01 & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---LARGE\_RM\\
011969092-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
011969092-03 & \nodata & FP & 1 & 0 & 1 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE---LARGE\_RM\\
011969988-01 & 4011.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
011970050-01 & 4893.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011970288-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011970288-02 & 7501.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
011970288-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011970288-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011970988-01 & 4129.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
011971323-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
011971335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011971449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---KIC\_OFFSET\\
011971449-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---KIC\_OFFSET\\
011971449-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
011971490-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
011971490-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
011971494-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
011971494-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011971494-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
011972526-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011972526-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011972526-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
011972666-01 & 0545.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
011972872-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
011973805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
011973921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
011974540-01 & 0129.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
011974942-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
011974942-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
011974942-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
011975363-01 & 6248.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
012004594-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
012004679-01 & 7502.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
012004680-01 & 7503.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_012004679-pri\\
012004689-01 & 7504.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_012004679-pri\\
012004971-01 & 3194.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
012008727-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012008872-01 & 2729.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012009347-01 & 3792.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012009347-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012009584-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012010534-01 & 6092.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012010534-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012011851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012011851-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012013615-01 & 7505.01 & FP & 0 & 1 & 0 & 0 & ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---FIT\_FAILED\\
012016243-01 & 7506.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
012016267-01 & 2590.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012017109-01 & 2106.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012017140-01 & 0358.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012017140-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
012017750-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012017750-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
012017894-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012017894-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---LARGE\_RM\\
012017921-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
012017921-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
012018798-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
012018805-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
012019440-01 & 0186.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012020218-01 & 1507.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012020252-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TOO\_FEW\_QUARTERS\\
012020329-01 & 0783.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012020365-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012020365-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012020365-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012020590-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
012020590-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012020590-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012020590-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012021387-01 & 3522.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
012021625-01 & 2996.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012022517-01 & 7507.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012022517-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012022718-01 & 7508.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
012023078-01 & 2888.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_012023089-01\\
012023089-01 & 3727.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
012024018-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012024120-01 & 0265.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012053628-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012053823-01 & 7509.01 & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
012055539-01 & 3261.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012055552-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
012055866-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012056139-01 & 3262.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012057840-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
012058147-01 & 2072.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012058204-01 & 2218.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012058204-02 & 2218.02 & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
012058931-01 & 0546.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012058931-02 & 0546.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012061096-01 & 2642.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
012061222-01 & 0484.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012061238-01 & 1502.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
012061605-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012061605-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012061756-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012061756-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012061969-01 & 2061.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012061969-02 & 2061.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012062339-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012062660-01 & 3746.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
012062660-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---KIC\_OFFSET---LARGE\_RM\\
012062667-01 & 1487.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3746.01\\
012066007-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---EYEBALL---SATURATED\\
012066335-01 & 0784.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012066335-02 & 0784.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012066447-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012066569-01 & 3282.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012066583-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012066629-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_012066630-pri\\
012066629-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_012066630-sec\\
012067780-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012067780-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012067780-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
012067960-01 & 7510.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012068180-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012068180-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
012068180-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012068180-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012068975-01 & 0623.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---KIC\_OFFSET---LARGE\_RM\\
012068975-02 & 0623.03 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012068975-03 & 0623.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012068975-04 & 0623.04 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012069252-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012069252-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012069252-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
012069414-01 & 4512.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
012069786-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012069786-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012070811-01 & 0785.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012071006-01 & 7511.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
012071006-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012071006-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---FIT\_FAILED\\
012071037-01 & 2388.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_012071006-pri\\
012071317-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---TOO\_FEW\_CENTROIDS\\
012071317-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012071317-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012071754-01 & 4914.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012072666-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012072872-01 & 3017.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012073334-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012073334-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012104897-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012104951-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012104951-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012104951-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012105051-01 & 0141.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
012105259-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
012105259-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012105259-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
012105785-01 & 7512.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---LARGE\_RM\\
012105785-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---LARGE\_RM\\
012106368-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012106875-01 & 7513.01 & FP & 0 & 0 & 0 & 1 & EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_3895.01\\
012106929-01 & 0359.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---KIC\_OFFSET---LARGE\_RM---PARENT\_IS\_3895.01\\
012106929-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012106934-01 & 3895.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_359.01\\
012107008-01 & 4297.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_3895.01\\
012107021-01 & 0360.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3895.01\\
012108293-01 & 4540.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_012108333-pri\\
012108293-02 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO---PARENT\_IS\_012108333-sec\\
012108312-01 & 1492.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_012108333-pri\\
012108364-01 & 4592.01 & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED---PARENT\_IS\_012108333-pri\\
012109267-01 & 4457.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012109297-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012109421-01 & \nodata & FP & 1 & 0 & 0 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_012157987-pri\\
012109845-01 & 3765.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
012110786-01 & 2665.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
012110942-01 & 0786.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012111004-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012111004-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012115188-01 & 2396.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012115188-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012115387-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012115810-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
012116380-01 & 2155.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012116489-01 & 0547.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012116489-02 & 0547.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012117099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012117276-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012117689-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012117689-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012117689-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012117945-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---FIT\_FAILED---PARENT\_IS\_005443837-02\\
012118993-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012119295-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012119295-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012119295-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012120077-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012120077-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012120077-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
012120307-01 & 2597.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012120307-02 & 2597.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012120307-03 & 2597.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
012120484-01 & 2407.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012120938-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012120943-01 & 1458.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012121470-01 & 2142.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
012121570-01 & 2290.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012154526-01 & 2004.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012154526-02 & 2004.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012154526-03 & 2004.03 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
012155015-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012155015-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012155928-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
012156174-01 & 3260.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012156347-01 & 2588.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012157971-01 & \nodata & FP & 1 & 0 & 1 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO---PARENT\_IS\_012157987-pri\\
012157983-01 & 7514.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_ALT---CLEAR\_APO---PARENT\_IS\_012157987-pri\\
012158032-01 & \nodata & FP & 1 & 0 & 0 & 1 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_012157987-pri\\
012159249-01 & 1536.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012159988-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
012160023-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012164564-01 & 2780.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012164634-01 & 3491.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012164634-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012164751-01 & 7515.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---FIT\_FAILED\\
012164770-01 & 2088.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_012164751-pri\\
012165113-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012165113-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012165113-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012166770-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012166874-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012166874-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012167139-01 & \nodata & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012167361-01 & 0980.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---SATURATED\\
012167585-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
012168993-01 & 3105.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012169181-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012169181-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012170648-01 & 2875.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012170648-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012202137-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012202143-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012202143-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012202143-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012202245-01 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
012202431-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012203455-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012204137-01 & 4590.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012206271-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012206271-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012206271-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012206313-01 & 2714.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012206313-02 & 2714.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012206313-03 & 2714.03 & PC & 0 & 0 & 0 & 0 & \nodata\\
012207099-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
012207099-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012207117-01 & 6249.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---INVERT\_DIFF\\
012207117-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
012208157-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012208157-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012208157-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012208483-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
012208631-01 & 2449.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012208631-02 & 2449.02 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
012208769-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012208769-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012208769-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012208769-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012208887-01 & 3333.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
012208887-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012208887-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---FIT\_FAILED\\
012216210-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012216210-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012216210-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012216210-04 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012216210-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012216278-01 & 2565.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
012216706-01 & 3644.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---SEASONAL\_DEPTH\_DIFFS\_IN\_DV\\
012217281-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012217283-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
012217403-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012217824-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
012217866-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012217866-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012217907-01 & 7516.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012217907-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012218917-01 & \nodata & FP & 1 & 0 & 0 & 1 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
012251650-01 & 0621.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012251779-01 & 7517.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012251779-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012252424-01 & 0153.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012252424-02 & 0153.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012253106-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
012253474-01 & 1947.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012253490-01 & 5961.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012253534-01 & 7619.01 & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
012253624-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012253769-01 & 3310.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012254378-01 & 2387.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012254389-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012254389-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012254419-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012254688-01 & 2384.01 & FP & 0 & 0 & 1 & 0 & LARGE\_RM\\
012254752-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012254792-01 & 1506.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012254909-01 & 2372.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012255382-01 & 3167.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
012255382-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
012256520-01 & 2264.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012257449-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012257449-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012257449-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012257851-01 & 5962.01 & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---CLEAR\_APO---PARENT\_IS\_012257908-pri\\
012257886-01 & 4148.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_012257908-pri\\
012257999-01 & 2577.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012258300-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012258300-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012258330-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012258330-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012258556-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
012265078-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012265150-01 & 5963.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
012265786-01 & 4595.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012266636-01 & 1522.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012266636-02 & 1522.02 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH\\
012267759-01 & \nodata & FP & 1 & 0 & 1 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---LARGE\_RM---PARENT\_IS\_012267718-sec\\
012268190-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012268190-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012268220-01 & 7518.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---EYEBALL---SATURATED\\
012268220-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---SATURATED\\
012268319-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012268319-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---TOO\_FEW\_QUARTERS\\
012268319-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012268319-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012268408-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012268579-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012268579-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012300524-01 & 5964.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012301181-01 & 2059.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012301181-02 & 2059.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012302104-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012302391-01 & 7519.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
012302530-01 & 0438.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012302530-02 & 0438.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012302530-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012303426-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012303426-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012304013-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012304202-01 & 7620.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012304728-01 & 7520.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012305407-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012305407-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012306058-01 & 2541.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012306058-02 & 2541.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012306284-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---KIC\_OFFSET\\
012306301-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TOO\_FEW\_QUARTERS\\
012306699-01 & 3858.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
012306808-01 & 7521.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
012314444-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012314580-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012314750-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
012314750-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012314973-01 & 0279.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012314973-02 & 0279.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012315060-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---CLEAR\_APO\\
012316431-01 & 0485.01 & FP & 0 & 1 & 1 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO---PARENT\_IS\_3575.01\\
012316447-01 & 3575.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
012316447-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012316447-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
012317342-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012317342-02 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---CLEAR\_APO\\
012349560-01 & 5965.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
012350110-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---TOO\_FEW\_QUARTERS\\
012351927-01 & 7522.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012351927-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012352290-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012352485-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
012352520-01 & 3094.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012353501-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
012353633-01 & 7523.01 & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---PARENT\_IS\_012554536-pri\\
012353648-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
012353648-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012353648-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012353648-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012353720-01 & 7524.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012353720-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012354328-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012356746-01 & 7525.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL---EYEBALL---LARGE\_RM\\
012356746-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
012356914-01 & 7526.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
012356914-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012356914-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
012356914-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
012356914-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
012357103-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012365000-01 & 7527.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012365000-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---FIT\_FAILED\\
012365015-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012365015-02 & 7528.01 & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012365184-01 & 1474.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012365420-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012365420-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012366084-01 & 0787.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012366084-02 & 0787.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012366084-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012366757-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012367017-01 & 7529.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---CLEAR\_APO\\
012367310-01 & 7530.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012367310-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012367464-01 & 6250.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012367464-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012400538-01 & 1503.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012400729-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012400729-02 & \nodata & FP & 1 & 0 & 0 & 0 & SAME\_P\_AS\_PREV\_NTL\_TCE\\
012400984-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW\\
012400984-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012400984-03 & \nodata & FP & 1 & 0 & 0 & 0 & ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012400984-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012400984-05 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
012401132-01 & 4829.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_QUARTERS\\
012401863-01 & 2331.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012403119-01 & 1478.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012403968-01 & 7531.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012403985-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012404086-01 & 0788.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012404305-01 & 0486.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012404890-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012404890-02 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS---PARENT\_IS\_005443837-02\\
012404954-01 & 0361.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012405333-01 & 3009.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012405950-01 & 3778.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012405950-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012405950-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012406610-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012406749-01 & 1476.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012406807-01 & 3091.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012407395-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012407395-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012407623-01 & 4370.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
012416661-01 & 3122.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012416987-01 & 2933.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012417370-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012417486-01 & 0622.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012417739-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS\\
012417739-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012418662-01 & 7532.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT\\
012418724-01 & 1516.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012418795-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---PARENT\_IS\_012418816-pri\\
012418816-01 & 7533.01 & PC & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET---FIT\_FAILED\\
012418891-01 & 4321.01 & FP & 0 & 0 & 0 & 1 & PARENT\_IS\_012418816-pri\\
012418966-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012453581-01 & 2424.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012453851-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012454043-01 & \nodata & FP & 1 & 0 & 0 & 0 & MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT\\
012454461-01 & 2463.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
012454800-01 & 7534.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012455315-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH\\
012455315-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012456063-01 & 4329.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012456601-01 & 2745.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012457978-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012457978-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012458437-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012458437-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012458437-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012458437-04 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012458605-01 & 4605.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012458666-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012458817-01 & 7535.01 & PC & 0 & 0 & 0 & 0 & TOO\_FEW\_CENTROIDS\\
012459731-01 & 3662.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
012459731-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
012459808-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH\\
012459913-01 & 0602.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012469800-01 & 2543.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012470041-01 & 6251.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012470317-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
012470317-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012470317-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012470530-01 & 7536.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---FIT\_FAILED\\
012470530-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012470530-03 & \nodata & FP & 1 & 0 & 0 & 0 & RESID\_OF\_PREV\_TCE---FIT\_FAILED\\
012470709-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012470709-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012470844-01 & 0790.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012470844-02 & 0790.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012470954-01 & 0439.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012504353-01 & 7537.01 & FP & 1 & 0 & 0 & 0 & TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012504988-01 & 0181.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012504988-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012505076-01 & 2154.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012505503-01 & 4190.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---INVERT\_DIFF\\
012505621-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012505621-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012505621-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012505654-01 & 2353.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012506342-01 & 7538.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_012506351-pri\\
012506351-01 & 1446.01 & FP & 0 & 1 & 0 & 0 & DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL---ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL\\
012506665-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
012506770-01 & 1577.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012507325-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012507325-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
012508335-01 & 0215.01 & PC & 0 & 0 & 0 & 0 & EYEBALL---LARGE\_RM\\
012508604-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012508604-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---FIT\_FAILED\\
012508604-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012509148-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012509148-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012509148-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012509829-01 & 4264.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---CLEAR\_APO\\
012509829-02 & \nodata & FP & 1 & 1 & 1 & 0 & THIS\_TCE\_IS\_A\_SEC---CLEAR\_APO\\
012519942-01 & 7539.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012520187-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012553358-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW\\
012553358-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE\\
012554212-01 & 5974.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012554510-01 & \nodata & FP & 1 & 0 & 0 & 1 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---PARENT\_IS\_012554536-pri\\
012554634-01 & 4714.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012555616-01 & 7540.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012555688-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---INVERT\_DIFF\\
012557548-01 & 3794.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012557713-01 & 7541.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH\\
012557713-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC\\
012599532-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---INVERT\_DIFF\\
012599700-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012600735-01 & 0548.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012602191-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---MARSHALL\_FAIL---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012602236-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---EYEBALL---SATURATED\\
012602314-01 & 2853.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012602335-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012602567-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012602567-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012602568-01 & 1583.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012643582-01 & 3626.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012643589-01 & 0376.01 & FP & 0 & 0 & 1 & 1 & CLEAR\_APO---PARENT\_IS\_3626.01\\
012643589-02 & 0376.02 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---LARGE\_RM\\
012643589-03 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---INVERT\_DIFF\\
012643933-01 & \nodata & FP & 1 & 0 & 0 & 0 & DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---TRANSITS\_NOT\_CONSISTENT---TOO\_FEW\_QUARTERS\\
012644712-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---TOO\_FEW\_QUARTERS\\
012644769-01 & 1611.01 & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---KIC\_OFFSET\\
012644769-02 & \nodata & FP & 1 & 1 & 0 & 0 & THIS\_TCE\_IS\_A\_SEC---KIC\_OFFSET\\
012644769-03 & \nodata & FP & 0 & 1 & 0 & 0 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---KIC\_OFFSET\\
012644774-01 & \nodata & FP & 0 & 1 & 0 & 1 & SIG\_SEC\_IN\_DV\_MODEL\_SHIFT---OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH---PERIOD\_ALIAS\_IN\_DV\_DATA\_SEEN\_AT\_10:1---PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_10:1---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_1611.01\\
012644774-02 & \nodata & FP & 1 & 1 & 0 & 1 & THIS\_TCE\_IS\_A\_SEC---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_1611.01\\
012644774-03 & \nodata & FP & 1 & 0 & 0 & 1 & SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---CLEAR\_APO---TOO\_FEW\_QUARTERS---PARENT\_IS\_1611.01\\
012644774-04 & 1555.01 & FP & 1 & 0 & 1 & 1 & RESID\_OF\_PREV\_TCE---CLEAR\_APO---PARENT\_IS\_1611.01\\
012644822-01 & 0791.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012645057-01 & 4497.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012645761-01 & 5976.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012647018-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012647070-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
012647070-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012647070-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012647577-01 & 4530.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012688835-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012688835-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---FIT\_FAILED\\
012688835-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---INVERT\_DIFF\\
012689656-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012691412-01 & 1983.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
012691831-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW\\
012691831-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012735740-01 & 3663.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012735830-01 & 3311.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012736056-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012736056-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---EYEBALL---SATURATED\\
012736056-03 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012736658-01 & 5980.01 & FP & 0 & 1 & 1 & 0 & SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT---LARGE\_RM\\
012737015-01 & 4245.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012784167-01 & 3848.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012784394-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---SATURATED\\
012785320-01 & 0298.01 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012785320-02 & 0298.02 & PC & 0 & 0 & 0 & 0 & KIC\_OFFSET\\
012833566-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---SATURATED\\
012833701-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---EYEBALL---LARGE\_RM\\
012834393-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---LARGE\_RM\\
012834874-01 & 0487.01 & PC & 0 & 0 & 0 & 0 & \nodata\\
012884588-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---TOO\_FEW\_CENTROIDS\\
012884589-01 & \nodata & FP & 1 & 0 & 1 & 0 & LPP\_DV\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---CLEAR\_APO\\
012885086-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---EYEBALL---SATURATED\\
012885086-02 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---LPP\_ALT\_TOO\_HIGH---SAME\_P\_AS\_PREV\_NTL\_TCE---EYEBALL---SATURATED\\
012885212-01 & 2184.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO\\
012885212-02 & 2184.02 & PC & 0 & 0 & 0 & 0 & \nodata\\
012934846-01 & \nodata & FP & 1 & 0 & 0 & 0 & LPP\_DV\_TOO\_HIGH---ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW---ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW---EYEBALL---INVERT\_DIFF\\
012935144-01 & 2847.01 & FP & 0 & 0 & 1 & 0 & CLEAR\_APO

